Plateau-Rayleigh instability of a soft layer coated on a rigid cylinder

We study the Plateau-Rayleigh instability of a viscoelastic soft solid layer coated on a rigid cylinder i.e., a soft fibre with a rigid core. The onset of instability is examined using a linear stability analysis. We find that increasing the rigid cylinder radius reduce the growth rate of the fastest growing mode. For each rigid cylinder radius, a critical elastocapillary number is found below which all wavelengths of disturbances are stable. The critical value for a soft fibre with a thick rigid cylindrical core can be several orders of magnitudes larger than that for a totally soft fibre (no rigid core), which highlights the strong stabilizing effect of the rigid core on the system. Increasing the relaxation timescale of the viscoelastic material also slows down the growth of disturbance, but has no effect on the critical elastocapillary number. Interestingly, the wavelength of the fastest growing mode is independent of the rigid cylinder radius for the purely elastic case.

==> ss.tex <==
@Article{Snoeijer13,
     author    = "Snoeijer, J. H. and Andreotti, B.",
     title     = "Moving contact lines: Scales, regimes, and dynamical transitions",
     journal   = "Ann. Rev. Fluid Mech.",
     volume    = "45",
     year      = "2013",
     pages     = "269",
}

@Article{Reiter2001,
     author    = "G. Reiter and A. Sharma",
     title     = "Auto-Optimisation of Dewetting Rates by Rim Instabilities in Slipping Polymer Films",
     journal   = "Phys. Rev. Lett.",
     volume    = "87",
     year      = "2001",
     pages     = "166103",
}


@Article{FKPA09,
     author    = "J.-B. Fournier and N. Khalifat and N. Puff and
                M. I. Angelova",
     title     = "Chemically triggered ejection of membrane tubules
            controlled by intermolecular friction",
     journal   = "Phys. Rev. Lett.",
     volume    = "102",
     year      = "2009",
     pages     = "018102",
}

@Article{FMA60,
     author    = "H. {von Foerster} and P. M. Mora and L. W. Amiot",
     title     = "Doomsday: Friday, 13 November, A.D. 2026",
     journal   = "Science",
     volume    = "132",
     year      = "1960",
     pages     = "1291",
}

@Article{Cahn2000,
     author    = "J. W. Cahn",
     title     = "Wetting and non-wetting near critical points in solids",
     journal   = "Physica A",
     volume    = "279",
     year      = "2000",
     pages     = "195",
}
@Article{ELowen,
     author    = "A. Esztermann and H. L{\"o}wen",
     title     = "Wetting of topographically structured surfaces by
                    crystalline phases",
     journal   = "J. Phys.: Condens. Matter",
     volume    = "17",
     year      = "2005",
     pages     = "S429",
}
@Article{Schweika,
     author    = "W. Schweika and H. Reichert and
           W. Babik and O. Klein and S. Engemann",
     title     = "Strain-induced incomplete wetting at CuAu(001) surfaces ",
     journal   = "Phys. Rev. B ",
     volume    = "70",
     year      = "2004",
     pages     = "041401(R)",
}
@Article{Gittes,
     author    = "F. T. Gittes and M. Schick",
     title     = "Complete and incomplete wetting by adsorbed solids",
     journal   = "Phys. Rev. B",
     volume    = "30",
     year      = "1984",
     pages     = "209",
}
@Article{HuseIC,
     author    = "D. A. Huse",
     title     = "Incomplete wetting by adsorbed solid films",
     journal   = "Phys. Rev. B",
     volume    = "29",
     year      = "1984",
     pages     = "6985",
}
@Article{Esztermann,
     author    = "A. Esztermann and M. Heni and  H. L{\"o}wen and
             J. Klier and M. Sohaili and P.  Leiderer",
     title     = "Triple-Point Wetting on Rough Substrates",
     journal   = "Phys. Rev. Lett. ",
     volume    = "88",
     year      = "2002",
     pages     = "055702",
}
@Article{MK96,
     author    = "L. Mahadevan and J. B.  Keller",
     title     = "Coiling of flexible ropes ",
     journal   = "Proc. Roy. Soc. London A",
     volume    = "452",
     year      = "1996",
     pages     = "1679",
}
@Article{MP99,
     author    = "L. Mahadevan and Y. Pomeau",
     title     = "Rolling droplets ",
     journal   = "Phys. Fluids",
     volume    = "11",
     year      = "1999",
     pages     = "2449",
}
@Article{KW56,
     author    = "J. B.  Keller and M. L. Weitz",
     title     = "Upward 'falling' jets and surface tension",
     journal   = "J. FLuid Mech.",
     volume    = "2",
     year      = "1956",
     pages     = "201",
}

@Article{B07,
     author    = "A. Boudaoud",
     title     = "Non-Newtonian thin films with normal stresses:
                  dynamics and spreading ",
     journal   = "Eur. Phys. J. E",
     volume    = "22",
     year      = "2007",
     pages     = "107",
}
@Article{BW58,
     author    = "G. Barnes and R. Woodcock",
     title     = "",
     journal   = "Am. J. Phys.",
     volume    = "26",
     year      = "1958",
     pages     = "205",
}
@Article{CL06,
     author    = "S. Chiu-Webster and J. R. Lister",
     title     = "The fall of a viscous thread onto a 	 surface:
         a 'fluid-mechanical sewing machine'",
     journal   = "J. Fluid Mech.",
     volume    = "569",
     year      = "2006",
     pages     = "89",
}
@Article{RHHHB06,
     author    = "N. M. Ribe and H. E. Huppert and M. A. Hallworth
         and M. Habibi and D. Bonn",
     title     = "Multiple coexisting states of liquid rope coiling",
     journal   = "J. Fluid Mech.",
     volume    = "555",
     year      = "2006",
     pages     = "275",
}
@Article{MHGRB04,
     author    = "M. Maleki and M. Habibi and R. Golestanian and
        N. M. Ribe and D.  Bonn",
     title     = "Liquid rope coiling on a solid surface",
     journal   = "Phys. Rev. Lett.",
     volume    = "93",
     year      = "2004",
     pages     = "214502",
}

@Article{dHL01,
     author    = "E. H. A. {de Hoog} and H. N. W. Lekkerkerker",
     title     = "Breakup of an elongated droplet in a centrifugal field",
     journal   = "J. Phys. Chem. B",
     volume    = "105",
     year      = "2001",
     pages     = "11636",
}

@Article{AS04,
     author    = "J. Ashmore and H. A. Stone",
     title     = "Instability of a rotating thread in a second immiscible
                    liquid",
     journal   = "Phys. Fluids",
     volume    = "16",
     year      = "2004",
     pages     = "29",
}

@Article{KW06,
     author    = "J. P. Kubitschek and P. D. Weidman",
     title     = "The effect of viscosity on the stability of a
          uniformly rotating liquid column in zero gravity",
     journal   = "J. Fluid Mech.",
     volume    = "572",
     year      = "2007",
     pages     = "261",
}

@Article{Aartswetting,
     author    = "D. G. A. L. Aarts and R. P. A. Dullens
        and H. N. W. Lekkerkerker and D. Bonn and R. {van Roij}",
     title     = "Interfacial tension and wetting in
             colloid-polymer mixtures",
     journal   = "J. Chem. Phys.",
     volume    = "120",
     year      = "2004",
     pages     = "1973",
}
@Article{BBSRDPBMI01,
     author    = "D. Bonn and E. Bertrand and N. Shahidzadeh and
        K. Ragil and  H. T. Dobbs and A. I. Posazhennikova and
          D. Broseta and J. Meunier and J. O. Indekeu",
     title     = "Complex wetting phenomena in liquid mixtures:
      frustrated-complete wetting and competing intermolecular forces",
     journal   = "J. Phys.: Condens. Matter",
     volume    = "13",
     year      = "2001",
     pages     = "4903",
}

@Article{HAWWELB06,
     author    = "Y. Hennequin and D. G. A. L. Aarts and J. H. {van der Wiel}
        and G. Wegdam and J. Eggers and H. N. W. Lekkerkerker and D. Bonn",
     title     = " Drop formation by thermal fluctuations at an
                 ultralow surface tension",
     journal   = "Phys. Rev. Lett.",
     volume    = "97",
     year      = "2006",
     pages     = "244503",
}
@Article{hennequin,
     author    = "Y. Hennequin and D. G. A. L. Aarts and J. O. Indekeu
          and H. N. W. Lekkerkerker and D. Bonn",
     title     = "Fluctuation forces and wetting layers in
         colloid-polymer mixture",
     journal   = "Phys. Rev. Lett.",
     volume    = "100",
     pages     = "178305",
     year      = "2008",
}
@Article{Indekeu94,
     author    = "J. O. Indekeu",
     title     = "Line tension at wetting",
     journal   = "Int. J. Mod. Phys. B",
     volume    = "8",
     pages     = "309-345",
     year      = "1994",
}
@Article{ACM02,
     author    = "D. B. Abraham and R. Cuerno and E. Moro",
     title     = "Microscopic model for thin film spreading",
     journal   = "Phys. Rev. Lett.",
     volume    = "88",
     year      = "2002",
     pages     = "206101"
}

@Book{AS68,
     author    = "M. Abramowitz and I. A. Stegun",
     title     = "Handbook of Mathematical Functions",
     publisher = "Dover",
     year      = "1968",
}

@Book{Goldstein1,
     author    = "S. Goldstein, Editor",
     title     = "Modern Developments in Fluids Dynamics, Vol I",
     publisher = "Oxford University Press",
     year      = "1938",
}
@Book{Goldstein2,
     author    = "S. Goldstein, Editor",
     title     = "Modern Developments in Fluids Dynamics, Vol II",
     publisher = "Oxford University Press",
     year      = "1938",
}
@Book{Vilenkin,
     author    = "A. Vilenkin and E. P. S. Shellard",
     title     = "Cosmic Strings and Other Topological Defects",
   publisher = {Cambridge University Press, Cambridge},
     year      = "2000",
}
@Book{Nye99,
     author    = "J. Nye",
     title     = "Natural Focusing and Fine Structure of Light:
          Caustics and Wave Dislocations",
     publisher = "Institute of Physics Publishing, Bristol",
     year      = "1999",
}
@Book{Abel,
     author    = "N. H. Abel",
     title     = "Oeuvres II",
     publisher = "Imprimerie de Gr{\o}ndahl {\&} S{\o}n, Christiania",
     pages     = "26",
     year      = "1881",
}
@Book{Lugt96,
     author    = "H. J. Lugt",
     title     = "Introduction to Vortex Theory",
     publisher = "Vortex Flow Press",
     year      = "1996",
}
@Article{Lugt87,
     author    = "H. J. Lugt",
     title     = "Local flow properties at a viscous free surface",
     journal   = "Phys. Fluids",
     volume    = "30",
     year      = "1987",
     pages     = "3647-3652"
}
@Article{S_Wu99,
     author    = "S. Wu",
     title     = "Well-posedness in Sobolev spaces of the full
                   water wave problem in 3-D",
     journal   = "J. Amer. Math. Soc. ",
     volume    = "12",
     year      = "1999",
     pages     = "445--495"
}
@Article{L87,
     author    = "H. J. Lugt",
     title     = "Local flow properties at a viscous free surface",
     journal   = "Phys. Fluids",
     volume    = "30",
     year      = "1987",
     pages     = "3647"
}
@Book{Wiggins03,
     author    = "S. Wiggins",
     title     = "Introduction to Applied Nonlinear Dynamical
                Systems and Chaos",
     publisher = "Springer",
     year      = "2003",
}
@Book{Alinhac95,
     author    = "S. Alinhac",
     title     = "Blowup for nonlinear hyperbolic equations",
     publisher = "Birkh{\"a}user",
     year      = "1995",
}
@Book{Birkhoff,
     author    = "G. Birkhoff and E. H. Zarantonello",
     title     = "Jets, wakes, and cavities",
     publisher = "Academic Press",
     year      = "1957",
}
@Book{Gurevich,
     author    = "M. I. Gurevich",
     title     = "Theory of Jets in an Ideal Fluid",
     publisher = "Pergamon Press",
     year      = "1966",
}
@Article{Berry07,
     author    = "M. V. Berry",
     title     = "Focused tsunami waves",
     journal   = "Proc. R. Soc. A",
     volume    = "463",
     year      = "2007",
     pages     = "3055"
}
@Article{AA03,
     author    = "S. B. Angenent and D. G. Aronson",
     title     = "The focusing problemfor eikonal equation",
     journal   = "J. evol. equ.",
     volume    = "3",
     year      = "2003",
     pages     = "137"
}
@Book{D69,
     author    = "A. Dupr{\'e}",
     title     = "Th{\'e}orie m{\'e}chanique de la chaleur",
     page      = "284",
     publisher = "Gauthier-Villars, Paris",
     year      = "1869",
}
@Book{DE86,
     author    = "M. Doi and S. F. Edwards",
     title     = "The theory of polymer dynamics",
     publisher = "Oxford University Press",
     year      = "1986",
}
@Book{T76,
     author    = "A. A. Townsend",
     title     = "The structure of turbulent shear flow",
   publisher = {Cambridge University Press, Cambridge},
     year      = "1976",
}
@Book{Risken,
     author    = "H. Risken",
     title     = "The Fokker-Planck Equation",
     publisher = "Springer: Berlin",
     year      = "1984",
}
@Book{Israelachvili,
     author    = "J. Israelachvili",
     title     = " Intermolecular and Surface Forces",
     publisher = "Academic Press: London",
     year      = "1992",
}

@Inproceedings{mckinley,
     author    = "G. H. McKinley and B. Ovryn",
     title     = "An interferometric investigation of contact line dynamics in
           spreading polymer melts and solutions",
     year      = "1998",
     booktitle = "Proceedings of the Fourth Microgravity
         Fluid Physics and Transport Phenomena Conference",
     editor    = "B. S. Singh",
     pages     = "384",
     publisher = "NASA",
}

@Inproceedings{S02,
     author    = "V. V. Serebryakov",
     title     = "The models of the supercavitation prediction for high
                  speed motion in water",
     year      = "2002",
     booktitle = "Proceedings of the International
         Summer Scientific School, High Speed Hydrodynamics,
                  Chebocsary",
     editor    = "G. G. Cherny and M. P. Tulin and A. G. Terentiev
                and V. V. Serebryakov",
     pages     = "71",
     publisher = "??"
}

@Article{S73,
     author    = "V. V. Serebryakov",
     journal   = "Dokl. Akad. Nauk Ukr. SSR. Ser. A",
     volume    = "12",
     pages     = "1119",
     year      = "1973",
}

@Article{AHHL96,
     author    = "T. Ala-Nissila and S. Herminghaus
         and T. Hjelt and P. Leiderer",
     title     = "Diffusive spreading of chainlike molecules on surfaces",
     journal   = "Phys. Rev. Lett.",
     volume    = "76",
     year      = "1996",
     pages     = "4003-4006",
}
@Article{HHAY98,
     author    = "T. Hjelt and S. Herminghaus and T. Ala-Nissila and
         and S. C. Ying",
     title     = "Dynamics of chainlike molecules on surfaces",
     journal   = "Phys. Rev. E",
     volume    = "57",
     year      = "1998",
     pages     = "1864-1872",
}

@Article{AOL92,
     author    = "U. Albrecht and A. Otto and P. Leiderer",
     title     = "Two-dimensional liquid polymer diffusion: experiment and
                      simulation",
     journal   = "Phys. Rev. Lett.",
     volume    = "68",
     year      = "1992",
     pages     = "3192-3195",
}

@Book{AT87,
     author    = "M. Allen and D. Tildesley",
     title     = "Computer simulations of liquids",
     Publisher = "Clarendon, New York",
     year      = "1987"
}

@Book{AL65,
     author    = "H. Ashley and M. Landahl",
     title     = "Aerodynamics of Wings and Bodies",
     Publisher = "Addison-Wesley, Reading, Mass.",
     year      = "1965"
}

@Article{APL86,
     author    = "D. Ausserre and A. M. Picard and L. L{\'e}ger",
     title     = "Existence and Role of the Precursor Film in
               the Spreading of Polymer Liquids",
     journal   = "Phys. Rev. Lett.",
     volume    = "57",
     year      = "1986",
     pages     = "2671-2674",
}

@Article{BB99,
     author    = "J.-L. Barrat and L. Bocquet",
     title     = "Large slip effect at a nonwetting fluid-solid interface",
     journal   = "Phys. Rev. Lett.",
     volume    = "82",
     year      = "1999",
     pages     = "4671-4674",
}

@Article{Duprat2012,
     author    = "C. Duprat and A. Y. Bebee and S. Protiere and H. A. Stone",
     title     = "Wetting of flexible fibre arrays",
     journal   = "Nature",
     volume    = "482",
     year      = "2012",
     pages     = "510-513",
}

@Article{CAR12,
     author    = "A. Carlson and G. Bellani and G. Amberg",
     title     = "Universality in dynamic wetting dominated by contact line friction",
     journal   = "Phys. Rev. E.",
     volume    = "85",
     year      = "2012",
     pages     = "045302",
}

@Article{Lui2015,
     author    = "C. Liu and Y. Xue and Y. Chen and Y. Zheng",
     title     = "Effective directional self-gathering of drops on spine of cactus with splayed capillary arrays",
     journal   = "Sci. Rep.",
    volume    = "5",
    year      = "2015",
    pages     = "17757",
}

@Article{BC96,
     author    = "I. B. Bazhlekov and A. K. Chesters",
     title     = "Numerical investigation of the dynamic influence of the
contact line region on the macroscopic meniscus shape",
     journal   = "J. Fluid Mech.",
     volume    = "329",
     year      = "1996",
     pages     = "137-146",
}

@Inproceedings{BCS64,
     author    = "W. D. Bascom and R. Cottington and C. Singleterry",
     title     = "Dynamic Surface Phenomena in the Spontaneous Spreading of
                  Oils on Solids",
     year      = "1964",
     booktitle = "Contact angle, wettability, and adhesion",
     editor    = "F. M. Fowkes",
     pages     = "355",
     Publisher = "American Chemical Society, Washington D.C.",
}

@Article{B89,
     author    = "D. Beaglehole",
     title     ="Profiles of the Precursor of Spreading
      Drops of Siloxane Oil on Glass, Fused Silica, and Mica",
     journal   = "J. Phys. Chem.",
     volume    = "93",
     year      = "1989",
     pages     = "893-899",
}

@Article{BGSMJMB03,
     author    = "J. Becker and G. Gr{\"u}n and R. Seemann and
            H. Mantz and K. Jacobs and K. R. Mecke and R. Blossey",
     title     = "Complex dewetting scenarios captured by thin-film models",
     journal   = "Nature Mat.",
     volume    = "2",
     year      = "2003",
     pages     = "59",
}

@Article{RMWB05,
     author    = "M. Rauscher and A. M{\"u}nch and B. Wagner and R. Blossey",
     title     = "A thin-film equation for viscoelastic liquids of
                   Jeffreys type ",
     journal   = "Eur. Phys. J. E",
     volume    = "17",
     year      = "2005",
     pages     = "373",
}
@Article{FJMWW05,
     author    = "R. Fetzer and K. Jacobs and A. M{\"u}nch and B. Wagner
              and T. P. Witelski",
     title     = "New slip regimes and the shape of dewtting thin liquid
                  films",
     journal   = "Phys. Rev. Lett.",
     volume    = "95",
     year      = "2005",
     pages     = "127801",
}
@Article{MWW05,
     author    = "A. M{\"u}nch and B. Wagner and T. P. Witelski",
     title     = "Lubrication models with small slip lengths",
     journal   = "J. Engin. Math.",
     volume    = "53",
     year      = "2005",
     pages     = "359",
}
@Article{VR05,
     author    = "T. Vilmin and E. Rapha{\"e}l",
     title     = "Dewetting of thin viscoelastic polymer films on
                     slippery substrates",
     journal   = "Europhys. Lett.",
     volume    = "72",
     year      = "2005",
     pages     = "781",
}
@Article{VRDSGHR06,
     author    = "T. Vilmin and E. Rapha{\"e}l and P. Damman and S. Sclavons
                   and S. Gabriele and M. Hamieh and G. Reiter",
     title     = "The role of nonlinear friction in the dewetting
                     of thin polymer films",
     journal   = "Europhys. Lett.",
     volume    = "73",
     year      = "2006",
     pages     = "906",
}
@Article{DBR06,
     author    = "P. Damman and N. Baudelet and G. Reiter",
     title     = "Dewetting near the Glass Transition: Transition
       from a Capillary Force Dominated to a Dissipation Dominated Regime",
     journal   = "Phys. Rev. Lett.",
     volume    = "91",
     year      = "2003",
     pages     = "216101",
}
@Article{GMR06,
     author    = "G. Gr{\"u}n and K. R. Mecke and M. Rauscher",
     title     = "Thin-film flow influenced by thermal noise",
     journal   = "J. Stat. Phys.",
     volume    = "122",
     year      = "2006",
     pages     = "1261",
}
@Article{MR05,
     author    = "K. R. Mecke and M. Rauscher",
     title     = "On thermal fluctuations in thin film flow",
     journal   = "J. Phys.: Condensed Matter",
     volume    = "17",
     year      = "2005",
     pages     = "S3515",
}
@Article{MWRB06,
     author    = "A. M{\"u}nch and B. Wagner and M. Rauscher and R. Blossey",
     title     = "A thin-film model for corotational Jeffreys fluids
                under strong slip",
     journal   = "Eur. Phys. J. E",
     volume    = "20",
     year      = "2006",
     pages     = "365",
}
@Article{JKMWW05,
     autor     = "K. Jacobs and R. Konrad and A. M{\"u}nch and
                T.  Witelski and B. Wagner",
     title     = " New slip regimes and the shape of dewetting
                thin liquid films",
     journal   = "Phys. Rev. Lett.",
     volume    = "95",
     year      = "2005",
     pages     = "1278016",
}
@Article{DMS05,
     author    = "B. Davidovitch and E. Moro and H. A. Stone",
     title     = "Spreading of viscous fluid drops on a solid substrate
                   assisted by thermal fluctuations",
     journal   = "Phys. Rev. Lett.",
     volume    = "95",
     year      = "2005",
     pages     = "244505",
}
@Article{ Blossey,
     author    = "R. Blossey and T. Kinoshita and J. Dupont-Roc",
     title     = "Random-field Ising model for the hysteresis of
  the prewetting transition on a disordered substrate",
     journal   = "Physica A",
     volume    = "248",
     year      = "1998",
     pages     = "247-272",
}
@Article{Bausch,
     author    = " R. Blossey",
     title     = "Nucleation at first-order wetting transitions",
     journal   = "Int. J. Mod. Phys.",
     volume    = "9",
     year      = "1995",
     pages     = "3489-3525",
}

@Article{BKVE96,
     author    = "S. Bekink and S. Karaborni and G. Verbist and K. Esselink",
     title     = "Simulating the spreading of a drop in the
                  terraced wetting regime. ",
     journal   = "Phys. Rev. Lett.",
     volume    = "76",
     year      = "1996",
     pages     = "3766",
}

@Article{BCP03,
     author    = "M. {Ben Amar} and L. J. Cummings and Y. Pomeau",
     title     = "Transition of a moving contact line from smooth to angular",
     journal   = "Phys. Fluids",
     volume    = "15",
     year      = "2003",
     pages     = "2949-2960",
}

@Article{BC01,
     author    = "M. {Ben Amar} and L. J. Cummings",
     title     = "Fingering instabilities in driven thin nematic films",
     journal   = "Phys. Fluids",
     volume    = "13",
     year      = "2001",
     pages     = "1160-1166",
}

@Article{BT80,
     author    = "D. J. Benney and W. J.  Timson",
     title     = "The rolling motion of a viscous fluid on
                      and off a rigid surface",
     journal   = "Stud.  Appl. Maths.",
     volume    = "63",
     year      = "1980",
     pages     = "93-98",
}

@Article{Mull57,
     author    = "W. W. Mullins",
     title     = "???",
     journal   = "J. Appl. Phys.",
     volume    = "28",
     year      = "1957",
     pages     = "333",
      }

@Article{Mull59,
     author    = "W. W. Mullins",
     title     = "???",
     journal   = "J. Appl. Phys.",
     volume    = "30",
     year      = "1959",
     pages     = "77",
      }

@Article{NM65,
     author    = "F. A. Nichols and W. W. Mullins",
     title     = "Morphological Changes of a Surface of Revolution
               due to Capillarity-Induced Surface Diffusion",
     journal   = "J. Appl. Phys.",
     volume    = "36",
     year      = "1965",
     pages     = "1826",
      }

@Article{IGRBE07,
     author    = "R. Ishiguro and F. Graner and E. Rolley and S. Balibar
                       and J. Eggers",
     title     = "Dripping of a crystal",
     journal   = "Phys. Rev. E",
     volume    = "75",
     year      = "2007",
     pages     = "041606",
      }

@Article{Balibar:2005,
     author    = "S. Balibar and H. Alles and A. Y. Parshin",
     title     = "???",
     journal   = "Rev. Mod. Phys.",
     volume    = "77",
     year      = "2005",
     pages     = "317",
}

@Book{MB02,
     author    = "A. J. Majda and A. L. Bertozzi",
     title     = "Vorticity and Incompressible Flow",
     publisher = {Cambridge University Press, Cambridge},
     year      = "2002",
}

@Article{BMFC98,
     author    = "A. L. Bertozzi and A. Munch and X. Fanton and A.-M. Cazabat",
     title     = "Contact line stability and ``undercompressive shocks''
                  in a driven thin film flow",
     journal   = "Phys. Rev. Lett.",
     volume    = "81",
     year      = "1998",
     pages     = "5169-5172",
}

@Article{BBW98,
     author    = "A. J. Bernoff and A. L. Bertozzi and T. P. Witelski",
     title     = "Axisymmetric surface diffusion: Dynamics and
             stability of self-similar pinch-off",
     journal   = "J. Stat. Phys.",
     volume    = "93",
     year      = "1998",
     pages     = "725-776",
}

@Article{BW98,
     author    = "M. P. Brenner and T. P. Witelski",
     title     = "On spherically symmetric gravitational collapse",
     journal   = "J. Stat. Phys.",
     volume    = "93",
     year      = "1998",
     pages     = "863",
}

@Article{VLW01a,
     author    = "D. Vaynblat and J. R. Lister and T. P. Witelski",
     title     = "Symmetry and self-similarity in rupture and pinchoff:
            A geometric bifurcation",
     journal   = "Eur. J. Appl. Math.",
     volume    = "12",
     year      = "2001",
     pages     = "209-232",
}

@Article{VLW01b,
     author    = "D. Vaynblat and J. R. Lister and T. P. Witelski",
     title     = "Rupture of Thin Viscous Films by van der Waals Forces:
                    Evolution and Self-similarity",
     journal   = "Phys. Fluids",
     volume    = "13",
     year      = "2001",
     pages     = "1130-1140",
}

@Article{MSTT00,
     author    = "I. Mizushima and T. Sato and S. Taniguchi
                and Y. Tsunashima",
     title     = "Empty-space-in-silicon technique for fabricating
                        a silicon-on-nothing structure",
     journal   = "Appl. Phys. Lett.",
     volume    = "77",
     year      = "2000",
     pages     = "3290-3292",
}

@Article{BB97,
     author    = "A. L. Bertozzi and M. P. Brenner",
     title     = "Linear stability and transient growth in
                driven contact lines",
     journal   = "Phys. Fluids",
     volume    = "9",
     year      = "1997",
     pages     = "530",
}

@Article{BMS99,
     author    = "A. L. Bertozzi and A. Munch and M. Shearer",
     title     = "Undercompressive shocks in thin film flows",
     journal   = "Physica D",
     volume    = "134",
     year      = "1999",
     pages     = "431-464",
}

@Article{BertrandPRL,
     author    = "E. Bertrand and H. Dobbs and
        D. Broseta and J. O. Indekeu and D. Bonn and  J. Meunier",
     title     = "First-order and critical wetting of alkanes ",
     journal   = "Phys. Rev. Lett.",
     volume    = "85",
     year      = "2000",
     pages     = "1282"
}
@Article{Bertrand,
     author    = "E. Bertrand and D. Bonn and D. Broseta and H. Dobbs
             and J. O. Indekeu and J. Meunier and K. Ragil and
                N. Shahidzadeh",
     title     = "Wetting of alkanes on water",
     journal   = "J. Petrol. Sci. Eng.",
     volume    = "33",
     year      = "2002",
     pages     = "217"
}
@Article{IndekeuJSP,
     author    = "J. O. Indekeu and K. Ragil and D. Bonn and D. Broseta
                  and J. Meunier",
     title     = "Wetting of alkanes on water from a Cahn-type theory:
          Effects of long-range forces ",
     journal   = "J. Stat. Phys.",
     volume    = "95",
     year      = "1999",
     pages     = "1009-1043"
}
@Article{ ragilJCP,
     author    = " K. Ragil and D. Bonn and D. Broseta and J. Meunier",
     title     = " Wetting of alkanes on water from a Cahn-type theory",
     journal   = "J. Chem. Phys.",
     volume    = "105",
     year      = "1996",
     pages     = "5160"
}
@Article{ joseph,
     author    = " J. O. Indekeu",
     title     = " Introduction to Wetting Phenomena",
     journal   = "Acta Physica Polonica",
     volume    = "26",
     year      = "1995",
     pages     = "1065"
}
@Article{ josephPS,
     author    = " J. O. Indekeu",
     title     = "Wetting and adsorption at substrates and grain boundaries",
     journal   = "Physica Scripta",
     volume    = "T35",
     year      = "1991",
     pages     = "31-33"
}
@Article{ kellayfluc,
     author    = "  H. Kellay and J. Meunier and B. P. Binks",
     title     = " Wetting properties of n-alkanes on AOT monolayers
                at the brine-air interface",
     journal   = "Phys. Rev. Lett.",
     volume    = "69",
     year      = "1992",
     pages     = "1220"
}
@Article{ helfrich1,
     author    = " W. Helfrich",
     title     = " Steric interaction of fluid membranes in
                     multilayer systems",
     journal   = "Z. Naturforsch. A",
     volume    = "33",
     year      = "1978",
     pages     = "305"
}
@Article{ helfrich2,
     author    = " W. Helfrich and R.-M. Servuss",
     title     = " Undulations, steric interaction and cohesion of fluid
                     membranes",
     journal   = "Nuovo Cimento D",
     volume    = "3",
     year      = "1984",
     pages     = "137"
}
@Article{ hill,
     author    = " R. M. Hill",
     title     = " Superspreading",
     journal   = "Curr. Opin. Coll. Interf. Sci.",
     volume    = "3",
     year      = "1998",
     pages     = "247"
}
@Article{ salicasi,
     author    = " S. Rafa{\"\i} and D. Bonn and J. Meunier",
     title     = " ????",
     journal   = "to be published",
     year      = "2006",
}
@Article{ monkrech,
     author    = " M. Krech",
     title     = "Casimir forces in binary liquid mixtures ",
     journal   = "Phys. Rev. E",
     volume    = "56",
     year      = "1997",
     pages     = "1642"
}
@Book{ KrechBook,
     author    = "M. Krech",
     title     = "The Casimir effect in critical systems",
     Publisher = "World Scientific, Singapore",
     year      = "1994",
}
@Article{ krechdietrich,
     author    = " M. Krech and S. Dietrich",
     title     = "Finite-size scaling for critical films",
     journal   = "Phys. Rev. Lett.",
     volume    = "66",
     year      = "1991",
     pages     = "345"
}
@Article{ casimir,
     author    = " H. B. G. Casimir",
     title     = " On the attraction between two perfectly conducting plates",
     journal   = "Proc. K. Ned. Akad. Wet.",
     volume    = " 51",
     year      = "1948",
     pages     = "793"
}
@Article{ josephcasi,
     author    = " J. O. Indekeu and M. P. Nightingale and W. V. Wang",
     title     = " Finite-size interaction amplitudes and their
         universality: Exact, mean-field, and renormalization-group results",
     journal   = "Phys. Rev. B",
     volume    = " 34",
     year      = "1986",
     pages     = "330"
}
@Article{ NighInd,
     author    = " M. P. Nightingale and J. O. Indekeu",
     title     = " Effect of criticality on wetting layers",
     journal   = "Phys. Rev. Lett.",
     volume    = " 54",
     year      = "1985",
     pages     = "1824"
}

@Article{ garcia,
     author    = " R. Garcia and M. H. W. Chan",
     title     = " Critical Fluctuation-Induced Thinning of He-4 Films
            near the Superfluid Transition",
     journal   = "Phys. Rev. Lett.",
     volume    = " 83",
     year      = "1999",
     pages     = "1187"
}
@Article{ garcia2,
     author    = " R. Garcia and M. H. W. Chan",
     title     = "Critical Casimir effect near the He-3-He-4
                     tricritical point ",
     journal   = "Phys. Rev. Lett.",
     volume    = " 88",
     year      = "2002",
     pages     = "086101"
}
@Article{ pershan,
     author    = " M. Fukuto and Y. F. Yano and P. S. Pershan",
     title     = " Critical Casimir effect in three-dimensional Ising
              systems: Measurements on binary wetting films",
     journal   = "Phys. Rev. Lett.",
     volume    = " 94",
     year      = "2005",
     pages     = "135702"
}
@Article{ zisman2,
     author    = " K. G. Kabza and J. E. Gestwicki and J. L. J. McGrath",
     title     = " Contact angle goniometry as a tool for surface
            tension measurements of solids, using Zisman Plot method.
                A Physical Chemistry experiment",
     journal   = "J. Chem. Educ.",
     volume    = " 77",
     year      = "2000",
     pages     = "63",
}
@Article{ lipo,
     author    = " R. Lipowsky",
     title     = " Upper critical dimension for wetting in systems with
                long-range forces",
     journal   = "Phys. Rev. Lett.",
     volume    = " 52",
     year      = "1984",
     pages     = "1429",
}
@Article{ lipo2,
     author    = " R. Lipowsky",
     title     = " ????",
     journal   = "Phys. Rev. B",
     volume    = " 32",
     year      = "1985",
     pages     = "1731",
}
@Article{ lipofisher,
     author    = " R. Lipowsky and M. E. Fisher",
     title     = " Scaling regimes and functional renormalization
                for wetting transitions",
     journal   = "Phys. Rev. B",
     volume    = " 36",
     year      = "1987",
     pages     = "2126",
}
@Article{ FisherReview,
     author    = " M. E. Fisher",
     title     = "Interface wandering in adsorbed and bulk phases, pure
              and impure ",
     journal   = "J. Chem. Soc. Faraday Trans.",
     volume    = " 282",
     year      = "1986",
     pages     = "1569",
}
@Article{ quereROP,
     author    = " D. Qu{\'e}r{\'e}",
     title     = " Non-sticking drops",
     journal   = "Rep. Prog. Phys.",
     volume    = " 68",
     year      = "2005",
     pages     = "2495",
}
@Article{ onda,
     author    = " T. Onda and N. Shibuichi and N. Satoh and K. Tsuji",
     title     = " Super-water-repellent fractal surfaces",
     journal   = "Langmuir",
     volume    = " 12",
     year      = "1996",
     pages     = "2125",
}
@Article{ naka,
     author    = " A. Nakajami and K. Hashimoto and T. Watanabe and
       K. Takai and G. Yamouchi and A. Fujishima",
     title     = " Transparent superhydrophobic thin films with
              self-cleaning properties",
     journal   = "Langmuir",
     volume    = " 16",
     year      = "2000",
     pages     = "7044",
}
@Article{ B03,
     author    = " R. Blossey",
     title     = " Self-cleaning surfaces-virtual realities",
     journal   = "Nature Mater.",
     volume    = " 2",
     year      = "2003",
     pages     = "301",
}
@Article{ cottin,
     author    = " C. Cottin-Bizonne and J.-L. Barrat and L. Boquet and
           E. Charlaix",
     title     = " Low-friction flows of liquid at nanopatterned interfaces",
     journal   = " Nature Mater.",
     volume    = " 2",
     year      = "2003",
     pages     = "237",
}
@Article{ journet,
     author    = " C. Journet and S. Moulinet and C. Ybert and
       S. Purcell and L. Bocquet",
     title     = " ????",
     journal   = " Europhys. Lett.",
     volume    = " 71",
     year      = " 2005",
     pages     = " 104-109",
}
@Article{ DYCB07,
     author    = " C. Duez and C. Ybert and C. Clanet and L. Bocquet",
     title     = " Making a splash with water repellency",
     journal   = " Nat. Phys.",
     volume    = " 3",
     year      = " 2007",
     pages     = " 180",
}
@Article{ Esmall,
     author    = " J. Eggers",
     title     = " Coupling the large and the small",
     journal   = " Nat. Phys.",
     volume    = " 3",
     year      = " 2007",
     pages     = " 145",
}

@Article{ CouderNature,
     author    = "Y. Couder and S. Proti{\`e}re and E. Fort and A. Boudaoud",
     title     = " Walking and orbiting droplets",
     journal   = " Nature",
     volume    = " 437",
     year      = " 2005",
     pages     = " 208",
}

@Article{ Gilet07,
     author    = "T. Gilet and N. Vandewalle and S. Dorbolo",
     title     = " Controlling the partial coalescence of a droplet
                on a vertically vibrated bath",
     journal   = " Phys. Rev. E",
     volume    = " 76",
     year      = " 2007",
     pages     = " 035302(R)"
}

@Article{ Yacine01,
     author    = " Y. Amarouchene and G. Cristobal and H. Kellay",
     title     = " Noncoalescing Drops",
     journal   = " Phys. Rev. Lett.",
     volume    = " 95",
     year      = " 2001",
     pages     = " 164504"
}

@Article{ bartolo,
     author    = " D. Bartolo and F. Bouamrirene and E. A. Buguin
          and P. Silberzan and S. Moulinet",
     title     = " Bouncing or sticky droplets: Impalement
          transitions on superhydrophobic micropatterned surfaces ",
     journal   = " Europhys. Lett.",
     volume    = " 74",
     year      = " 2006",
     pages     = " 299",
}
@Article{petrole,
     author    = "E. Bertrand and D. Bonn and D. Broseta and N. Shahidzadeh
          and K. Ragil and H. Dobbs and J. O. Indekeu and J. Meunier",
     title     = "Wetting of alkanes on water",
     journal   = "J. Petrol. Sci. Eng.",
     volume    = "33",
     year      = "2002",
     pages     = "217",
}

@Article{ BN01,
     author    = " M. Bestehorn and K. Neuffer",
     title     = "Surface patterns of laterally extended thin liquid films
in three dimensions ",
     journal   = " Phys. Rev. Lett.",
     volume    = " 87",
     year      = " 2001",
     pages     = " 046101",
}
@Article{ binder1,
     author    = " K. Binder and D. P. Landau",
     title     = " Wetting layering in the nearest-neighbor simple-cubic
              Ising lattice - a Monte-Carlo investigation",
     journal   = " Phys. Rev. B",
     volume    = " 37",
     year      = " 1988",
     pages     = " 1745-1765",
}

@Article{ binder2,
     author    = " K. Binder and D. P. Landau and D. M. Kroll",
     title     = " Critical wetting with short-range forces
                  - is mean-filed theory valid ?",
     journal   = " Phys. Rev. Lett. ",
     volume    = " 56",
     year      = " 1986",
     pages     = " 2272",
}
@Article{ binder3,
     author    = " K. Binder and D. P. Landau and S. Wansleben",
     title     = " Wetting transitions near the bulk critical point-
                  Monte-Carlo simulations for the Ising model",
     journal   = " Phys. Rev. B",
     volume    = " 40",
     year      = " 1989",
     pages     = " 6971-6979",
}
@Article{ BMQ99,
     author    = " J. Bico and C. Marzolin and D. Qu\'{e}r\'{e}",
     title     = " Pearl drops",
     journal   = " Europhys. Lett.",
     volume    = " 47",
     year      = " 1999",
     pages     = " 220-226",
}

@Article{ BCQ03,
     author    = " A.-L. Biance and C. Clanet and D. Qu\'{e}r\'{e}",
     title     = " First steps of the spreading of a liquid droplet",
     journal   = " Phys. Rev. E",
     volume    = " 69",
     year      = " 2004",
     pages     = " 016301",
}

@Article{ Bico,
     author    = " J. Bico and C. Tordeux and D. Qu\'{e}r\'{e}",
     title     = " Rough wetting",
     journal   = " Europhys. Lett.",
     volume    = " 55",
     year      = " 2001",
     pages     = " 214-220",
}

@Article{ BSHL96,
     author    = " J. Bischof and D. Scherer and S. Herminghaus
           and P. Leiderer",
     title     = " Dewetting modes of thin metallic films: nucleation of
holes and spinodal dewetting",
     journal   = " Phys. Rev. Lett.",
     volume    = " 77",
     year      = " 1996",
     pages     = " 1536",
}

@Inproceedings{ Blake93,
     author    = " T. D. Blake",
     title     = " Dynamic contact angles and wetting kinetics",
     pages     = " 251-309",
     year      = " 1993",
     Booktitle = " Wettability",
     editor    = " J. Berg.",
     volume    = " 49",
     publisher = " New York, Marcel Dekker",
}

@Article{ Blake06,
     author    = " T. D. Blake",
     title     = " The physics of moving wetting lines",
     year      = " 2006",
     journal   = " J. Colloid Inter. Sci.",
     volume    = " 299",
     pages     = " 1--13",
}

@Article{ BH69,
     author    = " T. D. Blake and J. M. Haynes",
     title     = " Kinetics of Liquid/Liquid Displacement",
     journal   = " J. Colloid Interface Sci.",
     volume    = " 30",
     year      = " 1969",
     pages     = " 421-423",
}

@Article{ BD02,
     author    = " T. D. Blake and J. {De Coninck}",
     title     = " The influence of
             solid-liquid interactions on dynamic wetting",
     journal   = " Adv. Colloid Interface Sci.",
     volume    = " 96",
     year      = " 2002",
     pages     = " 21-36",
}

@Article{ BS02,
     author    = " T. D. Blake and Y. D. Shikhmurzaev",
     title     = " Dynamic Wetting by Liquids of Different Viscosity",
     journal   = " Colloid Interface Sci.",
     volume    = " 253",
     year      = " 2002",
     pages     = " 196-202",
}

@Article{ BBS99,
     author    = " T. D. Blake and M. Bracke and Y. D. Shikhmurzaev",
     title     = " Experimental evidence of nonlocal hydrodynamic
               influence on the dynamic contact angle",
     journal   = " Phys. Fluids",
     volume    = " 11",
     year      = " 1999",
     pages     = " 1995-2007",
}

@Article{ BR79,
     author    = " T. D. Blake and K. J. Ruschak",
     title     = " A maximum speed of wetting.",
     journal   = " Nature",
     volume    = " 282",
     year      = " 1979",
     pages     = " 489-491",
}

@Inproceedings{ BR97,
     author    = " T. D. Blake and K. J. Ruschak",
     title     = " Wetting: static and dynamic contact lines",
     year      = " 1997",
     booktitle = " Liquid film coating",
     editor    = " S. F. Kistler and P. M. Schweizer",
     publisher  = " London, Chapman and Hall",
}

@Article{ BL37,
     author    = " K. B. Blodgett and I. Langmuir",
     title     = " Built-Up Films of Barium Stearate and
             Their Optical Properties",
     journal   = " Nature",
     volume    = " 282",
     year      = " 1937",
     pages     = " 489-491",
}

@Article{ Bonn2000,
     author    = " D. Bonn and E. Bertrand and J. Meunier and R. Blossey",
     title     = " Dynamics of wetting layer formation",
     journal   = " Phys. Rev. Lett.",
     volume    = " 84",
     year      = " 2000",
     pages     = " 4661",
}

@Article{ Bonn1994,
     author    = " D. Bonn and H. Kellay and J. Meunier",
     title     = " Metastable states and nucleation near
                  first-order wetting transitions",
     journal   = " Phys. Rev. Lett.",
     volume    = " 73",
     year      = " 1994",
     pages     = " 3560",
}

@Article{ Bonn1992,
     author    = " D. Bonn and H. Kellay and G. H. Wegdam",
     title     = " Experimental observation of
               hysteresis in a wetting transition ",
     journal   = " Phys. Rev. Lett.",
     volume    = " 69",
     year      = " 1992",
     pages     = " 1975",
}
@Article{ Findenegg,
     author    = " G. H. Findenegg and R. L{\"o}ring",
     title     = "Fluid adsorption up to the critical point.
         Experimental study of a wetting fluid/solid interface ",
     journal   = " J. Chem. Phys.",
     volume    = " 81",
     year      = " 1984",
     pages     = " 3270",
}

@Article{ B97,
     author    = " C. J. Boulter",
     title     = " When is short-range ''critical wetting not critical?",
     journal   = " Phys. Rev. Lett.",
     volume    = " 79",
     year      = " 1997",
     pages     = " 1897-1900",
}

@Article{ BB93,
     author    = " M. P. Brenner and A. L. Bertozzi",
     title     = " Spreading of Droplets on a Solid Surface",
     journal   = " Phys. Rev. Lett.",
     volume    = " 71",
     year      = " 1993",
     pages     = " 593-596",
}

@Article{ BHL83a,
     author    = " E. Br\'ezin and B. I. Halperin and S. Leibler",
     title     = " Critical wetting in 3 dimensions",
     journal   = " Phys. Rev. Lett.",
     volume    = " 50",
     year      = " 1983",
     pages     = " 1387-1390",
}
@Article{ BHL83b,
     author    = " E. Br\'ezin and B. I. Halperin and S. Leibler",
     title     = "Critical wetting : the domain of validity of mean
                  field theory",
     journal   = " J. Physique (Paris)",
     volume    = " 44",
     year      = " 1983",
     pages     = " 775-783",
}

@Article{ BWY04,
     author    = " A. J. Briant and A. J. Wagner and J. M. Yeomans",
     title     = " Lattice boltzmann simulations of contact line
               motion. I.Liquid-gas systems",
     journal   = " Phys. Rev. E",
     volume    = " 69",
     year      = " 2004",
     pages     = " 031602",
}

@Article{ BY04,
     author    = " A. J. Briant and J. M. Yeomans",
     title     = " Lattice boltzmann simulations of contact line
               motion. II.Binary fluids",
     journal   = " Phys. Rev. E",
     volume    = " 69",
     year      = " 2004",
     pages     = " 031603",
}

@Article{ BD90,
     author    = " F. Brochard-Wyart and J. Daillant",
     title     = " Drying of solids wetted by thin liquid films",
     journal   = " Can. J. Phys.",
     volume    = " 68",
     year      = " 1990",
     pages     = " 1084",
}

@Article{ BMQG91,
     author    = " F. Brochard-Wyart and J.-M. di Meglio and
                    D. Qu\'{e}r\'{e} and P.-G. {de Gennes}",
     title     = " Spreading of nonvolatile liquids in a continuum picture",
     journal   = " Langmuir",
     volume    = " 7",
     year      = " 1991",
     pages     = " 335-338",
}

@Article{ BMQ87,
     author    = " F. Brochard-Wyart and J.-M. di Meglio and
                    D. Qu\'{e}r\'{e} ",
     title     = " Dewetting - Growth of dry regions from a film covering
                     a flat solid or a fiber",
     journal   = " C. R. Acad. Sc. Paris S{\'e}rie II",
     volume    = " 304",
     year      = " 1987",
     pages     = " 553-558",
}

@Article{ dG86,
     author    = " P.-G. {de Gennes}",
     title     = " Transformation process for a horizontal soap film",
     journal   = " C. R. Acad. Sc. Paris S{\'e}rie II",
     volume    = " 303",
     year      = " 1986",
     pages     = " 1275-1277",
}

@Article{ FG78,
     author    = " M. E. Fisher and P.-G. {de Gennes}",
     title     = " Wall phenomena in a critical binary mixture",
     journal   = " C. R. Acad. Sci. Paris",
     volume    = " 287",
     year      = " 1978",
     pages     = " 207-209",
}

@Article{ BG92,
     author    = " F. Brochard-Wyart and P.-G. {de Gennes}",
     title     = " Dynamics of partial wetting",
     journal   = " Adv. Colloid Interface Sci.",
     volume    = " 39",
     year      = " 1992",
     pages     = " 1-11",
}

@Article{ DB93,
     author    = " R. A. de Bruijn",
     title     = " Tip streaming of drops in simple shear flows",
     journal   = " Chem. Eng. Sci.",
     volume    = " 48",
     year      = " 1993",
     pages     = " 277-284",
}

@Article{ B92,
     author    = " J. R. {de Bruyn}",
     title     = " Finger instability of a gravitationally
                 driven contact line",
     journal   = " Phys. Rev. A",
     volume    = " 46",
     year      = " 1992",
     pages     = " R4500",
}

@Article{ BBR92,
     author    = " J. B. Brzoska and F. Brochart-Wyart and F. Rondelez",
     title     = " Exponential growth of fingering instabilities
              of spreading films under horizontal thermal gradients",
     journal   = " Europhys. Lett.",
     volume    = " 19",
     year      = " 1992",
     pages     = " 97",
}

@Article{ BHM03,
     author    = " J. Buehrle and S. Herminghaus and F. Mugele",
     title     = " Interface profiles near three-phase contact
                lines in electric fields",
     journal   = " Phys. Rev. Lett.",
     volume    = " 91",
     year      = " 2003",
     pages     = " 086101",
}

@Article{ BOCM96,
     author    = " S. F. Burlatsky and G. Oshanin and A.-M. Cazabat
                and M. Moreau",
     title     = " Microscopic model of upward creep of an
                   ultrathin wetting film",
     journal   = " Phys. Rev. Lett.",
     volume    = " 76",
     year      = " 1996",
     pages     = " 86-89",
}

@Article{ BK76a,
     author    = " R. Burley and B. S. Kennedy",
     title     = " A study of the dynamic wetting behavior of polyester tapes",
     journal   = " Brit. Polym. J.",
     volume    = " 8",
     year      = " 1976",
     pages     = " 140-143",
}

@Article{ BK76b,
     author    = " R. Burley and B. S. Kennedy",
     title     = " An experimental study of air entrainment
               at a solid/liquid/gas interface",
     journal   = " Chem. Eng. Sci.",
     volume    = " 31",
     year      = " 1976",
     pages     = " 901-911",
}

@Article{ Ben07,
     author    = " H. Benkreira and M. I. Khan",
     title     = " Air entrainment in dip coating under reduced air pressures",
     journal   = " Chem. Eng. Sci.",
     volume    = " 63",
     year      = " 2008",
     pages     = " 448-459",
}
@Article{ Ben10,
     author    = " H. Benkreira and J. B. Ikin",
     title     = " Dynamic wetting and gas viscosity effects",
     journal   = " Chem. Eng. Sci.",
     volume    = " 65",
     year      = " 2010",
     pages     = " 1790-1796",
}



@Inproceedings{ BK78,
     author    = " R. Burley and B. S. Kennedy",
     title     = " Dynamic Wetting and Air Entrainment
                          at a Liquid-Solid-Gas Junction",
     year      = " 1978",
     booktitle = " Wetting, Spreading and Adhesion",
     editor    = " J. F. Padday",
     pages      = "327",
     publisher = " Academic Press, London",
}

@Article{ Cahn,
     author    = " J. W. Cahn",
     title     = " Critical Point Wetting",
     journal   = " J. Chem. Phys.",
     volume    = " 66",
     year      = " 1977",
     pages     = " 3667",
}

@Article{ Moldover,
     author    = " M. R. Moldover and J. W. Cahn",
     title     = " Interface phase transition - complete to partial wetting",
     journal   = " Science",
     volume    = " 207",
     year      = " 1980",
     pages     = " 1073-1075",
}

@Article{ M85,
     author    = " M. R. Moldover",
     title     = " Interfacial tension of fluids near critical points and
                  2-scale-factor universality",
     journal   = " Phys. Rev. A",
     volume    = " 31",
     year      = " 1985",
     pages     = " 1022-1033",
}

@Article{ heady,
     author    = " R. B. Heady and J. W. Cahn",
     title     = " Experimental test of classical nucleation theory
                in a liquid-liquid miscibility gap system ",
     journal   = " J. Chem. Phys.",
     volume    = " 58",
     year      = " 1973",
     pages     = " 896",
}

@Article{ CC86,
     author    = " A.-M. Cazabat and M. A. Cohen-Stuart",
     title     = " Dynamics of Wetting: Effects of Surface Roughness",
     journal   = " J. Phys. Chem.",
     volume    = " 90",
     year      = " 1986",
     pages     = " 5845-5849",
}

@Article{ CHTC90,
     author    = " A.-M. Cazabat and F. Heslot and S. M. Troian and P. Carles",
     title     = " Fingering instability of thin films
                    driven by temperature gradients",
     journal   = " Nature",
     volume    = " 346",
     year      = " 1990",
     pages     = " 824-826",
}

@Article{ CHCT92,
     author    = " A.-M. Cazabat and F. Heslot and P. Carles and S. M. Troian",
     title     = " Hydrodynamic fingering instability of driven wetting films",
     journal   = " Colloid Interface Sci.",
     volume    = " 39",
     year      = " 1992",
     pages     = " 61",
}

@Article{ CFHC92,
     author    = " A.-M. Cazabat and N. Fraysse and F. Heslot and P. Carles",
     title     = " Spreading at the microscopic scale",
     journal   = " J. Phys. Chem.",
     volume    = " 94",
     year      = " 1992",
     pages     = " 7581-7585",
}

@Article{ CGVV97,
     author    = " A.-M. Cazabat and S. Gerdes and
                    M. P. Valignat and S. Villette",
     title     = " Dynamics of wetting: from theory to experiment",
     journal   = " Interf. Sci.",
     volume    = " 5",
     year      = " 1997",
     pages     = " 129-139",
}
@Article{ VFCHL93,
     author    = "M. P. Valignat and N. Fraysse and A.-M. Cazabat and
                   F. Heslot and P. Levinson",
     title     = " An ellipsometric study of layered droplets",
     journal   = " Thin Solid Films",
     volume    = " 234",
     year      = " 1993",
     pages     = " 475-477",
}

@Article{ Chauve01,
     author    = " P. Chauve  and P. {Le Doussal} and  K. J. Wiese",
     title     = " Renormalization of pinned elastic system:
            how does it work beyond one loop ?",
     journal   = " Phys. Rev. Lett.",
     volume    = " 86",
     year      = " 2001",
     pages     = " 1785-1788",
}
@Article{ MBK82,
     author    = " S. R. McKay and A. N. Berker and S. Kirkpatrick",
     title     = " Spin-glass behavior in frustrated Ising models with
         chaotic renormalization-group trajectories",
     journal   = " Phys. Rev. Lett.",
     volume    = " 48",
     year      = " 1982",
     pages     = " 767",
}
@Article{ Ledoussal,
     author    = " P. {Le Doussal} and K. J. Wiese and E. Rapha{\"e}l and
              R. Golestanian",
     title     = " Can Non-Linear Elasticity Explain
               Contact-Line Roughness at Depinning?",
     journal   = " Phys. Rev. Lett.",
     volume    = " 96",
     pages     = " 015702",
     year      = " 2006"
}
@Article{ M06,
     author    = "M. E. M{\"o}bius",
     title     = " Clustering instability in a freely falling granular jet",
     journal   = " Phys. Rev. E",
     volume    = " 74",
     pages     = " 051304",
     year      = " 2006"
}
@Article{ Lemerle,
     author    = " S. Lemerle and J. Ferr\'{e} and C. Chappert and
               V. Mathet and T. Giamarchi and P. {Le Doussal}",
     title     = " Domain Wall Creep in an Ising Magnetic Film",
     journal   = " Phys. Rev. Lett.",
     volume    = " 80",
     year      = " 1998",
     pages     = " 849",
}

@Article{ ZCDS98,
     author    = " S. Zapperi and P. Cizeau and G. Durin
                  and H. E. Stanley",
     title     = " Dynamics of a ferromagnetic domain wall:
         Avalanches, depinning transition, and the Barkhausen effect",
     journal   = " Phys. Rev. B",
     volume    = " 58",
     year      = " 1998",
     pages     = " 6353-6366",
}
@Article{ ADR04,
     author    = " M. Alava and M. Dube and M. Rost",
     title     = " Imbibition in disordered media",
     journal   = " Adv. Phys.",
     volume    = " 53",
     year      = " 2004",
     pages     = " 83-175",
}
@Article{ Middelton,
     author    = " A. A. Middelton",
     title     = " Thermal rounding of the charge-density-wave
              depinning transition",
     journal   = " Phys. Rev. B",
     volume    = " 45",
     year      = " 1992",
     pages     = " R9465-9468.",
}
@Article{ CJV00,
     author    = " H.-Y. Chen and D. Jasnow and J. Vinals",
     title     = " Interface and contact line motion
           in a two-phase fluid under shear flow",
     journal   = " Phys. Rev. Lett.",
     volume    = " 85",
     year      = " 2000",
     pages     = " 1686-1689",
}

@Article{ CW89,
     author    = " J.-D. Chen and N. Wada",
     title     = " Wetting dynamics near the edge of a spreading drop",
     journal   = " Phys. Rev. Lett.",
     volume    = " 62",
     year      = " 1989",
     pages     = " 3050-3053",
}

@Article{ C88,
     author    = " J.-D. Chen",
     title     = " Experiments on a spreading drop and its contact
                  angle on a solid",
     journal   = " J. Colloid Interf. Sci.",
     volume    = " 122",
     year      = " 1988",
     pages     = " 60",
}

@Article{ CRG95,
     author    = " Q. Chen and E. Ram\'{e} and S. Garoff",
     title     = " The breakdown of asymptotic hydrodynamic
         models of liquid spreading at increasing capillary number",
     journal   = " Phys. Fluids",
     volume    = " 7",
     year      = " 1995",
     pages     = " 2631-2639",
}

@Article{ SRG99,
     author    = " K. Stoev and E. Ram\'{e} and S. Garoff",
     title     = " Effects of inertia on the hydrodynamics near moving
                   contact lines",
     journal   = " Phys. Fluids",
     volume    = " 11",
     year      = " 1999",
     pages     = " 3209",
}

@Article{ CRG97,
     author    = " Q. Chen and E. Ram\'{e} and S. Garoff",
     title     = " The velocity field near moving contact lines",
     journal   = " J. Fluid Mech.",
     volume    = " 337",
     year      = " 1997",
     pages     = " 49-66",
}

@Article{ ChengRMP,
     author    = " E. Cheng and M. W. Cole and J. Dupont-Roc and W. F. Saam",
     title     = " Novel wetting behaviour in quantum films",
     journal   = " Rev. Mod. Phys.",
     volume    = " 65",
     year      = " 1993",
     pages     = " 557",
}

@Article{ Chiz,
     author    = " A. Chizmeshya and M. W. Cole and E. Zaremba",
     title     = " Weak binding potentials and wetting transitions",
     journal   = " J. Low Temp. Phys.",
     volume    = " 110",
     year      = " 1998",
     pages     = " 677",
}

@Article{ BFGLV94,
     author    = " G. Blatter and M. V. Feigelman and V. B. Geshkenbein
        and A. I. Larkin and V. M. Vinokur",
     title     = " Vortices in high-temperature superconductors",
     journal   = " Rev. Mod. Phys.",
     volume    = " 66",
     year      = " 1994",
     pages     = " 1125",
}

@Article{ Dalfovo,
     author    = "F. Dalfovo and A. Lastri and L. Pricaupenko and
              S. Stringari and J. Treiner",
     title     = " Structural and dynamical properties of
          superfluid helium: A density-functional approach",
     journal   = " Phys. Rev. B",
     volume    = " 52",
     year      = " 1995",
     pages     = " 1193",
}

@Article{ Cheng91,
     author    = " E. Cheng and M. W. Cole and W. F. Saam and J. Treiner",
     title     = " Helium prewetting and nonwetting on
                    weak-binding substrates",
     journal   = " Phys. Rev. Lett.",
     volume    = " 67",
     year      = " 1991",
     pages     = " 1007",
}

@Article{ Cheng93,
     author    = " E. Cheng and G. Mistura and H. C. Lee and
       M. H. C. Chan and M. W.  Cole and C. Carraro and
               W. F. Saam and F. Toigo",
     title     = " Wetting transitions of liquid-hydrogen films",
     journal   = " Phys.  Rev. Lett.",
     volume    = " 70",
     year      = " 1993",
     pages     = " 1854",
}

@Article{ CRG04,
     author    = " X. Chen and E. Rame and S. Garoff",
     title     = " The effects of thin and ultrathin
                liquid films on dynamic wetting",
     journal   = " Phys. Fluids",
     volume    = " 16",
     year      = " 2004",
     pages     = " 287-297",
}

@Article{ CLR04,
     author    = " J.-H. J. Cho and B. M. Law and F. Rieutord",
     title     = " Dipole-dependent slip of Newtonian liquids
     at smooth solid hydrophibic surfaces",
     journal   = " Phys. Rev. Lett.",
     volume    = " 92",
     year      = " 2004",
     pages     = " 166102",
}
@Article{ Law,
     author    = " B. M. Law",
     title     = " Surface amplitude rations near a critical end-point",
     journal   = " Phys. Rev. Lett.",
     volume    = " 67",
     year      = " 1991",
     pages     = " 1555-1558",
}

@Article{ CQ02,
     author    = " C. Clanet and D. Qu\'{e}r\'{e}",
     title     = " Onset of menisci",
     journal   = " J. Fluid Mech.",
     volume    = " 460",
     year      = " 2002",
     pages     = " 131-149",
}

@Article{ CLHMN01,
     author    = " I. Cohen and H. Li and J. Hougland and
                   M. Mrksich and S. R. Nagel",
     title     = " Using selective withdrawal to coat microparticles,",
     journal   = " Science",
     volume    = " 292",
     year      = " 2001",
     pages     = " 265",
}

@Article{ deegan,
     author    = " R. D. Deegan and O. Bakajin and T. F. Dupont and G. Huber
             and S. R. Nagel and T. A. Witten",
     title     = " Capillary flow as the cause of ring stains
                       from dried liquid drops",
     journal   = " Nature",
     volume    = " 389",
     year      = " 1997",
     pages     = " 827-829",
}

@Article{ deegan2,
     author    = " R. D. Deegan and O. Bakajin and T. F. Dupont and G. Huber
             and S. R. Nagel and T. A. Witten",
     title     = " Contact line deposits in an evaporating drop",
     journal   = " Phys. Rev. E",
     volume    = " 62",
     year      = " 2000",
     pages     = " 756-765",
}

@Article{ deegan3,
     author    = " R. D. Deegan",
     title     = " Pattern formation in drying drops",
     journal   = " Phys. Rev. E",
     volume    = " 61",
     year      = " 2000",
     pages     = " 475-485",
}

@Article{ bourges,
     author    = " C. Bourges-Monnier and M. E. R.  Shanahan",
     title     = " Influence of evaporation on contact-angle",
     journal   = " Langmuir",
     volume    = " 11",
     year      = " 1995",
     pages     = " 2820-2829",
}

@Article{ CC99,
     author    = " M. Cachile and A.-M. Cazabat",
     title     = " Spontaneous spreading of surfactant solutions on
     hydrophilic surfaces: $C_nE_m$ in Ethylene and Diethylene glycol",
     journal   = " Langmuir",
     volume    = " 15",
     year      = " 1999",
     pages     = " 1515",
}

@Article{ cazabat02a,
     author    = " M. Cachile and O. Benichou and A.-M. Cazabat",
     title     = " Evaporating droplets of completely wetting liquids",
     journal   = " Langmuir",
     volume    = " 18",
     year      = " 2002",
     pages     = " 7985-7990",
}

@Article{ cazabat02b,
     author    = " M. Cachile and O. Benichou and C. Poulard
             and A.-M. Cazabat",
     title     = " Evaporating droplets",
     journal   = " Langmuir",
     volume    = " 18",
     year      = " 2002",
     pages     = " 8070-8078",
}

@Article{ arezki,
     author    = " C. Poulard and G. Guena and A.-M. Cazabat and
           A. Boudaoud and M. {Ben Amar}",
     title     = " Rescaling the dynamics of evaporating drops",
     journal   = " Langmuir",
     volume    = " 21",
     year      = " 2005",
     pages     = " 8226",
}

@Article{ MK08,
     author    = " N. Murisic and L. Kondic",
     title     = " Modeling Evaporation of Sessile Drops with
            Moving Contact Lines",
     journal   = " Phys. Rev. E",
     volume    = " 78",
     year      = " 2008",
     pages     = " 065301",
}


@Article{ GMvdV02,
     author    = " A. Y. Gunawan and J. Molenaar and A. A. F. {van de Ven}",
     title     = " In-phase and out-of-phase break-up of two immersed
          liquid threads under influence of surface tension",
     journal   = " Eur. J. Mech. B-Fluids",
     volume    = " 21",
     year      = " 2002",
     pages     = " 399",
}

@Article{ GMvdV04,
     author    = " A. Y. Gunawan and J. Molenaar and A. A. F. {van de Ven}",
     title     = " Break-up of a set of liquid threads under influence
                   of surface tension",
     journal   = " J. Engin. Math.",
     volume    = " 50",
     year      = " 2004",
     pages     = " 25",
}

@Article{ cazabat03,
     author    = " C. Poulard and O. Benichou and A.-M. Cazabat",
     title     = " Freely receding evaporating droplets",
     journal   = " Langmuir",
     volume    = " 19",
     year      = " 2003",
     pages     = " 8828-8834",
}

@Article{ sultan,
     author    = " E. Sultan and A. Boudaoud and
                      M. {Ben Amar}",
     title     = " Diffusion-limited evaporation of thin polar liquid films",
     journal   = " J. Engin. Math.",
     volume    = " 50",
     year      = " 2004",
     pages     = " 209-222",
}

@Article{ davis,
     author    = " S. H. Davis",
     title     = " Thermocapillay instabilities",
     journal   = " Annu. Rev. Fluid Mech.",
     volume    = " 19",
     year      = " 1987",
     pages     = " 403-435",
}

@Article{ bonn/meunier,
     author    = " D. Bonn and J. Meunier",
     title     = " Evaporation preempts complete wetting - Comment",
     journal   = " Europhys. Lett.",
     volume    = " 39",
     year      = " 1997",
     pages     = " 341-342",
}

@Article{ noushineevap,
     author    = " N. Shahidzadeh-Bonn and S. Rafa{\"\i} and
                  A. Azouni and D. Bonn",
     title     = " Evaporating droplets",
     journal   = " J. Fluid Mech.",
     volume    = " 549",
     year      = " 2006",
     pages     = " 307",
}

@Article{ SWDDD09,
     author    = " K. Sefiane and S. K. Wilson and S. David and
        G. J. Dunn and B. R. Duffy",
     title     = " On the effect of the atmosphere on the evaporation of
              sessile droplets of water ",
     journal   = " Phys. Fluids",
     volume    = " 21",
     year      = " 2009",
     pages     = " 062101"
}

@Article{ ansini,
     author    = " L. Ansini and L. Giacomelli",
     title     = " Shear-thinning liquid films: macroscopic and
     asymptotic behaviour by quasi-self-similar solutions",
     journal   = " Nonlinearity",
     volume    = " 15",
     year      = " 2002",
     pages     = " 2147-2164",
}

@Article{ carre97,
     author    = " A. Carr{\'e} and F. Eustache",
     title     = " Dynamique d'\'etalement d'un liquide rh\'eofluidifiant",
     journal   = " C. R. Acad. Sci. Paris",
     volume    = " 325",
     year      = " 1997",
     pages     = " 709-718",
}

@Article{ carre00,
     author    = " A. Carr{\'e} and F. Eustache",
     title     = " Spreading kinetics of shear-thinning
        fluids in wetting and dewetting modes",
     journal   = " Langmuir",
     volume    = " 16",
     year      = " 2000",
     pages     = " 2936--2940",
}

@Article{ carre02,
     author    = " A. Carr{\'e} and P. Woehl",
     title     = " Hydrodynamic behaviour at the triple line
  of spreading liquids and the divergence problem",
     journal   = " Langmuir",
     volume    = " 18",
     year      = " 2002",
     pages     = " 3600-3603",
}

@Article{ CCSC05,
     author    = " C. Cottin-Bizonne and B. Cross and
              A. Steinberger and E. Charlaix",
     title     = " Boundary slip on smooth hydrophobic surfaces:
               intrinsic effets and possible artifacts",
     journal   = " Phys. Rev. Lett.",
     volume    = " 94",
     year      = " 2005",
     pages     = " 056102",
}
@Article{ CC,
     author    = " J. Crassous and E. Charlaix",
     title     = " Contact angle hysteresis on a heterogeneous substrate
in the limit of a weakly distorted contact line",
     journal   = " Europhys. Lett.",
     volume    = " 28",
     year      = " 1994",
     pages     = " 415-420",
}

@Article{ C86,
     author    = " R. G. Cox",
     title     = " The dynamics of the spreading of liquids
           on a solid surface. Part 1. Viscous flow",
     journal   = " J. Fluid Mech.",
     volume    = " 168",
     year      = " 1986",
     pages     = " 169-194",
}

@Article{ Cox83,
     author    = " R. G. Cox",
     title     = " The spreading of a liquid on a rough solid surface",
     journal   = " J. Fluid Mech.",
     volume    = " 131",
     year      = " 1983",
     pages     = " 1-26",
}

@Article{ C98,
     author    = " R. G. Cox",
     title     = " Inertial and viscous effects on dynamic contact angles",
     journal   = " J. Fluid Mech.",
     volume    = " 357",
     year      = " 1998",
     pages     = " 249-278",
}

@Article{ C66,
     author    = " R. G. Cox",
     title     = " The steady motion of a particle of arbitrary shape
                    at small Reynolds numbers",
     journal   = " J. Fluid Mech.",
     volume    = " 23",
     year      = " 1966",
     pages     = " 625",
}

@misc{ DKM88,
     author    = " C. W. Deneka and G. Kar and T. O. Mensah",
     title     = " Method of coating optical waveguide fiber",
     howpublished    = " US Patent no.= 4792347",
     year      = " 1988",
}

@misc{ B_pr,
     author    = " D. Bonn",
     howpublished     = " private communication",
     year      = " 2007"
       }

@misc{ Nagel07,
     author    = " S. R. Nagel ",
     howpublished     = " private communication",
     year      = " 2007"
       }

@misc{ Cohen07,
     author    = " I. Cohen ",
     howpublished     = " private communication",
     year      = " 2007"
       }

@misc{ Mos_pr,
     author    = " M. Moseler",
     howpublished     = " private communication",
     year      = " 2007"
       }

@misc{footcurv,
note={At small ${\rm Ca}$ viscous effects become negligable
whenever $h'\mbox{\ \raisebox{-.9ex}{$\stackrel{\textstyle
>}{\sim}$}\ } 1$, so that the equation remains valid in the bath.}
}

@Article{ HCMS07,
     author    = " B. Henrich and C. Cupelli and M. Moseler and M. Santer",
     title     = " An adhesive DPD wall model for dynamic wetting",
     journal   = " Europhys. Lett.",
     volume    = " 80",
     year      = " 2007",
     pages     = " 60004",
}

@Article{ HK92,
     author    = " P. J. Hoogerbrugge and J. M. V. A. Koelman",
     title     = " Simulating  microscopic hydrodynamic phenomena
                with  dissipative  particle  dynamics",
     journal   = " Europhys. Lett.",
     volume    = " 19",
     year      = " 1992",
     pages     = " 155",
}

@Article{ HCSM08,
     author    = " B. Henrich and C. Cupelli and M. Santer and M. Moseler",
     title     = " Continuum concepts in nanoscale capillary impregnation",
     journal   = " New J. Phys.",
     volume    = " 10",
     pages     = " 113022",
     year      = " 2008",
   }
@Article{ DT03a,
     author    = " J. M. Davis and S. M. Troian",
     title     = " On a generalized approach to the linear stability
                     of spatially nonuniform thin film flows",
     journal   = " Phys. Fluids",
     volume    = " 15",
     year      = " 2003",
     pages     = " 1344",
}

@Article{ DT03b,
     author    = " J. M. Davis and S. M. Troian",
     title     = " Influence of attractive van der Waals
interactions on the optical excitations in thermocapillary-driven spreading",
     journal   = " Phys. Rev. E",
     volume    = " 67",
     year      = " 2003",
     pages     = " 016308",
}

@Article{ Decker,
     author    = " E. L. Decker and  S. Garoff",
     title     = " Contact line structure and
           dynamics on surfaces with contact angle hysteresis",
     journal   = " Langmuir",
     volume    = " 13",
     year      = " 1997",
     pages     = " 6321-6332",
}
@Article{ DeC,
     author    = " J. {De Coninck} and J. Ruiz and S. Miracle-Sole",
     title     = " Generalized Young's equation for rough and
 heterogeneous substrates: A microscopic proof",
     journal   = " Phys. Rev. E",
     volume    = " 65",
     year      = " 2002",
     pages     = " 036139",
}

@Article{ DHVC93,
     author    = " J. {De Coninck} and S. Hoorelbeke and
               M. P. Valignat and A.-M. Cazabat ",
     title     = " Effective microscopic model for the dynamics of spreading",
     journal   = " Phys. Rev. E",
     volume    = " 48",
     year      = " 1993",
     pages     = " 4549-4555",
}

@Article{ JC95,
     author    = "V. de Jonghe and D. Chatain",
     title     = " Experimental study of wetting hysteresis on
     surfaces with controlled geometrical defects and/or chemical defects",
     journal   = " Acta. Metall. Mater.",
     volume    = " 43",
     year      = " 1995",
     pages     = " 1505-1515",
}

@Article{ DR04,
     author    = " C. Denniston and M. O. Robbins",
     title     = " Mapping molecular models to continuum
              theories for partially miscible fluids",
     journal   = " Phys. Rev. E",
     volume    = " 69",
     year      = " 2004",
     pages     = " 021505",
}

@Article{ Dettre,
     author    = " R. H. Dettre and R. E. Johnson",
     title     = " Contact angle hysteresis. IV.
         Contact angle measurement on heterogeneous surfaces ",
     journal   = " J. Phys. Chem",
     volume    = " 69",
     year      = " 1965",
     pages     = " 1507-1515",
}

@Article{ Kirilyuk,
     author    = " A. Kirilyuk and J. Ferr\'{e} and V. Grolier and
             J.-P. Jamet and D. Renard",
     title     = " Magnetization reversal in ultrathin ferromagnetic films with
              perpendicular anisotropy",
     journal   = " Journal of Magnetism and Magnetic Materials",
     volume    = " 171",
     year      = " 1997",
     pages     = " 45-63",
}

@Article{ D40,
     author    = " B. V. Deryaguin",
     title     = " ",
     journal   = " Zh. Fiz. Khim",
     volume    = " 14",
     year      = " 1940",
     pages     = " 137",
}

@Article{ D43,
     author    = " B. V. Deryaguin",
     title     = " On the thickness of a layer of liquid remaining on the
    walls of vessels after their emptying, and the theory of the application
            of photoemulsion after coating on the cine film",
     journal   = " Acta physico-chimica USSR",
     volume    = " 20",
     year      = " 1943",
     pages     = " 349",
}

@Article{ Der40,
     author    = " B. V. Deryaguin",
     title     = " A theory of capillary condensation in the pores of
                 sorbents and of other capillary phenomena taking into
                  account the disjoining action of polymolecular
                  liquid films",
     journal   = " Acta physico-chimica USSR",
     volume    = " 12",
     year      = " 1940",
     pages     = " 181",
}

@Article{ EM85,
     author    = " R. Evans and U. {Marini Bettolo Marconi}",
     title     = " The role of wetting films in capillary condensation
                   and rise: influence of long-range forces",
     journal   = " Chem. Phys. Lett.",
     volume    = " 114",
     year      = " 1985",
     pages     = " 415",
}

@Book{ DCM87,
     author    = " B. V. Deryaguin and N. V. Curaev and V. M. Muller",
     title     = " Surface Forces",
     publisher = " Consultants Bureau, New York",
     year    = " 1987",

}
@Book{ Carrier,
     author    = " G. F. Carrier and M. Krook and C. E. Pearson",
     title     = " Functions of a complex variable",
     publisher = " McGraw-Hill, New York",
     year    = " 1966",

}
@Book{ B59,
     author    = " C. V. Boys",
     title     = " Soap Bubbles, their colors and forces which mold them",
     publisher = " reprinted Dover, New York",
     year    = " 1959",

}
@Article{ B90,
     author    = " C. V. Boys",
     title     = " Notes on photographs of rapidly moving objects,
                  and on the oscillating electric spark",
     journal   = " Phil. Mag.",
     volume    = " 30",
     year      = " 1890",
     pages     = " 248",

}

@Book{ DL64,
     author    = " B. V. Deryaguin and S. M. Levi",
     title     = " Film Coating Theory",
     publisher = " Focal, London",
     year      = " 1964",

}

@Incollection{ N92,
     author    = " P. Nozi{\`e}res",
     title     = " Shape and growth of crystals",
     booktitle     = "Solids far from equilibrium",
     year      = "1992",
     editor    = " C. Godr{\`e}che",
     publisher = {Cambridge University Press, Cambridge},
     pages = " 1-154",
}

@Incollection{ BC05,
     author    = " M. Z. Bazant and D. Crowdy",
     title     = " Conformal mapping methods for interfacial dynamics",
     booktitle     = "Handbook of Materials Modeling",
     year      = "2005",
     editor    = " S. Yip",
     publisher = {Springer},
     pages = " 1417",
}

@Article{ P46,
     author    = " T. Pearcey",
     title     = " The structure of the electromagnetic field
                   in the neighbourhood of a cusp of a caustic",
     journal   = " Phil. Mag.",
     volume    = " 37",
     year      = " 1946",
     pages     = " 311-317"
}
@Incollection{ Berry92,
     author    = " M. V. Berry",
     title     = " Rays, wavefronts and phase: a picture book
                     of cusps",
     booktitle     = "Huygens' principle 1690-1990: Theory and
             Applications",
     year      = "1992",
     editor    = " H. Blok, H. A. Ferwerda, H. K. Kuiken",
     publisher = " Elsevier",
     pages = " 97",
}

@Incollection{ Prandtl,
     author    = " L. Prandtl",
     title     = " {\"U}ber Fl{\"u}ssigkeitsbewegung bei sehr kleiner
                     Reibung",
     booktitle     = "Ludwig Prandtl, Gesammelte Abhandlungen, Vol. II",
     year      = "1961",
     editor    = " W. Tollmien and H. Schlichting and H. G{\"o}rtler",
     publisher = " Springer",
     pages = " 575-584",
}

@Incollection{ Dietrich,
     author    = " S. Dietrich",
     title     = " Wetting Phenomena",
     booktitle     = " Phase Transitions and Critical Phenomena",
     year      = "1988",
     volume    = " 12",
     editor    = " C. Domb and J. L. Lebowitz ",
     publisher = " London: Academic",
     pages = " 1-218",
}

@Incollection{ E_history,
     author    = " J. Eggers",
     title     = " A brief history of drop formation",
     booktitle     = "Nonsmooth Mechanics and Analysis",
     year      = "2006",
     editor    = " P. Alart and O. Maisonneuve and R. T. Rockafellar",
     publisher = " Springer",
     pages = " 163",
}
@Article{DEJ03,
     author    = "L. Duchemin and J. Eggers and C. Josserand",
     title     = "Inviscid coalescence of drops",
     journal   = "J. Fluid Mech.",
     volume    = "487",
     year      = "2003",
     pages     = "167",
}
@Article{ DMQ90,
     author    = " J.-M. {Di Meglio} and D. Qu\'{e}r\'{e}",
     title     = " Contact Angle Hysteresis:
a First analysis of the noise of the creeping motion of the contact line",
     journal   = " Europhys. Lett.",
     volume    = " 11",
     year      = " 1990",
     pages     = " 163-168",
}

@Article{ DiMeglio92,
     author    = " J.-M. {Di Meglio}",
     title     = " Contact angle hysteresis and interacting
surface defects",
     journal   = " Europhys. Lett.",
     volume    = " 17",
     year      = " 1992",
     pages     = " 607",
}

@Article{ DW97,
     author    = " B. R. Duffy and S. K. Wilson",
     title     = " A third-order differential
      equation arising in thin-film flows and relevant to Tanner's law",
     journal   = " Appl. Math. Lett.",
     volume    = " 10",
     year      = " 1997",
     pages     = " 63",
}

@Article{ DAMHL03,
     author    = " D. Duft and T. Achtzehn and R. M{\"u}ller and
     B. A. Huber and T. Leisner",
     title     = " Coulomb fission: Rayleigh jets from levitated
                          microdroplets",
     journal   = " Nature",
     volume    = " 421",
     year      = " 2003",
     pages     = " 128",
}

@Article{ D79,
     author    = " E. B. {Dussan V.}",
     title     = " On the spreading of liquids on solid surfaces:
    static and dynamic contact lines",
     journal   = " Ann. Rev. Fluid Mech.",
     volume    = " 11",
     year      = " 1979",
     pages     = " 371-400",
}

@ARTICLE{Stone94,
   author = "H. A. Stone",
   title     = "Dynamics of drop deformation and breakup
           in viscous fluids",
   year = "1994",
   journal = "Annu. Rev. Fluid Mech.",
   volume = "26",
   pages =  "65"
}

@Article{ DC83,
     author    = " E. B. {Dussan V.} and R. T.-P. Chow ",
     title     = " On the ability of drops or bubbles to stick to
                   non-horizintal surfaces of solids",
     journal   = " J. Fluid Mech.",
     volume    = " 137",
     year      = " 1983",
     pages     = " 1-29",
}

@Article{ DD74,
     author    = " E. B. {Dussan V.} and S. H. Davis",
     title     = " On the motion of a fluid-fluid interface along a solid
                     surface",
     journal   = " J. Fluid Mech.",
     volume    = " 65",
     year      = " 1974",
     pages     = " 71-95",
}

@Article{ DLP,
     author    = " I. Dzyaloshinskii and E. M. Lifshitz and L. P. Pitaevskii",
     title     = " Dispersion forces",
     journal   = " Adv. Phys.",
     volume    = " 10",
     year      = " 1961",
     pages     = " 165",
}

@Article{ Ebner/Saam87,
     author    = " C. Ebner and W. F. Saam",
     title     = " New Reentrant wetting phenomena and
           critical-behaviour near bulk critical-points",
     journal   = " Phys. Rev. Lett.",
     volume    = " 58",
     year      = " 1987",
     pages     = " 587-590",
}
@Article{ Ebner/Saam77,
     author    = " C. Ebner and W. F. Saam",
     title     = " New phase-transition phenomena in thin argon films",
     journal   = " Phys. Rev. Lett.",
     volume    = " 38",
     year      = " 1977",
     pages     = " 1486-1489",
}

@Article{ E97,
     author    = " J. Eggers",
     title     = " Nonlinear dynamics and breakup of free-surface flows",
     journal   = " Rev. Mod. Phys.",
     volume    = " 69",
     year      = " 1997",
     pages     = " 865-929"
}

@Article{ BEIMR09,
     author    = " D. Bonn and J. Eggers and J. Indekeu and J. Meunier
                        and E. Rolley",
     title     = " Wetting and Spreading",
     journal   = " Rev. Mod. Phys.",
     volume    = " 81",
     year      = " 2009",
     pages     = " 739 "
}

@Article{ ELS99,
     author    = " J. Eggers and J. R. Lister and H. A. Stone",
     title     = " Coalescence of Liquid Drops",
     journal   = " J. Fluid Mech.",
     volume    = " 401",
     year      = " 1999",
     pages     = " 293-310",
}


@Article{ EV08,
     author    = " J. Eggers and E. Villermaux",
     title     = " Physics of liquid jets",
     journal   = " Rep. Progr. Phys.",
     volume    = " 71",
     pages     = " 036601",
     year      = " 2008",
}

@Article{ TL02,
     author    = " M.-L. Timmermans and J. R. Lister",
     title     = " The effect of surfactant on the stability of a
                     liquid thread",
     journal   = " J. Fluid Mech.",
     volume    = " 459",
     year      = " 2002",
     pages     = " 289",
}

@Article{ W75,
     author    = " S. Whitaker",
     title     = " Studies of the drop-weight method for surfactant
       solutions III: drop stability, the effect of surfactants on the
         stability of a column of liquid",
     journal   = " J. Colloid Interf. Sci.",
     volume    = " 54",
     year      = " 1975",
     pages     = " 231",
}

@Article{ SW89,
     author    = " A. H. P. Skelland and P. G. Walker",
     title     = " The effects of surface active agents on jet breakup
                   in liquid-liquid systems",
     journal   = " Can. J. Chem. Engin.",
     volume    = " 67",
     year      = " 1989",
     pages     = " 762",
}

@Article{ BB74,
     author    = " H. C. Burkholder and J. C. Berg",
     title     = " Effect of mass transfer on laminar jet breakup I:
                   liquid jets in gases",
     journal   = " AIChE J.",
     volume    = " 20",
     year      = " 1974",
     pages     = " 863",
}

@Article{ CB83,
     author    = " R. W. Coyle and J. C. Berg",
     title     = " The effects of mass transfer and solute adsorption
                on the stability of liquid jets in liquids to
                asymmetric disturbances",
     journal   = " Phys. Chem. Hydrod.",
     volume    = " 4",
     year      = " 1983",
     pages     = " 11",
}

@Article{ CMP02,
     author    = " R. V. Craster and O. K. Matar and D. T. Papageorgiou",
     title     = " Pinchoff and satellite formation in surfactant
                    covered viscous threads",
     journal   = " Phys. Fluids",
     volume    = " 14",
     year      = " 2002",
     pages     = " 1364",
}

@Article{ MB06,
     author    = " P. T. McGough and O. A. Basaran",
     title     = " Repeated formation of fluid threads in breakup
                   of a surfactant-covered jet",
     journal   = " Phys. Rev. Lett.",
     volume    = " 96",
     year      = " 2006",
     pages     = " 054502",
}

@Article{ KP01,
     author    = " S. Kwak and C. Pozrikidis",
     title     = " Effect of surfactants on the instability of a liquid
                   thread or annular layer",
     journal   = " Int. J. Multiphase Flow",
     volume    = " 27",
     year      = " 2001",
     pages     = " 1",
}

@Article{ KFP01,
     author    = " S. Kwak and M. M. Fyrillas and C. Pozrikidis",
     title     = " Effect of surfactants on the instability of a liquid
                   Part II: extensional flow",
     journal   = " Int. J. Multiphase Flow",
     volume    = " 27",
     year      = " 2001",
     pages     = " 39"
}

@Article{ P98,
     author    = " C. Pozrikidis",
     title     = " Numerical studies of cusp formation at fluid
             interfaces in Stokes flow",
     journal   = " J. Fluid Mech.",
     volume    = " 357",
     year      = " 1998",
     pages     = " 29"
}

@Article{ P90,
     author    = " C. Pozrikidis",
     title     = " The deformation of a liquid drop moving normal to
                    a plane wall",
     journal   = " J. Fluid Mech.",
     volume    = " 215",
     year      = " 1990",
     pages     = " 331"
}

@Book{ Pozbook,
     author    = " C. Pozrikidis",
     title     = " Boundary Integral and singularity methods for linearized
               flow",
     publisher = {Cambridge University Press, Cambridge},
     year      = " 1992",
}

@Article{ B68,
     author    = " E. Bart",
     title     = " The slow unsteady settling of a fluid sphere
                     toward a flat fluid interface",
     journal   = " Chem. Engin. Sci. ",
     volume    = " 23",
     year      = " 1968",
     pages     = " 193"
}

@Article{ Blake71,
     author    = " J. R. Blake",
     title     = " A note on the image system for a stokeslet in a
                 no slip boundary",
     journal   = " Proc. Camb. Phil. Soc",
     volume    = " 70",
     year      = " 1972",
     pages     = " 303"
}

@Article{ HPM99,
     author    = " S. Hansen and G. W. M. Peters and H. E. H. Meijer",
     title     = " The effect of surfactant on the stability of a fluid
                   filament embedded in a viscous fluid",
     journal   = " J. Fluid Mech.",
     volume    = " 382",
     year      = " 1999",
     pages     = " 331"
}

@Article{ E02,
     author    = " J. Eggers",
     title     = " Dynamics of Liquid Nanojets",
     journal   = " Phys. Rev. Lett.",
     volume    = " 89",
     year      = " 2002",
     pages     = " 084502-(1-4)",
}

@Article{ FP02,
     author    = " H. C. Fogedby and V. Poutkaradze",
     title     = " Power laws and stretched exponentials in
                    a noisy finite-time singularity model",
     journal   = " Phys. Rev. E",
     volume    = " 66",
     year      = " 2002",
     pages     = " 021103",
}

@Article{ FB02,
     author    = " H. C. Fogedby and A. Brandenburg",
     title     = " Solitons in the noisy Burgers equation",
     journal   = " Phys. Rev. E",
     volume    = " 66",
     year      = " 2002",
     pages     = " 016604",
}

@Article{ ES04,
     author    = " J. Eggers and H. A. Stone",
     title     = " Characteristic lengths at moving contact lines
                         for a perfectly wetting fluid:
            the influence of speed on the dynamic contact angle",
     journal   = " J. Fluid Mech.",
     volume    = " 505",
     year      = " 2004",
     pages     = " 309-321",
}

@Article{ E04a,
     author    = " J. Eggers",
     title     = " Toward a description of contact line
             motion at higher capillary numbers",
     journal   = " Phys. Fluids",
     volume    = " 16",
     year      = " 2004",
     pages     = " 3491",
}

@Article{ E04b,
     author    = " J. Eggers",
     title     = " Hydrodynamic theory of forced dewetting",
     journal   = " Phys. Rev. Lett.",
     volume    = " 93",
     year      = " 2004",
     pages     = " 094502",
}

@Article{ SLLSE07,
     author    = " J. Snoeijer and N. {Le Grand} and L. Limat and
                    H. A. Stone and J. Eggers",
     title     = " Cornered drop and rivulets",
     journal   = " Phys. Fluids",
     volume    = " 19",
     year      = " 2007",
     pages     = " 042104",
}

@Article{ E05,
     author    = " J. Eggers",
     title     = " Existence of receding and advancing contact lines",
     journal   = " Phys. Fluids",
     volume    = " 17",
     year      = " 2005",
     pages     = " 082106",
}

@Article{ E05p,
     author    = " J. Eggers",
     title     = " Contact line motion for partially wetting fluids",
     journal   = " Phys. Rev. E",
     volume    = " 72",
     year      = " 2005",
     pages     = " 061605",
}

@Article{ EE04,
     author    = " J. Eggers and R. Evans",
     title     = " Comment on Dynamic Wetting by liquids of
     different viscosity, by T. D. Blake and Y. D. Shikhmurzaev",
     journal   = " J. Colloid Interf. Sci.",
     volume    = " 280",
     year      = " 2004",
     pages     = " 537",
}
@Article{ Evans,
     author    = " D. Nicolaides and R. Evans",
     title     = " Monte-Carlo study of phase transitions
                in a confined lattice gas",
     journal   = " Phys. Rev. B",
     volume    = " 39",
     year      = " 1989",
     pages     = " 9336-9342",
}

@Article{ Ehr93,
     author    = " P. Ehrhard",
     title     = " Experiments on isothermal and non-isothermal spreading",
     journal   = " J. Fluid Mech.",
     volume    = " 257",
     year      = " 1993",
     pages     = " 463-483",
}

@Article{ ED91,
     author    = " P. Ehrhard and S. H. Davis",
     title     = " Non-isothermal spreading of liquid drops
                            on horizontal plates",
     journal   = " J. Fluid Mech.",
     volume    = " 229",
     year      = " 1991",
     pages     = " 365-388",
}

@Article{ ESR00,
     author    = " M. H. Eres and L. W. Schwartz and R. V. Roy",
     title     = " Fingering phenomena for driven coating films",
     journal   = " Phys. Fluids",
     volume    = " 12",
     year      = " 2000",
     pages     = " 1278-1295",
}

@Article{ EK,
     author    = " D. Ertas and M. Kardar",
     title     = " Critical dynamics of contact line depinning",
     journal   = " Phys. Rev. E",
     volume    = " 49",
     year      = " 1994",
     pages     = " R2532-2535",
}

@Book{ E41,
     author    = " H. J. Eyring",
     title     = " The Theory of Rate Processes",
     publisher = " McGraw-Hill, New York",
     year      = " 1941",
}

@Incollection{ E90,
     author    = " R. Evans",
     title     = " Microscopic theories of simple fluids and their interfaces",
     booktitle = " Liquids at Interfaces, Les Houches Session XLVIII",
     editor    = " J. Charvolin and J.-F. Joanny and J. Zinn-Justin",
     publisher = " Amsterdam: Elsevier",
     year      = " 1990",
     pages     = " 1-98",
}

@Article{ FKB96,
     author    = " D. E. Finlow and P. R. Kota and A. Bose",
     title     = " Investigation of wetting hydrodynamics
                        using numerical simulations",
     journal   = " Phys. Fluids",
     volume    = " 8",
     year      = " 1996",
     pages     = " 302",
}

@misc{ F04,
     author    = " M. Fermigier",
     year      = " 2004",
     howpublished     = " private communication"
}


@Article{ FJ88,
     author    = " M. Fermigier and P. Jenffer",
     title     = " Dynamics of a liquid-liquid interface in a capillary",
     journal   = " Ann. Physique",
     volume    = " 13",
     year      = " 1988",
     pages     = " 37-42",
}

@Article{ FJ91,
     author    = " M. Fermigier and P. Jenffer",
     title     = " An experimental investigation of the dynamic
              contact angle in liquid-liquid systems.",
     journal   = " J. Coll. Int. Sci.",
     volume    = " 146",
     year      = " 1991",
     pages     = " 226-241",
}

@Article{ FW92,
     author    = " M. E. Fisher and H. Wen",
     title     = " Interfacial stiffness and the wetting paramter - the
                   simple cubic Ising model",
     journal   = " Phys. Rev. Lett.",
     volume    = " 68",
     year      = " 1992",
     pages     = " 3654-3654",
}
@Article{ DeGennes,
     author    = " P.-G. de Gennes",
     title     = " Effet des forces {\`a} longue port{\'e}e sur les
              transitions de mouillage",
     journal   = " C. R. Acad. Sc. Paris",
     volume    = " 297:II",
     year      = " 1983",
     pages     = " 9-12",
}

}
@Article{ DeGennesWSD,
     author    = " P.-G. de Gennes",
     title     = "Wetting: Statics and Dynamics",
     journal   = "Rev. Mod. Phys.",
     volume    = " 57",
     year      = " 1985",
     pages     = " 827",
}

@Article{ Getal90,
     author    = " G. Gompper and D. M. Kroll and R. Liposky",
     title     = " Nonclassical wetting behavior in the solid-on-solid
              limit of the 3-dimensional Ising model",
     journal   = " Phys. Rev. B",
     volume    = " 42",
     year      = " 1990",
     pages     = " 961964",
}

@Article{ GK88a,
     author    = " G. Gompper and D. M. Kroll",
     title     = " Critical behavior of effective interface models for
                 wetting in 3 dimensions",
     journal   = " Europhys. Lett.",
     volume    = " 5",
     year      = " 1988",
     pages     = " 49-53",
}

@Article{ GK88b,
     author    = " G. Gompper and D. M. Kroll",
     title     = " Monte-Carlo study of nonuniversal wetting behavior in
      (2+1) dimensions",
     journal   = " Phys. Rev. B",
     volume    = " 37",
     year      = " 1988",
     pages     = " 3821-3824",
}

@Article{ Durian,
     author    = " D. J. Durian and C. Franck",
     title     = " Wall phenomena in a critical binary mixture",
     journal   = " Phys. Rev. Lett.",
     volume    = " 59",
     year      = " 1987",
     pages     = " 555",
}

@Article{ Fisher,
     author    = " M. E. Fisher and A. J. Jin",
     title     = " Is short-range critical wetting a 1st order transition ?",
     journal   = " Phys. Rev. Lett.",
     volume    = " 69",
     year      = " 1992",
     pages     = " 792",
}

@Article{ FM93,
     author    = " M. L. Forcada and C. M. Mate",
     title     = " Molecular layering during evaporation of
                        ultrathin liquid films",
     journal   = " Nature",
     volume    = " 363",
     year      = " 1993",
     pages     = " 527-529",
}

@Article{ ,
     author    = " C. Fradin and A. Braslau and A. Luzat and D. Smilgies
              and M. Alba and N. Boudet and K. R. Mecke and J. Daillant",
     title     = " Reduction in the surface energy of liquid interfaces
                   at short length scales",
     journal   = " Nature",
     volume    = " 403",
     year      = " 2000",
     pages     = " 871",
}

@Article{ FH94,
     author    = " N. Fraysse and G. M. Homsy",
     title     = " An experimental study of rivulet instabilities
              in centrifugal spin coating of viscous Newtonian
                 and non-Newtonian fluids, ",
     journal   = " Phys. Fluids",
     volume    = " 6",
     year      = " 1994",
     pages     = " 1491",
}

@Article{ F65,
     author    = " G. Friz",
     title     = " {\"U}ber den dynamischen Randwinkel im Fall der
                  vollst{\"a}ndigen Benetzung",
     journal   = " Zeitschr. angew. Phys.",
     volume    = " 19",
     year      = " 1965",
     pages     = " 374-378",
}

@Article{ GGS03,
     author    = " N. Garnier and R. O. Grigoriev and M. F. Schatz",
     title     = " Optical manipulation of microscale fluid flow",
     journal   = " Phys. Rev. Lett.",
     volume    = " 91",
     year      = " 2003",
     pages     = " 054501",
}

@Article{ Gau,
     author    = " H. Gau and S. Herminghaus and P. Lenz and R. Lipowsky",
     title     = " Liquid morphologies on structured surfaces:
                    From microchannels to microchips",
     journal   = " Science",
     volume    = " 283",
     year      = " 1999",
     pages     = " 46",
}

@Article{ lenz,
     author    = " P. Lenz and R. Lipowsky",
     title     = " Morphological transitions of wetting layers on
                   structured surfaces",
     journal   = " Phys. Rev. Lett.",
     volume    = " 80",
     year      = " 1998",
     pages     = " 1920-1923",
}

@Article{ rascon1,
     author    = " C. Rasc{\'o}n and A. O. Parry",
     title     = " ???",
     journal   = " Nature",
     volume    = " 407",
     year      = " 2000",
     pages     = " 986",
}

@Article{ rascon2,
     author    = " A. O. Parry and A. J. Wood and C. Rasc{\'o}n",
     title     = " Wedge filling, cone filling and the strong
                     fluctuation regime",
     journal   = " Journal of Physics: Condensed Matter",
     volume    = " 13",
     year      = " 2001",
     pages     = " 4591",
}
@Article{ BCM02,
     author    = " L. Bruschi and A. Carlin and G. Mistura",
     title     = " Complete wetting on a linear wedge",
     journal   = " Phys. Rev. Lett.",
     volume    = " 89",
     year      = " 2002",
     pages     = " 166101"
}

@Article{ oil,
     author    = " N. Shahidzadeh-Bonn and E. Bertrand and
             J. P. Dauplait and D. Bonn",
     title     = " ???",
     journal   = " J. Petroleum Science \& Engineering",
     volume    = " 39",
     year      = " 2003",
     pages     = " 409"
}
@Article{ civil,
     author    = " E. C. Childs",
     title     = " ???",
     journal   = " Proc. Roy. Soc. A",
     volume    = " 201",
     year      = " 1950",
     pages     = " 392"
}

@Article{ poon,
     author    = " W. C. K. Poon",
     title     = " The physics of a model colloid-polymer mixture",
     journal   = " J. Phys.: Condens. Matter",
     volume    = " 14",
     year      = " 2002",
     pages     = " R859"
}

@Article{ asakura1,
     author    = " S. Asakura and F. Oosawa",
     title     = " On interaction between two bodies immersed in a
             solution of macromolecules",
     journal   = " J. Chem. Phys.",
     volume    = " 22",
     year      = " 1954",
     pages     = " 1255"
}

@Article{ asakura2,
     author    = " S. Asakura and F. Oosawa",
     title     = " Interaction between particles suspended
                      in solutions of macromolecules",
     journal   = " J. Pol. Sci.",
     volume    = " 33",
     year      = " 1958",
     pages     = " 183"
}

@Article{ G85,
     author    = " P.-G. {de Gennes}",
     title     = " Wetting: statics and dynamics",
     journal   = " Rev. Mod. Phys.",
     volume    = " 57",
     year      = " 1985",
     pages     = " 827-863",
}

@Article{ G86,
     author    = " P.-G. {de Gennes}",
     title     = " Deposition of Langmuir-Blodget layers",
     journal   = " Coll. Pol. Sci.",
     volume    = " 264",
     year      = " 1986",
     pages     = " 463-465",
}

@Article{ Gennes1981,
     author    = " P.-G. {de Gennes}",
     title     = " Effect of long-range forces on wetting phenomena",
     journal   = " J. Phys. Lett.",
     volume    = " 42",
     year      = " 1981",
     pages     = " L377",
}

@Article{ GC90,
     author    = " P.-G. {de Gennes} and A.-M. Cazabat",
     title     = " Spreading of a stratified incompressible droplet",
     journal   = " C. R. Acad. Sci. Paris, Serie",
     volume    = " 310",
     year      = " 1990",
     pages     = " 1601",
}

@Article{ GHL90,
     author    = " P.-G. {de Gennes} and X. Hua and P. Levinson",
     title     = " Dynamics of wetting: local contact angles",
     journal   = " J. Fluid Mech.",
     volume    = " 212",
     year      = " 1990",
     pages     = " 55-63",
}

@Book{ GBQ03,
     author    = " P.-G. {de Gennes} and F. Brochart-Wyart and
               D. Qu\'{e}r\'{e}",
     title     = " Capillarity and Wetting Phenomena: Drops,
                 Bubbles, Pearls, Waves",
     publisher = " Springer",
     year      = " 2003",

}

@Article{ GLGM01,
     author    = " Y. Gogotsi and J. A. Libera and C. Guvenc-Yazicioglu
                          and C. M. Megaridis",
     title     = " Multiphase fluid experiments in hydrothermal carbon
                        nanotubes",
     journal   = " Appl. Phys. Lett.",
     volume    = " 79",
     year      = " 2001",
     pages     = " 1021-1023",
}

@misc{ GR_pr,
     author    = " R. Golestanian and  E. Rapha{\"e}l",
     year = {2004},
     howpublished     = " private communication"
}

@Article{ GR01,
     author    = " R. Golestanian and  E. Rapha{\"e}l",
     title     = " Relaxation of a moving contact line
              and the Landau-Levich effect",
     journal   = " Europhys. Lett.",
     volume    = " 55",
     year      = " 2001",
     pages     = " 228-234",
}

@Article{ GolestanianR01,
     author    = " R. Golestanian and  E. Rapha{\"e}l",
     title     = " Dissipation in the dynamics of a moving contact line",
     journal   = " Phys. Rev. E",
     volume    = " 64",
     year      = " 2001",
     pages     = " 031601-1-7",
}
@Article{ GR03,
     author    = " R. Golestanian and  E. Rapha{\"e}l",
     title     = " Roughening transition in a moving contact line",
     journal   = " Phys. Rev. E",
     volume    = " 67",
     year      = " 2003",
     pages     = " 031603",
}

@Article{ GH91,
     author    = " R. Goodwin and  G. M. Homsy",
     title     = " Viscous flow down a slope in the vicinity
                       of a contact line",
     journal   = " Phys. Fluids A ",
     volume    = " 3",
     year      = " 1991",
     pages     = " 515",
}

@Article{ G90,
     author    = " V. A. Gorodtsov",
     title     = " Spreading of a film of nonlinearly viscous liquid over a
              horizontal smooth surface",
     journal   = " J. Engrg. Phys.",
     volume    = " 57",
     year      = " 1990",
     pages     = " 879-884",
}

@Article{ GMH04,
     author    = " C. M. Gramlich and A. Mazouchi and G. M. Homsy",
     title     = " Time-dependent free surface Stokes flow with a
              moving contact line.II. Flow over wedges and trenches",
     journal   = " Phys. Fluids",
     volume    = " 16",
     year      = " 2004",
     pages     = " 1660-1667",
}

@Article{ G78,
     author    = " H. P. Greenspan",
     title     = " On the motion of a small viscous droplet that
                    wets the surface",
     journal   = " J. Fluid Mech.",
     volume    = " 84",
     year      = " 1978",
     pages     = " 125-143",
}

@Article{ G03,
     author    = " R. O. Grigoriev",
     title     = " Contact line instability and pattern selection in
                 thermally driven liquid film flows",
     journal   = " Phys. Fluids",
     volume    = " 15",
     year      = " 2003",
     pages     = " 1363",
}

@Article{ G05,
     author    = " R. O. Grigoriev",
     title     = " Transient growth in driven contact lines",
     journal   = " Physica D",
     volume    = " 209",
     year      = " 2005",
     pages     = " 105-116",
      }

@Article{ GK82,
     author    = " E. B. Gutoff and C. E. Kendrick",
     title     = " Dynamic contact angles",
     journal   = " AIChE J.",
     volume    = " 28",
     year      = " 1982",
     pages     = " 459-466",
}

@Article{ HP97,
     author    = " N. G. Hadjiconstantinou and A. T. Patera",
     title     = " Heterogeneous atomistic-continuum
                  representation for dense fluid systems",
     journal   = " Int. J. Modern Phys. C",
     volume    = " 8",
     year      = " 1997",
     pages     = " 967",
}

@Article{ H99a,
     author    = " N. G. Hadjiconstantinou",
     title     = " Combining atomistic and continuum simulations of
              contact-line motion",
     journal   = " Phys. Rev. E",
     volume    = " 59",
     year      = " 1999",
     pages     = " 2475-2478",
}

@Article{ H99b,
     author    = " N. G. Hadjiconstantinou",
     title     = " Hybrid Atomistic-Continuum Formulations
                  and the moving contact-line problem",
     journal   = " J. Comp. Phys.",
     volume    = " 154",
     year      = " 1999",
     pages     = " 245-265",
}

@Article{ H03,
     author    = " N. G. Hadjiconstantinou",
     title     = " A molecular view of Tanner's law: molecular dynamics of
droplet spreading",
     journal   = " J. Fluid Mech.",
     volume    = " 497",
     year      = " 2003",
     pages     = " 123-132",
}

@Article{ Halpin-Healy,
     author    = " T. Halpin-Healy and E. Br{\'e}zin",
     title     = " Ginzburg criterium for short-range critical wetting",
     journal   = " Phys. Rev. Lett.",
     volume    = " 58",
     year      = " 1987",
     pages     = " 1220",
}

@Article{ HT71,
     author    = " R. J. Hansen and T. Y. Toong",
     title     = " Interface behavior as one fluid completely displaces
another from a small-diameter tube",
     journal   = " J. Colloid Interf. Sci",
     volume    = " 36",
     year      = " 1971",
     pages     = " 410-413",
}

@Article{ H19,
     author    = " W. P. Hardy",
     title     = " The Spreading of Fluids on Glass",
     journal   = " Philos. Mag.",
     volume    = " 38",
     year      = " 1919",
     pages     = " 49-55",
}

@Article{ Q77,
     author    = " G. H. Quincke",
     title     = " Ueber den Randwinkel und die Ausbreitung von
                Fl{\"u}ssigkeiten auf festen K{\"o}rpern",
     journal   = " Wied. Ann.",
     volume    = " 2",
     year      = " 1877",
     pages     = " 145",
}

@Article{ HR93,
     author    = " R. A. Hayes and J. Ralston",
     title     = " Forced liquid movement on low energy surfaces",
     journal   = " J. Colloid Int. Sc.",
     volume    = " 159",
     year      = " 1993",
     pages     = " 429-438",
}

@Article{ HM,
     author    = " A. Hazareesing and  M. M\'ezard",
     title     = " Wandering of a contact line at thermal equilibrium",
     journal   = " Phys. Rev. E",
     volume    = " 60",
     year      = " 1999",
     pages     = " 1269-1278",
}

@Article{ HG84,
     author    = " H. Hervet and P.-G. {de Gennes}",
     title     = " The Dynamics of Wetting: Precursor Films in the Wetting
of ``Dry'' Solids ",
     journal   = " C. R. Acad. Sc. Paris, Serie II",
     volume    = " 299",
     year      = " 1984",
     pages     = " 499-503",
}

@Article{ HSj02,
     author    = " S. Herminghaus and R. Seemann and K. Jacobs",
     title     = " Generic morphologies of viscoelastic dewetting fronts",
     journal   = " Phys. Rev. Lett.",
     volume    = " 89",
     year      = " 2002",
     pages     = " 056101",
}

@Article{ HCL89,
     author    = " F. Heslot and A.-M. Cazabat and P. Levinson",
     title     = " Dynamics of wetting of tiny drops:
            ellipsometric study of the late stages of spreading",
     journal   = " Phys. Rev. Lett.",
     volume    = " 62",
     year      = " 1989",
     pages     = " 1286-1289",
}

@Article{ HFC89,
     author    = " F. Heslot and N. Fraysse and A.-M. Cazabat",
     title     = " Molecular layering in the spreading of
                     wetting liquid drops",
     journal   = " Nature",
     volume    = " 338",
     year      = " 1989",
     pages     = " 640-642",
}

@Article{ krim,
     author    = " J. Krim and J. G. Dash and J. Suzanne",
     title     = " Triple-point wetting of light molecular gases on
                       Au(111) surfaces",
     journal   = " Phys. Rev. Lett.",
     volume    = " 52",
     year      = " 1984",
     pages     = " 640-643",
}

@Article{ Hess,
     author    = " G. B. Hess and M. J. Sabatini and M. H. W. Chan",
     title     = " Nonwetting of cesium by neon near its critical point",
     journal   = " Phys. Rev. Lett.",
     volume    = " 78",
     year      = " 1997",
     pages     = " 1739",
}

@Book{ Hinch91,
     author    = " E. J. Hinch",
     title     = " Perturbation methods",
     publisher = {Cambridge University Press, Cambridge},
     year      = " 1991",

}

@Article{ H76,
     author    = " L. M. Hocking",
     title     = " A moving fluid interface on a rough surface",
     journal   = " J. Fluid Mech.",
     volume    = " 76",
     year      = " 1976",
     pages     = " 801-817",
}

@Article{ Hock77,
     author    = " L. M. Hocking",
     title     = " A moving fluid interface. Part 2.
          The removal of the force singularity by a slip flow",
     journal   = " J. Fluid Mech.",
     volume    = " 79",
     year      = " 1977",
     pages     = " 209-229",
}

@Article{ H81,
     author    = " L. M. Hocking",
     title     = " Sliding and spreading of a thin two-dimensional drops",
     journal   = " Q. J. Mech. Appl. Math.",
     volume    = " 34",
     year      = " 1981",
     pages     = " 37-55",
}

@Article{ H83,
     author    = " L. M. Hocking",
     title     = " The spreading of a thin drop by gravity and capillarity",
     journal   = " Q. J. Mech. Appl. Math.",
     volume    = " 36",
     year      = " 1983",
     pages     = " 55-69",
}

@Article{ H82,
     author    = " L. M. Hocking and  A. D. Rivers",
     title     = " The spreading of a drop by capillary action",
     journal   = " J. Fluid Mech.",
     volume    = "121",
     year      = " 1982",
     pages     = " 425-442",
}

@Article{ H90,
     author    = " L. M. Hocking",
     title     = " Spreading and instability of a viscous fluid sheet",
     journal   = " J. Fluid Mech.",
     volume    = " 221",
     year      = " 1990",
     pages     = " 373",
}

@Article{ H92,
     author    = " L. M. Hocking",
     title     = " Rival contact-angle models and the spreading of drops",
     journal   = " J. Fluid Mech.",
     volume    = " 239",
     year      = " 1992",
     pages     = " 671-681",
}

@Article{ H93,
     author    = " L. M. Hocking",
     title     = " The influence of intermolecular forces on
                          thin fluid layers",
     journal   = " Phys. Fluids A",
     volume    = " 5",
     year      = " 1993",
     pages     = " 793-799",
}

@Article{ H94,
     author    = " L. M. Hocking",
     title     = " The spreading of drops with intermolecular forces",
     journal   = " Phys. Fluids",
     volume    = " 6",
     year      = " 1994",
     pages     = " 3224-3228",
}

@Article{ H95,
     author    = " L. M. Hocking",
     title     = " On contact angles in evaporating liquids",
     journal   = " Phys. Fluids",
     volume    = " 7",
     year      = " 1995",
     pages     = " 2950"
}

@Article{ H01,
     author    = " L. M. Hocking",
     title     = " Meniscus draw-up and draining",
     journal   = " Euro. J. Appl. Math.",
     volume    = " 12",
     year      = " 2001",
     pages     = " 195-208",
}

@Article{ HM93,
     author    = " L. M. Hocking and M. J. Miksis",
     title     = " Stability of a ridge of liquid",
     journal   = " J. Fluid Mech.",
     volume    = " 247",
     year      = " 1993",
     pages     = " 157",
}

@Article{ H75,
     author    = " R. L. Hoffman",
     title     = " A Study of the Advancing Interface",
     journal   = " J. Coll. Interface Sci.",
     volume    = " 50",
     year      = " 1975",
     pages     = " 228-241",
}

@Article{ HH77,
     author    = " P. C. Hohenberg and B. I. Halperin",
     title     = " Theory of dynamic critical phenomena",
     journal   = " Rev. Mod. Phys.",
     volume    = " 49",
     year      = " 1977",
     pages     = " 435-479",
}

@Article{ HM77,
     author    = " C. Huh and S. G. Mason",
     title     = " The steady movement of a liquid meniscus
                     in a capillary tube",
     journal   = " J. Fluid Mech.",
     volume    = " 81",
     year      = " 1977",
     pages     = " 401-419",
}

@Article{HS71,
     author    = " C. Huh and L. E. Scriven",
     title     = " Hydrodynamic model of steady movement of a
               solid/liquid/fluid contact line",
     journal   = " J. Coll. Int. Sci.",
     volume    = " 35",
     year      = " 1971",
     pages     = " 85-101",
}

@Article{ H82a,
     author    = " H. E. Huppert",
     title     = " Flow and instability of a viscous current down a slope",
     journal   = " Nature",
     volume    = " 300",
     year      = " 1982",
     pages     = " 427-429",
}

@Article{ H82b,
     author    = " H. E. Huppert",
     title     = " The propagation of two-dimensional and axisymmetric
           viscous gravity currents over a rigid horizontal surface",
     journal   = " J. Fluid Mech.",
     volume    = " 121",
     year      = " 1982",
     pages     = " 43-58",
}

@Incollection{ IndekeuFCW,
     author    = " J. O. Indekeu and K. Ragil and D. Broseta and
         D. Bonn  and J. Meunier",
     title     = " Wetting phase transitions and petroleum reservoirs",
     booktitle     = " New approaches to Problems in Liquid State Theory",
     editor     = " C. Caccamo and J.-P. Hansen and G. Stell",
     publisher = " Kluwer Academic Publishers",
     year      = " 1999",
     pages     = " 337-344",
}
@Article{ BI95,
     author    = " D. Bonn and J. O. Indekeu",
     title     = " Nucleation and wetting near surface spinodals",
     journal   = " Phys. Rev. Lett.",
     volume    = " 74",
     year      = " 1995",
     pages     = " 3844",
}
@Article{ Ragil1,
     author    = " K. Ragil and D. Bonn and D. Broseta and J. Meunier",
     title     = " Wetting of alkanes on water from a Cahn-type theory",
     journal   = " J. Chem. Phys.",
     volume    = " 105",
     year      = " 1996",
     pages     = " 5160-5167",
}
@Article{ Ragil2,
     author    = " K. Ragil and J. Meunier and D. Broseta and
              J. O. Indekeu and D. Bonn",
     title     = " Experimental observation of critical wetting",
     journal   = " Phys. Rev. Lett.",
     volume    = " 77",
     year      = " 1996",
     pages     = " 1532",
}

@Article{ Indekeu,
     author    = " J. O. Indekeu and K. Ragil and D. Bonn and
         D. Broseta  and J. Meunier",
     title     = " Wetting of alkanes on water from a
            Cahn-type theory: effects of long-range forces",
     journal   = " J. Stat. Phys.",
     volume    = " 95",
     year      = " 1990",
     pages     = " 1009",
}

@misc{ I69a,
     author    = " G. Inverarity",
     title     = " The wetting of glass fibres by liquids and polymers",
     howpublished = " Ph.D. Thesis, Univ. of Manchester",
     year      = " 1969",

}

@Article{ I69b,
     author    = " G. Inverarity",
     title     = " Dynamic wetting of glass fibre and polymer fibre",
     journal   = " Brit. Polym. J.",
     volume    = " 1",
     year      = " 1969",
     pages     = " 245",
}

@Article{ IT02,
     author    = " C. Iwamoto and S. Tanaka",
     title     = " Atomic morphology and chemical
           reactions of the reactive wetting front",
     journal   = " Acta Mater",
     volume    = " 50",
     year      = " 2002",
     pages     = " 749-755",
}

@Incollection{ I88,
     author    = " J. A. {de Feijter}",
     title     = " Thermodynamics of thin liquid films",
     booktitle     = " Thin liquid films",
     editor     = " I. B. Ivanov",
     publisher = " Marcel Dekker, New York",
     year      = " 1988",
     pages      = " 1-47",

}

@Article{ JMH98,
     author    = " K. Jacobs and K. R. Mecke and S. Herminghaus",
     title     = " Thin liquid film rupture via defects",
     journal   = " Langmuir",
     volume    = " 14",
     year      = " 1998",
     pages     = " 965",
}

@Article{ Feigel,
     author    = " M. V. Feigel'man and V. B. Geshkenbein and A. I. Larkin
                        and V. M. Vinokur",
     title     = " Theory of collective flux creep",
     journal   = " Phys. Rev. Lett.",
     volume    = " 63",
     year      = " 1989",
     pages     = " 2303",
}

@Article{ J00,
     author    = " D. Jacqmin",
     title     = " Contact-line dynamics of a diffuse fluid interface",
     journal   = " J. Fluid Mech.",
     volume    = " 402",
     year      = " 2000",
     pages     = " 57-88",
}

@Article{ JM92,
     author    = " J.-T. Jeong and H. K. Moffatt",
     title     = " Free-surface cusps associated with a flow at
                        low Reynolds numbers",
     journal   = " J. Fluid Mech.",
     volume    = " 241",
     year      = " 1992",
     pages     = " 1-22",
}

@Article{ R68,
     author    = " S. Richardson",
     title     = " Two-dimensional bubbles in slow viscous flows",
     journal   = " J. Fluid Mech.",
     volume    = " 33",
     year      = " 1968",
     pages     = " 476",
}

@Article{ R72,
     author    = " S. Richardson",
     title     = " Hele-Shaw flows with a free boundary produced by the
                injection of fluid into a narrow channel",
     journal   = " J. Fluid Mech.",
     volume    = " 56",
     year      = " 1972",
     pages     = " 609"
}

@Article{ How86,
     author    = " S. D. Howison",
     title     = " Cusp Development in Hele-Shaw Flow with a Free Surface",
     journal   = " SIAM J. Appl. Math",
     volume    = " 46",
     year      = " 1986",
     pages     = " 20"
}

@Article{ PK45a,
     author    = " P. Ya. Polubarinova-Kochina",
     title     = " On a problem of the motion of the contour of a
                      petroleum shell",
     journal   = " Dokl. Akad Nauk USSR",
     volume    = "47 ",
     year      = " 1945",
     pages     = " 254-257"
}

@Article{ PK45b,
     author    = " P. Ya. Polubarinova-Kochina",
     title     = " Concerning unsteady motions in the theory of
                filtration",
     journal   = " Prikl. Matem. Mech.",
     volume    = "9 ",
     year      = " 1945",
     pages     = " 79-90"
}

@Article{ Ga45,
     author    = "  L. A. Galin",
     title     = " Unsteady seepage with a free surface",
     journal   = " Dokl. Akad. Nauk. SSSR",
     volume    = " 47 ",
     year      = " 1945",
     pages     = " 246-249"
}

@Article{ CHS99,
     author    = " H. D. Ceniceros and T. Y. Hou and H. Si",
     title     = " Numerical study of Hele-Shaw flow with suction",
     journal   = " Phys. Fluids",
     volume    = " 11",
     year      = " 1999",
     pages     = " 2471",
}

@Article{ CeniS00,
     author    = " H. D. Ceniceros and H. Si",
     title     = " Computation of Axi-Symmetric Suction Flow through
        Porous Media in the Presence of Surface Tension",
     journal   = " J. Comput. Phys.",
     volume    = " 165",
     year      = " 2000",
     pages     = " 237",
}

@Article{ DH95,
     author    = " C. R. Dun and G. C. Hocking",
     title     = "  Withdrawal of fluid through a line sink beneath a
                   free surface above a sloping boundary",
     journal   = " J. Engin. Math.",
     volume    = " 29",
     year      = " 1995",
     pages     = " 1-10",
}

@Article{ FH90,
     author    = " L. K. Forbes and G. C. Hocking",
     title     = "  Flow caused by a point sink in a fluid having a
                      free surface",
     journal   = " J. Austral. Math. Soc. B",
     volume    = " 32",
     year      = " 1990",
     pages     = " 231-249",
}

@Article{ TV84,
     author    = " E. O. Tuck and J.-M. Vanden Broeck",
     title     = "  A cusp-like free-surface flow due to a
          submerged source or sink",

     journal   = " J. Austral. Math. Soc. Ser. B",
     volume    = " 25",
     year      = " 1984",
     pages     = " 443-450"
}

@Article{ TS90,
     author    = " E. O. Tuck and L. W. Schwartz",
      title     = "A numerical and asymptotic study of some 3rd-order ordinary differential equations relevant to draining and coating flows",
      journal   = "SIAM Review",
     volume    = " 32",
     year      = " 1990",
     pages     = " 453-469"
}


@Article{ MvB91,
     author    = "H. Mekias and Jean-Marc Vanden-Broeck",
     title     = "Subcritical flow with a stagnation point due to a
             source beneath a free surface",
     journal   = " Phys. Fluids A",
     volume    = " 3",
     year      = " 1991",
     pages     = "2652-2658"
}

@Article{ vBK87,
     author    = "Jean-Marc Vanden-Broeck and J. B. Keller",
     title     = "Free surface flow due to a sink",
     journal   = " J. Fluid Mech.",
     volume    = " 175",
     year      = " 1987",
     pages     = "109-117"
}

@Article{ ZHB97,
     author    = " H. Zhang and G. C. Hocking and D. A. Barry",
     title     = " An analytical solution for critical withdrawal of
           layered fluid through a line sink in a porous medium",
     journal   = " J. Austral. Math. Soc. B",
     volume    = " 39",
     year      = " 1997",
     pages     = " 271-279",
}

@Article{ ZH96,
     author    = " H. Zhang and G. C. Hocking",
     title     = " Withdrawal of layered fluid through a line sink
                in a porous medium",
     journal   = " J. Austral. Math. Soc. B",
     volume    = " 38",
     year      = " 1996",
     pages     = " 240-254",
}

@Article{ Kirch69,
     author    = " G. Kirchhoff",
     title     = " Zur {T}heorie freier {F}l{\"u}ssigkeitsstrahlen",
     journal   = " J. reine angew. Math.",
     volume    = " 70",
     year      = " 1869",
     pages     = " 289",
}

@Article{ Planck,
     author    = " M. Planck",
     title     = "Zur {T}heorie der {F}l{\"u}ssigkeitsstrahlen",
     journal   = " Wied. Ann.",
     volume    = " 21",
     year      = " 1884",
     pages     = " 499-509",
}

@Article{ Ho98,
     author    = " B. Hopkinson",
     title     = " Discontinuous fluid motions involving
                       sources and vortices",
     journal   = " Proc. Lond. Math. Soc.",
     volume    = " 29",
     year      = " 1898",
     pages     = " 142-164",
}

@Article{ Lo91,
     author    = " A. E. H. Love",
     title     = " On the theory of discontinuous fluid motion in two
                   dimensions",
     journal   = " Proc. Camb. Phil. Soc.",
     volume    = " 7",
     year      = " 1891",
     pages     = " 175-201",
}

@Article{ Cr49,
     author    = " A. Craya",
     title     = " Theoretical research on the flow of nonhomogeneous
                         fluids",
     journal   = " La Houille Blanche",
     volume    = " 4",
     year      = " 1949",
     pages     = " 44-55",
}

@Article{ Sau01,
     author    = " C. Sautreaux",
     title     = " Mouvement d'un liquide parfait soumis \`a la pesanteur.
             {D}\'etermination des lignes de courant.",
     journal   = " J. Math. Pures Appl.",
     volume    = " 7",
     year      = " 1901",
     pages     = " 125-159"
}

@Article{ 95,
     author    = " C. R. Dun and G. C. Hocking",
     title     = "  Withdrawal of fluid through a line sink beneath a
                   free surface above a sloping boundary",
     journal   = " J. Engin. Math.",
     volume    = " 29",
     year      = " 1995",
     pages     = " 1-10",
}

@Article{ Moffatt63,
     author    = " H. K. Moffatt",
     title     = " Viscous and resistive eddies near a sharp corner",
     journal   = " J. Fluid Mech.",
     volume    = " 18",
     year      = " 1963",
     pages     = " 1-18"
}

@Article{ C13,
     author    = " S. D. Carothers",
     title     = " Plane strain in a wedge, with application to masonry dams",
     journal   = " Proc. Roy. Soc. Edinburgh",
     volume    = " 23",
     year      = " 1912",
     pages     = " 292"
}

@Article{ SK58,
     author    = " E. Sternberg and W. T. Koiter",
     title     = " The wedge under a concentrated couple: a paradox
             in the two-dimensional theory of elasticity",
     journal   = " J. Appl. Mech.",
     volume    = " 25",
     year      = " 1958",
     pages     = " 575"
}

@Article{ JB92,
     author    = " J. M. Jerret and J. R. {de Bruyn}",
     title     = " Fingering instability of a gravitationally
                        driven contact line",
     journal   = " Phys. Fluids A",
     volume    = " 4",
     year      = " 1992",
     pages     = " 234",
}

@Article{ JG84,
     author    = " J.-F. Joanny and P.-G. {de Gennes}",
     title     = " Competition Between Wetting and Adverse
               Macroscopic Forces [in French]",
     journal   = " C. R. Acad. Sc. Paris, Serie II",
     volume    = " 299",
     year      = " 1984",
     pages     = " 605-608",
}
@Article{ JoannyR90,
     author    = " J.-F. Joanny and M. O. Robbins",
     title     = " Motion of a contact line on a heterogeneous substrate",
     journal   = " J. Chem. Phys.",
     volume    = " 92",
     year      = " 1990",
     pages     = " 3206-3212",
}

@Article{ JdG84,
     author    = " J.-F. Joanny and P.-G. de Gennes",
     title     = " A model for contact angle hysteresis",
     journal   = " J. Chem. Phys.",
     volume    = " 81",
     year      = " 1984",
     pages     = " 552-562",
}

@misc{ JL87,
     author    = " C. M. G. Jochem and J. W. C. van der Ligt",
     title     = " Method of and arrangement for coating a fibre",
     howpublished = " US Patent No. 4704307 ",
     year      = " 1987",

}

@Article{ JSMB99,
     author    = " M. F. G. Johnson and R. A. Schluter and
          M. J. Miksis and S. G. Bankoff",
     title     = " Experimental study of rivulet formation on an
              inclined plate by fluorescent imaging",
     journal   = " J. Fluid Mech.",
     volume    = " 394",
     year      = " 1999",
     pages     = " 339",
}

@Incollection{ JohnsonD93,
     author    = " R. E. Johnson and R. H. Dettre",
     title     = " Wetting of low energy surfaces",
     booktitle= " Wettability",
     editor    = " J. C. Berg ",
     publisher = " Marcel Dekker, New York",
     year      = " 1993",
     pages      = " 1-74",
}
@Book{ Cole(book),
     author    = " W. Bruch and M. W. Cole and E. Zaremba",
     title     = " Physical Adsorption: Forces and Phenomena",
     publisher = " Clarendon: New York",
     year      = " 1997",
}

@Book{ Guggenheim,
     author    = " E. A. Guggenheim",
     title     = " Thermodynamics",
     publisher = " North Holland",
     year      = " 1967",
}

@Article{ JYTB05,
     author    = " L. Joly and C. Ybert and E. Trizac and L. Bocquet",
     title     = " Hydrodynamics within the electric double
                 layer on slipping surfaces",
     journal   = " Phys. Rev. Lett.",
     volume    = " ",
     year      = " 2005",
     pages     = " ",
}

@Article{ JNRR91,
     author    = " D. D. Joseph and J. Nelson and M. Renardy and Y. Renardy",
     title     = " Two-dimensional cusped interfaces",
     journal   = " J. Fluid Mech.",
     volume    = " 223",
     year      = " 1991",
     pages     = " 383-409",
}

@Article{ RPDRZJDRCQ03,
     author    = " Y. Renardy and S. Popinet and L. Duchemin and M. Renardy
 and S. Zaleski and C. Josserand and M. A. Drumright-Clarke and D. Richard
      and C. Clanet and D. Qu\'{e}r\'{e}",
     title     = "Pyramidal and toroidal water drops after impact
                  on a solid surface ",
     journal   = " J. Fluid Mech.",
     volume    = " 484",
     year      = " 2003",
     pages     = " 69",
}

@Article{ PQCM96,
     author    = "M. Pasandideh-Fard and Y. M. Qiao and S. Chandra and
          J. Mostaghime",
     title     = "Capillary effects during droplet impact on a solid surface",
     journal   = " Phys. Fluids",
     volume    = " 8",
     year      = " 1996",
     pages     = " 650",
}

@Article{ KFC00,
     author    = "H.-Y. Kim and Z. C. Feng and J.-H. Chun",
     title     = "Instability of a liquid jet emerging from a droplet
           upon collision with a solid surface",
     journal   = " Phys. Fluids",
     volume    = " 12",
     year      = " 2000",
     pages     = " 531",
}

@Article{ BCM00,
     author    = "M. Bussmann and S. Chandra and J. Mostaghimi",
     title     = "Modeling the splash of a drop impacting on a solid surface",
     journal   = " Phys. Fluids",
     volume    = " 12",
     year      = " 2000",
     pages     = " 3121",
}

@Article{ RQ00,
     author    = "D. Richard and D. Qu{\'e}r{\'e}",
     title     = "Bouncing water drops",
     journal   = " Europhys. Lett.",
     volume    = " 50",
     year      = " 2000",
     pages     = " 769",
}

@Article{ CBRQ04,
     author    = "C. Clanet and C. B{\'e}guin and D. Richard and
               D. Qu\'{e}r\'{e}",
     title     = "Maximal deformation of an impacting drop",
     journal   = " J. Fluid Mech.",
     volume    = " 517",
     year      = " 2004",
     pages     = " 199",
}

@Article{ EF_pre09,
     author    = " J. Eggers and M. Fontelos",
     title     = " Cusps in interfacial problems ",
     journal         = "http://arxiv:math-ph/0910.3499",
     year      = " 2009"
}

@misc{ EFJZ08,
     author    = " J. Eggers and M. Fontelos and
                     C. Josserand and S. Zaleski",
     title     = "Splat! ",
     journal   = " preprint",
     year      = " 2008",
}

@misc{ Josserand,
     author    = " C. Josserand",
     title     = " Christoph's recent simulations",
     year      = " 2008",
}

@Article{ KD79,
     author    = " F. Y. Kafka and E. B. {Dussan V.}",
     title     = " On the interpretation of dynamic contact angles
                     in capillaries",
     journal   = " J. Fluid Mech.",
     volume    = " 95",
     year      = " 1979",
     pages     = " 539-565",
}

@Article{ Sabisky/Anderson,
     author    = " E. S. Sabisky and C. H. Anderson",
     title     = " Verification of the Lifshitz Theory of the van der
            Waals Potential Using Liquid-Helium Films",
     journal   = " Phys. Rev. A",
     volume    = " 7",
     year      = " 1973",
     pages     = " 790",
}

@Article{ KC94,
     author    = " S. Kalliadasis and H.-C. Chang",
     title     = " Apparent dynamic contact angle of an advancing
                   gas-liquid meniscus",
     journal   = " Phys. Fluids",
     volume    = " 6",
     year      = " 1994",
     pages     = " 12-23",
}

@Article{ CDK99,
     author    = " H.-C. Chang and E. A. Demekhin and E. Kalaidin",
     title     = " Iterated stretching of viscoelastic jets",
     journal   = " Phys. Fluids",
     volume    = " 11",
     year      = " 1999",
     pages     = " 1717",
         }

@Article{ MZZC08,
     author    = " S. Maheshwari and L. Zhang and Y. Zhu and H.-C. Chang",
     title     = " Coupling between precipitation and contact-line
              dynamics: multi-ring stains and stick-slip motion",
     journal   = " Phys. Rev. Lett.",
     volume    = " 100",
     year      = " 2008",
     pages     = " 044503",
         }

@Article{ KT97,
     author    = " D. E. Kataoka and S. M. Troian",
     title     = " A theoretical study of instabilities at the
              advancing front of thermally driven coating films",
     journal   = " J. Colloid Interf. Sci.",
     volume    = " 192",
     year      = " 1997",
     pages     = " 350",
}

@Article{ KT98,
     author    = " D. E. Kataoka and S. M. Troian",
     title     = " Stabilizing the advancing front
           of thermally driven advancing films",
     journal   = " J. Colloid Interf. Sci.",
     volume    = " 203",
     year      = " 1998",
     pages     = " 335",
}

@Article{ KOM02,
     author    = " H. P. Kavehpour and B. Ovryn and G. H. McKinley",
     title     = " Evaporatively-driven Marangoni instabilities of volatile
liquid films spreading on thermally active substrates",
     journal   = " Coll. Surf. A",
     volume    = " 206",
     year      = " 2002",
     pages     = " 409-423",
}

@Article{ KOM03,
     author    = " H. P. Kavehpour and B. Ovryn and G. H. McKinley",
     title     = " Microscopic and macroscopic structure of the precursor
                   layer in spreading viscous drops",
     journal   = " Phys. Rev. Lett.",
     volume    = " 91",
     year      = " 2003",
     pages     = " 196104",
}

@Article{ KSM85,
     author    = " R. F. Kayser and J. W. Schmidt and M. R. Moldover",
     title     = " Wetting layers and dispersion forces
     for a fluid in contact with a vertical wall",
     journal   = " Phys. Rev. Lett.",
     volume    = " 54",
     year      = " 1985",
     pages     = " 707",
}
@Article{ Kayser,
     author    = " R. F. Kayser and M. R. Moldover and J. W. Schmidt",
     title     = " What controls the thicknesses of wetting layers?",
     journal   = " J. Chem. Soc. Faraday Trans. II",
     volume    = " 82",
     year      = " 1986",
     pages     = " 1701-1719",
}
@Article{ Schmidt,
     author    = " J. W. Schmidt and M. R. Moldover",
     title     = " A search for the wetting line",
     journal   = " J. Chem. Phys",
     volume    = " 84",
     year      = " 1986",
     pages     = " 4563-4568",
}

@Article{ Kellay,
     author    = " H. Kellay and D. Bonn and J. Meunier",
     title     = " Prewetting  in a binary liquid mixture",
     journal   = " Phys. Rev. Lett.",
     volume    = " 71",
     year      = " 1993",
     pages     = " 2607",
}
@Article{ bertrand01,
     author    = " E. Bertrand and D. Bonn and H. Kellay and
      B. Binks and J. Meunier",
     title     = " Fluctuation effects on wetting films",
     journal   = " Europhys. Lett.",
     volume    = " 55",
     year      = " 2001",
     pages     = " 827-833",
}
@Article{ BR01,
     author    = " D. Bonn and D. Ross",
     title     = " Wetting transitions",
     journal   = " Rep. Progr. Phys.",
     volume    = " 64",
     year      = " 2001",
     pages     = " 1085",
}

@Article{ Klier,
     author    = " J. Klier and P. Stefanyi and A. F. G. Wyatt",
     title     = " Contact-angle of liquid-HE-4 on a CS surface",
     journal   = " Phys. Rev. Lett.",
     volume    = " 75",
     year      = " 1995",
     pages     = " 3709",
}

@Incollection{ jking,
     author    = " J. R. King",
     title     = " Thin-film flows and high-order degenerate
                 parabolic equations",
     booktitle = " Free Surface Flows",
     editors   = " A. C. King and Y. D. Shikhmurzaev",
     year      = " 2001",
     publisher = " Kluwer, Dordrecht",
     pages     = " 7-18",
}

@Incollection{ jking2,
     author    = " J. R. King",
     title     = " The spreading of power-law fluids",
     booktitle = " Free Surface Flows",
     editors   = " A. C. King and Y. D. Shikhmurzaev",
     year      = " 2001",
     publisher = " Kluwer, Dordrecht",
     pages     = " 153-160",
}

@Article{ neogi,
     author    = " P. Neogi and R. M. Ybarra",
     title     = " The absence of a rheological effect on
            the spreading of some drops",
     journal   = " J. Chem. Phys.",
     volume    = " 115",
     year      = " 2001",
     pages     = " 7811-7813",
}

@Article{ YN04,
     author    = " R. M. Ybarra and P. Neogi",
     title     = " Dynamic contact angles under evaporation",
     journal   = " J. Chem. Phys.",
     volume    = " 120",
     year      = " 2004",
     pages     = " 5755-5760"
}

@Incollection{ rosenblat,
     author    = "S. Rosenblat and S. H. Davis",
     title     = " How do liquid drops spread on solids?",
     booktitle = " Frontiers in Fluid Mechanics",
     editors   = " S. H. Davis and J. L. Lumley",
     year      = " 1985",
     publisher = " Springer",
     pages     = " 171-183",
}

@Article{ salima,
     author    = " S. Rafa{\"\i} and D. Bonn and A. Boudaoud",
     title     = " Spreading of non-Newtonian fluids on hydrophilic surfaces",
     journal   = " J. Fluid Mech.",
     volume    = " 513",
     year      = " 2004",
     pages     = " 77-85",
}

@Article{ super,
     author    = " S. Rafa{\"\i} and D. Sarker and V. Bergeron
                  and J. Meunier and D. Bonn",
     title     = " Superspreading: Aqueous surfactant drops
         spreading on hydrophobic surfaces",
     journal   = " Langmuir",
     volume    = " 18",
     year      = " 2002",
     pages     = " 10486-10488",
}

@Article{ starov,
     author    = " V. M. Starov and A. N. Tyatyushkin and
          M. G. Velarde and S. A. Zhdanov",
     title     = " Spreading of non-newtonian liquids over solid substrates",
     journal   = " J. Coll. Int. Sci.",
     volume    = " 257",
     year      = " 2003",
     pages     = " 284-290",
}

@Incollection{ K93,
     author    = " S. Kistler",
     title     = " Hydrodynamics of wetting",
     booktitle = " Wettability",
     editor    = " J. C. Berg",
     year      = " 1993",
     publisher = " Marcel Dekker, New York",
     pages     = " 311-429",
}

@Book{ Berg93,
     author    = " J. C. Berg, ed.",
     title     = " Wettability",
     publisher = " Marcel Dekker, New York",
     year      = " 1993",
 }

@Book{ Rosen63,
     author    = " L. Rosenhead",
     title     = " Laminar boundary layers",
     publisher = " Oxford University Press",
     year      = " 1963",
 }

@Book{ SVR07,
     author    = " V. M. Starov and M. G. Velarde and C. J. Radke",
     title     = " Wettability",
     publisher = " CRC Press, Boca Raton",
     year      = " 2007",
 }

@Book{ dC,
     author    = " M. P. {do Carmo}",
     title     = " Differential geometry of curves and surfaces",
     publisher = " Prentice-Hall, Englewood Cliffs, N. J.",
     year      = " 1976",
 }

@Article{ K03,
     author    = " L. Kondic",
     title     = " Instabilities in gravity driven fow of thin fluid films",
     journal   = " SIAM Review",
     volume    = " 45",
     year      = " 2003",
     pages     = " 95-115",
}

@Article{ KB99,
     author    = " L. Kondic and A. L. Bertozzi",
     title     = " Nonlinear dynamics and transient
                  growth of driven contact lines",
     journal   = " Phys. Fluids",
     volume    = " 11",
     year      = " 1999",
     pages     = " 3560-3562",
}

@Article{ KBW89,
     author    = " J. Koplik and J. R. Banavar and J. F. Willemsen",
     title     = " Molecular dynamics of fluid flow at solid surfaces",
     journal   = " Phys. Fluids A",
     volume    = " 1",
     year      = " 1989",
     pages     = " 781-794",
}

@Article{ kumar,
     author    = " S. Kumar and D. H. Reich and M. O. Robbins",
     title     = " Critical dynamics of
                    contact line motion",
     journal   = " Phys. Rev. E",
     volume    = " 52",
     year      = " 1995",
     pages     = " R5776-5779",
}

@Article{ L82,
     author    = " A. A. Lacey",
     title     = " The motion with slip of a thin viscous
       droplet over a solid surface",
     journal   = " Stud. Appl. Math.",
     volume    = " 67",
     year      = " 1982",
     pages     = " 217-230",
}

@Article{ LL42,
     author    = " L. D. Landau and B. V. Levich",
     title     = " Dragging of a liquid by a moving plate",
     journal   = " Acta physico-chimica USSR",
     volume    = " 17",
     year      = " 1942",
     pages     = " 42",
}

@Book{ L99,
     author    = " R. G. Larson",
     title     = " The structure and rheology of complex fluids",
     publisher = " Oxford University Press, New York",
     year      = " 1999",

}

@Article{ LEGAS88,
     author    = " L. L{\'e}ger and M. Erman and
       A. M. Guinet-Picard and D. Ausserre and C. Strazielle",
     title     = " Precursor film profiles of spreading liquid drops",
     journal   = " Phys. Rev. Lett.",
     volume    = " 60",
     year      = " 1988",
     pages     = " 2390-2393",
}

@Article{ LJ92,
     author    = " L. L{\'e}ger and J.-F. Joanny",
     title     = " Liquid spreading",
     journal   = " Rep. Prog. Phys.",
     volume    = " 55",
     year      = " 1992",
     pages     = " 431-486",
}

@Article{ LCCHN88,
     author    = " P. Levinson and A.-M. Cazabat and M. A. Cohen-Stuart
                and F. Heslot and S. Nicolet",
     title     = " The spreading of macroscopic droplets",
     journal   = " Revue Phys. Appl.",
     volume    = " 23",
     year      = " 1988",
     pages     = " 1009-1016",
}

@Book{ L62,
     author    = " V. G. Levich",
     title     = " Physicochemical Hydrodynamics",
     publisher = " Prentice-Hall, Englewood Cliffs, N.J.",
     year      = " 1962",
     pages     = " ",
}

@Article{ LRM04,
     author    = " S. Lichter and A. Roxin and S. Mandre",
     title     = " Mechanisms for liquid slip at solid surfaces",
     journal   = " Phys. Rev. Lett.",
     volume    = " 93",
     year      = " 2004",
     pages     = " 086001",
}

@Article{ LS03,
     author    = " L. Limat and H. A. Stone",
     title     = " Three-dimensional lubrication model of a
              contact line corner singularity",
     journal   = " Europhys. Lett.",
     volume    = " 65",
     year      = " 2004",
     pages     = " 365",
}

@Article{ LKZ83,
     author    = " R. Lipowsky and D. M. Kroll and R. K. P. Zia",
     title     = " Effective field theory for interface delocalization
                      transitions",
     journal   = " Phys. Rev. B",
     volume    = " 27",
     year      = " 1983",
     pages     = " R4499-4502",
}

@Article{ Lipowsky84,
     author    = " R. Lipowsky",
     title     = " Upper critical dimension for wetting in systems
                     with long-range forces",
     journal   = " Phys. Rev. Lett.",
     volume    = " 52",
     year      = " 1984",
     pages     = " 1429",
}

@Article{ Lipowsky,
     author    = " R. Lipowsky and D. M. Kroll",
     title     = " Critical wetting in systems with long-range forces",
     journal   = " Phys. Rev. Lett.",
     volume    = " 52",
     year      = " 1984",
     pages     = " 2303",
}

@Article{ L75,
     author    = " G. Lippmann",
     title     = " Relation entre les phenomenes electriques et capillaires",
     journal   = " Ann. Chim. Phys.",
     volume    = " 5",
     year      = " 1875",
     pages     = " 494",
}

@Article{ LMR76,
     author    = " J. Lopez and C. A. Miller and E. Ruckenstein",
     title     = " Spreading kinetics of of liquid drops on solids",
     journal   = " J. Colloid Interface Sci.",
     volume    = " 56",
     year      = " 1976",
     pages     = " 460-468",
}

@Article{ LQE04,
     author    = " E. Lorenceau and D. Qu\'{e}r\'{e} and J. Eggers",
     title     = " Air Entrainment by a Viscous Jet Plunging into a Bath",
     journal   = " Phys. Rev. Lett.",
     volume    = " 93",
     year      = " 2004",
     pages     = " 254501",
}

@Article{ Bin93,
     author    = " A. K. Bin",
     title     = " Gas entrainment by plunging liquid jets",
     journal   = " Chem. Eng. Sci.",
     volume    = " 48",
     year      = " 1993",
     pages     = " 3585-3630",
}

@Article{ LD66,
     author    = " T. J. Lin and H. G. Donnelly",
     title     = " Gas bubble entrainment by plunging laminar liquid jets",
     journal   = " A. I. Ch. E. J.",
     volume    = " 12",
     year      = " 1966",
     pages     = " 563",
}

@Article{ Lucht,
     author    = " R. Lucht and C. H. Bahr",
     title     = " Prewetting critical point in a binary liquid-crystal system",
     journal   = " Phys. Rev. Lett.",
     volume    = " 80",
     year      = " 1998",
     pages     = " 3783",
}

@Article{ MGD93,
     author    = " J. A. Marsh and S. Garoff and E. B. {Dussan V.} ",
     title     = " Dynamic contact angles and hydrodynamics
               near a moving contact line",
     journal   = " Phys. Rev. Lett.",
     volume    = " 70",
     year      = " 1993",
     pages     = " 2778-2781",
}
@Article{ DRG91,
     author    = " E. B. {Dussan V.} and E. Ram\'{e} and S. Garoff",
     title     = " On identifying the appropriate boundary condition
                    at a moving contact line: an experimental investigation",
     journal   = " J. Fluid Mech.",
     volume    = " 230",
     year      = " 1991",
     pages     = " 97",
}

@Article{ MGH04,
     author    = " A. Mazouchi and C. M.  Gramlich and G. M. Homsy",
     title     = " Time-dependent free surface Stokes flow with a
             moving contact line I. Flow over planar surfaces",
     journal   = " Phys. Fluids",
     volume    = " 16",
     year      = " 2004",
     pages     = " 1647-1659",
}

@Article{ MNRB95,
     author    = " G. McHale and M. I. Newton and S. M. Rowan and M. Banerjee",
     title     = " The spreading of small viscous stripes of oil",
     journal   = " J. Phys. D: Appl. Phys.",
     volume    = " 28",
     year      = " 1995",
     pages     = " 1925-1929",
}

@Article{ MJF89,
     author    = " F. Melo and J.-F. Joanny and S. Fauve",
     title     = " Fingering instability of spinning drops",
     journal   = " Phys. Rev. Lett.",
     volume    = " 63",
     year      = " 1989",
     pages     = " 1958",
}

@Conference{ mckinley,
     author    = " G. H. McKinley and B. Ovryn",
     title     = " An interferometric investigation of contact
              line dynamics in spreading polymer melts and solutions",
     conference= " Proceedings of the Fourth Microgravity
          Fluid Physics and Transport Phenomena Conference",
     year      = " 1998",
     place     = " Cleveland, Ohio",
}

@Book{ M95,
     author    = " S. Middleman",
     title     = " Modeling Axisymmetric Flows",
     publisher = " Academic, San Diego",
     year      = " 1995",
}

@Article{ MABT99,
     author    = " G. Mistura and F. Ancilotto and L. Bruschi and F. Toigo",
     title     = " Wetting of argon on CO2",
     journal   = " Phys. Rev. Lett.",
     volume    = " 82",
     year      = " 1999",
     pages     = " 795",
}

@Article{ M93,
     author    = " V. S. Mitlin",
     title     = "Dewetting of solid surface: analogy with spinodal
             decomposition ",
     journal   = " J. Colloid Interface Sci.",
     volume    = " 156",
     year      = " 1993",
     pages     = " 491",
}

@Article{ MLWGS01,
     author    = " J. Moon and J. Lowekamp and P. Wynblatt and S. Garoff
             and R. M. Suter",
     title     = " Effects of concentration dependent
      diffusivity on the growth of precursing films of Pb on Cu",
     journal   = " Surf. Sci.",
     volume    = " 488",
     year      = " 2001",
     pages     = " 73-82",
}

@Article{ ML94,
     author    = " J. F. de la Mora and I. G. Loscertales",
     title     = " The current emitted by highly conducting Taylor cones",
     journal   = " J. Fluid Mech.",
     volume    = " 260",
     year      = " 1994",
     pages     = " 155-184",
}

@Article{ cerro,
     author    = " C. Del Cerro and G. J. Jameson",
     title     = " The behavior of pentane, hexane, and heptane on water",
     journal   = " J. Colloid Interf. Sci.",
     volume    = " 78",
     year      = " 1980",
     pages     = " 362-375",
}

@Article{ MS92,
     author    = " J. A. Moriarty and L. W. Schwartz",
     title     = " Effective slip in numerical calculations of
         moving-contact-line problems",
     journal   = " J. Eng. Math.",
     volume    = " 26",
     year      = " 1992",
     pages     = " 81",
}

@Article{ Moulinet1,
     author    = " S. Moulinet and C. Guthmann and E. Rolley",
     title     = " Roughness and dynamics of a contact line of a
                 viscous fluid on a disordered substrate",
     journal   = " Eur. Phys. J. E",
     volume    = " 8",
     year      = " 2002",
     pages     = " 437-443",
}

@Article{ Moulinet2,
     author    = " S. Moulinet and C. Guthmann and E. Rolley",
     title     = " Dissipation in the dynamics of a moving contact line: effect of the substrate disorder",
     journal   = " Eur. Phys. J. B",
     volume    = " 37",
     year      = " 2004",
     pages     = " 127",
}

@Article{ Moulinet3,
     author    = " S. Moulinet and A. Rosso and W. Krauth and E. Rolley ",
     title     = " Width distribution of contact lines on a
                disordered substrate",
     journal   = " Phys. Rev. E",
     volume    = " 69",
     year      = " 2004",
     pages     = " 035103(R)",
}
@Article{ Muller,
     author    = " X. M{\"u}ller and J. Dupont-Roc",
     title     = " Prewetting transition on a weakly disordered
            substrate: Evidence for a creeping film dynamics",
     journal   = " Europhys. Lett.",
     volume    = " 54",
     year      = " 2001",
     pages     = " 533-539",
}

@Article{ ML00,
     author    = " M. Moseler and U. Landman",
     title     = " Formation, Stability, and Breakup of Nanojets",
     journal   = " Science",
     volume    = " 289",
     year      = " 2000",
     pages     = " 1165-1169",
}

@Article{ MKBSH05,
     author    = " F. Mugele and A. Klingner and J. Buehrle
     and D. Steinhauser and S. Herminghaus",
     title     = " Electrowetting: a covenient way to
         switchable wettability patterns",
     journal   = " J. Phys.: Condens. Matter",
     volume    = " 17",
     year      = " 2005",
     pages     = " S559",
}

@Article{ MB07,
     author    = " F. Mugele and J. Buehrle",
     title     = " Equilibrium drop surface profiles in electric fields",
     journal   = " J. Phys.: Condens. Matter",
     volume    = " 19",
     year      = " 2007",
     pages     = " 375112",
}

@Article{ MB05,
     author    = " F. Mugele and J.-C. Baret",
     title     = " Electrowetting: from basics to applications",
     journal   = " J. Phys.: Condens. Matter",
     volume    = " 17",
     year      = " 2005",
     pages     = " R705",
}

@Article{ Mumley,
     author    = " T. E. Mumley and C. J. Radke and M. C. Williams",
     title     = " ",
     journal   = " J. of Colloid Interface Sci.",
     volume    = " 109",
     year      = " 1986",
     pages     = " 398",
}

@Article{ Nacher,
     author    = " P. J. Nacher and J. Dupont-Roc",
     title     = " Experimental-evidence for nonwetting with
                 superfluid-helium ",
     journal   = " Phys. Rev. Lett.",
     volume    = " 67",
     year      = " 1991",
     pages     = " 2966",
}

@Article{ Nadkarni,
     author    = " G. D. Nadkarni and S. Garoff",
     title     = " An investigation of microscopic
                      aspects of contact angle hysteresis:
              Pinning of the Contact Line on a Single Defect",
     journal   = " Europhys. Lett.",
     volume    = " 20",
     year      = " 1992",
     pages     = " 523-528",
}

@Article{ NC04,
     author    = " G. Nagayama and P. Cheng",
     title     = " Effects of interface wettability on microscale flow by
molecular dynamics simulation",
     journal   = " Int. J. Heat Mass Trans.",
     volume    = " 47",
     year      = " 2004",
     pages     = " 501-513",
}

@Article{ Nakanishi,
     author    = " H. Nakanishi and M. E. Fisher",
     title     = " Multicriticality of wetting, pre-wetting,
             and surface transitions",
     journal   = " Phys. Rev. Lett.",
     volume    = " 49",
     year      = " 1982",
     pages     = " 1565",
}
@Article{ Kozhevnikov,
     author    = " V. F. Kozhevnikov and D. I. Arnold and S. P. Naurzakov
                   and M. E. Fisher",
     title     = " Prewetting transitions in a near-critical metallic vapor",
     journal   = " Phys. Rev. Lett.",
     volume    = " 78",
     year      = " 1997",
     pages     = " 1735-1738",
}
@Article{ fisherhuse,
     author    = " D. S. Fisher and D. A. Huse",
     title     = " Multicriticality of wetting, pre-wetting,
             and surface transitions",
     journal   = " Phys. Rev. B",
     volume    = " 32",
     year      = " 1985",
     pages     = " 247-256",
}

@Article{ NF92,
     author    = " O. Narayan and D. S. Fisher",
     title     = " Critical behavior of sliding
        charge-density waves in 4- epsilon dimensions",
     journal   = " Phys. Rev. B",
     volume    = " 46",
     year      = " 1992",
     pages     = " 11520-11549",
}

@Article{ N23,
     author    = " C. L. Navier",
     title     = " Sur les lois du mouvement des fluides",
     journal   = " Mem. Acad. R. Sci. France",
     volume    = " 6",
     year      = " 1827",
     pages     = " 389-440",
}

@Article{ NCR04,
     author    = " X. Nie and S. Chen and M. O. Robbins",
     title     = " Hybrid continuum-atomistic simulation of
                   singular corner flow",
     journal   = " Phys. Fluids",
     volume    = " 16",
     year      = " 2004",
     pages     = " 3579-3591",
}

@Article{ NWCKPK02,
     author    = " A. D. Nikolov and D. T. Wasan and A. Chengara
        and K. Koczoand G. A. Policello and I. Kolossvary",
     title     = " Superspreading driven by Marangoni flow",
     journal   = " Adv. Colloid Interf. Sci.",
     volume    = " 96",
     year      = " 2002",
     pages     = " 325-338",
}

@Article{ WKN94,
     author    = "  D. T. Wasan and K. Koczo and A. D. Nikolov",
     title     = " Mechanisms of aqueous foam stability and antifoaming action
                         with and without oil - a thin film approach",
     journal   = " Adv. Chem.",
     volume    = " 242",
     year      = " 1994",
     pages     = " 47-111",
}

@Article{ NVB01,
     author    = " P. Notz and A. U. Chen and O. A. Basaran",
     title     = " Satellite drops: Unexpected
    dynamics and change of scaling during pinch-off",
     journal   = " Phys. Fluids",
     volume    = " 13",
     year      = " 2001",
     pages     = " 549-552",
}

@Article{ OT95,
     author    = " S. T. O'Connell and P. A. Thompson",
     title     = " Molecular dynamics-continuum hybrid computation: A tool for studying complex fluid flows",
     journal   = " Phys. Rev. E",
     volume    = " 52",
     year      = " 1995",
     pages     = " R5792-R5795",
}

@Article{ OTAT74,
     author    = " V. A. Ogarev and T. N. Timonina and V. V. Arslanov and
                      A. A. Trapeznikov",
     title     = " Spreading of polydimethylsiloxane drops on solid
              horizontal surfaces",
     journal   = " J. Adhesion",
     volume    = " 6",
     year      = " 1974",
     pages     = " 337-356",
}

@Article{ ASB96,
     author    = " C. Andrieu and C. Sykes and F. Brochard",
     title     = " Dynamics of fast dewetting on model solid substrates",
     journal   = " J. Adhesion",
     volume    = " 58",
     year      = " 1996",
     pages     = " 15-24",
}

@misc{ Andrieu95,
     author    = " C. Andrieu",
     title     = " Angles de contact et d{\'e}moulliage",
     howpublished = " Ph.D. Thesis, Universit{\'e} Paris VI",
     year      = " 1995",

}

@Article{ ODB97,
     author    = " A. Oron and S. H. Davis and S. G. Bankoff",
     title     = " Long-scale evolution of thin liquid films",
     journal   = " Rev. Mod. Phys.",
     volume    = " 69",
     year      = " 1997",
     pages     = " 931-980",
}

@Article{ AD95,
     author    = " D. M. Anderson and S. H. Davis",
     title     = " The spreading of volatile liquid droplets on heated
              surfaces",
     journal   = " Phys. Fluids",
     volume    = " 7",
     year      = " 1995",
     pages     = " 248"
}

@Article{ Morris00,
     author    = " S. J. S. Morris",
     title     = " A phenomenological model for the contact region of an
            evaporating meniscus on a superheated slab",
     journal   = " J. Fluid Mech.",
     volume    = " 411",
     year      = " 2000",
     pages     = " 59",
}

@Article{ CM09,
     author    = " R. V. Craster and O. K. Matar",
     title     = " Dynamics and stability of thin liquid films",
     journal   = " Rev. Mod. Phys.",
     volume    = " 81",
     year      = " 2009",
     pages     = " 1131-1198",
}

@Article{ OKYK04,
     author    = " M. Oron and T. Kerle and R. Yerushalmi-Rozon and J. Klein",
     title     = " Pesistent droplet motion in liquid-liquid dewetting",
     journal   = " Phys. Rev. Lett.",
     volume    = " 92",
     year      = " 2004",
     pages     = " 236104",
}

@Article{ Parryreview,
     author    = " A. O. Parry",
     title     = " Three-dimensional wetting revisited",
     journal   = " J. Phys. Cond. Matt.",
     volume    = " 8",
     year      = " 1996",
     pages     = " 10761-10778",
}
@Article{ ParryPRL,
     author    = " A. O. Parry and J. M. Romero-Enrique and A. Lazarides",
     title     = " Non-locality and short-range wetting phenomena",
     journal   = " Phys. Rev. Lett.",
     volume    = " 93",
     year      = " 2004",
     pages     = " 086104",
}
@Article{ ParryJPCM,
     author    = " A. O. Parry and C. Rasc\'on and
      N. R. Bernardino and J. M. Romero-Enrique",
     title     = " Derivation of a non-local interfacial Hamiltonian for short-ranged wetting: I. Double-parabola approximation",
     journal   = " J. Phys. Cond. Matt.",
     volume    = " 18",
     year      = " 2006",
     pages     = " 6433-6451",
}
@Article{ Henderson,
     author    = " J. R. Henderson",
     title     = " An elegant advance in the physics of wetting",
     journal   = " J. Phys. Cond. Matt.",
     volume    = " 18",
     year      = " 2006",
     pages     = " V11-V14",
}
@Article{ P91,
     author    = " A. O. Parry and B. Evans and K. Binder",
     title     = " Critical amplitude ratios for critical wetting in 3
  dimensions - observation of nonclassical behavior in the Ising model",
     journal   = " Phys. Rev. B",
     volume    = " 43",
     year      = " 1991",
     pages     = " 11535-11538",
}

@Article{ P59,
     author    = " R. E. Pattle",
     title     = " Diffusion from an instantaneous point source with
           concentration-dependent coefficient",
     journal   = " Q. J. Mech. Appl. Math.",
     volume    = " 12",
     year      = " 1959",
     pages     = " 407-409",
}


@Article{ PKM80,
     author    = " J. G. Petrov and H. Kuhn and D.  Mobius",
     title     = " Three-Phase Contact Line Motion in the Deposition
of Spread Monolayers",
     journal   = " J. Colloid Interf. Sci.",
     volume    = " 73",
     year      = " 1980",
     pages     = " 66-75",
}


@Article{ PR81,
     author    = " J. G. Petrov and B. P. Radoev",
     title     = " Steady motion of the three phase contact line in model
Langmuir-Blodgett systems",
     journal   = " Colloid Polymer Sci.",
     volume    = " 259",
     year      = " 1981",
     pages     = " 753-760",
}

@Article{ PS85,
     author    = " J. G. Petrov and R. V. Sedev",
     title     = " On the existence of a maximum speed of wetting",
     journal   = " Colloids Surfaces",
     volume    = " 13",
     year      = " 1985",
     pages     = " 313-322",
}


@Article{ PP98,
     author    = " J. G. Petrov and P. G. Petrov",
     title     = " Molecular-Hydrodynamic Description of Langmuir-Blodgett
                  Deposition",
     journal   = " Colloid Polymer Sci.",
     volume    = " 259",
     year      = " 1998",
     pages     = " 753-760",
}

@Article{ PP92,
     author    = "P. G. Petrov and J. G. Petrov",
     title     = " A combined molecular-hydrodynamic approach to wetting
                      kinetics",
     journal   = " Langmuir",
     volume    = " 8",
     year      = " 1992",
     pages     = " 1762",
}

@Article{ Milchev,
     author    = " A. Milchev and M. Mueller and K. Binder and D. P. Landau",
     title     = " Interface localization-delocalization in a double wedge:
 a new universality class with strong fluctuations and anisotropic scaling",
     journal   = " Phys. Rev. Lett.",
     volume    = " 90",
     year      = " 2003",
     pages     = " 136101",
}
@Article{ rascon3,
     author    = " C. Rasc{\'o}n and A. O. Parry",
     title     = " Geometry dependent critical exponents at complete wetting",
     journal   = " J. Chem. Phys.",
     volume    = " 112",
     year      = " 2000",
     pages     = " 5175-5180",
}
@Article{ PRSH03a,
     author    = " J. G. Petrov and J. Ralston and
           M. Schneemilch and R. A. Haynes",
     title     = " Dynamics of partial wetting and dewetting
              of an amorphous fluoropolymer by pure liquids",
     journal   = " Langmuir",
     volume    = " 19",
     year      = " 2003",
     pages     = " 2795-2801",
}

@Article{ PRSH03b,
     author    = " J. G. Petrov and J. Ralston and
                  M. Schneemilch and R. A. Haynes",
     title     = " Dynamics of partial wetting and dewetting in
well-defined systems",
     journal   = " J. Phys. Chem.",
     volume    = " 107",
     year      = " 2003",
     pages     = " 1634-1645",
}

@Article{ PP00,
     author    = " L. M. Pismen and Y. Pomeau",
     title     = " Disjoijning potential and spreading of thin layers in
                   the diffuse interface model coupled to hydrodynamics",
     journal   = " Phys. Rev. E",
     volume    = " 62",
     year      = " 2000",
     pages     = " 2480-2492",
}

@Article{ LP01,
     author    = " L. M. Pismen",
     title     = " Nonlocal diffuse interface theory of thin films
            and moving contact line",
     journal   = " Phys. Rev. E",
     volume    = " 64",
     year      = " 2001",
     pages     = " 021603",
}

@Article{ LP02,
     author    = " L. M. Pismen",
     title     = " Mesoscopic hydrodynamics of contact line motion",
     journal   = " Colloids and Surfaces A",
     volume    = " 206",
     year      = " 2002",
     pages     = " 11-30",
}

@Article{ LP04,
     author    = " L. M. Pismen",
     title     = " Spinodal dewetting in a volatile liquid film",
     journal   = " Phys. Rev. E",
     volume    = " 70",
     year      = " 2004",
     pages     = " 021601",
}

@Article{ LP06,
     author    = " L. M. Pismen",
     title     = " Perturbation theory for traveling droplet",
     journal   = " Phys. Rev. E",
     volume    = " 74",
     year      = " 2006",
     pages     = " 041605",
}

@Incollection{ LP08,
     author    = " L. M. Pismen",
     title     = " Thin film and droplet patterns shaped by surface forces",
     booktitle     = " Pattern Formation at Interfaces",
     editor     = " P. Colinet and A. A. Nepomnyashchy",
     publisher = " Springer, Berlin",
     year      = " 2008",
     pages      = "to appear",

}

@Article{ WP08,
     author    = " O. Weinstein and L.M. Pismen",
     title     = " Scale dependence of contact line computations",
     journal   = " MMNP",
     volume    = " 3",
     year      = " 2008",
     pages     = " 98-107",
}

@Article{ PFL01,
     author    = " T. Podgorski and J. M. Flesselles and  L. Limat",
     title     = " Corners, cusps, and pearls in running drops",
     journal   = " Phys. Rev. Lett.",
     volume    = " 87",
     year      = " 2001",
     pages     = " 036102(1)-(4)",
}

@Article{ P00,
     author    = " Y. Pomeau",
     title     = " Representation of the moving contact line in
  the eqautions of fluid mechanics (in French)",
     journal   = " C. R. Acad. Sci. Paris",
     volume    = " 328",
     year      = " 2000",
     pages     = " 411-416",
}

@Article{ P02,
     author    = " Y. Pomeau",
     title     = " Recent progress in the moving contact line problem:
                  a review",
     journal   = " C. R. Mecanique",
     volume    = " 330",
     year      = " 2002",
     pages     = " 207-222",
}

@Article{ PD04,
     author    = " M. N. Popescu and S. Dietrich",
     title     = " Model for spreading of liquid monolayers",
     journal   = " Phys. Rev. E",
     volume    = " 69",
     year      = " 2004",
     pages     = " 061602",
}
@Article{ DPR05,
     author    = " S. Dietrich and M. N. Popescu and M. Rauscher",
     title     = " Wetting on structured substrates",
     journal   = " J. Phys.: Condens. Matter",
     volume    = " 17",
     year      = " 2005",
     pages     = " S577",
}
@Article{ RDK07,
     author    = " M. Rauscher and S. Dietrich and J. Koplik",
     title     = " Shear Flow Pumping in Open Micro- and Nanofluidic
                    Systems",
     journal   = " Phys. Rev. Lett.",
     volume    = " 98",
     year      = " 2007",
     pages     = " 224504",
}
@Article{ MRD06,
     author    = " Moosavi, A. and Rauscher, M. and Dietrich, S.",
     title     = " Motion of Nnaodroplets near Edges and Wedges",
     journal   = " Phys. Rev. Lett.",
     volume    = " 97",
     year      = " 2006",
     pages     = " 236101",
}
@Article{ KLRD06,
     author    = " J. Koplik and T. S. Lo and M. Rauscher and S. Dietrich",
     title     = " Pearling instability of nanoscale fluid flow
                    confined to a chemical channel",
     journal   = " Phys. Fluids",
     volume    = " 18",
     year      = " 2006",
     pages     = " 032104",
}
@Article{ PDO05,
     author    = " M. N. Popescu and S. Dietrich and G. Oshanin",
     title     = " Diffusive spreading and mixing of fluid monolayers",
     journal   = " J. Phys.: Condens. Matter",
     volume    = " 17",
     year      = " 2005",
     pages     = " S4189",
}
@Article{ Dietschick,
     author    = " S. Dietrich and M. Schick",
     title     = " Critical wetting of surfaces in systems with long-range
                      forces",
     journal   = " Phys. Rev. B",
     volume    = " 31",
     year      = " 1985",
     pages     = " 4718-4720",
}
@Article{ Hauge,
     author    = " E. H. Hauge and M. Schick",
     title     = " Continuous and1st-order wetting transition from the
              van-der-Waals theory of fluids",
     journal   = " Phys. Rev. B",
     volume    = " 27",
     year      = " 1983",
     pages     = " 4288",
}
@Article{ Pandit,
     author    = " R. Pandit and M. Schick and M. Wortis",
     title     = " Systematics of multilayer adsorption phenomena
             on attractive substrates",
     journal   = " Phys. Rev. B",
     volume    = " 26",
     year      = " 1982",
     pages     = " 5112-5140",
}

@Article{ DietrichNapiorkow,
     author    = " S. Dietrich and M. Napiorkowski",
     title     = " Analytical results for wetting transitions in the presence
             of van-der-Waals tails",
     journal   = " Phys. Rev. A",
     volume    = " 43",
     year      = " 1991",
     pages     = " 1861-1885",
}


@Article{ Prevost02,
     author    = " A. Prevost and E. Rolley and C. Guthmann",
     title     = " Dynamics of a helium-4 meniscus on a strongly
            disordered cesium substrate",
     journal   = " Phys. Rev. B",
     volume    = " 65",
     year      = " 2002",
     pages     = " 064517",
}
@Article{ Poujade,
     author    = " M. Poujade and C. Guthmann and E. Rolley",
     title     = " Propagative modes along a superfluid Helium-4 meniscus",
     journal   = " Europhys. Lett.",
     volume    = " 59",
     year      = " 2002",
     pages     = " 862",
}

@Article{ PomeauV,
     author    = " Y. Pomeau and J. Vannimenus",
     title     = " Contact angle on heterogeneous
           surfaces: weak heterogeneities",
     journal   = " J. Colloid Int. Sc.",
     volume    = " 104",
     year      = " 1985",
     pages     = " 477-488",
}

@Article{ Prevost99,
     author    = " A. Prevost and E. Rolley and C. Guthmann",
     title     = " Thermally activated motion of the contact line of a
               liquid Helium-4 meniscus on a Cesium substrate",
     journal   = " Phys. Rev. Lett.",
     volume    = " 83",
     year      = " 1999",
     pages     = " 348-351",
}
@Article{ Rolley,
     author    = " E. Rolley and C. Guthmann",
     title     = " Optical measurement of contact angle of liquid
                 helium on cesium",
     journal   = " J. Low Temp. Phys.",
     volume    = " 108",
     year      = " 1997",
     pages     = " 1-9",
}

@Article{ QWS03,
     author    = " T. Qian and X.-P. Wang and P. Sheng",
     title     = " Molecular scale contact line
               hydrodynamics of immiscible flows",
     journal   = " Phys. Rev. E",
     volume    = " 68",
     year      = " 2003",
     pages     = " 016306",
}

@Article{ QWS04,
     author    = " T. Qian and X.-P. Wang and P. Sheng",
     title     = " Power-law slip profile of the moving
             contact line in two-phase immiscible flows",
     journal   = " Phys. Rev. Lett.",
     volume    = " 93",
     year      = " 2004",
     pages     = " 094501",
}

@Article{ QWS06,
     author    = " T. Qian and X.-P. Wang and P. Sheng",
     title     = " A variational approach to moving contact line
                      hydrodynamics ",
     journal   = " J. Fluid Mech.",
     volume    = " 564",
     year      = " 2006",
     pages     = " 333",
}

@Article{ RE07,
     author    = " W. Ren and W. E",
     title     = " Boundary conditions for the moving contact line problem",
     journal   = " Phys. Fluids",
     volume    = " 19",
     year      = " 2007",
     pages     = " 022101",
}

@Article{ Q91,
     author    = " D. Qu\'{e}r\'{e}",
     title     = " On the minimal velocity of forced spreading in
             partial wetting (in French)",
     journal   = " C. R. Acad. Sci. Paris, Serie II",
     volume    = " 313",
     year      = " 1991",
     pages     = " 313-318",
}

@Article{ Q99,
     author    = " D. Qu{\'e}r{\'e}",
     title     = " Fluid coating on a fiber",
     journal   = " Annu Rev. Fluid Mech.",
     volume    = " 31",
     year      = " 1999",
     pages     = " 347",
}

@Article{ QB01,
     author    = " C. Quilliet and B. Berge",
     title     = " Electrowetting: a recent outbreak",
     journal   = " Curr. Op. Colloid Interface Sci.",
     volume    = " 6",
     year      = " 2001",
     pages     = " 34-39",
}

@Article{ BVQM06,
     author    = " M. Bienia and M. Vallade and C. Quilliet and F. Mugele",
     title     = " Electrical-field-induced curvature increase
                    on a drop of conducting liquid",
     journal   = " Europhysics Letters",
     volume    = " 74",
     year      = " 2006",
     pages     = " 103-109",
}

@Article{ casteletto,
     author    = " V. Castelletto and I. Cantat and D. Sarker and
      R. Bausch and D. Bonn and J. Meunier",
     title     = " Stability of soap films: Hysteresis and
             nucleation of black films",
     journal   = " Phys. Rev. Lett.",
     volume    = " 90",
     year      = " 2003",
     pages     = " 048302",
}

@Article{ Rafai,
     author    =  "S. Rafa{\"\i} and D. Bonn and E. Bertrand and
         J. Meunier and V. C. Weiss and J. O. Indekeu",
     title     = " Long-range critical wetting: Observation of
             a critical end point",
     journal   = " Phys. Rev. Lett.",
     volume    = " 92",
     year      = " 2004",
     pages     = " 245701",
}
@Article{ bergeron,
     author    = " V. Bergeron and D. Bonn and J.-Y. Martin and
             L. Vovelle",
     title     = " Controlling droplet deposition with polymer additives",
     journal   = " Nature",
     volume    = " 405",
     year      = " 2000",
     pages     = " 772-775",
}
@Article{ RafaiPhysicaA,
     author    = " S. Rafa{\"\i}",
     title     = " Spreading of non-Newtonian fluids and surfactant
            solutions on solid surfaces ",
     journal   = " Physica A",
     volume    = " 358",
     year      = " 2005",
     pages     = " 58",
}

@Article{ Ramos,
     author    = " S. M. M. Ramos and E. Charlaix
                  and A. Benyagoub and M. Toulemonde",
     title     = " Wetting on nanorough surfaces",
     journal   = " Phys. Rev. E",
     volume    = " 67",
     year      = " 2003",
     pages     = " 031604",
}
@Article{ RaphaeldG89,
     author    = " E. Rapha{\"e}l and P.-G. de Gennes",
     title     = " Dynamics of wetting with nonideal surfaces",
     journal   = " J. Chem. Phys.",
     volume    = " 90",
     year      = " 1989",
     pages     = " 7577-7584",
}

@Article{ RBR91,
     author    = " C. Redon and F. Brochard-Wyart and F. Rondelez",
     title     = " Dynamics of dewetting",
     journal   = " Phys. Rev. Lett.",
     volume    = " 66",
     year      = " 1991",
     pages     = " 715",
}

@Article{ Rascon,
     author    = " C. Rasc{\'o}n and A. O. Parry",
     title     = " Geometry-dominated fluid adsorption on sculpted
                   solid substrates",
     journal   = " Nature",
     volume    = " 407",
     year      = " 2000",
     pages     = " 986",
}

@Article{ R92,
     author    = " G. Reiter",
     title     = " Dewetting of thin polymer films",
     journal   = " Phys. Rev. Lett.",
     volume    = " 68",
     year      = " 1992",
     pages     = " 75",
}

@Article{ RY02,
     author    = " S. N. Resnik and A. L. Yarin",
     title     = " Strong squeezing flow between parallel plates leads
     to rolling motion at the contact line",
     journal   = " Int. J. Multiphase Flow",
     volume    = " 28",
     year      = " 2002",
     pages     = " 911-924",
}

@Article{ RJ87,
     author    = " M. O. Robbins and J.-F. Joanny",
     title     = " Contact angle hysteresis on
random surfaces",
     journal   = " Europhys. Lett.",
     volume    = " 3",
     year      = " 1987",
     pages     = " 729-735",
}

@Article{ Rolley98,
     author    = " E. Rolley and C. Guthmann and R. Gombrowicz and V. Repain",
     title     = " The roughness of the contact line on a
                        disordered substrate,",
     journal   = " Phys. Rev. Lett.",
     volume    = " 80",
     year      = " 1998",
     pages     = " 2865-2868",
}

@Article{ Rolley98b,
     author    = " E. Rolley and A. Prevost and C. Guthmann",
     title     = " Depinning of a superfluid He4-Cs contact line",
     journal   = " J. Low Temp. Phys.",
     volume    = " 113",
     year      = " 1998",
     pages     = " 787-798",
}

@Article{ Rossnature,
     author    = " D. Ross and D. Bonn and J. Meunier",
     title     = " Observation of short-range critical wetting",
     journal   = " Nature",
     volume    = " 400",
     year      = " 1999",
     pages     = " 737",
}
@Article{ Rossetal01b,
     author    = " D. Ross and D. Bonn and A. I. Posazhennikova and
      J. O. Indekeu and J. Meunier",
     title     = " Crossover from first-order to critical wetting:
              Short-range tricritical wetting",
     journal   = " Phys. Rev. Lett.",
     volume    = " 87",
     year      = " 2001",
     pages     = " 176103",
}

@Article{ Ross96,
     author    = " D. Ross and J. E. Rutledge and P. Taborek",
     title     = " Triple point dewetting transitions of helium
                  mixtures on cesium",
     journal   = " Phys. Rev. Lett.",
     volume    = " 76",
     year      = " 1996",
     pages     = " 2350",
}
@Article{ Ross97,
     author    = " D. Ross and J. A. Phillips and J. E. Rutledge and
           P. Taborek",
     title     = " Adsorption of He-3 on cesium",
     journal   = " J. Low Temp. Phys.",
     volume    = " 106",
     year      = " 1997",
     pages     = " 81-92",
}
@Article{ Ross98,
     author    = " D. Ross and P. Taborek and J. E. Rutledge",
     title     = " Contact angle of superfluid helium droplets on a
                     cesium surface",
     journal   = " J. Low Temp. Phys.",
     volume    = " 111",
     year      = " 1998",
     pages     = " 1-10",
}

@Article{ Rossetal01a,
     author    = " D. Ross and D. Bonn and J. Meunier",
     title     = " Wetting of methanol on the n-alkanes:
          Observation of short-range critical wetting",
     journal   = " J. Chem. Phys.",
     volume    = " 114",
     year      = " 2001",
     pages     = " 2784-2792",
}
@Article{ Rosso01,
     author    = " A. Rosso and W. Krauth",
     title     = " Origin of the roughness exponent in
        elastic strings at the depinning threshold",
     journal   = " Phys. Rev. Lett.",
     volume    = " 87",
     year      = " 2001",
     pages     = " 187002",
}

@Article{ Rosso02,
     author    = " A. Rosso and W. Krauth",
     title     = " Roughness at the depinning threshold for a
             long-range elastic string",
     journal   = " Phys. Rev. E",
     volume    = " 65",
     year      = " 2002",
     pages     = " 025101(R)",
}

@Article{ Rosso03,
     author    = " A. Rosso and W. Krauth and P. {Le Doussal}
           and J. Vannimenus and K. J. Wiese",
     title     = " Universal interface width distributions at the
          depinning threshold",
     journal   = " Phys. Rev. E",
     volume    = " 68",
     year      = " 2003",
     pages     = " 036128",
}

@Book{ Rowlinson,
     author    = " J. S. Rowlinson and B. Widom",
     title     = " Molecular Theory of Capillarity",
     publisher = " Oxford: Clarendon",
     year      = " 1982",
}

@Book{ pismen_book,
     author    = " L. M. Pismen",
     title     = " Vortices in nonlinear fields: From Liquid
   Crystals to Superfluids, from Non-equilibrium Patterns to Cosmic Strings",
     publisher = " Oxford: Clarendon",
     year      = " 1999",
}

@Book{ Rowlinson-cohesion,
     author    = " J. S. Rowlinson",
     title     = " Cohesion",
     publisher = {Cambridge University Press, Cambridge},
     year      = " 2002",
}

@Book{ Barabasi,
     author    = " A.-L. Barabasi and H. E. Stanley",
     title     = " Fractal Concepts in Surface Growth",
     publisher = " Cambridge University Press, Cambridge",
     year      = " 1995",
}

@Article{ RJ74,
     author    = " E. Ruckenstein and R. K. Jain",
     title     = " Spontaneous rupture of thin liquid films",
     journal   = " J. Chem. Soc. Faraday Trans. 2",
     volume    = " 70",
     year      = " 1974",
     pages     = " 132",
}

@Article{ RCO99,
     author    = " M. J. de Ruijter and J. {De Coninck} and G. Osanin",
     title     = " Droplet spreading: partial wetting regime revisited",
     journal   = " Langmuir",
     volume    = " 15",
     year      = " 1999",
     pages     = " 2209-2216",
}
@Article{ Borgs,
     author    = " C. Borgs and J. {De Coninck} and R. Kotecky
                    and M. Zinque",
     title     = " Does the roughness of the substrate enhance wetting?",
     journal   = " Phys. Rev. Lett.",
     volume    = " 74",
     year      = " 1995",
     pages     = " 2292",
}

@Article{ Mistura94,
     author    = " G. Mistura and H. C. Lee and M. H. W. Chan",
     title     = " Hydrogen adsorption on alkali-metal surfaces -
               wetting, prewetting, and triple-point wetting",
     journal   = " J. Low Temp. Phys.",
     volume    = " 96",
     year      = " 1994",
     pages     = " 221-244",
}

@Article{ RQ98a,
     author    = " A. {de Ryck} and D. Qu\'{e}r\'{e}",
     title     = " Gravity and Inertia Effects in Plate Coating",
     journal   = " J. Colloid Interf. Sci.",
     volume    = " 203",
     year      = " 1998",
     pages     = " 278-285",
}

@Article{ RQ98b,
     author    = " A. {de Ryck} and D. Qu\'{e}r\'{e}",
     title     = " Fluid coating from a polymer solution",
     journal   = " Langmuir",
     volume    = " 14",
     year      = " 1998",
     pages     = " 1911",
}

@Article{ RBC99,
     author    = " M. J. Ruijter and T. D. Blake and J. {De Coninck}",
     title     = " Dynamic wetting studied by  molecular modeling simulations of droplet spreading",
     journal   = " Langmuir",
     volume    = " 15",
     year      = " 1999",
     pages     = " 7836-7847",
}

@Article{ Rutledge,
     author    = " J. E. Rutledge and P. Taborek",
     title     = " Prewetting phase-diagram of HE-4 on cesium",
     journal   = " Phys. Rev. Lett.",
     volume    = " 69",
     year      = " 1992",
     pages     = " 937",
}

@Article{ RSS89,
     author    = " W. B. Russel and D. A. Saville and W. R. Schowalter",
     title     = " Colloidal Suspensions",
     publisher = {Cambridge University Press, Cambridge},
     year      = " 1989",
     pages     = " 148, table 5.3",
}

@Article{ G06,
     author    = " J. D. Goddard",
     title     = " A dissipative anisotropic fluid model for
           non-colloidal particle dispersions",
     journal   = " J. Fluid Mech.",
     volume    = " 568",
     pages     = " 1",
     year      = " 2006",
}

@Article{ SRG02,
     author    = " F. Saulnier and E. Rapha{\"e}l and P.-G. de Gennes",
     title     = " Dewetting of thin-film polymers",
     journal   = " Phys. Rev. E",
     volume    = " 66",
     year      = " 2002",
     pages     = " 061607",
}

@Article{ SRG02b,
     author    = " F. Saulnier and E. Rapha{\"e}l and P.-G. de Gennes",
     title     = " Dewetting of thin polymer films near the glass
                         transition",
     journal   = " Phys. Rev. Lett.",
     volume    = " 88",
     year      = " 2002",
     pages     = " 196101",
}

@Article{ SchafferWong,
     author    = " E. Sch{\"a}ffer and P. Z. Wong",
     title     = " Contact line dynamics near the pinning
        threshold: A capillary rise and fall experiment",
     journal   = " Phys. Rev. E",
     volume    = " 61",
     year      = " 2000",
     pages     = " 5257-5277",
}
@Article{ Shibuichi,
     author    = " S. Shibuichi and T. Onda and N. Satoh and K. Tsujii",
     title     = " Super Water-Repellent Sufaces Resulting from
               Fractal Structure",
     journal   = " J. Phys. Chem.",
     volume    = " 100",
     year      = " 1996",
     pages     = " 19512-19517",
}
@Article{ SchwarzF,
     author    = " J. M. Schwarz and D. S. Fisher",
     title     = " Depinning with Dynamic Stress Overshoots:
            Mean Field Theory",
     journal   = " Phys. Rev. Lett.",
     volume    = " 87",
     year      = " 2001",
     pages     = " 096107",
}

@Incollection{ Schick,
     author    = " M. Schick",
     title     = " Introduction to wetting phenomena",
     booktitle = " Liquids at Interfaces, Les Houches Session XLVIII",
     editor    = " J. Charvolin and J.-F. Joanny and J. Zinn-Justin",
     publisher = " Amsterdam: Elsevier",
     year      = " 1990",
     pages     = " 415-497",
}

@Article{ S89,
     author    = " L. W. Schwartz",
     title     = " Viscous flows down an inclined plane:
                 Instability and finger formation",
     journal   = " Phys. Fluids A",
     volume    = " 1",
     year      = " 1989",
     pages     = " 443",
}

@Article{ SchwartzTajeda,
     author    = " A. Schwartz and S. B. Tejeda",
     title     = " ????",
     journal   = " J. Colloid Interface Sci.",
     volume    = " 38",
     year      = " 1972",
     pages     = " 359",
}

@Article{ SP91,
     author    = " R. V. Sedev and J. G. Petrov",
     title     = " The critical condition for transition
            from steady wetting to film entrainment",
     journal   = " Colloids and Surfaces",
     volume    = " 53",
     year      = " 1991",
     pages     = " 147",
}

@Article{ SP92,
     author    = " R. V. Sedev and J. G. Petrov",
     title     = " Influence of geometry on steady dewetting kinetics",
     journal   = " Colloids and Surfaces",
     volume    = " 62",
     year      = " 1992",
     pages     = " 141-151",
}

@Article{ SHJ01a,
     author    = " R. Seemann and S. Herminghaus and K. Jacobs",
     title     = " Gaining control of pattern formation of
                    dewetting liquid films",
     journal   = " J. Phys. Condens. Mat.",
     volume    = " 13",
     year      = " 2001",
     pages     = " 4925",
}

@Article{ SHJ01b,
     author    = " R. Seemann and S. Herminghaus and K. Jacobs",
     title     = " Dewetting patterns and molecular forces: A reconciliation",
     journal   = " Phys. Rev. Lett.",
     volume    = " 86",
     year      = " 2001",
     pages     = " 5534-5537",
}

@Article{ SB92,
     author    = " J. E. Seebergh and J. C. Berg",
     title     = " A comparison of force and optical techniques
               for the measurement of dynamic contact angles",
     journal   = " Chem. Engin. Sci.",
     volume    = " 47",
     year      = " 1992",
     pages     = " 4468-4470",
}

@Article{ S96,
     author    = " P. Seppecher",
     title     = " Moving contact lines in the Cahn-Hilliard theory",
     journal   = " Int. J. Engng. Sci.",
     volume    = " 34",
     year      = " 1996",
     pages     = " 977-992",
}

@Article{ Shahidzadeh,
     author    = " N. Shahidzadeh and D. Bonn and K. Ragil
         and D. Broseta  and J. Meunier",
     title     = " Sequence of two wetting transitions induced by
tuning the Hamaker constant",
     journal   = " Phys. Rev. Lett.",
     volume    = " 80",
     year      = " 1998",
     pages     = " 3992",
}
@Article{ Baumberger,
     author    = " T. Baumberger and P. Berthoud and C. Caroli",
     title     = " Physical analysis of the state- and rate-dependent
     friction law. II. Dynamic friction",
     journal   = " Phys. Rev. B",
     volume    = " 60",
     year      = " 1999",
     pages     = " 3928",
}
@Article{ Hamaker,
     author    = " H. C. Hamaker",
     title     = " The London-van der Waals attraction between
                    spherical particles",
     journal   = " Physica",
     volume    = " 4",
     year      = " 1937",
     pages     = " 1058-1072",
}
@Article{ noushineNature,
     author    = " J. B. Brzoska and N. Shahidzadeh and F. Rondelez",
     title     = " Evidence of a transition-temperature for the optimum
                  deposition of grafted monolayer coatings",
     journal   = " Nature",
     volume    = " 360",
     year      = " 1992",
     pages     = " 719-721",
}
@Article{ noushineTPM,
     author    = " N. Shahidzadeh and E. Bertrand and J.-P. Dauplait and
          J.-C. Borgotti and D. Bonn",
     title     = "Effect of wetting on gravity drainage in porous media",
     journal   = " Transp. Porous Media",
     volume    = " 52",
     year      = " 2003",
     pages     = " 213-227",
}

@Article{ SR98,
     author    = " C. Shen and D. W. Ruth",
     title     = " Experimental and numerical investigations of the
             interface profile close to a moving contact line",
     journal   = " Phys. Fluids",
     volume    = " 10",
     year      = " 1998",
     pages     = " 789-799",
}

@Article{ Shenoy,
     author    = " V. B. Shenoy and W. F. Saam",
     title     = " Continuous wetting transitions in XE
             adsorbed on NAF and on plated CS and RB substrates",
     journal   = " Phys. Rev. Lett.",
     volume    = " 75",
     year      = " 1995",
     pages     = " 4086",
}

@Article{ Yao,
     author    = " M. Yao and F. Hensel",
     title     = " Wetting of mercury on sapphire",
     journal   = " J. Phys.: Condens. Matter",
     volume    = " 8",
     year      = " 1996",
     pages     = " 9547-9551",
}

@Incollection{ Diehl,
     author    = " H. W. Diehl",
     title     = " ????",
     booktitle = " Phase Transitions and Critical Phenomena",
     year      = " 1986",
     volume    = " 10",
     editor    = " C Domb and JL Lebowitz ",
     publisher = " London: Academic",
     pages     = " 75-267",
}
@Incollection{ LipowskyR,
     author    = " R. Lipowsky",
     title     = " Scaling properties of interfaces and membranes",
     booktitle = " Random fluctuations and pattern growth",
     year      = " 1988",
     volume    = " NATO ASI Series E, Vol. 157",
     editor    = " H. E. Stanley and N. Ostrowsky",
     publisher = " Kluwer Acad. Publ., Dordrecht",
     pages     = " 227-245",
}
@Article{ Checco,
     author    = " A. Checco and P. Guenoun and J. Daillant",
     title     = " Nonlinear dependence
of the contact angle of nanodroplets on contact line curvature",
     journal   = " Phys. Rev. Lett.",
     volume    = " 91",
     year      = " 2003",
     pages     = " 186101",
}
@Article{ SchwartzGaroff,
     author    = " L. W. Schwartz and S. Garoff",
     title     = " Contact angle hysteresis on heterogeneous surfaces",
     journal   = " Langmuir",
     volume    = " 1",
     year      = " 1985",
     pages     = " 219-230",
}
@Article{ Helfrich,
     author    = " W. Helfrich",
     title     = " Elastic properties of lipid bilayers:
                 theory and possible experiments",
     journal   = " Z. Naturforsch. C",
     volume    = " 28",
     year      = " 1973",
     pages     = " 693-703",
}
@Article{ Cassie,
     author    = " A. B. D. Cassie",
     title     = " Contact angles",
     journal   = " Discuss. Faraday Soc.",
     volume    = " 57",
     year      = " 1952",
     pages     = " 5041",
}
@Article{ W36,
     author    = " R. N. Wenzel",
     title     = " Resistance of Solid Surfaces to Wetting by Water",
     journal   = " Ind. Engin. Chem.",
     volume    = " 28",
     year      = " 1936",
     pages     = " 988-994",
}
@Article{ GM06a,
     author    = " L. Gao and T. J. McCarthy",
     title     = " Contact angle hysteresis explained",
     journal   = " Langmuir",
     volume    = " 22",
     year      = " 2006",
     pages     = " 6234",
}
@Article{ GM06b,
     author    = " L. Gao and T. J. McCarthy",
     title     = " The {"Lotus Effect"} Explained: Two Reasons Why Two Length
           Scales of Topography Are Important",
     journal   = " Langmuir",
     volume    = " 22",
     year      = " 2006",
     pages     = " 2966",
}
@Article{ sigl/fenzl,
     author    = " L. Sigl and W. Fenzl",
     title     = " Order parameter exponent $\beta_1$ of a binary liquid
                     mixture at a boundary",
     journal   = " Phys. Rev. Lett.",
     volume    = " 57",
     year      = " 1986",
     pages     = " 2191",
}
@Article{ Trejo,
     author    = " L. M. Trejo and J. Garcia and C. Varea and A. Robledo",
     title     = " Possibility of continuous wetting transition at the
             liquid-vapor interface of the binary liquid
               mixture cyclohexane + acetonitrile",
     journal   = " Europhys. Lett.",
     volume    = " 7",
     year      = " 1988",
     pages     = " 537-542",
}

@Article{ saamshenoy,
     author    = " W. F. Saam and V. B. Shenoy",
     title     = " Continuous wetting transitions in adsorbed Xe films",
     journal   = " J. Low. Temp. Phys.",
     volume    = " 101",
     year      = " 1995",
     pages     = " 225-230",
}

@Article{ Shikh94,
     author    = " Y. D. Shikhmurzaev",
     title     = " Mathematical modeling of wetting hydrodynamics",
     journal   = " Fluid Dyn. Res.",
     volume    = " 13",
     year      = " 1994",
     pages     = " 45-64",
}

@Article{ Shikh97,
     author    = " Y. D. Shikhmurzaev",
     title     = " Moving contact lines in liquid/liquid/solid systems",
     journal   = " J. Fluid Mech.",
     volume    = " 334",
     year      = " 1997",
     pages     = " 211-249",
}

@Article{ Shikh05,
     author    = " Y. D. Shikhmurzaev",
     title     = " ",
     journal   = " IMA J. Appl. Math.",
     volume    = " 70",
     year      = " 2005",
     pages     = " 880",
}

@Article{ Silber,
     author    = " P. Silberzan and L. L\'eger and
       D. Ausserre and J. J. Benattar",
     title     = " Silanation of silica surfaces. A new method of
                constructing pure or mixed monolayers",
     journal   = " Langmuir",
     volume    = " 7",
     year      = " 1991",
     pages     = " 1647"
}

@Article{ Swain,
     author    = " P. Swain and R. Lipowsky",
     title     = " Contact angles on heterogeneous surfaces:
          a new look at Cassie's and Wenzel's laws",
     journal   = " Langmuir",
     volume    = " 14",
     year      = " 1998",
     pages     = " 6772-6780",
}

@Article{ Vandembroucq,
     author    = " D. Vandembroucq and R. Skoe and S. Roux",
     title     = " Univeral depinning
          force fluctuations of an elastic line: Application to finite
                       temperature behavior",
     journal   = " Phys. Rev. E",
     volume    = " 70",
     year      = " 2004",
     pages     = " 051101",
}
@Article{ Wenzel,
     author    = " R. N. Wenzel",
     title     = " Resistance of solid surfaces to wetting by water",
     journal   = " Ind. Eng. Chem.",
     volume    = " 28",
     year      = " 1936",
     pages     = " 988-994",
}

@Article{ SD85,
     author    = " N. Silve and E. B. {Dussan V.}",
     title     = " On the rewetting of an inclinsolid surface by a liquid",
     journal   = " Phys. Fluids",
     volume    = " 28",
     year      = " 1985",
     pages     = " 5",
}

@Article{ SK00,
     author    = " P. G. Simpkins and V. J. Kuck",
     title     = " Air entrapment in coatings by way of a
                tip-streaming meniscus",
     journal   = " Nature",
     volume    = " 403",
     year      = " 2000",
     pages     = " 641-643",
}

@Article{ SK03,
     author    = " P. G. Simpkins and V. J. Kuck",
     title     = " On air entrainment in coatings",
     journal   = " J. Col. Interf. Sci.",
     volume    = " 263",
     year      = " 2003",
     pages     = " 562",
}

@Article{ SRLL05,
     author    = " J. H. Snoeijer and E. Rio and N. {Le Grand} and L. Limat",
     title     = " Self-similar flow and contact
           line geometry at the rear of cornered drops",
     journal   = " Phys. Fluids",
     volume    = " 17",
     year      = " 2005",
     pages     = " 072101",
}

@Article{ RDAL05,
     author    = " E. Rio and A. Daerr and B. Andreotti and L. Limat",
     title     = " Boundary Conditions in the Vicinity of a Dynamic
                 Contact Line: Experimental Investigation of Viscous
                 Drops Sliding Down an Inclined Plane ",
     journal   = " Phys. Rev. Lett.",
     volume    = " 94",
     year      = " 2005",
     pages     = " 024503",
}

@Article{ SDAF06,
     author    = " J. H. Snoeijer and G. Delon and M. Fermigier and
              B. Andreotti",
     title     = " Avoided critical behavior in dynamically forced wetting",
     journal   = " Phys. Rev. Lett.",
    volume    = " 96",
     year      = " 2006",
     pages     = " 174504",
}

@phdThesis{ Dthese,
     author    = " G. Delon",
     title     = " Thesis ",
     school    = "Universit{\'e} Paris VI",
     year      = " 2007",
}

@Article{ SZAFE08,
     author    = " J. H. Snoeijer and J. Ziegler and B. Andreotti and
                    M. Fermigier and J. Eggers ",
     title     = "  Thick films coating a plate withdrawn from a bath",
     journal   = " Phys. Rev. Lett.",
     year      = " 2008",
     volume    = " 100",
     pages     = " 244502"
  }

@Article{ SBE09,
     author    = " J. H. Snoeijer, P. Brunet, J. Eggers",
     title     = " Maximum size of drops levitated by an air cushion",
     journal   = " Phys. Rev. E",
     year      = " 2009",
     volume    = " 79",
     pages     = " 036307",
  }

@Article{ ZSE09,
     author    = " J. Ziegler and J. H. Snoeijer and J. Eggers ",
     title     = " Film transitions of receding contact lines",
     journal   = " Eur. Phys. J. Special Topics",
     volume    = " 166",
     pages     = " 177",
     year      = " 2009",
  }


@Article{ BED09,
     author    = " P. Brunet and J. Eggers and R. D. Deegan",
     title     = " Motion of a drop driven by substrate vibrations",
     journal   = " Eur. Phys. J. Special Topics",
     volume    = " 166",
     pages     = " 11",
     year      = " 2009",
  }

@Article{ SADF07,
     author    = " J. H. Snoeijer and B. Andreotti and G. Delon and
                    M. Fermigier",
     title     = " Relaxation of a dewetting contact line Part 1:
        A full-scale hydrodynamic calculation",
     journal   = " J. Fluid Mech.",
     volume    = " 579",
     year      = " 2007",
     pages     = " 63",

}

@Article{ DFSA07,
     author    = " G. Delon and M. Fermigier and J. H. Snoeijer and
                 B. Andreotti",
     title     = " Relaxation of a dewetting contact line Part 2:
                   Experiments",
     journal   = " J. Fluid Mech.",
     volume    = " 604",
     year      = " 2008",
     pages     = " 55",
}

@Article{ SB00,
     author    = " S. Somalinga and A. Bose",
     title     = " Numerical investigations of boundary
          conditions for moving contact line problems",
     journal   = " Phys. Fluids",
     volume    = " 12",
     year      = " 2000",
     pages     = " 499",
}

@Article{ SH96,
     author    = " M. A. Spaid and G. M. Homsy",
     title     = " Stability of Newtonian and viscoelastic
                    dynamic contact lines",
     journal   = " Phys. Fluids",
     volume    = " 8",
     year      = " 1996",
     pages     = " 460",
}

@Article{ SLW02,
     author    = " H. A. Stone and L. Limat and S. K. Wilson and
       J. M. Flesselles and T. Podgorski",
     title     = " Corner singularity of a contact line
     moving on a solid substrate",
     journal   = " C. R. Physique",
     volume    = " 3",
     year      = " 2002",
     pages     = " 103-110",
}

@Article{ LDL05,
     author    = " N. {Le Grand} and A. Daerr and L. Limat",
     title     = " Shape and motion of drops sliding down
                      an inclined plane",
     journal   = " J. Fluid Mech.",
     volume    = " 541",
     year      = " 2005",
     pages     = " 293-315",
}

@Article{ SWRJT05,
     author    = " S. Sikalo and H. D. Wilhelm and I. V. Roisman and
       S. Jakirlic and C. Tropea",
     title     = " Dynamic contact angle of spreading droplets:
           Experiments and simulations",
     journal   = " Phys. Fluids",
     volume    = " 17",
     year      = " 2005",
     pages     = " 062103",
}

@Article{ RoRioTr02,
     author    = " I. V. Roisman and R. Rioboo and C. Tropea",
     title     = " Normal impact of a liquid drop on a dry surface:
        model for spreading and receding",
     journal   = " Proc. R. Soc. Lond. A",
     volume    = " 458",
     year      = " 2002",
     pages     = " 1411--1430"
}

@Article{ Korob08,
     author    = " A. Korobkin and A. Ellis and F. Smith",
     title     = " Trapping of air in impact between a body and shallow water",
     journal   = " J. Fluid Mech.",
     volume    = " 611",
     year      = " 2008",
     pages     = " 365-394"
}

@Article{ Mandre09,
     author    = " S. Mandre and M. Mani and M. P. Brenner",
     title     = " Precursors to Splashing of Liquid Droplets on
              a Solid Surface",
     journal   = " Phys. Rev. Lett.",
     volume    = " 102",
     year      = " 2009",
     pages     = " 134502"
}

@Article{ BenPouli93,
     author    = " T. Bennett and D. Poulikakos",
     title     = " Splat-quench solidification: estimating the maximum
         spreading of a droplet impacting a solid surface",
     journal   = " J. Mater. Sci.",
     volume    = " 28",
     year      = " 1993",
     pages     = " 963--970"
}

@Article{ PCM02,
     author    = " M. Pasandideh-Fard and S. Chandra and J. Mostaghimi",
     title     = " A three-dimensional model of droplet impact and
             solidification",
     journal   = " Int. J. Heat Mass Trans.",
     volume    = " 45",
     year      = " 2002",
     pages     = " 2229-2242"
}

@Article{ BJB05,
     author    = " D. Bartolo and C. Josserand and D. Bonn",
     title     = " Retraction dynamics of aqueous drops upon impact
       on non-wetting surfaces",
     journal   = " J. Fluid Mech.",
     volume    = " 545",
     year      = " 2005",
     pages     = " 329--338"
}

@Article{ Rois09a,
     author    = "I. V. Roisman and E. Berberovi{\'c} and C. Tropea",
     title     = " Inertia dominated drop collisions.
              I. On the universal flow in the lamella",
     journal   = " Phys. Fluids",
     volume    = " 21",
     year      = " 2009",
     pages     = " 052103",
}

@Article{ Rois09b,
     author    = "I. V. Roisman",
     title     = " Inertia dominated drop collisions. II. An analytical
            solution of the Navier-Stokes equations for a spreading
                viscous film",
     journal   = " Phys. Fluids",
     volume    = " 21",
     year      = " 2009",
     pages     = " 052104",
}

@Incollection{ LBS05,
     author    = " E. Lauga and M. P. Brenner and H. A. Stone",
     title     = " Microfluidics: the no-slip boundary condition",
     booktitle = " Springer Handbook of Experimental Fluid Mechnaics",
     editor    = " C. Tropea and J. F. Foss and A. Yarin",
     year      = " 2008",
     publisher = " Springer",
     pages     = " 1219-1240",
}

@Article{ SFSR90a,
     author    = " G. Str{\"o}m and M. Fredriksson and
              P. Stenius and B. Radoev",
     title     = " Kinetics of Steady-State wetting",
     journal   = " J. Colloid Interf. Sci.",
     volume    = " 134",
     year      = " 1990",
     pages     = " 107-116",
}

@Article{ SFSR90b,
     author    = " G. Str{\"o}m and M. Fredriksson and
                   P. Stenius and B. Radoev",
     title     = " Kinetics of Oil displacement from a solid surface by
                 an aqueous solution",
     journal   = " J. Colloid Interf. Sci.",
     volume    = " 134",
     year      = " 1990",
     pages     = " 117-121",
}

@Incollection{ Sullivan,
     author    = " D. E. Sullivan and M. M. {Telo da Gama}",
     title     = "Wetting transition and multilayer adsorption at
                    fluid interfaces",
     booktitle = " Fluid  interfacial Phenomena",
     publisher = " New York: Wiley",
     editor    = " CA Croxton",
     year      = " 1986",
     pages     = " 45-134 ",
}

@Book{ tabeling,
     author    = " P. Tabeling",
     title     = " Microfluidics",
     publisher = " EDP Sciences: Paris",
     year      = " 2004",
}

@Article{ SMHY05,
     author    = " Y. Sumino and N. Magome and T. Hamada and K. Yoshikawa",
     title     = " Self-running droplet: emergence of regular
            motion from nonequilibrium noise",
     journal   = " Phys. Rev. Lett.",
     volume    = " 94",
     year      = " 2005",
     pages     = " 068301",
}

@Article{ SBB03,
     author    = " J. Sur and A. L. Bertozzi and R. P. Behringer",
     title     = " Reverse undercompressive shock
                  structures in driven thin film flow",
     journal   = " Phys. Rev. Lett.",
     volume    = " 90",
     year      = " 2003",
     pages     = " 126105",
}


@Article{ Taborek92,
     author    = " P. Taborek and J. E. Rutledge",
     title     = " Novel wetting behavior of He-4 on Cesium",
     journal   = " Phys. Rev. Lett.",
     volume    = " 68",
     year      = " 1992",
     pages     = " 2184",
}

@Article{ Taborek93,
     author    = " P. Taborek and J. E. Rutledge",
     title     = " Tuning the wetting transition -
       prewetting and superfluidity of He-4 on a thin Cesium substrate",
     journal   = " Phys. Rev. Lett.",
     volume    = " 71",
     year      = " 1993",
     pages     = " 263",
}

@Article{ T79,
     author    = " L. H. Tanner",
     title     = " The spreading of silicone oil drops on horizontal surfaces",
     journal   = " J. Phys. D: Appl. Phys.",
     volume    = " 12",
     year      = " 1979",
     pages     = " 1473-1478",
}

@Article{ T34,
     author    = " G. I. Taylor",
     title     = " The formation of emulsions in definable fields of flow",
     journal   = " Proc. Roy. Soc. London A",
     volume    = " 146",
     year      = " 1934",
     pages     = " 501",
}

@Article{ TDS88,
     author    = " G. F. Teletzke and H. T. Davis and L. E. Scriven",
     title     = " Wetting hydrodynamics",
     journal   = " Revue Phys. Appl.",
     volume    = " 23",
     year      = " 1988",
     pages     = " 989-1007",
}

@Article{ BBD88,
     author    = " J. P. Burelbach and S. G. Bankoff and S. H. Davis",
     title     = " Nonlinear stability of evaporating/condensing
                    liquid films",
     journal   = " J. Fluid Mech.",
     volume    = " 195",
     year      = " 1988",
     pages     = " 463",
}

@Article{ Carey,
     author    = " B. S. Carey and L. E. Scriven and H. T. Davis",
     title     = " Semi-empirical theory of surface tensions of pure normal
                alkanes and alcohols",
     journal   = " AIChE Journal",
     volume    = " 24",
     year      = " 1978",
     pages     = " 1076-1080",
}

@Article{ T03,
     author    = " U. Thiele",
     title     = " Open questions and promising new fields in dewetting",
     journal   = " Eur. Phys. J. E",
     volume    = " 12",
     year      = " 2003",
     pages     = " 409",
}

@Article{ TK03,
     author    = " U. Thiele and E. Knobloch",
     title     = " Front and back instability of a liquid film on a
slightly inclined plane",
     journal   = " Phys. Fluids",
     volume    = " 15",
     year      = " 2003",
     pages     = " 892-907",
}

@Article{ TR89,
     author    = " P. A. Thompson and M. O. Robbins",
     title     = " Simulations of contact-line motion:
        slip and the dynamic contact angle",
     journal   = " Phys. Rev. Lett.",
     volume    = " 63",
     year      = " 1989",
     pages     = " 766-769",
}

@Article{ TT97,
     author    = " P. A. Thompson and S. M. Troian",
     title     = " A general boundary condition for liquid flow
                        at solid surfaces",
     journal   = " Nature",
     volume    = " 389",
     year      = " 1997",
     pages     = " 360-362",
}

@Article{ TC94,
     author    = " F. Tiber and A.-M. Cazabat",
     title     = " Spreading of thin films of ordered nonionic
       surfactants. Origin of the stepped shape of the spreading precursor",
     journal   = " Langmuir",
     volume    = " 10",
     year      = " 1994",
     pages     = " 2301-2306",
}

@Article{ TTRD93,
     author    = " L. N. Trevethen and A. E. Trefethen and
                S. C. Reddy and T. A. Driscoll",
     title     = " Hydrodynamic stability without eigenvalues",
     journal   = " Science",
     volume    = " 261",
     year      = " 1993",
     pages     = " 578",
}

@Article{ THSJ89,
     author    = " S. M. Troian and E. Herbolzheimer and
                          S. A. Safran and J.-F. Joanny",
     title     = " Fingering instability of driven spreading films",
     journal   = " Europhys. Lett.",
     volume    = " 10",
     year      = " 1989",
     pages     = " 25-30",
}

@Article{ BG88,
     author    = " M. S. Borgas and J. B. Grotberg",
     title     = " Monolayer flow on a thin film",
     journal   = " J. Fluid Mech.",
     volume    = " 193",
     year      = " 1988",
     pages     = " 151-170",
}

@Article{ JG92,
     author    = " O. E. Jensen and J. B. Grotberg",
     title     = " Insoluble surfactant spreading on a thin viscous film:
                    shock evolution and film rupture",
     journal   = " J. Fluid Mech.",
     volume    = " 240",
     year      = " 1992",
     pages     = " 259-288",
}

@Article{ MT99,
     author    = " O. K. Matar and S. M. Troian",
     title     = " The development of transient fingering patterns
                    during the spreading of surfactant coated films",
     journal   = " Phys. Fluids",
     volume    = " 11",
     year      = " 1999",
     pages     = " 3232-3246",
}

@Article{ WCM04,
     author    = " M. R. E. Warner and R. V. Craster and O. K. Matar",
     title     = " Fingering phenomena associated with insoluble
                     surfactant spreading on thin liquid films",
     journal   = " J. Fluid Mech.",
     volume    = " 510",
     year      = " 2004",
     pages     = " 169-200",
}

@Article{ CSHC02,
     author    = " M. Cachile and M. Schneemilch and
               A. Hamraoui and A.-M. Cazabat",
     title     = " Films driven by surface tension gradients",
     journal   = " J. Colloid Interf. Sci.",
     volume    = " 96",
     year      = " 2002",
     pages     = " 59-74",
}

@Article{ TWS89,
     author    = " S. M. Troian and X. L. Wu and S. A. Safran",
     title     = " Fingering instability in thin wetting films",
     journal   = " Phys. Rev. Lett.",
     volume    = " 62",
     year      = " 1989",
     pages     = " 1496",
}



@Article{ ueno,
     author    = " T. Ueno and S. Balibar and T. Mizusaki
        and F. Caupin and E. Rolley ",
     title     = " Critical Casimir effect and wetting by helium mixtures",
     journal   = " Phys. Rev. Lett.",
     volume    = " 90",
     year      = " 2003",
     pages     = " 116102",
}

@Article{ V76,
     author    = " O. V. Voinov",
     title     = " Hydrodynamics of wetting [English translation]",
     journal   = " Fluid Dynamics",
     volume    = " 11",
     year      = " 1976",
     pages     = " 714-721",
}

@Article{ V77,
     author    = " O. V. Voinov",
     title     = " Inclination angles of the boundary in
              moving liquid layers [English translation]",
     journal   = " J. Appl. Mech. Tech. Phys.",
     volume    = " 18",
     year      = " 1977",
     pages     = " 216-222",
}

@Article{ V78,
     author    = " O. V. Voinov",
     title     = " Asymptote to the free surface of a viscous liquid
creeping on a surface and the velocity dependence of the angle
                  of contact [English translation]",
     journal   = " Sov. Phys. Dokl.",
     volume    = " 23",
     year      = " 1978",
     pages     = " 891-893",
}

@Article{ V94,
     author    = " O. V. Voinov",
     title     = " Closure of the hydrodynamic theory of wetting in a
small-scale region",
     journal   = " J. Appl. Mech. Techn. Phys.",
     volume    = " 35",
     year      = " 1994",
     pages     = " 1-12",
}

@Article{ V95,
     author    = " O. V. Voinov",
     title     = " Motion of line of contact of three phases
on a solid: thermodynmics and asymptotic theory",
     journal   = " Int. J. Multiphase Flow",
     volume    = " 21",
     year      = " 1995",
     pages     = " 801-816",
}

@Article{ V00a,
     author    = " O. V. Voinov",
     title     = " Wetting: Inverse Dynamic Problem and
              Equations for Microscopic Parameters",
     journal   = " J. Colloid Interf. Sci.",
     volume    = " 226",
     year      = " 2000",
     pages     = " 5-15",
}

@Article{ V00b,
     author    = " O. V. Voinov",
     title     = " Wetting line dynamics in the process of drop spreading",
     journal   = " J. Colloid Interf. Sci.",
     volume    = " 226",
     year      = " 2000",
     pages     = " 22-28",
}

@Incollection{ R02,
     author    = " E. Ram\'{e}",
     title     = " Moving contact line problem: state of the contact
                    angle boundary condition",
     booktitle = " Encyclopedia of Surface and Colloid Science",
     publisher = " New York, Marcel Dekker",
     year      = " 2002",
     pages     = " 3602-3618",
}
@Incollection{ Vreview,
     author    = " O. V. Voinov",
     title     = " Dynamics of wetting of a solid by a liquid:
                    movement of thin liquid films",
     booktitle = " Encyclopedia of Surface and Colloid Science",
     publisher = " New York, Marcel Dekker",
     year      = " 2002",
     pages     = " 1546-1559",
}

@Article{ VVOCC98,
     author    = " M. Voue and M. P. Valignat and G. Oshanin
    and A.-M. Cazabat and J. {De Coninck}",
     title     = " Dynamics of spreading of liquid mircodroplets
             on substrates of increasing surface energies",
     journal   = " Langmuir",
     volume    = " 14",
     year      = " 1998",
     pages     = " 5951-5958",
}

@Article{ V66,
     author    = " A. Vrij",
     title     = " Possible mechanism for the spontaneous rupture of thin,
              free liquid films",
     journal   = " Discuss. Faraday Soc.",
     volume    = " 42",
     year      = " 1966",
     pages     = " 23",
}

@Article{ Vr76,
     author    = " A. Vrij",
     title     = " Polymers at interfaces and the interactions in
            colloidal dispersions",
     journal   = " Pure Appl. Chem.",
     volume    = " 48",
     year      = " 1976",
     pages     = " 471",
}

@Article{ joanny,
     author    = " J.-F. Joanny and L. Leibler and P.-G. {de Gennes}",
     title     = " Effects of polymer solutions on colloid stability",
     journal   = " J. Polym. Sci.: Polym.",
     volume    = " 17",
     year      = " 2003",
     pages     = " 1073",
}
@Article{ Lekkerkerker,
     author    = " H. N. W. Lekkerkerker and W. C. K. Poon and P. N. Pusey
        and A. Stroobants and P. B. Warren",
     title     = " PHASE-BEHAVIOR OF COLLOID PLUS POLYMER MIXTURES",
     journal   = " Europhys. Lett.",
     volume    = " 20",
     year      = " 1992",
     pages     = " 559",
}

@Article{ Aartscodef,
     author    = " D. G. A. L. Aarts and H. N. W. Lekkerkerker",
     title     = " Confocal scanning laser microscopy on fluid-fluid
                  demixing colloid-polymer mixtures",
     journal   = " J. Phys.: Condens. Matter",
     volume    = " 16",
     year      = " 2004",
     pages     = " S4231",
}

@Article{ Aartsjpcb,
     author    = " D. G. A. L. Aarts",
     title     = " The capillary length in a fluid-fluid demixed
                  colloid-polymer mixture",
     journal   = " J. Phys. Chem. B",
     volume    = " 109",
     year      = " 2005",
     pages     = " 7407",
}

@Article{ SE05,
     author    = " M. C. Stewart and R. Evans",
     title     = " Wetting and drying at a curved substrate:
                   long-ranged forces",
     journal   = " Phys. Rev. E",
     volume    = " 71",
     year      = " 2005",
     pages     = " 011602",
}

@Article{ MW09,
     author    = " N. Marheineke and R. Wegener",
     title     = " Asymptotic model for the dynamics of curved viscous
                   fibres with surface tension",
     journal   = " J. Fluid Mech.",
     volume    = " 622",
     year      = " 2009",
     pages     = " 345-369",
}

@Article{ Wessels,
     author    = " P. P. F. Wessels and M. Schmidt and H. L{\"o}wen",
     title     = " The contact angle of the colloidal liquid-gas
             interface and a hard wall",
     journal   = " J. Phys.: Condens. Matter",
     volume    = " 16",
     year      = " 2004",
     pages     = " S4169",
}

@Article{ Dijkstra,
     author    = " M. Dijkstra and R. {van Roij}",
     title     = " Entropic wetting and many-body induced layering
      in a model colloid-polymer mixture",
     journal   = " Phys. Rev. Lett.",
     volume    = " 89",
     year      = " 2002",
     pages     = " 208303",
}

@Article{ Aartskonstanz,
     author    = " D. G. A. L. Aarts and J. H. {van der Wiel} and
        H. N. W. Lekkerkerker",
     title     = " Interfacial dynamics and the static profile near a
            single wall in a model colloid-polymer mixture",
     journal   = " J. Phys.: Condens. Matter",
     volume    = " 15",
     year      = " 2003",
     pages     = " S245",
}

@Article{ wijting1,
     author    = " W. K. Wijting and N. A. M. Besseling and
                     M. A. {Cohen-Stuart}",
     title     = " Wetting in a colloidal liquid-gas system",
     journal   = " Phys. Rev. Lett.",
     volume    = " 90",
     year      = " 2003",
     pages     = " 196101",
}

@Article{ wijting2,
     author    = " W. K. Wijting and N. A. M. Besseling and
                     M. A. {Cohen-Stuart}",
     title     = " Wetting behavior in colloid-polymer mixtures at
               different substrates",
     journal   = " J. Phys. Chem. B",
     volume    = " 107",
     year      = " 2003",
     pages     = " 10565",
}

@Article{ likos,
     author    = " C. N. Likos",
     title     = " Effective interactions in soft condensed matter physics",
     journal   = " Phys. Rep.",
     volume    = " 348",
     year      = " 2001",
     pages     = " 267",
}

@Article{ Fuchs,
     author    = " M. Fuchs and K. S. J. Schweizer",
     title     = " Structure of colloid-polymer suspensions",
     journal   = " J. Phys.: Condens. Matter",
     volume    = " 14",
     year      = " 2002",
     pages     = " R239",
}

@Article{ Tuinier,
     author    = " R. Tuinier and J. Rieger and C. G. {de Kruif}",
     title     = " Depletion-induced phase separation in
        colloid-polymer mixtures",
     journal   = " Adv. Coll. Interface Sci.",
     volume    = " 103",
     year      = " 2003",
     pages     = " 1",
}

@Article{ Aartsscience,
     author    = " D. G. A. L. Aarts and M. Schmidt and
                     H. N. W. Lekkerkerker",
     title     = " Direct visual observation of thermal capillary waves",
     journal   = " Science",
     volume    = " 304",
     year      = " 2004",
     pages     = " 847",
}

@Article{ W93,
     author    = " P. C. Wayner",
     title     = " Spreading of a Liquid Film with a Finite Contact
              Angle by the Evaporation/Condensation Process",
     journal   = " Langmuir",
     volume    = " 9",
     year      = " 1993",
     pages     = " 294-299",
}

@Article{ WGH03,
     author    = " E. B. {Webb III} and G. S. Grest and D. R. Heine",
     title     = " Precursor film controlled wetting of Pb on Cu",
     journal   = " Phys. Rev. Lett.",
     volume    = " 91",
     year      = " 2003",
     pages     = " 236102",
}

@Article{ WS93,
     author    = " D. E. Weidner and L. W. Schwartz",
     title     = " Contact-line motion of shear-thinning liquids",
     journal   = " Phys. Fluids",
     volume    = " 6",
     year      = " 1994",
     pages     = " 3535-3538",
}

@Article{ XSBMRS04,
     author    = " H. Xu and D. Shirvanyants and K. Beers
      and K. Matyjaszewski and M. Rubinstein and S. S. Sheiko",
     title     = " Molecular motion in a spreading precursor film",
     journal   = " Phys. Rev. Lett.",
     volume    = " 93",
     year      = " 2004",
     pages     = " 206103-(1)-(4)",
}
@Article{ Y05,
     author    = " T. Young",
     title     = " An essay on the cohesion of fluids",
     journal   = " Phil. Trans. R. Soc. London ",
     volume    = " 95",
     year      = " 1805",
     pages     = " 65-87",
}
@Article{ Zisman,
     author    = " H. W. Fox and W. A. Zisman",
     title     = " The spreading of liquids on low energy surfaces.
                   I. Polytetrafluoroethylene",
     journal   = " J. Colloid. Sci.",
     volume    = " 5",
     year      = " 1950",
     pages     = " 514-531",
}

@Article{ ZS90,
     author    = " M.-Y Zhou and P. Sheng",
     title     = " Dynamics of Immiscible-Fluid Displacement in
                    a Capillary Tube",
     journal   = " Phys. Rev. Lett.",
     volume    = " 64",
     year      = " 1990",
     pages     = " 882-885",
}

@Book{ Zhou,
     author    = " Y. Zhou",
     title     = " Critical dynamics of contact lines",
     publisher = " PhD Thesis, Johns Hopkins University, Baltimore.",
     year      = " 1999",

}
@Book{ L07,
     author    = " P. S. {de Laplace}",
     title     = " M\'{e}canique C\'{e}leste, Suppl\'{e}ment au Xieme Livre ",
     publisher = " Courcier, Paris",
     year      = " 1807",

}

@Article{ B66,
     author    = " D. J. Benney",
     title     = " Long waves on liquid films",
     journal   = " J. Math. Phys. (N. Y.)",
     volume    = " 45",
     year      = " 1966",
     pages     = " 150-155",
}
@Article{ SN06,
     author    = " J. H. Snoeijer",
     title     = " Free surface flows with large slopes:
              beyond lubrication theory",
     journal   = " Phys. Fluids",
     volume    = " 18",
     year      = " 2006",
     pages     = " 021701",
}
@Article{ G04,
     author    = " G. Gr{\"u}n",
     title     = " Droplet spreading under weak slippage-existance for
                     the {C}auchy problem",
     journal   = " Comm. Partial Diff. Eqs.",
     volume    = " 29",
     year      = " 2004",
     pages     = " 1697-1744"
}
@Article{ BG05,
     author    = " J. Becker and G. Gr{\"u}n",
     title     = " The thin-film equation: recent advances and some
                     new perspectives",
     journal   = " J. Phys.: Condens. Matter",
     volume    = " 17",
     year      = " 2005",
     pages     = " S291-S307"
}
@Article{ PMP89,
     author    = " A. Pumir and P. Manneville and Y. Pomeau",
     title     = " On solitary waves running down an inclined plane",
     journal   = " J. Fluid Mech.",
     volume    = " 135",
     year      = " 1983",
     pages     = " 27-50",
}
@Article{ BF03,
     author    = " S. I. Betelu and M. A. Fontelos",
     title     = " Capillarity driven spreading of power-law fluids",
     journal   = " Appl. Math. Lett.",
     volume    = " 16",
     year      = " 2003",
     pages     = " 1315-1320",
}
@Article{ Betelu,
     author    = " S. I. Betelu and D. G. Aronson",
     title     = " Focusing of Noncircular Self-Similar Shock Waves",
     journal   = " Phys. Rev. Lett.",
     volume    = " 87",
     year      = " 2001",
     pages     = " 074501",
}
@Article{ BF04,
     author    = " S. I. Betelu and M. A. Fontelos",
     title     = " Capillarity driven spreading of circular drops
             of shear-thinning fluid",
     journal   = " Math. Computer Modelling",
     volume    = " 40",
     year      = " 2004",
     pages     = " 729-734",
}
@Article{ FF04,
     author    = " M. A. Fontelos and A. Friedman",
     title     = " Symmetry breaking bifurcations of charged drops",
     journal   = " Arch. Ration. Mech. Anal.",
     volume    = " 172",
     year      = " 2004",
     pages     = " 267",
}
@Article{ LF03,
     author    = " J. Li and M. A. Fontelos",
     title     = " Drop dynamics on the beads-on-string structure of
                      viscoelastic jets: a numerical study",
     journal   = " Phys. Fluids",
     volume    = " 15",
     year      = " 2003",
     pages     = " 922",
}
@Article{ FL04,
     author    = " M. A. Fontelos and J. Li",
     title     = " On the evolution and rupture of filaments in
                     Giesekus and FENE models",
     journal   = " J. Non-Newtonian Fluid Mech.",
     volume    = " 118",
     year      = " 2004",
     pages     = " 1",
}
@misc{ Y03,
     author    = " C. Yang",
     title     = " Dynamic point-formation in dielectric fluids",
     url       = "http://uk.arxiv.org/abs/physics/0303122",
     year      = " 2003",
}

@Article{ BFKV06,
     author   = " S. I. Betel{\'u} and M. A. Fontelos and
           U. Kindel{\'a}n and O. Vantzos",
     title     = " Singularities on charged viscous droplets",
     journal   = " Phys. Fluids",
     volume    = " 18",
     year      = " 2006",
     pages     = " 051706",
}

@Article{ FK08,
     author   = " M. A. Fontelos and U. Kindel{\'a}n",
     title     = " The shape of charged drops over a solid surface and
                  symmetry-breaking instabilities",
     journal   = " SIAM J. Appl. Math.",
     volume    = " 69",
     pages     = " 126",
     year      = " 2008",
}

@misc{ BFKV07,
     author    = " S. I. Betel{\'u} and M. A. Fontelos and
           U. Kindela{\'a}n and O. Vantzos",
     howpublished = "unpublished simulations",
     year      = " 2007",
}
@Article{ RBB04,
     author    = " S. Rafa{\"\i} and D. Bonn and A. Boudaoud",
     title     = " Spreading of non-Newtonian fluids on hydrophilic surfaces",
     journal   = " J. Fluid Mech.",
     volume    = " 513",
     year      = " 2004",
     pages     = " 77-85",
}
@Article{ Fenistein,
     author    = " D. Fenistein and D. Bonn and S. Rafa{\"\i} and G. H. Wegdam
    and J. Meunier and A. O. Parry and M. M. {Telo da Gama}",
     title     = " What controls the thickness of wetting
                      layers near bulk criticality? ",
     journal   = " Phys. Rev. Lett.",
     volume    = " 89",
     year      = " 2002",
     pages     = " 096101",
}
@Article{ PR01,
     author    = " L. M. Pismen and B. Y. Rubinstein",
     title     = " Kinetic slip condition, can der Waals forces,
                     and dynamic contact angle",
     journal   = " Langmuir",
     volume    = " 17",
     year      = " 2001",
     pages     = " 5265-5270",
}
@Article{ PP04,
     author    = " L. M. Pismen and Y. Pomeau",
     title     = " Mobility and interactions of weakly nonwetting droplets",
     journal   = " Phys. Fluids",
     volume    = " 16",
     year      = " 2004",
     pages     = " 2604-2612",
}
@Article{ I85,
     author    = " J. N. Israelachvili",
     title     = " Measurement of the viscosity of liquids in very thin films",
     journal   = " J. Colloid Interf. Sci.",
     volume    = " 110",
     year      = " 1986",
     pages     = " 263-271",
}

@Article{ RM98,
     author    = " C. Ruyer-Quil and P. Manneville",
     title     = " Modeling film flows down inclined planes",
     journal   = " Eur. Phys. J. B",
     volume    = " 6",
     year      = " 1998",
     pages     = " 277-292",
}
@Article{ SRTKLC04,
     author    = " B. Scheid and C. Ruyer-Quil and U. Thiele
            and O. A. Kabov and J. C. Legros and P. Colinet",
     title     = " Validity domain of the Benney equation
         including the Marangoni effect for closed and open flows",
     journal   = " J. Fluid Mech.",
     volume    = " 527",
     year      = " 2004",
     pages     = " 303-335",
}
@Article{ Bill02,
     author    = " J. Billingham",
     title     = " Nonlinear sloshing in zero gravity",
     journal   = " J. Fluid Mech.",
     volume    = " 464",
     year      = " 2002",
     pages     = " 365-391",
}
@Article{ dropweight,
     author    = " A. Ferguson",
     title     = " Some notes on the drop-weight method for the
                  measurement of surface tension",
     journal   = " J. Sci. Instrum.",
     volume    = " 6",
     year      = " 1929",
     pages     = " 163",
}
@Incollection{ amouroux,
     author    = " S. Wu",
     title     = " Modifications of polymer surfaces : mechanisms of
          wettability and bondability improvements",
     booktitle     = "Polymer Interfaces and Adhesion",
     editor    = " ",
     publisher = " Marcel Dekker, New York",
     year      = " 1982",
     pages     = " 279-329",
}
@Article{ PT06,
     author    = " L. M. Pismen and U. Thiele",
     title     = " Asymptotic theory for a moving droplet driven by
                     a wettability gradient",
     journal   = "Phys. Fluids",
     volume    = "18",
     pages     = "042104",
     year      = " 2006",
}
@article{TJB04,
  author =	 {Thiele, U. and John, K. and B{\"a}r, M.},
  title =	 {Dynamical Model for Chemically Driven Running
                  Droplets},
  year =	 {2004},
  journal =	 {Phys. Rev. Lett.},
  volume =	 {93},
  pages =	 {027802},
                          }
@Article{ WeissInd,
    author    = " V. C. Weiss and J. O. Indekeu",
    title     = " Effect of ion hydration on the
     first-order transition in the sequential wetting of hexane on brine",
    journal   = " J. Chem. Phys.",
     volume    = " 118",
     year      = " 2003",
     pages     = " 10741-10751",
          }

@Article{ WeissNew,
     author    = " V. C. Weiss and E. Bertrand and S. Rafa{\"\i}
                  and J. O. Indekeu and D. Bonn",
     title     = "  Effective exponents in the long-range critical
              wetting of alkanes on aqueous substrates",
     journal   = "  Phys. Rev. E",
     volume    = " 76",
     pages     = " 051602",
     year      = " 2007",
               }

@misc{ See05,
author = " R. Seemann",
year = "2005",
howpublished = "private communication"
}

@misc{ M_pr,
author = " G. H. McKinley",
year = "2005",
howpublished = "private communication",
}

@Article{rolley2007,
     author    = "E. Rolley and C. Guthmann",
     title     = " Hysteresis and dynamics of the contact line",
     journal   = " Phys. Rev. Lett.",
     volume    = "98",
     year      = "2007",
     pages     = "166105",
}
@Article{AL78,
     author    = "A.  Acrivos and T. S.  Lo ",
     title     = "Deformation and breakup of a single slender
      drop in an extensional flow",
     journal   = "J. Fluid Mech.",
     volume    = "86",
     year      = "1978",
     pages     = "641",
}

@article{YA76,
author = "Youngren, G. K. and Acrivos, A.",
title = "On the shape of a gas bubble in a viscous extensional flow",
journal = "Journal of Fluid Mechanics",
year = "1976",
volume = "76",
number = "3",
pages ="433--442"
}

@Article{AF95,
     author    = " I. Aguirre-de-Carcer and  J. {Fernandez de la Mora}",
     title     = " ",
     journal   = "J. Colloid Interface Sci.",
     volume    = "171",
     year      = "1995",
     pages     = "512",
}

@Article{ABB96,
     author    = "R. Almgren and A. L. Bertozzi and M. P. Brenner ",
     title     = "Stable and unstable singularities in the unforced
                    Hele-Shaw cell ",
     journal   = "Phys. Fluids",
     volume    = "8",
     year      = "1996",
     pages     = "1356",
}

@Article{A96,
     author    = "R. Almgren",
     title     = "Singularity formation in Hele-Shaw bubbles ",
     journal   = "Phys. Fluids",
     volume    = "8",
     year      = "1996",
     pages     = "344",
}

@Article{Alvalow03,
     author    = "E. Alvarez-Lacalle and J. Casademunt and J. Ort\'{\i}n",
     title     = "",
     journal   = "Phys. Fluids",
     volume    = "16",
     year      = "2004",
     pages     = "908",
}

@Article{Alvarez01,
     author    = "E. Alvarez-Lacalle and J. Casademunt and J. Ort\'{\i}n",
     title     = "",
     journal   = "Phys. Rev. E",
     volume    = "64",
     year      = "2001",
     pages     = "016302",
}

@Article{Lee02a,
     author    = "H-G. Lee and J. S. Lowengrub and J. Goodman",
     title     = "",
     journal   = "Phys. Fluids",
     volume    = "14",
     year      = "2002",
     pages     = "492",
}

@Article{Lee02b,
     author    = "H-G. Lee and J. S. Lowengrub and J. Goodman",
     title     = "",
     journal   = "Phys. Fluids",
     volume    = "14",
     year      = "2002",
     pages     = "514",
}

@Article{Tryggvason85,
     author    = "G. Tryggvason and H. Aref",
     title     = "",
     journal   = "J. Fluid Mech.",
     volume    = "154",
     year      = "1985",
     pages     = "287",
}

@Article{AAG95,
     author    = "S. Altschuler and S.  Angenent and Y.  Giga ",
     title     = "Mean curvature flow through singularities
        for surfaces of rotation",
     journal   = "J. Geom. Anal.",
     volume    = "5",
     year      = "1995",
     pages     = "293",
}

@Book{A78,
     author    = "D. J. Amit ",
     title     = "Field theory the renormalization group
           and critical phenomena",
     publisher = "New York: McGraw-Hill",
     year      = "1978"
}

@Book{Coddington,
     author    = "E. A. Coddington and N. Levinson",
     title     = "Theory of Ordinary Dierential Equations",
     publisher = "McGraw-Hill",
     year      = "1955"
}

@Book{Levitan,
     author    = "B. M. Levitan and I. S. Sargsjan",
     title     = "Sturm-Liouville and Dirac Operators",
     publisher = "Springer",
     year      = "1990"
}

@Book{Christie,
     author    = "L. {da Vinci} ",
     title     = "Codex Leicester",
     publisher = "Christie's London",
     year      = "1980"
}

@Article{ABMK01,
     author    = "Y. Amarouchene and D.  Bonn and
                   J. Meunier and H. Kellay ",
     title     = " Inhibition of the Finite-Time Singularity during
          Droplet Fission of a Polymeric Fluid",
     journal   = "Phys. Rev. Lett.",
     volume    = "86",
     year      = "2001",
     pages     = "3558",
}

@Article{AM01,
     author    = "S. L.  Anna and G. H.   McKinley ",
     title     = "Elasto-capillary Thinning and Breakup of
                  Model Elastic Liquids ",
     journal   = "J. Rheol.",
     volume    = "45",
     year      = "2001",
     pages     = "115",
}

@Article{MT90,
     author    = "J. E. Matta and R. P. Tytus",
     title     = "Liquid stretching using a falling cylinder",
     journal   = "J. Non-Newtonian Fluid Mech.",
     volume    = "35",
     year      = "1990",
     pages     = "215",
}

@Article{TS93,
     author    = "V. Tirtaatmadja and T. Sridhar",
     title     = "A filament stretching device for measurement of
                  extensional viscosity",
     journal   = "J. Rheology",
     volume    = "37",
     year      = "1993",
     pages     = "1081",
}

@Article{TMC06,
     author    = "V. Tirtaatmadja and G. H. McKinley and J. J. Cooper-White",
     title     = " ",
     journal   = "Phys. FLuids",
     volume    = "18",
     year      = "2006",
     pages     = "043101",
}

@Article{AMB95,
     author    = "N.  Ashgriz and F.   Mashayek ",
     title     = " ",
     journal   = "J. Fluid Mech.",
     volume    = "293",
     year      = "1995",
     pages     = "163",
}



@Book{B88,
     author    = "A. G. Bailey ",
     title     = "Electrostatic Spraying of Liquids",
     publisher = "Wiley",
     year      = "1988"
}

@Article{BMO80,
     author    = "G. R. D.  Baker and I.  Meiron and S. A. Orszag ",
     title     = " ",
     journal   = "Phys. Fluids",
     volume    = "23",
     year      = "1980",
     pages     = "1485",
}

@Article{BMO,
     author    = "G. R. D.  Baker and I.  Meiron and S. A. Orszag ",
     title     = "Generalized
             vortex methods for free-surface flow problems ",
     journal   = "J. Fluid Mech.",
     volume    = "123",
     year      = "1982",
     pages     = "477-501",
}

@Article{FdlH,
     author    = "M. A. Fontelos and F. {de la Hoz}",
     title     = "Singularities in water
       waves and the Rayleigh-Taylor problem",
     journal   = "J. Fluid Mech.",
     volume    = "??",
     year      = "2010",
     pages     = "???",
}

@Article{BM94,
     author    = "R.  Ziv and E. Moses ",
     title     = " ",
     journal   = "Phys. Rev. Lett.",
     volume    = "73",
     year      = "1994",
     pages     = "1392",
}

@Article{BZ72,
     author    = "G. I. Barenblatt and Y. B. Zel'dovich",
     title     = "Self-similar solutions as intermediate asymptotics",
     journal   = "Annu. Rev. Fluid Mech.",
     volume    = "4",
     year      = "1972",
     pages     = "285-312"
}

@Book{Sachdev,
     author    = "P. L. Sachdev",
     title     = "Shock Waves and Explosions",
     publisher = "Chapman and Hall",
     year      = "2004"
}

@Book{Sedov,
     author    = "L. I. Sedov",
     title     = "Similarity and dimensional methods in mechanics",
     publisher = "CRC Press",
     year      = "1993"
}

@Book{B96,
     author    = "G. I. Barenblatt ",
     title     = "Similarity Self-Similarity and Intermedeate Asymptotics",
     publisher = {Cambridge University Press, Cambridge},
     year      = "1996"
}

@Book{Barenblatt,
     author    = "G. I. Barenblatt ",
     title     = "Scaling",
     publisher = {Cambridge University Press, Cambridge},
     year      = "2003"
}

@Article{B-BA73,
     author    = "D. {Barth{\`e}s-Biesel} and A. Acrivos ",
     title     = "Deformation and burst of a liquid droplet freely
        suspended in a linear shear field",
     journal   = "J. Fluid Mech.",
     volume    = "61",
     year      = "1973",
     pages     = "1",
}
@Article{B02,
     author    = "O. A. Basaran ",
     title     = " ",
     journal   = "AICHE",
     volume    = "48",
     year      = "2002",
     pages     = "1842",
}

@Article{XB07,
     author    = "Q. Xu and O. A. Basaran ",
     title     = "Computational analysis of drop-on-demand drop formation",
     journal   = "Phys. Fluids",
     volume    = "19",
     year      = "2007",
     pages     = "102111",
}

@Article{DC06,
     author    = "H. Dong and W. W. Carr",
     title     = "An experimental study of drop-on-demand drop formation",
     journal   = "Phys. Fluids",
     volume    = "18",
     year      = "2006",
     pages     = "072102",
}

@Article{BBCF95,
     author    = "S. E.  Bechtel and K. Bolinger and G. Cao and M. G. Forest ",
     title     = " ",
     journal   = "SIAM J. Appl. Math.",
     volume    = "55",
     year      = "1995",
     pages     = "58",
}

@Article{BCF95,
     author    = "S. E.  Bechtel and C. D.  Carlson and M. G. Forest ",
     title     = " ",
     journal   = "Phys. Fluids",
     volume    = "7",
     year      = "1995",
     pages     = "2957",
}

@Article{BFL92,
     author    = "S. E. Bechtel and M. G.  Forest and K. J. Lin ",
     title     = " ",
     journal   = "SAACM ",
     volume    = "2",
     year      = "1992",
     pages     = "59",
}

@Article{BHK91,
     author    = "E. W. Becker and J. Hiller and T. A.  Kowalewski ",
     title     = " ",
     journal   = "J. Fluid Mech.",
     volume    = "231",
     year      = "1991",
     pages     = "189",
}

@Article{BHK94,
     author    = "E. W. Becker and J.  Hiller and T. A. Kowalewski ",
     title     = " ",
     journal   = "J. Fluid Mech.",
     volume    = "258",
     year      = "1994",
     pages     = "191",
}

@Book{BO78,
     author    = "C. M.  Bender and S. A. Orszag ",
     title     = "Advanced mathematical methods for scientists and engineers",
     publisher = "Mc Graw-Hill: New York",
     year      = "1978"
}

@Article{B86,
     author    = "D. Bensimon and L. P. Kadanoff and S. Liang and
           B. I. Shraiman and C. Tang",
     title     = " Viscous flows in two dimensions",
     journal   = "Rev Mod Phys",
     volume    = "58",
     year      = "1986",
     pages     = "977",
}

@Article{BL86a,
     author    = "B. J.  Bentley and L. G. Leal ",
     title     = " ",
     journal   = "J. Fluid Mech.",
     volume    = "167",
     year      = "1986a",
     pages     = "219",
}

@Article{BL86b,
     author    = "B. J.  Bentley and L. G. Leal ",
     title     = " ",
     journal   = "J. Fluid Mech.",
     volume    = "167",
     year      = "1986b",
     pages     = "241",
}

@Article{Ber88,
     author    = "S. A. Berger ",
     title     = " ",
     journal   = "SIAM J. Appl. Math.",
     volume    = "48",
     year      = "1988",
     pages     = "973",
}

@Inproceedings{Bertozzi,
     author    = "A. L. Bertozzi and M. P.  Brenner and
         T. F.  Dupont and L. P. Kadanoff ",
     title     = "Trends and Perspectives in Applied Mathematics",
     year      = "1994",
     booktitle = "Applied Mathematics Series Vol 100",
     editor    = "L. Sirovich",
     pages     = "115",
     publisher = "Springer: New York",
          }

@Article{B23,
     author    = "G. Bidone ",
     title     = " ",
     journal   = "Mem. Accad. della scienza di Torino",
     volume    = "27",
     year      = "1823",
     pages     = "83",
}

@Book{BAH87,
     author    = "R. B. Bird and R. C.  Armstrong and O. Hassager ",
     title     = "Dynamics of Polymeric Liquids Volume I:
             Fluid Mechanics; Volume I:     Kinetic Theory",
     publisher = "Wiley: New York",
     year      = "1987"
}

@Article{B78a,
     author    = "D. B. Bogy ",
     title     = " ",
     journal   = "J. Appl. Mech.",
     volume    = "45",
     year      = "1978a",
     pages     = "469",
}
@Article{B78b,
     author    = "D. B. Bogy ",
     title     = " ",
     journal   = "Phys. Fluids",
     volume    = "21",
     year      = "1978",
     pages     = "190",
}

@Article{B79a,
     author    = "D. B. Bogy ",
     title     = " ",
     journal   = "Phys. Fluids",
     volume    = "22 & 23",
     year      = "1979",
     pages     = "224 & 421",

}

@Article{B79b,
     author    = "D. B. Bogy ",
     title     = " ",
     journal   = "Annu. Rev. Fluid Mech.",
     volume    = "11",
     year      = "1979b",
     pages     = "207",
}

@Article{BST80,
     author    = "D. B.  Bogy and S. J.  Shine and F. E. Talke ",
     title     = " ",
     journal   = "J. Comput. Phys.",
     volume    = "38",
     year      = "1980",
     pages     = "294",
}

@Article{B09,
     author    = "N. Bohr ",
     title     = "Determination of the surface-tension of water by
                  the method of jet vibration ",
     journal   = "Phil. Trans. Roy. Soc. A",
     volume    = "209",
     year      = "1909",
     pages     = "281",
}

@Article{B10,
     author    = "N. Bohr ",
     title     = "On the determination of the tension of a recently formed
                  water-surface",
     journal   = "Phil. Trans. Roy. Soc. A",
     volume    = "84",
     year      = "1910",
     pages     = "395",
}

@Article{BKMD86,
     author    = "D. W.  Bousfield and R. Keunigs and
         G. Marrucci and M. M. Denn ",
     title     = " ",
     journal   = "J. Non-Newtonian Fluid Mech.",
     volume    = "21",
     year      = "1986",
     pages     = "79",
}

@Article{BS78,
     author    = "S. G.  Bradley and C. D. Stow ",
     title     = " ",
     journal   = "Phil. Trans. R. Soc. London A",
     volume    = "287",
     year      = "1978",
     pages     = "635",
}

@Article{BSN94,
     author    = "M. P.  Brenner and X. D.  Shi and S. R. Nagel ",
     title     = "Iterated instabilities during droplet fission",
     journal   = "Phys. Rev. Lett.",
     volume    = "73",
     year      = "1994",
     pages     = "3391",
}


@Article{BEJNS97,
     author    = "M. P.  Brenner and J.  Eggers and K. Joseph
              and S. R.  Nagel and X. D. Shi ",
     title     = " ",
     journal   = "Phys. Fluids",
     volume    = "9",
     year      = "1997",
     pages     = "1573",
}

@Article{BLS96,
     author    = "M. P. Brenner and J. R.  Lister and H. A. Stone ",
     title     = " Pinching threads, singularities and the number 0.0304...",
     journal   = "Phys. Fluids",
     volume    = "8",
     year      = "1996",
     pages     = "2827",
}

@Article{CB04,
     author    = "H. H. Chen and M. P. Brenner",
     title     = "The Optimal Faucet",
     journal   = "Phys. Rev. Lett.",
     volume    = "92",
     year      = "2004",
     pages     = "166106",
}

@Article{BGM90,
     author    = "U.  Brosa and S.  Grossmann and A. M{\"u}ller ",
     title     = "Nuclear Scission",
     journal   = "Phys. Rep.",
     volume    = "197",
     year      = "1990",
     pages     = "167",
}

@article{B72,
author = "Buckmaster, J. D.",
title = "Pointed bubbles in slow viscous flow",
journal = "J. Fluid Mech.",
year = "1972",
volume = "55",
pages ="385"
}

@article{BN78,
author = "J. D. Buckmaster and A. Nachman",
title = "The buckling and stretching of a viscida II. Effects of surface
               tension",
journal = "J. Mech. Appl. Math.",
year = "1978",
volume = "31",
pages ="157"
}

@article{B73,
author = "Buckmaster, J. D.",
title = "Viscous gravity spreading of an oil slick",
journal = "Journal of Fluid Mechanics",
year = "1973",
volume = "59",
pages ="481"
}

@Article{CR80,
     author    = "K. C.  Chaudhary and L. G. Redekopp ",
     title     = " ",
     journal   = "J. Fluid Mech.",
     volume    = "96",
     year      = "1980",
     pages     = "257",
}

@Article{CM80a,
     author    = "K. C.  Chaudhary and T. Maxworthy ",
     title     = " ",
     journal   = "J. Fluid Mech.",
     volume    = "96",
     year      = "1980a",
     pages     = "275",
}

@Article{CM80b,
     author    = "K. C.  Chaudhary and T. Maxworthy ",
     title     = " ",
     journal   = "J. Fluid Mech.",
     year      = "1980b",
     pages     = "287",
}

@Article{CEFLM06,
     author    = "C. Clasen and J. Eggers and
          M. A.  Fontelos and J.  Li and G. H. McKinley ",
     title     = "The beads-on-string structure of viscoelastic jets",
     journal   = "J. Fluid Mech.",
     volume    = "556",
     year      = "2006",
     pages     = "283",
}

@misc{EF_caus,
     author    = "J. Eggers and M. A.  Fontelos",
     title     = "Caustics in interfacial problems",
     journal   = "preprint",
     year      = "2009",
}

@Article{YCM06,
     author    = "B. Yesilata and C. Clasen and G. H. McKinley ",
     title     = " Nonlinear shear and extensional flow dynamics of wormlike
                 surfactant solutions",
     journal   = "J. Non-Newtonian Fluid Mech.",
     volume    = "133",
     year      = "2006",
     pages     = "73",
}

@Article{CA78,
     author    = "H. E.  Cline and T. R. Anthony ",
     title     = " ",
     journal   = "J. Appl. Phys.",
     volume    = "49",
     year      = "1978",
     pages     = "3203",
}

@Article{CBEN99,
     author    = "I. Cohen and M. P. Brenner and J. Eggers and S. R. Nagel ",
     title     = "Two fluid drop snap-off problem: experiment and theory",
     journal   = "Phys. Rev. Lett.",
     volume    = "83",
     year      = "1999",
     pages     = "1147",
}

@Article{ML02,
     author    = "I. N. Milosevic and E. K. Longmire",
     title     = "Pinch-Off Modes and Satellite Formation in
                          Liquid-Liquid Jet Systems",
     journal   = "Int. J. Multiphase Flow",
     volume    = "28",
     year      = "2002",
     pages     = "1853",
}

@Article{CDGKSZ93,
     author    = "P. Constantin and T. F.  Dupont and R. E. Goldstein
        and L. P. Kadanoff and M. J.  Shelley and {S.-M.} Zhou ",
     title     = "Droplet breakup in a model of the Hele-Shaw cell",
     journal   = "Phys. Rev. E",
     volume    = "47",
     year      = "1993",
     pages     = "4169",
}

@Article{Goldstein93,
     author    = "R. E. Goldstein and A. I. Pesci and M. J. Shelley",
     title     = "",
     journal   = "Phys. Rev. Lett.",
     volume    = "70",
     year      = "1993",
     pages     = "3043",
}

@Article{Goldstein95,
     author    = "R. E. Goldstein and A. I. Pesci and M. J. Shelley",
     title     = "",
     journal   = "Phys. Rev. Lett.",
     volume    = "75",
     year      = "1995",
     pages     = "3665",
}

@Article{DGKZ93,
     author    = "T. F.  Dupont and R. E. Goldstein
        and L. P. Kadanoff and {S.-M.} Zhou ",
     title     = " Finite-time singularity formation in Hele-Shaw systems",
     journal   = "Phys. Rev. E",
     volume    = "47",
     year      = "1993",
     pages     = "4182",
}

@Article{CCFF04,
     author    = "A.  Cordoba and D.  Cordoba
                and C. L.  Fefferman and M. A. Fontelos ",
     title     = " ",
     journal   = "Adv. Math.",
     volume    = "187",
     year      = "2004",
     pages     = "228",
}

@Article{CE06,
     author    = "S. {Courrech du Pont} and J. Eggers ",
     title     = "Sink flow deforms the interface between
         a viscous liquid and air into a tip singularity",
     journal   = "Phys. Rev. Lett.",
     volume    = "96",
     year      = "2006",
     pages     = "034501"
}

@Article{EC09,
     author    = "J. Eggers and S. {Courrech du Pont}",
     title     = "Numerical analysis of tip singularities in viscous flow ",
     journal   = "Phys. Rev. E",
     volume    = "79",
     year      = "2009",
     pages     = "066311"
}

@Article{SLE09,
     author    = "J. S{\'e}billeau and L. Limat and J. Eggers",
     title     = "Flow separation from a stationary meniscus",
     journal   = "J. Fluid Mech.",
     volume    = "633",
     year      = "2009",
     pages     = "137",
}

@Article{EH09,
     author    = "J. Eggers and J. Hoppe",
     title     = "Singularity formation for timelike extremal hypersurfaces",
     journal   = "Phys. Lett. B",
     volume    = "680",
     pages     = "274",
     year      = "2009"
}

@Article{CBM64,
     author    = "L. S. Crane and S.  Birch and P. O. McCormack ",
     title     = " ",
     journal   = "Brit. J. Appl. Phys.",
     volume    = "15",
     year      = "1964",
     pages     = "743",
}

@Article{D87,
     author    = "C. M. Dafermos ",
     title     = " ",
     journal   = "SIAM J. Math. Anal.",
     volume    = "18",
     year      = "1987",
     pages     = "409",
}

@Inproceedings{Da-Riva,
     author    = "I. Da-Riva",
     title     = "Applications of Space Development",
     year      = "1981",
     booktitle = "XXXI International Astronautical Congress",
     editor    = "L. G. Napolitano,",
     pages     = "69",
     publisher = "Pergamon",
}

@Inproceedings{daVinci,
     author    = "L. {da Vinci}",
     title     = "Codex Leicester",
     year      = "1508",
     booktitle = "The Notebooks of Leonardo da Vinci",
     editor    = "translated in MacCurdy",
     pages     = "756",
     publisher = "George Brazillier: New York",
}

@Article{DHL98,
     author    = "R. F. Day and E. J.  Hinch and J. R. Lister ",
     title     = "Self-similar capillary Pinchoff of an inviscid fluid ",
     journal   = "Phys. Rev. Lett.",
     volume    = "80",
     year      = "1998",
     pages     = "704",
}

@Article{LH96,
     author    = "M. Loewenberg and E. J. Hinch",
     title     = "Numerical simulation of a concentrated emulsion in
          shear flow",
     journal   = "J. Fluid Mech.",
     volume    = "321",
     year      = "1996",
     pages     = "395-419",
}

@Article{D97,
     author    = "K. Deckelnick ",
     title     = " ",
     journal   = "Nonlinearity",
     volume    = "10",
     year      = "1997",
     pages     = "655",
}

@Article{DOW92,
     author    = "J. N. Dewynne and J. R. Ockenden and P. Wilmott ",
     title     = " ",
     journal   = "J. FLuid Mech.",
     volume    = "244",
     year      = "1992",
     pages     = "323",
}

@Article{DHW94,
     author    = "J. N.  Dewynne and P. D. Howell and P. Wilmott ",
     title     = " ",
     journal   = "Quarterly J. Mech. Appl. Math.",
     volume    = "47",
     year      = "1994",
     pages     = "541",
}

@Article{D92,
     author    = "J. W. Dold ",
     title     = " ",
     journal   = "J. Comp. Phys.",
     volume    = "103",
     year      = "1992",
     pages     = "90",
}

@Article{Lind05,
     author    = "H. Lindblad ",
     title     = "Well-posedness for the motion of an incompressible
                  liquid with free surface boundary  ",
     journal   = "Ann. Math.",
     volume    = "162",
     year      = "2005",
     pages     = "109",
}

@Article{DY87,
     author    = "D. G.  Dommermuth and D. K. P. Yue ",
     title     = " ",
     journal   = "J. Fluid Mech.",
     volume    = "178",
     year      = "1987",
     pages     = "195",
}

@Article{DG66,
     author    = "R. J.  Donnelly and W. Glaberson ",
     title     = " ",
     journal   = "Proc. Roy. Soc. London A",
     volume    = "290",
     year      = "1966",
     pages     = "547",
}

@Article{DCZSHBN03,
     author    = "P. Doshi and I. Cohen and W. W.  Zhang and
          M. Siegel and P. Howell and O. A. Basaran and S. R. Nagel ",
     title     = " Persistence of memory in drop breakup: the
                  breakdown of universality",
     journal   = "Science",
     volume    = "302",
     year      = "2003",
     pages     = "1185",
}

@Article{S99,
     author    = "M. Siegel ",
     title     = "Influence of surfactant on rounded and pointed bubbles
                 in two-dimensional Stokes flow",
     journal   = "SIAM J. Appl. Math.",
     volume    = "59",
     year      = "1999",
     pages     = "1998",
}

@Article{DB04,
     author    = "P. Doshi and O. A. Basaran",
     title     = "Self-similar pinch-off of power law fluids",
     journal   = "Phys. Fluids",
     volume    = "16",
     year      = "2004",
     pages     = "585",
}

@Article{YB01,
     author    = "O. E. Yildirim and O. A. Basaran",
     title     = "Deformation and breakup of stretching bridges of
                  Newtonian and shear-thinning liquids: comparison of
                  one- and two-dimensional models",
     journal   = "Chem. Engin. Sci.",
     volume    = "56",
     year      = "2001",
     pages     = "211",
}

@Article{DSYMB03,
     author    = "P. Doshi and R. Suryo and O. E. Yildirim and
                 G. H. McKinley and O. A. Basaran",
     title     = "Scaling in pinch-off of generalized Newtonian liquids",
     journal   = "J. Non-Newtonian Fuid Mech.",
     volume    = "113",
     year      = "2003",
     pages     = "1",
}

@misc{D93,
     author    = "T. F. Dupont ",
     year      = "1993",
     howpublished = "private communication"
}

@Article{EHT37,
     author    = "H. E.  Edgerton and E. A.  Hauser and W. B. Tucker ",
     title     = " ",
     journal   = "J. Phys. Chem.",
     volume    = "41",
     year      = "1937",
     pages     = "1029",
}

@Book{E77,
     author    = "H. E. Edgerton ",
     title     = "Stopping time: the photographs of Harold Edgerton",
     year      = "1977",
     publisher = "Abrams: New York",
}

@Article{E95a,
     author    = "J. Eggers ",
     title     = "Theory of drop formation ",
     journal   = "Phys. Fluids",
     volume    = "7",
     year      = "1995",
     pages     = "941",
}

@Article{E00,
     author    = "J. Eggers ",
     title     = "Singularities in droplet pinching with vanishing viscosity",
     journal   = "SIAM J. Appl. Math.",
     volume    = "60",
     year      = "2000",
     pages     = "1997",
}

@Article{E01,
     author    = "J. Eggers ",
     title     = " Air entrainment through free-surface cusps",
     journal   = "Phys. Rev. Lett.",
     volume    = "86",
     year      = "2001",
     pages     = "4290",
}

@Article{SLB99,
     author    = "H. A. Stone and J. R. Lister and M. P. Brenner",
     title     = "Drops with conical ends in electric and magnetic fields ",
     journal   = "Proc. Roy. Soc. Lond. A",
     volume    = "455",
     year      = "1999 ",
     pages     = "329",
}

@Article{L89,
     author    = "J. R. Lister",
     title     = "Selective withdrawal from a viscous two-layer system",
     journal   = "J. Fluid Mech.",
     volume    = "198",
     year      = "1989 ",
     pages     = "231-254"
}


@Article{LCL79,
     author    = "S. H. Lee and R. S. Chadwick and L. G. Leal",
     title     = "Motion of a sphere in the presence of a plane interface.
       Part 1. An approximate solution by generalization of the method of
                Lorentz",
     journal   = "J. Fluid Mech.",
     volume    = "93",
     year      = "1979 ",
     pages     = "705-726"
}

@Article{LL80,
     author    = "S. H. Lee and L. G. Leal",
     title     = "Motion of a sphere in the presence of a plane interface.
            Part 2. An exact solution in bipolar co-ordinates",
     journal   = "J. Fluid Mech.",
     volume    = "98",
     year      = "1980 ",
     pages     = "193-224",
}

@Article{ED94,
     author    = "J.  Eggers and T. F. Dupont ",
     title =   {Drop formation in a one-dimensional approximation
          of the Navier-Stokes equation.},
     journal   = "J. Fluid Mech.",
     volume    = "262",
     year      = "1994",
     pages     = "205",
}

@Article{EY84,
     author    = "V. M.  Entov and A. L. Yarin ",
     title     = "The dynamics of thin liquid jets in air ",
     journal   = "J. Fluid Mech.",
     volume    = "140",
     year      = "1984",
     pages     = "91",
}

@Article{EH97,
     author    = "V. M.  Entov and E. J. Hinch",
     title     = "Effect of a spectrum of relaxation times on the capillary
                  thinning of a filament of elastic liquids",
     journal   = "J. Non-Newt. Fluid Mech.",
     volume    = "72",
     year      = "1997",
     pages     = "31",
}

@Article{BELR97,
     author    = "A. V. Bazilevskii and V. M. Entov and M. M. Lerner
          and A. N. Rozhkov",
     title     = "Failure of polymer solution filaments ",
     journal   = "Polym. Sci. Ser. A",
     volume    = "39",
     year      = "1997",
     pages     = "316",
}

@Inproceedings{BER90,
     author    = "A. V. Bazilevskii and V. M. Entov and A. N. Rozhkov",
     title     = "Liquid Filament Microrheometer and Some of its Applications",
     year      = "1990",
     booktitle = "Proceedings of the Third European Rheology Conference",
     editor    = "D. R. Oliver",
     pages     = "41",
     publisher = "Elsevier Applied Science"
}

@Article{BVER81,
     author    = "A. V. Bazilevskii and S. I. Voronkov and V. M. Entov
              and A. N. Rozhkov",
     title     = "Orientational effects in the decomposition of
        streams and strands of diluted polymer solutions",
     journal   = "Sov. Phys. Dokl.",
     volume    = "26",
     year      = "1981",
     pages     = "333"
}

@Article{RYZB06,
     author    = "S. N. Reznik and A. L. Yarin and E. Zussman
               and L. Bercovici",
     title     = " ",
     journal   = "Phys. Fluids",
     volume    = "18",
     year      = "2006",
     pages     = "062101",
}

@Article{EY80,
     author    = "V. M.  Entov and A. L. Yarin ",
     title     = " ",
     journal   = "Fluid Dyn.",
     volume    = "15",
     year      = "1980",
     pages     = "644",
}

@Article{EYa84,
     author    = "V. M.  Entov and A. L. Yarin ",
     title     = "Influence of elastic stresses on the capillary breakup
                   of dilute polymer solutions ",
     journal   = "Fluid Dyn.",
     volume    = "19",
     year      = "1984",
     pages     = "21",
}

@Article{EKKSY80,
     author    = "V. M.  Entov and W. E. Kordonskii and V. A. Kuz'min
                Z. P. Shul'man and A. L. Yarin ",
     title     = " ",
     journal   = "Zh. Prikl. Mekh. i Tekh. Fiz.",
     volume    = "3",
     year      = "1980",
     pages     = "90",
}

@Article{FZ04,
     author    = "L. G. Fel and Y. Zimmels",
     title     = " ",
     journal   = "J. Exp. Theor. Phys.",
     volume    = "98",
     year      = "2004",
     pages     = "960",
}

@Article{FMMWW89,
     author    = "J. B. Fenn and M. Mann and C. K. Meng and
        S. F.  Wong and C. M.  Whitehouse ",
     title     = " ",
     journal   = "Science",
     volume    = "246",
     year      = "1989",
     pages     = "64",
}

@Article{FL94,
     author    = " J. {Fernandez de la Mora} and I. G.  Loscertales ",
     title     = " ",
     journal   = "J. Fluid Mech.",
     volume    = "260",
     year      = "1994",
     pages     = "155",
}

@Article{FW90,
     author    = "M. G.  Forest and Q. Wang ",
     title     = " ",
     journal   = "J. Theor. Comp. Fluid Dyn.",
     volume    = "2",
     year      = "1990",
     pages     = "1",
}

@Article{FW94,
     author    = "M. G.  Forest and Q. Wang ",
     title     = " ",
     journal   = "SIAM J. Appl. Math.",
     volume    = "54",
     year      = "1994",
     pages     = "996",
}

@Article{FW85,
     author    = "I.  Frankel and D. Weihs ",
     title     = " ",
     journal   = "J. Fluid Mech.",
     volume    = "155",
     year      = "1985",
     pages     = "289",
}

@Book{F95,
     author    = "U. Frisch ",
     title     = "Turbulence",
     year      = "1995",
     publisher = {Cambridge University Press, Cambridge},
}

@Article{F84,
     author    = "J. E. Fromm ",
     title     = " ",
     journal   = "IBM J. Res. Develop.",
     volume    = "28",
     year      = "1984",
     pages     = "322",
}

@Article{G83,
     author    = "M. D. Gabovich ",
     title     = " ",
     journal   = "Usp. Fiz. Nauk.",
     volume    = "140",
     year      = "1983",
     pages     = "137",
}

@Article{G83b,
     author    = "M. D. Gabovich ",
     title     = " ",
     journal   = "Sov. Phys. Usp.",
     volume    = "26",
     year      = "1983",
     pages     = "447",
}

@Article{G98,
     author    = "A. M. Ga{\~n}{\'a}n-Calvo",
     title     = "Generation of Steady Liquid Microthreads and
  Micron-Sized Monodisperse Sprays in Gas Streams",
     journal   = "Phys. Rev. Lett.",
     volume    = "80",
     year      = "1998",
     pages     = "285",
          }

@Article{GHG06,
     author    = "A. M. Ga{\~n}{\'a}n-Calvo and M. A.
                Herrada and P. Garstecki",
     title     = " ",
     journal   = "Phys. Rev. Lett.",
     volume    = "96",
     year      = "2006",
     pages     = "124504",
}

@Article{GGRHF07,
     author    = "A. M. Ga{\~n}{\'a}n-Calvo and R. Gonz{\'a}lez-Prieto
             and P. Riesco-Chueca and M. A. Herrada and M. Flores-Mosquera",
     title     = "Focusing capillary jets close to the continuum limit ",
     journal   = "Nature Phys.",
     volume    = "3",
     year      = "2007",
     pages     = "737",
}

@Article{MFRRCCG05,
     author    = "L. Martin-Banderas and M. Flores-Mosquera and
          P. Riesco-Chueca and A. Rodriguez-Gil and A. Cebolla-Ramirez
        and S. {Chavez de Diego} and A. M. Ga{\~n}an-Calvo",
     title     = "Flow Focusing: a Versatile Technology to Produce
                 Size-Controlled and Specific-Morphology Microparticles",
     journal   = "Small",
     volume    = "1",
     year      = "2005",
     pages     = "688"
}

@Article{G-C07,
     author    = "A. M. Ga{\~n}{\'a}n-Calvo",
     title     = " Absolute instability of a viscous hollow jet",
     journal   = "Phys. Rev. E",
     volume    = "75",
     year      = "2007",
     pages     = "027301",
}

@Article{G-C07b,
     author    = "A. M. Ga{\~n}{\'a}n-Calvo",
     title     = " Electro-Flow Focusing: The High-Conductivity
            Low-Viscosity Limit",
     journal   = "Phys. Rev. Lett.",
     volume    = "98",
     year      = "2007",
     pages     = "027301",
}

@Article{BS07,
     author    = "O. A. Basaran and R. Suryo",
     title     = "The invisible jet",
     journal   = "Nature Phys.",
     volume    = "3",
     year      = "2007",
     pages     = "679",
}

@Article{SB06,
     author    = "R. Suryo and O. A. Basaran",
     title     = "Tip streaming from a liquid drop forming from a tube
                  in a co-flowing outer liquid",
     journal   = "Phys. Fluids ",
     volume    = "18",
     year      = "2006",
     pages     = "082102",
}

@Article{GC94,
     author    = "F. J.  Garcia and A. Castellanos ",
     title     = " ",
     journal   = "Phys. Fluids",
     volume    = "6",
     year      = "1994",
     pages     = "276",
}

@Article{G82,
     author    = "H. Giesekus ",
     title     = " ",
     journal   = "J. Non-Newtonian Fluid Mech.",
     volume    = "11",
     year      = "1982",
     pages     = "69",
}

@Article{BR02,
     author    = "L. Berg{\'e} and J. J.  Rasmussen",
     title     = "Collapsing dynamics of attractive Bose-Einstein condensates",
     journal   = "Phys. Lett. A",
     volume    = "304",
     year      = "2002",
     pages     = "136",
}

@Article{MGF03,
     author    = "K. D. Moll and A. L. Gaeta and G. Fibich",
     title     = "Self-similar optical wave collapse: Observation
              of the Townes profile",
     journal   = "Phys. Rev. Lett.",
     volume    = "90",
     year      = "2003",
     pages     = "203902",
}

@Article{GK85,
     author    = "Y.  Giga and R. V. Kohn ",
     title     = "Asymptotically self-similar blow-up of
        seminlinear heat-equations",
     journal   = "Comm. Pure Appl. Math.",
     volume    = "38",
     year      = "1985",
     pages     = "297",
}

@Article{FK92,
     author    = "S. Filippas and R. V. Kohn",
     title     = "Refined asymptotics for the blowup of
                      $u\sb t-\Delta u=u\sp p$",
     journal   = "Comm. Pure Appl. Math.",
     volume    = "45",
     year      = "1992",
     pages     = "821-869",
}

@Article{GK87,
     author    = "Y.  Giga and R. V. Kohn ",
     title     = "Characterizing blowup using similarity variables ",
     journal   = "Indiana University Math. J.",
     volume    = "36",
     year      = "1987",
     pages     = "1",
}

@Article{GK89,
     author    = "Y.  Giga and R. V. Kohn ",
     title     = "Nondegeneracy of blowup for semilinear heat-equations ",
     journal   = "Comm. Pure Appl. Math.",
     volume    = "42",
     year      = "1989",
     pages     = "845",
}

@Article{GD71,
     author    = "R. D.  Gillette and D. C. Dyson ",
     title     = "Stability of fluid interfaces of revolution between
                equal solid circular plates",
     journal   = "Chemical Engineering",
     volume    = "2",
     year      = "1971",
     pages     = "44",
}

@Article{GY70,
     author    = "E. F.  Goedde and M. C. Yuen ",
     title     = " ",
     journal   = "J. Fluid Mech.",
     volume    = "40",
     year      = "1970",
     pages     = "495",
}

@Article{GYPS69,
     author    = "M. Goldin and J. Yerushalmi and R. Pfeffer and R. Shinnar ",
     title     = "Breakup of a laminar capillary jet of a viscoelastic
                  fluid ",
     journal   = "J. Fluid Mech.",
     volume    = "38",
     year      = "1969",
     pages     = "689",
}

@Article{GG82,
     author    = "S. L. Goren and M. Gottlieb",
     title     = "Surface-tension-driven breakup of viscoelastic driven
                   threads",
     journal   = "J. Fluid Mech.",
     volume    = "120",
     year      = "1982",
     pages     = "245",
}

@Article{LL06,
     author    = " Z. Liu and Z. Liu",
     title     = "Linear analysis of three-dimensional instability
                of non-Newtonian liquid jets",
     journal   = "J. Fluid Mech.",
     volume    = "559",
     year      = "2006",
     pages     = "451",
}

@Book{GR80,
     author    = "I. S.  Gradshteyn and I. M. Ryzhik ",
     title     = "Table of Integrals Series and Products",
     year      = "1980",
     publisher = "Academic: New York ",
}

@Article{GM66,
     author    = "R. P.  Grant and S. Middleman ",
     title     = " ",
     journal   = "AICHE J.",
     volume    = "12",
     year      = "1966",
     pages     = "669",
}

@Article{GS91,
     author    = "R. Grauer and T. C. Sideris ",
     title     = " ",
     journal   = "Phys. Rev. Lett.",
     volume    = "67",
     year      = "1991",
     pages     = "3511",
}

@Article{M00,
     author    = "H. K. Moffatt",
     title     = "The interaction of skewed vortex pairs:
     a model for blow-up of the Navier-Stokes equations",
     journal   = "J. Fluid Mech.",
     volume    = "409",
     year      = "2000",
     pages     = "51",
}

@Article{GMG98,
     author    = "R. Grauer and C. Marliani and K. Germaschewski",
     title     = "Adaptive mesh refinement for singular
           solutions of the incompressible Euler equations",
     journal   = "Phys. Rev. Lett.",
     volume    = "80",
     year      = "1998",
     pages     = "4177",
}

@Article{GMS03,
     author    = "J. D. Gibbon and D. R. Moore and J. T. Stuart",
     title     = "Exact, infinite energy, blow-up solutions of the
              three-dimensional Euler equations",
     journal   = "Nonlinearity",
     volume    = "16",
     year      = "2003",
     pages     = "1823",
}

@Article{PLGG08,
     author    = "Y. Pomeau and M. {Le Berre} and P. Guyenne and S. Grilli",
     title     = "Wave-breaking and generic singularities of nonlinear
           hyperbolic equations",
     journal   = "Nonlinearity",
     volume    = "21",
     year      = "2008",
     pages     = "T61-T79"
}

@Article{CFMR05,
     author    = "D. C{\'o}rdoba and M. A. Fontelos and
            A. M.  Mancho and J. L. Rodrigo",
     title     = "Evidence of singularities for a family of
          contour dynamics equations",
     journal   = "PNAS",
     volume    = "102",
     year      = "2005",
     pages     = "5949",
}

@Article{G76,
     author    = "A. E. Green ",
     title     = " ",
     journal   = "Int. J. Engng. Sci.",
     volume    = "14",
     year      = "1976",
     pages     = "49",
}

@Article{GL66,
     author    = "A. E.  Green and N. Laws ",
     title     = " ",
     journal   = "Proc. Roy. Soc. London A",
     volume    = "293",
     year      = "1966",
     pages     = "145",
}

@Article{G93,
     author    = "D. Greenspan ",
     title     = " ",
     journal   = "SAMS",
     volume    = "11",
     year      = "1993",
     pages     = "87",
}

@Article{GH91,
     author    = "D.  Greenspan and L. F. Heath ",
     title     = " ",
     journal   = "J. Phys D: Appl. Phys.",
     volume    = "24",
     year      = "1991",
     pages     = "2121",
}

@Article{GM84,
     author    = "S.  Grossmann and A. M{\"u}ller ",
     title     = "Instabilities and decay rates of charged
                viscous liquid jets ",
     journal   = "Z. Phys. B",
     volume    = "57",
     year      = "1984",
     pages     = "161",
}

@Article{Grundy83,
     author    = "R. E. Grundy",
     title     = "Local similarity solutions for the initial
            value problem in nonlinear diffusion",
     journal   = "IMA J. Appl. Math.",
     volume    = "30",
     year      = "1983",
     pages     = "209-214",
}

@Article{GB93,
     author    = "R. E. Grundy and V. A. Bell",
     title     = "Waiting time solutions of the shallow water equations",
     journal   = "Proc. Roy. Soc. London Ser. A",
     volume    = "441",
     year      = "1993",
     pages     = "641-648",
}

@Article{Guderley,
     author    = "G. Guderley ",
     title     = "Starke Kugelige und Zylindrische Verdichtungsst{\"o}{\ss}e
      in der N{\"a}he des Kugelmittelpunktes bzw. der Zylinderachse ",
     journal   = "Luftfahrtforschung",
     volume    = "19",
     year      = "1942",
     pages     = "302",
}

@Article{G64,
     author    = "F. Guthrie ",
     title     = " ",
     journal   = "Proc. Roy. Soc.",
     volume    = "13",
     year      = "1864",
     pages     = "444",
}

@Article{H31,
     author    = "A. Haenlein ",
     title =   {\"Uber den Zerfall eines Fl\"ussigkeitsstrahles.},
     journal   = "Forschung  auf dem Gebiete des Ingenieurwesens",
     volume    = "2",
     year      = "1934",
     pages     = "139",
}

@Article{H49,
     author    = "G. Hagen ",
     title     = " ",
     journal   = "Verhandlungen Preuss. Akad. Wissenschaften",
     year      = "1849",
     pages     = "281",
}

@Book{HB83,
     author    = "J.  Happel and H. Brenner ",
     title     = "Low Reynolds Number Hydrodynamics",
     year      = "1983",
     publisher = "Martinus Nijhoff Publishers, The Hague",
}

@Article{HB19,
     author    = "W. D.  Harkins and F. E. Brown ",
     title     = " ",
     journal   = "J. Am. Chem. Soc.",
     volume    = "41",
     year      = "1919",
     pages     = "499",
}

@Article{HB93,
     author    = "M. T.  Harris and O. A. Basaran ",
     journal   = "J. Colloid Interface Sci.",
     volume    = "161",
     year      = "1993",
     pages     = "389",
}

@Article{HEHC36,
     author    = "E. A.  Hauser and H. E.  Edgerton and B. M.  Holt and
     J. T. {Cox Jr.}",
     title     = " ",
     journal   = "J. Phys. Chem.",
     volume    = "40",
     year      = "1936",
     pages     = "973",
}

@Article{HBT86,
     author    = "I. Hayati and A. I.  Bailey and T. F. Tadros ",
     title     = " ",
     journal   = "Nature",
     volume    = "319",

     pages     = "41",
}

@Article{HBT87,
     author    = "I.  Hayati and A. I.  Bailey and T. F. Tadros ",
     title     = " ",
     journal   = "J. Colloid Interface Sci.",
     volume    = "117",
     year      = "1987",
     pages     = "205",
}

@Article{HN81,
     author    = "C. W.  Hirt and B. D. Nichols ",
     title     = " ",
     journal   = "J. Comp. Phys.",

     year      = "1981",
     pages     = "201",
}

@Book{Hoppe92,
     author    = " J. Hoppe ",
     title     = "Lectures on Integrable Systems",
     year      = "1992",
     publisher = "Springer ",
}

@Book{CC09,
     author    = "E. Cosserat and F. Cosserat",
     title     = "Th{\'e}orie des Corps D{\'e}formables",
     year      = "1909",
     publisher = "Hermann, Paris",
     webpage   = "http://historical.library.cornell.edu/cgi-bin/
               cul.math/docviewer?did=06420001&seq=9"
}

@misc{Hop95,
     author    = " J. Hoppe ",
     howpublished = "private communication",
     year      = "1995",
}

@Article{HK89,
     author    = "W. J.  Hiller and T. A. Kowalewski ",
     title     = " ",
     journal   = "Optical Engineering",
     volume    = "28",
     year      = "1989",
     pages     = "197",
}

@Article{H77,
     author    = "E. J. Hinch ",
     title     = " ",
     journal   = "Phys. Fluids",
     volume    = "20",
     year      = "1977",
     pages     = "22",
}

@Article{HA79,
     author    = "E. J.  Hinch and A. Acrivos ",
     title     = "Steady long slender droplets in two-dimensional
             straining motion",
     journal   = "J. Fluid Mech.",
     volume    = "91",
     year      = "1979",
     pages     = "401",
}

@Article{HA80,
     author    = "E. J.  Hinch and A. Acrivos ",
     title     = " ",
     journal   = "J. Fluid Mech.",
     volume    = "98",
     year      = "1980",
     pages     = "305",
}

@Article{H91,
     author    = "G. Huisken ",
     title     = " ",
     journal   = "J. Diff. Geom.",
     volume    = "31",
     year      = "1991",
     pages     = "285",
}
@Article{Huis93,
     author    = "G. Huisken ",
     title     = "Local and global behaviour of
          hypersurfaces moving by mean curvature ",
     journal   = "Proc. of Symposia in Pure Math.",
     volume    = "54",
     year      = "1993",
     pages     = "175-191",
}

@Article{IF90,
     author    = "I. I.  Inculet and J. M. Floryan ",
     title     = " ",
     journal   = "Int. J. Microgravity Research Applications",
     volume    = "3",
     year      = "1990",
     pages     = "148",
}

@Book{J75,
     author    = "J. D. Jackson ",
     title     = "Classical Electrodynamics",
     year      = "1975",
     publisher = "Wiley",
}

@Article{JME85,
     author    = "G. R. Johnson and E.  Marschall and J. H. Esdorn ",
     title     = " ",
     journal   = "Rev. Sci. Instrum.",
     volume    = "56",
     year      = "1985",
     pages     = "264",
}

@Article{JKHSP91,
     author    = "M. Johnson and R. D. Kamm and L. W. Ho
               and A.  Shapiro and T. J. Pedley ",
     title     = " ",
     journal   = "J. Fluid Mech.",
     volume    = "233",
     year      = "1991",
     pages     = "141",
}

@Article{J91,
     author    = "D. D. Joseph and J. Nelson and M. Renardy and Y. Renardy",
     title     = " ",
     journal   = "J. Fluid Mech.",
     volume    = "223",
     year      = "1991",
     pages     = "383",
}

@Article{KLAS03,
     author    = "A.  Kalaaji and B. Lopez and P. Attan{\'e}
                   and A.  Soucemarianadin ",
     title     = " Breakup length of forced liquid jets",
     journal   = "Phys. Fluids",
     volume    = "15",
     year      = "2003 ",
     pages     = "2469",
}

@Article{GG06,
     author    = "H. Gonz{\'a}lez and F. J. Garcia",
     title     = " Comment on Breakup length of forced liquid jets ",
     journal   = "Phys. Fluids",
     volume    = "18",
     year      = "2006 ",
     pages     = "019101",
}

@Article{A06,
     author    = "P. Attan{\'e} ",
     title     = " Response to Comment on Breakup length of
                forced liquid jets ",
     journal   = "Phys. Fluids",
     volume    = "18",
     year      = "2006 ",
     pages     = "019102",
}

@Article{XBSAA96,
     author    = "J. H. Xing and A. Boguslawsky and A. Soucemarianadin
           and P. Atten and P. Attan{\'e}",
     title     = " Experimental investigation of capillary instability:
                results on jet stimulated by pressure modulations",
     journal   = "Exp. Fluids",
     volume    = "20",
     year      = "1996 ",
     pages     = "302",
}

@Article{BAS97,
     author    = "B. Barbet and P. Atten and A. Soucemarianadin",
     title     = " Two-mode EHD stimulation of a continuous jet:
                generation of drops and satellites",
     journal   = "J. Imaging Sci. Techn.",
     volume    = "41",
     year      = "1997 ",
     pages     = "570",
}

@Article{SS75,
     author    = "A. Sterling and C. Sleicher ",
     title     = " The instability of capillary jets",
     journal   = "J. Fluid Mech.",
     volume    = "68",
     year      = "1975 ",
     pages     = "477",
}

@Article{K90,
     author    = "N. Khamontoff ",
     title     = " ",
     journal   = "Phil. Mag.",
     volume    = "30",
     year      = "1890",
     pages     = "506",
}

@Article{K90-2,
     author    = "N. Khamontoff ",
     title     = "Applications of photography to studying the structure
                   of jets of liquids and powders",
     journal   = "Journal of the Russian Physico-Chemical Society of
                  Saint Petersburg",
     volume    = "22",
     year      = "1890",
     pages     = "281",
}

@Article{K83,
     author    = "J. B. Keller ",
     title     = " ",
     journal   = "Phys. Fluids",
     volume    = "26",
     year      = "1983",
     pages     = "506",
}

@Article{KKT95,
     author    = "J. B.  Keller and A.  King and L. Ting ",
     title     = " ",
     journal   = "Phys. Fluids",
     volume    = "7",
     year      = "1995",
     pages     = "226",
}

@Article{KM83,
     author    = "J. B.  Keller and M. J. Miksis ",
     title     = " ",
     journal   = "SIAM J. Appl. Math.",
     volume    = "43",
     year      = "1983",
     pages     = "268",
}

@Article{HK67,
     author    = "R. A. Handelsman and J. B.  Keller",
     title     = "Axially symmetric potential flow around a slender body ",
     journal   = "J. Fluid Mech.",
     volume    = "28",
     year      = "1967",
     pages     = "131",
}

@Article{Sell99,
     author    = "A. Sellier",
     title     = "Asymptotic solution for the electrostatic field
             around a slender conducting body",
     journal   = "IMA J. Appl. Math.",
     volume    = "62",
     year      = "1999",
     pages     = "167",
}

@Article{HK67b,
     author    = "R. A. Handelsman and J. B.  Keller",
     title     = "The electrostatic field around a slender conducting
                 body of revolution",
     journal   = "SIAM J. Appl. Math.",
     volume    = "15",
     year      = "1967",
     pages     = "824",
}


@Article{M63,
     author    = "J. P. Moran",
     title     = "Line source distribution and slender-body theory",
     journal   = "J. Fluid Mech.",
     volume    = "17",
     year      = "1963",
     pages     = "285",
}

@Article{KRT73,
     author    = "J. B. Keller and S. I.  Rubinov and Y. O. Tu ",
     title     = " ",
     journal   = "Phys. Fluids",
     volume    = "16",
     year      = "1973",
     pages     = "2052",
}

@Article{KKL88,
     author    = "D. A. Kessler and J. Koplik and H. Levine ",
     title     = " ",
     journal   = "Adv. Phys.",
     volume    = "37",
     year      = "1988",
     pages     = "255",
}

@Article{K86,
     author    = "R. Keunings ",
     title     = " ",
     journal   = "J. Comp. Phys.",
     volume    = "62",
     year      = "1986",
     pages     = "199",
}

@Article{KB92,
     author    = "J.  Koplik and J. R. Banavar ",

     journal   = "Science",
     volume    = "257",
     year      = "1992",
     pages     = "1664",
}

@Article{KB93,
     author    = "J.  Koplik and J. R. Banavar ",
     title     = " ",
     journal   = "Phys. Fluids A",
     volume    = "5",
     year      = "1993",
     pages     = "521",
}

@Article{K96,
     author    = "T. A. Kowalewski ",
     title     = " ",
     journal   = "Fluid Dyn. Res.",
     volume    = "17",
     pages     = "121-145",
     year      = "1996",
        }

@Book{L69,
     author    = "O. Ladyzhenskaya ",
     title     = "The Mathematical Theory of Viscous Incompressible Flow",
     year      = "1969",
     publisher = "Gordon \& Breach",
}

@Article{LNSZZ94,
     author    = "B.  Lafaurie and C. Nardone and R. Scardovelli
                 and S. Zaleski and G. Zanetti ",
     title     = " ",
     journal   = "J. Comput. Physics",
     volume    = "113",
     year      = "1994",
     pages     = "134",
}

@Article{La75,
     author    = "P. Lafrance ",
     title     = " ",
     journal   = "Phys. Fluids",
     volume    = "18",
     year      = "1975",
     pages     = "428",
}

@Article{LART74,
     author    = "P. Lafrance and G. Aiello and R. C. Ritter and J. S. Trefil",
     title     = "Drop spectrometry of laminar and turbulent jets ",
     journal   = "Phys. Fluids",
     volume    = "17",
     year      = "1974",
     pages     = "1469",
}

@Article{GM67,
     author    = "J. Gavis and M. Modan",
     title     = "Expansion and contraction of jets of Newtonian
                   liquids in air: the effect of tube length",
     journal   = "Phys. Fluids",
     volume    = "10",
     year      = "1967",
     pages     = "487",
}

@Article{A77,
     author    = "G. Aiello",
     title     = "Effect of velocity profile upon the asymptotic
                contraction ratio of horizontal jets",
     journal   = "Phys. Fluids",
     volume    = "20",
     year      = "1977",
     pages     = "165",
}

@Article{LR77,
     author    = "P. Lafrance and R. C. Ritter",
     title     = " ",
     journal   = "ASME J. Appl. Mech.",
     volume    = "44",
     year      = "1977",
     pages     = "385",
}

@Article{RZS74,
     author    = "R. C. Ritter and N. R. Zinner and A. M. Sterling",
     title     = "Analysis of drop intervals in jets modelling obstruction
                  of the urinary tract",
     journal   = "Phys. Med. Biol.",
     volume    = "19",
     year      = "1974",
     pages     = "161",
}

@Article{RSZ77,
     author    = "R. C. Ritter and A. M. Sterling and N. R. Zinner",
     title     = "Physical information in the external urinary stream
          of the normal and obstructed male",
     journal   = "Brit. J. Urol.",
     volume    = "49",
     year      = "1977",
     pages     = "293",
}

@Book{LL84a,
     author    = "L. D.  Landau and E. M. Lifshitz ",
     title     = "Fluid Mechanics",
     year      = "1984",
     publisher = "Pergamon: Oxford",
}

@Book{Batch67,
     author    = "G. K. Batchelor",
     title     = "An introduction to Fluid Dynamics",
     year      = "1967",
     publisher = {Cambridge University Press, Cambridge},
}

@Book{Acheson,
     author    = "D. J. Acheson",
     title     = "Elementary Fluid Dynamics",
     year      = "1990",
     publisher = {Clarendon Press, Oxford},
}

@Book{Yih69,
     author    = "C.-S. Yih",
     title     = "Fluid Dynamics",
     year      = "1969",
     publisher = {McGraw-Hill, New York},
}

@Book{LL84b,
     author    = "L. D.  Landau and E. M. Lifshitz ",
     title     = "Electrodynamics of M Continuous edia",
     year      = "1984b",
     publisher = "Pergamon: Oxford",
}

@Book{L05,
     author    = "P. S. {de Laplace}",
     title     = "Mechanique Celeste Supplement au X Libre",
     year      = "1805",
     publisher = "Courier: Paris",
}

@Article{L74,
     author    = "H. C. Lee ",
     title     = " ",
     journal   = "IBM J. Res. Develop.",
     volume    = "18",
     year      = "1974",
     pages     = "364",
}

@Article{LG86,
     author    = "S. J.  Leib and M. E. Goldstein ",
     title     = " ",
     journal   = "J. Fluid Mech.",
     volume    = "168",
     year      = "1986",
     pages     = "479",
}

@Article{LG86b,
     author    = "S. J.  Leib and M. E. Goldstein ",
     title     = "Convective and absolute instability of a
                 viscous liquid jet",
     journal   = "Phys. Fluids",
     volume    = "29",
     year      = "1986",
     pages     = "952",
}

@Article{Lenard87,
     author    = "P. Lenard ",
     title     = "Ueber die Schwingungen fallender Tropfen ",
     journal   = "Ann. Phys. Chem.",
     volume    = "30",
     year      = "1887",
     pages     = "209",
}

@Article{L10,
     author    = "P. Lenard ",
     title     = "{\"U}ber die Spannung frischer Wasseroberfl{\"a}chen
             und {\"u}ber die Messung derselben durch schwingende Tropfen",
     journal   = "Sitzungsber. Heidelberger Akad. Wiss.",
     volume    = "18. Abhandlung",
     year      = "1910",
     pages     = "3",
}

@Article{SHK93,
     author    = "B. St{\"u}ckrad and W. J. Hiller and T. A. Kowalwski",
     title     = "Measurement of dynamic surface tension by the oscillating
                   droplet method",
     journal   = "Exp. Fuids",
     volume    = "15",
     year      = "1993",
     pages     = "332",
}

@Article{LHL94,
     author    = "H. Li and T. C.  Halsey and A. Lobkovsky ",
     title     = " ",
     journal   = "Europhys Lett.",
     volume    = "27",
     year      = "1994",
     pages     = "575",
}

@Article{LK87,
     author    = "S. P.  Lin and D. J. Kang ",
     title     = " ",
     journal   = "Phys. Fluids",
     volume    = "30",
     year      = "1987",
     pages     = "2000",
}

@Article{LW94,
     author    = "S. P.  Lin and R. D.  Webb ",
     title     = " ",
     journal   = "Phys. Fluids",
     volume    = "6",
     year      = "1994",
     pages     = "2671",
}

@Article{LS96,
     author    = "J. R.  Lister and H. A. Stone ",
     title     = "Time-dependent viscous deformation of a drop
         in a rapidly rotating fluid ",
     journal   = "J. Fluid Mech.",
     volume    = "317",
     year      = "1996",
     pages     = "275",
}

@Article{LS98,
     author    = "J. R.  Lister and H. A. Stone ",
     title     = "Capillary breakup of a viscous thread surrounded
             by another viscous fluid ",
     journal   = "Phys. Fluids",
     volume    = "10",
     year      = "1998",
     pages     = "2758",
}

@Article{L-HC76,
     author    = "M. S.  Longuet-Higgins and E. D. Cokelet ",
     title     = " ",
     journal   = "Proc. Roy. Soc. London A",
     volume    = "350",
     year      = "1976",
     pages     = "1",
}

@Article{M55,
     author    = "G. Magnus ",
     title     = " ",
     journal   = "Ann. Phys. Chem.",
     volume    = "95",
     year      = "1855",
     pages     = "1",
}

@Article{M59,
     author    = "G. Magnus ",
     title     = " ",
     journal   = "Ann. Phys. Chem.",
     volume    = "106",
     year      = "1859",
     pages     = "1",
}

@Article{M91,
     author    = "A. J. Majda ",
     title     = " ",
     journal   = "SIAM Review",
     volume    = "33",
     year      = "1991",
     pages     = "349",
}

@Article{ML90,
     author    = "N. N.  Mansour and T. S. Lundgren ",
     title     = " ",
     journal   = "Phys Fluids A",
     volume    = "2",
     year      = "1990",
     pages     = "1141",
}

@Book{H71,
     author    = "A. R. Manwell ",
     title     = "The Hodograph Equations",
     year      = "1971",
     publisher = "Hafner",
}

@Article{MS72,
     author    = "M. P.  Markova and V. Ya. Shkadov",
     title     = " ",
     journal   = "Izw. Akad. Nauk SSSR Mekh. Zhid. Gaza",
     volume    = "3",
     year      = "1972",
     pages     = "30",
}

@Article{Marschall85,
     author    = "E. Marschall ",
     title     = " ",
     journal   = "Ver. Deutscher Ingen. Forschungsheft",
     volume    = "632",
     year      = "1985",
     pages     = "13",
}

@Article{MP69,
     author    = " M. A. Matovitch and J. R. A. Pearson ",
     title     = " ",
     journal   = "Ind. Eng. Chem. Fundamentals",
     volume    = "8",
     year      = "1969",
     pages     = "512",
}

@Article{M75,
     author    = "J. C. Maxwell ",
     title     = "Encyclopedia Britannica",
     year      = "1875",
     edition   = "9th edition",
}

@Article{MM74,
     author    = "M. J.  Mc Carthy and N. A. Malloy ",
     title     = " ",
     journal   = "Chem. Engng. J.",
     volume    = "7",
     year      = "1974",
     pages     = "1",
}

@Article{M92,
     author    = "F. Merle ",
     title     = " ",
     journal   = "Comm. Pure Appl. Math.",
     volume    = "55",
     year      = "1992",
     pages     = "203",
}

@Article{Ishiguro,
     author    = "R. Ishiguro and F. Graner and E. Rolley and S.
               Balibar",
     title     = "Coalescence of Crystalline Drops ",
     journal   = "Phys. Rev. Lett.",
     volume    = "93",
     year      = "2004",
     pages     = "235301",
}

@Article{SCB07,
     author    = "S. Sasaki and F. Caupin and S. Balibar",
     title     = "Wetting properties of grain boundaries in solid He-4",
     journal   = "Phys. Rev. Lett.",
     volume    = "99",
     year      = "2007",
     pages     = "205302",
}

@Article{AV97,
     author    = "S. B. Angenent and J. J. L. Vel{\'a}zquez",
     title     = "Degenerate neckpinches in mean curvature flow",
     journal   = "J. reine angew. Math.",
     volume    = "482",
     year      = "1997",
     pages     = "15",
}

@Article{BCG98,
     author    = "C. J. Budd and G. J. Collins and V. A. Galaktionov",
     title     = "An asymptotic and numerical description of self-similar
               blow-up in quasilinear parabolic equations",
     journal   = "J. Comp. Appl. Math.",
     volume    = "97",
     year      = "1998",
     pages     = "51",
}

@Article{BKL94,
     author    = "J. Bricmont and A. Kupiainen and G. Lin",
     title     = "Renormalization group and asymptotics of
                solutions of nonlinear parabolic equations ",
     journal   = "Comm. Pure Appl. Math.",
     volume    = "47",
     year      = "1994",
     pages     = "893",
}

@Article{CDGK04,
     author    = "L. Chen and P. G. Debenedetti and
         C. W. Gear and I. G. Kevrekidis",
     title     = "From molecular dynamics to coarse self-similar
      solutions: a simple example using equation-free computation",
     journal   = "J. Non-Newtonian Fluid Mech.",
     volume    = "120",
     year      = "2004",
     pages     = "215",
}

@Book{Goldenfeld93,
     author    = "N. Goldenfeld",
     title     = "Lectures on phase transitions and the
              renormalization group",
     publisher = "Addison-Wesley",
     year      = "1993",
}

@Article{MM04,
     author    = "H. Matano and F. Merle",
     title     = " ",
     journal   = "Comm. Pure Appl. Math.",
     volume    = "57",
     year      = "2004",
     pages     = "1494",
}

@Article{M83,
     author    = "J. Meseguer ",
     title     = " ",
     journal   = "J. Fluid Mech.",
     volume    = "130",
     year      = "1983",
     pages     = "122",
}

@Article{MS85,
     author    = "J.  Meseguer and A. Sanz ",
     title     = " ",
     journal   = "J. Fluid Mech.",

     year      = "1985",
     pages     = "83",
}

@Article{MSL86,
     author    = "J. Meseguer and A.  Sanz and J. Lopez ",
     title     = " ",
     journal   = "J. Christal Growth",
     volume    = "78",
     year      = "1986",
     pages     = "325",
}

@Article{M94,
     author    = "A. J. Mestel ",
     title     = " ",
     journal   = "J. Fluid Mech.",
     volume    = "274",
     year      = "1994",
     pages     = "93",
}

@Article{MW76,
     author    = "D. H.  Michael and P. G. Williams ",
     title     = " ",
     journal   = "Proc. R. Soc. London Ser. A",
     volume    = "351",
     year      = "1976",
     pages     = "117",
}

@Article{M81,
     author    = "M. J. Miksis ",
     title     = " ",
     journal   = "Phys. Fluids",
     volume    = "24",
     year      = "1981",
     pages     = "1967",
}

@misc{M95,
     author    = "H. K. Moffatt ",
     year      = "1995",
     howpublished = "private communication"
}

@misc{suppl_riv,
     howpublished = "EPAPS Document No"
}

@Article{Moore83,
     author    = "D. W. Moore ",
     title     = " ",
     journal   = "IMA J. Appl. Math.",
     volume    = "31",
     year      = "1983",
     pages     = "1",
}

@Article{K89,
     author    = "T. Kambe ",
     title     = "Spiral vortex solution of Birkhoff-Rott equation ",
     journal   = "Physica D",
     volume    = "37",
     year      = "1989",
     pages     = "463",
}

@Article{MG85,
     author    = "A.  M{\"u}ller and S. Grossmann ",
     title     = " ",
     journal   = "Z. Naturforsch.",
     volume    = "40",
     year      = "1985",
     pages     = "968",
}

@Article{N70,
     author    = "A. H. Nayfeh ",
     title     = " ",
     journal   = "Phys. Fluids",
     volume    = "14",
     year      = "1970",
     pages     = "841",
}

@Article{NJT96,
     author    = "M. R.  Nobari and Y-J. Jan and G. Tryggvason ",
     title     = " ",
     journal   = "Phys Fluids",
     volume    = "8",
     year      = "1996",
     pages     = "29",
}

@Article{OP90,
     author    = "H. N. O{\~g}uz and A. Prosperetti ",
     title     = " ",
     journal   = "J. Fluid Mech.",
     volume    = "219",
     year      = "1990",
     pages     = "143",
}

@Article{O36,
     author    = "W. {v. Ohnesorge}",
     title     = " Die Bildung von Tropfen an D{\"u}sen und die
            Aufl{\"o}sung fl{\"u}ssiger Strahlen",
     journal   = "ZAMM",
     volume    = "16",
     year      = "1936",
     pages     = "355",
}

@Article{ON88,
     author    = "P. J.  Olver and Y. Nutku ",
     title     = " ",
     journal   = "J. Math. Phys.",
     volume    = "29",
     year      = "1988",
     pages     = "1610",
}

@Article{PGB94,
     author    = "C. Pantano and A. M. Ga{\~n}{\'a}n-Calvo and A. Barrero",
     title     = "Zeroth order, electrohydrostatic solution for
        electrospraying in cone-jet mode",
     journal   = "J. Aerosol Sci.",
     volume    = "25",
     year      = "1994",
     pages     = "1065",
}

@Article{P95,
     author    = "D. T. Papageorgiou ",
     title     = "On the breakup of viscous liquid threads ",
     journal   = "Phys. Fluids",
     volume    = "7",
     year      = "1995",
     pages     = "1529",
}

@Article{Papa95,
     author    = "D. T. Papageorgiou ",
     title     = " Analytical description of the breakup of liquid jets",
     journal   = "J. Fluid Mech.",
     volume    = "301",
     year      = "1995",
     pages     = "109",
}

@Article{PM69,
     author    = "J. R. A.  Pearson and M. A. Matovitch ",
     title     = " ",
     journal   = "Ind. Eng. Chem. Fundamentals",
     volume    = "8",
     year      = "1969",
     pages     = "605",
}

@Article{PTM92,
     author    = "N. A.  Pelekasis and J. A. Tsamopoulos and G. D. Manolis ",
     title     = " ",
     journal   = "J. Comp. Phys.",
     volume    = "101",
     year      = "1992",
     pages     = "231",
}

@Article{PM92,
     author    = "J. M.  Perales and J. Meseguer ",
     title     = " ",
     journal   = "Phys. Fluids",
     volume    = "4",
     year      = "1992",
     pages     = "1110",
}

@Article{PSS90,
     author    = "D. H. Peregrine and G. Shoker and A. Symon ",
     title     = "The bifurcation of liquid bridges ",
     journal   = "J. Fluid Mech.",
     volume    = "212",
     year      = "1990",
     pages     = "25 ",
}

@Article{P81,
     author    = "D. H. Peregrine",
     title     = "The fascination of fluid mechanics ",
     journal   = "J. Fluid Mech.",
     volume    = "106",
     year      = "1981",
     pages     = "59 ",
}

@Book{P72,
     author    = "D. H. Peregrine ",
     title     = " ",
     journal   = "Waves on Beaches",
     editor    = "R. E. Meyer ",
     year      = "1972",
     pages     = "95",
     publisher = "Academic",
}

@Article{P76,
     author    = "W. T. Pimbley ",
     title     = " ",
     journal   = "IBM J. Res. Develop.",
     volume    = "20",
     year      = "1976",
     pages     = "148",
}

@Article{PL77,
     author    = "W. T.  Pimbley and H. C. Lee ",
     title     = " ",
     journal   = "IBM J. Res. Develop.",
     volume    = "21",
     year      = "1977",
     pages     = "21",
}

@Article{P43,
     author    = "J. A. F. Plateau ",
     title     = "M{\'e}moire sure les ph{\'e}nom{\`e}nes que
                  pr{\'e}sente une masse liquide libre
                 et soustraite a l'action de la pesanteur, 1st series",
     journal   = "Acad. Sci. Bruxelles Mem.",
     volume    = "16",
     year      = "1843",
     pages     = "3",
}

@Article{P49,
     author    = "J. A. F. Plateau ",
     title     = "Recherches exp{\'e}rimental et th{\'e}orique
                 sur les figures d'{\'e}quilibre d'une masse
               liquide sans pesanteur, 2nd series",
     journal   = "Acad. Sci. Bruxelles Mem.",
     volume    = "23",
     year      = "1849",
     pages     = "5",
}

@Article{P57,
     author    = "J. A. F. Plateau ",
     title     = "Recherches exp{\'e}rimental et th{\'e}orique
                 sur les figures d'{\'e}quilibre d'une masse
               liquide sans pesanteur, 3d series",
     journal   = "Acad. Sci. Bruxelles Mem.",
     volume    = "29",
     year      = "1857",
     pages     = "3",
}

@Article{P58,
     author    = "J. A. F. Plateau ",
     title     = "Recherches exp{\'e}rimental et th{\'e}orique
                 sur les figures d'{\'e}quilibre d'une masse
               liquide sans pesanteur, 4th series",
     journal   = "Acad. Sci. Bruxelles Mem.",
     volume    = "31",
     year      = "1859",
     pages     = "3",
}

@Book{P73,
     author    = "J. A. F. Plateau ",
     title     = "Statique exp{\'e}rimentale
      et theorique des liquides soumis aux seules forces mol{\'e}culaires ",
     volume    = "2 ",
     year      = "1873",
     pages     = "319",
     publisher = "Gauthier Villars: Paris",
}

@Article{P94,
     author    = "Y. Pomeau ",
     title     = " ",
     journal   = "C. R. Acad. Sci. Paris",
     volume    = "318",
     year      = "1994",
     pages     = "865",
}

@Book{PYVF92,
     author    = "W. H.  Press and S. A. Teukolski and
             W. T.  Vetterling and B. P. Flannery ",
     title     = "Numerical Recipes",
     publisher = {Cambridge University Press, Cambridge},
     year      = "1992",
}

@Article{LF82,
     author    = "R. A. London and B. P. Flannery ",
     title     = "Hydrodynamics of x-ray induced stallar winds",
     journal   = "Astrophys. J.",
     volume    = "258",
     year      = "1982",
     pages     = "260"
}

@Article{PS92,
     author    = "A.  Pumir and E. D. Siggia ",
     title     = "Development of singular solutions to the axisymmtric
                  Euler equations",
     journal   = "Phys. Fluids A",
     volume    = "4",
     year      = "1992",
     pages     = "1472",
}

@Article{PS92b,
     author    = "A.  Pumir and E. D. Siggia ",
     title     = "Finite-time singularities in the axisymmetric
                   three-dimensional Euler equations",
     journal   = "Phys. Rev. Lett.",
     volume    = "68",
     year      = "1992",
     pages     = "1511",
}

@Article{PS87,
     author    = "A.  Pumir and E. D. Siggia ",
     title     = "Vortex dynamics and the existence of solutions to the
                Navier-Stokes equations",
     journal   = "Phys. Fluids",
     volume    = "30",
     year      = "1987",
     pages     = "1606",
}

@Article{PSS92,
     author    = "A.  Pumir and B. I. Shraiman and E. D. Siggia",
     title     = "Vortex morphology and Kelvin's theorem",
     journal   = "Phys. Rev. A",
     volume    = "45",
     year      = "1992",
     pages     = "R5351",
}

@Article{ES94,
     author    = "W. E and C.-W. Shu",
     title     = "Small-scale structures in Boussinesq convection",
     journal   = "Phys. Fluids",
     volume    = "6",
     year      = "1994",
     pages     = "49",
}

@Article{QSTC86,
     author    = " S. X.  Quian and J. B. Snow and
          H. M.  Tzeng and R. K. Chang ",
     title     = " ",
     journal   = "Science",
     volume    = "2341",
     year      = "1986",
     pages     = "486",
}

@Article{RA78,
     author    = "J. M.  Rallison and A. Acrivos ",
     title     = "A numerical study of the deformation and burst of a
           viscous drop in an extensional flow ",
     journal   = "J. Fluid Mech.",
     volume    = "89",
     year      = "1978",
     pages     = "191",
}

@Article{R84,
     author    = "J. M. Rallison ",
     title     = "The deformation of small viscous drops and bubbles
                           in shear flows ",
     journal   = "Annu. Rev. Fluid Mech.",
     volume    = "16",
     year      = "1984",
     pages     = "45",
}

@Article{R93,
     author    = "N. A. Razumovski ",
     title     = " ",
     journal   = "Zh. Tekh. Fiz [Technical Physics {\bf 38} 752 (1993)]",
     volume    = "63",
     year      = "1993",
     pages     = "26",
}

@Article{R79a,
     author    = "Lord Rayleigh",
     title     = "On the instability of jets ",
     journal   = "Proc. Roy. Soc. London",
     volume    = "10",
     year      = "1879",
     pages     = "4",
}

@Article{R79b,
     author    = "Lord Rayleigh",
     title     = "On the capillary phenomenon of jets ",
     journal   = "Proc. Roy. Soc. London",
     volume    = "29",
     year      = "1879",
     pages     = "94",
}

@Article{Ray82,
     author    = "Lord Rayleigh",
     title     = "Further observations upon liquid jets, in continuation
                 of those recorded in the Royal Society's 'Proceedings'
                   for March and May, 1879 ",
     journal   = "Proc. Roy. Soc. London",
     volume    = "1882",
     year      = "34",
     pages     = "130",
}

@Article{R90,
     author    = "Lord Rayleigh",
     title     = "On the tension of recently formed liquid surfaces ",
     journal   = "Proc. Roy. Soc. London",
     volume    = "47",
     year      = "1890 ",
     pages     = "281",
}

@Article{BKNT02,
     author    = "S. E. Bechtel and K. W. Koelling and W. Nguyen and G. Tan",
     title     = "A new technique for the measurement of the dynamic
               evolution of surface tension",
     journal   = "J. Colloid Interf. Sci.",
     volume    = "245",
     year      = "2002 ",
     pages     = "142",
}

@Article{KNR74,
     author    = "N. N. Kochurova and B. A. Noskov and A. I. Rusanov",
     title     = "Taking account of the velocity profile in determining
                  surface tension by the method of an oscillating jet",
     journal   = "Kolloid Zh.",
     volume    = "36",
     year      = "1974 ",
     pages     = "559",
}

@Article{KR81,
     author    = "N. N. Kochurova and A. I. Rusanov",
     title     = "Dynamic surface properties of water: surface tension
                  and surface potential",
     journal   = "J. Colloid Interf. Sci.",
     volume    = "81",
     year      = "1981 ",
     pages     = "297",
}

@Article{R96,
     author    = "Lord Rayleigh",
     title     = "Phil. Mag.",
     journal   = " ",
     volume    = "34",
     year      = "1896",
     pages     = "145",
}

@Book{Ray78,
     author    = "Lord Rayleigh",
     title     = "The Theory of Sound, Vol 2",
     publisher = "Macmillan, reprinted 1945 Dover",
     year      = "1978",
     pages     = "351",
}

@Article{R99,
     author    = "Lord Rayleigh",
     title     = "Investigation in capillarity ",
     journal   = "Phil. Mag.",
     volume    = "48",
     year      = "1899",
     pages     = "321",
}

@Article{RH91,
     author    = "H.  Rehage and H. Hoffmann ",
     title     = " ",
     journal   = "Molecular Physics",
     volume    = "74",
     year      = "1991 ",
     pages     = "933",
}

@Article{R82,
     author    = "M. Renardy ",
     title     = " ",
     journal   = "SIAM J. Math. Anal.",
     volume    = "13",
     year      = "1982",
     pages     = "226",
}

@Article{R94,
     author    = "M. Renardy ",
     title     = " ",
     journal   = "Non-Newtonian Fluid Mech.",
     volume    = "51",
     year      = "1994",
     pages     = "97",
}

@Article{R95,
     author    = "M. Renardy ",
     title     = " ",
     journal   = "Non-Newtonian Fluid Mech.",
     volume    = "59",
     year      = "1995",
     pages     = "267",
}

@Article{R05,
     author    = "M. Renardy ",
     title     = " ",
     journal   = "IMA J. App. Math.",
     volume    = "70",
     year      = "2005",
     pages     = "353",
}

@Article{Ren02,
     author    = "M. Renardy ",
     title     = "Similarity solutions for jet break-up for various models
                  of viscoelastic fluids",
     journal   = "J. Non-Newtonian Fluid Mech.",
     volume    = "104",
     year      = "2002",
     pages     = "65",
}

@Article{RL02,
     author    = "M. Renardy and D. Losh",
     title     = "Similarity solutions for jet breakup in a Giesekus
                  fluid with inertia",
     journal   = "J. Non-Newtonian Fluid Mech.",
     volume    = "106",
     year      = "2002",
     pages     = "17",
}

@Article{RR04,
     author    = "M. Renardy and Y. Renardy",
     title     = "Similarity solutions for breakup of jets of
                  power law fluids",
     journal   = "J. Non-Newtonian Fluid Mech.",
     volume    = "122",
     year      = "2004",
     pages     = "303",
}

@Article{MR85,
     author    = "P. Markovich and M. Renardy ",
     title     = " ",
     journal   = "J. Non-Newtonian Fluid Mech.",
     volume    = "17",
     year      = "1985",
     pages     = "13",
}

@Article{R86,
     author    = "O. Reynolds ",
     title     = "On the Theory of Lubrication and its Application to Mr.
    Beauchamp Tower's Experiments, Including an Experimental
   Determination of the Viscosity of Olive Oil",
     journal   = "Phil. Trans. Roy. Soc.",
     volume    = "177",
     year      = "1886",
     pages     = "157-234",
}

@Article{RLB94,
     author    = "J. R  Richards and A. M.  Lenhoff and A. N.  Beris ",
     title     = " ",
     journal   = "Phys. Fluids",
     volume    = "6",
     year      = "1994",
     pages     = "2640",
}

@Article{RRR03,
     author    = "A.  Rothert and R.  Richter and I. Rehberg ",
     title     = " Formation of a drop: viscosity dependance of
                         three flow regimes ",
     journal   = "New J. Phys.",
     volume    = "5",
     year      = "2003",
     pages     = "59",
}

@Article{RJ70,
     author    = "D. F.  Rutland and G. J.  Jameson ",
     title     = " ",
     journal   = "Chem. Eng. Sci.",
     volume    = "25",
     year      = "1970",
     pages     = "1689",
}

@Article{H60,
     author    = "L. M. Hocking",
     title     = "The stability of a rigidly rotating column of liquid ",
     journal   = "Mathematika",
     volume    = "7",
     year      = "1960",
     pages     = "1",
}

@Article{GK61,
     author    = "J. Gillis and B. Kaufman",
     title     = "The stability of rotating viscous jet ",
     journal   = "Q. J. appl. Math.",
     volume    = "19",
     year      = "1961",
     pages     = "301",
}

@Article{P67,
     author    = "T. J. Pedley",
     title     = "The stability of rotating flows with a cylindrical
                 free surface",
     journal   = "J. Fluid Mech.",
     volume    = "30",
     year      = "1967",
     pages     = "127",
}

@Article{RJ71,
     author    = "D. F.  Rutland and G. J. Jameson ",
     title     = " ",
     journal   = "J. Fluid Mech.",
     volume    = "46",
     year      = "1971",
     pages     = "267",
}

@misc{EB06,
     author    = "J. Eggers and D. Bonn",
     year      = "2006",
     pages     = "unpublished",
}

@Inproceedings{EB99,
     author    = "J. Eggers and M. P. Brenner",
     title     = " Spinning jets ",
     year      = "1999",
     booktitle = "Proceedings of the IUTAM Symposium on
      Nonlinear Waves in Multi-Phase Flow",
     editor    = "H.-C. Chang",
     pages     = "185",
     publisher = "Kluwer",
}

@Article{SZ99,
     author    = "A. Scardiovelli and S. Zaleski ",
     title     = " Direct numerical simulation of free-surface and
                       interfacial flow",
     journal   = "Annu. Rev. Fluid Mech.",
     volume    = "31",
     year      = "1999",
     pages     = "567",
}

@Article{SLHC67,
     author    = "J. M.  Schneider and N. R.  Lindblatt and
         C. D.  {Hendricks Jr} and and J. M. Crowley ",
     title     = " ",
     journal   = "J. Appl. Phys.",
     volume    = "38",
     year      = "1967",
     pages     = "2599",
}

@Article{S93,
     author    = "R. M. S. M. Schulkes ",
     title     = " ",
     journal   = "Phys. Fluids A",
     volume    = "5",
     year      = "1993",
     pages     = "2121",
}

@Article{S94a,
     author    = "R. M. S. M. Schulkes ",
     title     = "The evolution of capillary fountains ",
     journal   = "J. Fluid Mech.",
     volume    = "261",
     year      = "1994a",
     pages     = "223",
}

@Article{S94b,
     author    = "R. M. S. M. Schulkes ",
     title     = "The evolution and bifurcation of a pendant drop ",
     journal   = "J. Fluid Mech.",
     volume    = "278",
     year      = "1994b",
     pages     = "83",
}

@Article{SD82,
     author    = "W. W.  Schultz and S. H.  Davis ",
     title     = " ",
     journal   = "J. Rheol",
     volume    = "26",
     year      = "1982",
     pages     = "331",
}

@Article{S46,
     author    = "L. I. Sedov ",
     title     = " ",
     journal   = "Prikl. Mat. Mekh.",
     volume    = "10",
     year      = "1946",
     pages     = "241",
}

@Article{S81,
     author    = "J. D.  Sherwood ",
     title     = " Spindle-shaped drops in a viscous extensional flow",
     journal   = "Math. Proc. Camb. Phil. Soc.",
     volume    = "90",
     year      = "1981",
     pages     = "529",
}

@Article{S84,
     author    = "J.  D. Sherwood ",
     title     = "Tip streaming from slender drops in a nonlinear
               extensional flow",
     journal   = "J. Fluid Mech.",
     volume    = "144",
     year      = "1984",
     pages     = "281",
}

@Article{SBN94,
     author    = "X. D.  Shi and M. P.  Brenner and S. R. Nagel ",
     title     = " ",
     journal   = "Science",
     volume    = "265",
     year      = "1994",
     pages     = "157",
}

@Article{CN07,
     author    = "S. C. Case and S. R. Nagel",
     title     = " Spout States in the Selective Withdrawal of
   Immiscible Fluids through a Nozzle Suspended above a Two-Fluid Interface",
     journal   = "Phys. Rev. Lett.",
     volume    = "98",
     year      = "2007",
     pages     = "114501",
}

@Article{TBT86,
     author    = "T. W.  Shield and D. B.  Bogy and F. E.  Talke ",
     title     = " ",
     journal   = "J. Comput. Phys.",
     volume    = "67",
     year      = "1986",
     pages     = "327",
}

@Article{SDK91,
     author    = "R. W. G.  Shipman and M. M.  Denn and R. Keunings ",
     title     = " ",
     journal   = "J. Non-Newtonian Fluid Mech.",
     volume    = "40",
     year      = "1991",
     pages     = "281",
}

@Article{SE87,
     author    = "F.  Shokoohi and H. G.  Elrod ",
     title     = " ",
     journal   = "J. Comput. Phys.",
     volume    = "71",
     year      = "1987",
     pages     = "324",
}

@Article{SE90,
     author    = "F.  Shokoohi and H. G.  Elrod ",
     title     = " ",
     journal   = "J. Comput. Phys.",
     volume    = "89",
     year      = "1990",
     pages     = "483",
}

 @Article{SL03,
     author    = "A.  Sierou and J. R.  Lister ",
     title     = "Self-similar solutions for viscous capillary pinch-off ",
     journal   = "J. Fluid Mech.",
     volume    = "497",
     year      = "2003",
     pages     = "381"
}

 @Article{SL04,
     author    = "A.  Sierou and J. R.  Lister ",
     title     = "Self-similar recoil of inviscid drops",
     journal   = "Phys. Fluids",
     volume    = "16",
     year      = "2004",
     pages     = "1379"
}

@Article{SHH95,
     author    = "C. A.  Spangler and J. H.  Hilbing and S. D. Heister ",
     title     = " ",
     journal   = "Phys. Fluids",
     volume    = "7",
     year      = "1995",
     pages     = "964",
}
@Article{HH96,
     author    = "J. H. Hilbing and S. D. Heister ",
     title     = "Droplet size control in liquid breakup ",
     journal   = "Phys. Fluids",
     volume    = "8",
     year      = "1996",
     pages     = "1574",
}

@Article{SAM96,
     author    = "S. H. Spiegelberg and D. C.  Ables and  G. H. McKinley",
     title     = " ",
     journal   = "J. Non-Newtonian Fluid Mech.",
     volume    = "64",
     year      = "1996",
     pages     = "229",
}

@Article{SM96,
     author    = "S. H. Spiegelberg and G. H.  McKinley ",
     title     = " ",
     journal   = "Non-Newtonian Fluid Mech.",
     volume    = "67",
     year      = "1996",
     pages     = "49",
}

@Article{STNG91,
     author    = "T. S. Sridhar and V. Tirtaatmadja
              and D. A.  Nguyen and R. K. Gupta ",
     title     = " ",
     journal   = "J. Non-Newtonian Fluid Mech.",
     volume    = "40",
     year      = "1991",
     pages     = "271",
}

@Article{SBL86,
     author    = "H. A. Stone and B. J.  Bentley and L. G. Leal ",
     title     = " ",
     journal   = "J. Fluid Mech.",
     volume    = "173",
     year      = "1986",
     pages     = "131",
}

@Article{SL89a,
     author    = "H. A.  Stone and L. G. Leal ",
     title     = " ",
     journal   = "J. Fluid Mech.",
     volume    = "198",
     year      = "1989a ",
     pages     = "399",
}

@Article{SL89b,
     author    = "H. A.  Stone and L. G. Leal ",
     title     = " ",
     journal   = "J. Fluid Mech.",
     volume    = "206",
     year      = "1989b ",
     pages     = "223",
}

@Article{SB96,
     author    = "H. A.  Stone and M. P.  Brenner ",
     title     = " ",
     journal   = "J. Fluid Mech.",
     volume    = "318",
     year      = "1996",
     pages     = "373",
}

@Article{T64,
     author    = "T. Tate ",
     title     = " ",
     journal   = "Phil. Mag",
     volume    = "27",
     year      = "1864",
     pages     = "176",
}

@Article{Taub76,
     author    = "H. H. Taub ",
     title     = " ",
     journal   = "Phys. Fluids",
     volume    = "19",
     year      = "1976",
     pages     = "1124",
}

@Article{T32,
     author    = "G. I. Taylor ",
     title     = " ",
     journal   = "Proc. Roy. Soc. London A",
     volume    = "138",
     year      = "1932",
     pages     = "41",
}

@Article{T64a,
     author    = "G. I. Taylor ",
     title     = " ",
     journal   = "Proc. Roy. Soc. London A",
     volume    = "280",
     year      = "1964",
     pages     = "383",
}

@Article{T69,
     author    = "G. I. Taylor ",
     title     = " ",
     journal   = "Proc. Roy. Soc. London A",
     volume    = "313",
     year      = "1969",
     pages     = "453",
}

@Article{TK90,
     author    = "L.  Ting and J. B. Keller ",
     title     = " Slender jets and thin sheets with surface tension",
     journal   = "SIAM J. Appl. Math.",
     volume    = "50",
     year      = "1990",
     pages     = "1533",
}

@Article{TO91,
     author    = "M.  Tjahjadi and J. M. Ottino ",
     title     = " ",
     journal   = "J. Fluid Mech.",
     volume    = "232",
     year      = "1991",
     pages     = "191",
}

@Article{TSO92,
     author    = "M.  Tjahjadi and H. A.  Stone and J. M. Ottino ",
     title     = " ",
     journal   = "J. Fluid Mech.",
     volume    = "243",
     year      = "1992 ",
     pages     = "297",
}

@Article{T88,
     author    = "P. A. Torpey ",
     title     = " ",
     journal   = "Phys. Fluids A ",
     volume    = "1",
     year      = "1988",
     pages     = "661",
}

@Article{TY96,
     author    = "W.-T. Tsai and D. K. P. Yue ",
     title     = " ",
     journal   = "Annu. Rev. Fluid Mech.",
     volume    = "28",
     year      = "1996",
     pages     = "249",
}

@Article{TY93,
     author    = "A. V.  Tur and V. V. Yanovsky ",
     title     = " ",
     journal   = "J. Fluid Mech.",
     volume    = "248",
     year      = "1993",
     pages     = "67",
}

@Article{VSCWR03,
     author    = "N. Vaago and A. Spiegel and P. Couty and
                 F. R.  Wagner and B. Richerzhagen ",
     title     = " ",
     journal   = "Exp. Fluids",
     volume    = "35",
     year      = "2003",
     pages     = "303",
}

@Article{V75,
     author    = "M. {Van Dyke} ",
     title     = " ",
     journal   = "Perturbation Methods in Fluid Mechanics",
     volume    = "sec edition Parabolic",
     year      = "1975",
}

@Article{VA91,
     author    = "P. Vassallo and N. Ashgriz ",
     title     = " ",
     journal   = "Proc. Roy. Soc. London A",
     volume    = "433",
     year      = "1991",
     pages     = "269",
}

@Article{WABE05,
     author    = "C. Wagner and Y. Amarouchene and D. Bonn and J. Eggers ",
     title     = "Droplet detachment and satellite bead formation in
                visco-elastic fluids ",
     journal   = "Phys. Rev. Lett.",
     volume    = "95",
     year      = "2005",
     pages     = "164504"
}

@Article{SWE08,
     author    = "R. Sattler and C. Wagner and J. Eggers",
     title     = "Blistering pattern and formation of nanofibers in
              capillary thinning of polymer solutions",
     journal   = "Phys. Rev. Lett.",
     volume    = "100",
     year      = "2008",
     pages     = "164502"
}

@Article{W68,
     author    = "D. P. Wang ",
     title     = " ",
     journal   = "J. Fluid Mech.",
     volume    = "34",
     year      = "1968",
     pages     = "299",
}

@Book{W78,
     author    = "R. C.  Weast (ed)",
     title     = "Handbook of Chemistry and Physics",
     publisher = "CRC Press",
     year      = "1978"
}

@Book{Arnold84,
     author    = "V. I. Arnold",
     title     = "Catastrophe Theory",
     publisher = "Springer",
     year      = "1984"
}

@Book{Arnold90,
     author    = "V. I. Arnold",
     title     = "Huygens \& Barrow, Newton \& Hooke",
     publisher = "Birkh{\"a}user",
     year      = "1990"
}

@Book{PS78,
     author    = "T. Poston and I. Stewart",
     title     = "Catastrophe Theory and Its Applications",
     publisher = "Dover Publications, Mineola",
     year      = "1978"
}

@Article{W31,
     author    = "C. Weber ",
     title     = " ",
     journal   = "ZAMM",
     volume    = "11",
     year      = "1931",
     pages     = "136",
}

@Article{W88,
     author    = "S. D. R. Wilson ",
     title     = "The slow dripping of a viscous fluid",
     journal   = "J. Fluid Mech.",
     volume    = "190",
     year      = "1988",
     pages     = "561",
}

@Article{AW05,
     author    = "M. A. M. {Al Khatib} and S. D. R. Wilson ",
     title     = "Slow dripping of yield-stress fluids",
     journal   = "J. Fluids Ingen.",
     volume    = "127",
     year      = "2005",
     pages     = "687",
}

@Article{WJ83,
     author    = "S. D. R. Wilson and A. F. Jones",
     title     = "The entry of a falling film into a pool and the
          air-entrainment. problem",
     journal   = "J. Fluid Mech.",
     volume    = "128",
     year      = "1983",
     pages     = "219",
}

@Article{Jones78,
     author    = "A. F. Jones and S. D. R. Wilson",
     title     = "The film drainage problem in droplet coalescence",
     journal   = "J. Fluid Mech.",
     volume    = "87",
     year      = "1978",
     pages     = "263",
}

@Article{Lister06,
     author    = "J. R. Lister and N. F. Morrison and J. M. Rallison",
     title     = "Sedimentation of a two-dimensional drop towards a
             rigid horizontal plane",
     journal   = "J. Fluid Mech.",
     volume    = "552",
     year      = "2006",
     pages     = "345",
}

@Article{Lister08,
     author    = "J. R. Lister and A. B. Thompson and A. Perriot and L.
                  Duchemin",
     title     = "Shape and stability of axisymmetric levitated viscous drops",
     journal   = "J. Fluid Mech.",
     volume    = "617",
     year      = "2008",
     pages     = "167",
}

@Article{ACDS07,
     author    = "C. Almarcha and P. Clavin and L. Duchemin and J. Sanz",
     title     = "Ablative Rayleigh-Taylor instability with strong
        temperature dependence of the thermal conductivity",
     journal   = "J. Fluid Mech.",
     volume    = "579",
     year      = "2007",
     pages     = "481",
}

@Article{CG05,
     author    = "P. Coussot and F. Gaulard",
     title     = "Gravity flow instability of viscoplastic materials:
                the ketchup drip",
     journal   = "Phys. Rev. E",
     volume    = "72",
     year      = "2005",
     pages     = "031409",
}

@Article{ST04,
     author    = "Y. M. Stokes and E. O. Tuck",
     title     = " ",
     journal   = "J. FLuid Mech.",
     volume    = "498",
     year      = "2004",
     pages     = "205",
}

@Article{LMW02,
     author    = "E. W. Llewellin and H. M. Marder and S. D. R. Wilson ",
     title     = " ",
     journal   = "Proc. Roy. Soc. London A",
     volume    = "458",
     year      = "2002",
     pages     = "987",
}

@Article{Llewellinetal02,
     author    = "E. W. Llewellin and H. M. Mader and S. D. R. Wilson ",
     title     = "The constitutive equation and flow dynamics
                          of bubbly magmas",
     journal   = "Geophys. Res. Lett.",
     volume    = "29",
     year      = "2002",
     pages     = "23",
}

@Article{W81,
     author    = "A. M. Worthington ",
     title     = " ",
     journal   = "Proc. Roy. Soc. London",
     volume    = "32",
     year      = "1881",
     pages     = "362",
}

@Book{L84,
     author    = "K. J. Lissant",
     title     = "Emulsions and Emulsion Technology",
     publisher = "Marcel Dekker",
     year      = "1984"
}

@Article{Kemp98,
     author    = "M. Kemp",
     title     = "Stilled splashes ",
     journal   = "Nature",
     volume    = "396",
     year      = "1998",
     pages     = "633",
}

@Book{W08,
     author    = "A. M. Worthington ",
     title     = "A Study of Splashes",
     publisher = "Longmans: London",
     year      = "1908"
}

@Article{Y92,
     author    = "H. Q. Yang ",
     title     = " ",
     journal   = "Phys. Fluids A",
     volume    = "4",
     year      = "1992",
     pages     = "681",
}

@Book{Y93,
     author    = "A. L. Yarin ",
     title     = "Free liquid jets and films: Hydrodynamics and rheology",
     publisher = "Wiley: New York",
     year      = "1993"
}

@Book{Freund,
     author    = " L. B. Freund ",
     title     = "Dynamic Fracture Mechanics",
     publisher = "Cambridge",
     year      = "1998"
}

@Article{YW95,
     author    = "A. L.  Yarin and D. A. Weiss ",
     title     = " ",
     journal   = "J. Fluid Mech.",
     volume    = "283",
     year      = "1995",
     pages     = "141",
}

@Article{WY99,
     author    = "D. A. Weiss and A. L.  Yarin",
     title     = "Single drop impact onto liquid films: neck distortion,
                 jetting, tiny bubble entrainment, and crown formation ",
     journal   = "J. Fluid Mech.",
     volume    = "385",
     year      = "1999",
     pages     = "229",
}

@Article{MST95,
     author    = "C. Mundo and M. Sommerfeld and C. Tropea",
     title     = "Droplet-wall collisions: experimental studies of
           the determination and breakup process",
     journal   = "Int. J. Multiphase. Flow",
     volume    = "21",
     year      = "1995",
     pages     = "151",
}

@Article{YA75,
     author    = "G. K.  Youngren and A. Acrivos ",
     title     = " ",
     journal   = "J. Fluid Mech",
     volume    = "69",
     year      = "1975",
     pages     = "377",
}

@Article{Y68,
     author    = "M.-C. Yuen",
     title     = " ",
     journal   = "J. Fluid Mech",
     volume    = "33",
     year      = "1968",
     pages     = "151",
}

@Article{Z14,
     author    = "J. Zeleny ",
     title     = " ",
     journal   = "Phys. Rev",
     volume    = "3",
     year      = "1914",
     pages     = "69",
}

@Article{Z15,
     author    = "J. Zeleny ",
     title     = " ",
     journal   = "Proc. Camb. Phil. Soc.",
     volume    = "18",
     year      = "1915",
     pages     = "71",
}

@Article{Z17,
     author    = "J. Zeleny ",
     title     = " ",
     journal   = "Phys. Rev",
     volume    = "10",
     year      = "1917",
     pages     = "1",
}

@Article{ZB95,
     author    = "X.  Zhang and O. A. Basaran ",
     title     = " ",
     journal   = "Phys. Fluids",
     volume    = "7",
     year      = "1995",
     pages     = "1184",
}

@Article{ZS97,
     author    = "D. F. Zhang and H. A. Stone",
     journal   = "Phys. Fluids",
     volume    = "9",
     year      = "1997",
     pages     = "2234",
}

@Article{SP00,
     author    = "M. Sussman and E. G. Pucket",
     journal   = "J. Comp. Phys.",
     volume    = "162",
     year      = "2000",
     pages     = "301",
}
@Article{TBEJ01,
     author    = "G. Tryggvason and B. Bunner and A. Esmaeeli and
         D. Juric and N. Al-Rawahi and W. Tauber and J. Han and Y.-J. Jan",
     journal   = "J. Comp. Phys.",
     volume    = "169",
     year      = "2001",
     pages     = "708",
}
@Article{WPB99,
     author    = "E. D. Wilkes and S. D. Phillips and O. A. Basaran",
     journal   = "Phys. Fluids",
     volume    = "11",
     year      = "1999",
     pages     = "3577",
}
@Article{NCB01,
     author    = "P. K. Notz and A. U. Chen and O. A. Basaran",
     journal   = "Phys. Fluids",
     volume    = "13",
     year      = "2001",
     pages     = "549",
}
@Article{CB02,
     author    = "A. U. Chen and O. A. Basaran",
     journal   = "Phys. Fluids",
     volume    = "14",
     year      = "2002",
     pages     = "L1",
}
@Article{CNB02,
     author    = "A. U. Chen and P. K. Notz and O. A. Basaran",
     title     = "Computational and. Experimental Analysis of
                Pinch-off and Scaling ",
     journal   = "Phys. Rev. Lett.",
     volume    = "88",
     year      = "2002",
     pages     = "174501",
}
@Article{ASPB04,
     author    = "B. Ambravaneswaran and H. J. Subramani and S. D. Phillips
             and O. A. Basaran",
     title     = " Dripping-Jetting Transitions in a Dripping Faucet",
     journal   = "Phys. Rev. Lett.",
     volume    = "93",
     year      = "2004",
     pages     = "034501",
}
@Article{APB00,
     author    = "B. Ambravaneswaran and S. D. Phillips and O. A. Basaran",
     journal   = "Phys. Rev. Lett.",
     volume    = "85",
     year      = "2000",
     pages     = "5332",
}
@Article{AWB02,
     author    = "B. Ambravaneswaran and E. D. Wilkes and O. A. Basaran",
     journal   = "Phys. FLuids",
     volume    = "14",
     year      = "2002",
     pages     = "2606",
}
@Article{CMR05,
     author    = "P. Coullet and L. Mahadevan and C. S. Riera",
     journal   = "J. Fluid Mech.",
     volume    = "526",
     year      = "2005",
     pages     = "1",
}
@Article{FIK99,
     author    = "N. Fuchikami and S. Ishioka and K. Kiyono",
     journal   = "J. Phys. Soc. Jap.",
     volume    = "68",
     year      = "1999",
     pages     = "1185",
}
@Article{SYSXAB06,
     author    = "H. J. Subramani and H. K. Yeoh and R. Suryo and
 Q. Xu and B. Ambravaneswaran and O. A. Basaran",
     journal   = "Phys. Fluids",
     volume    = "18",
     year      = "2006",
     pages     = "032106",
}
@Article{AB99,
     author    = "B. Ambravaneswaran and O. A. Basaran",
     title     = "Effects of insoluble surfactants on the nonlinear
            deformation and breakup of stretching liquid bridges",
     journal   = "Phys. Fluids",
     volume    = "11",
     year      = "1999",
     pages     = "997",
}
@Article{LFB06,
     author    = "Y.-C. Liao and E. I. Franses and O. A. Basaran",
     title     = "Deformation and breakup of a stretching liquid bridge
                     covered with an insoluble surfactant momolayer",
     journal   = "Phys. Fluids",
     volume    = "18",
     year      = "2006",
     pages     = "022101",
}
@Article{DSXCS06,
     author    = "V. Dravid and S. Songsermpong and Z. Xue and
                C. A. Corvalan and P. E. Sojka",
     title     = "Two-dimensional modeling of the effects of insoluble
               surfactant on the breakup of a liquid ligament",
     journal   = "Chem. Engin. Sci.",
     volume    = "61",
     year      = "2006",
     pages     = "3577",
}
@Article{CF95,
     author    = "C.-H. Chang and E. I. Franses",
     title     = "Adsorption dynamics of surfactant at the air/water
                   interface: A critical review of mathematical models,
                   data, and mechanisms",
     journal   = "Colloids Surf.",
     volume    = "100",
     year      = "1995",
     pages     = "1",
}
@Article{FBC96,
     author    = "E. I. Franses and O. A. Basaran and C.-H. Chang",
     title     = "Adsorption dynamics of surfactant at the air/water
                   interface: A critical review of mathematical models,
                   data, and mechanisms",
     journal   = "Current Opinion Colloid Interf. Sci.",
     volume    = "1",
     year      = "1996",
     pages     = "296",
}
@Article{JGS06,
     author    = "F. Jin and N. R. Gupta and K. J. Stebe",
     journal   = "Phys. Fluids",
     volume    = "18",
     year      = "2006",
     pages     = "022103",
}
@Article{ETS01,
     author    = "C. D. Eggleton and Tse-Min Tsai and K. J. Stebe",
     title     = "Tip Streaming from a Drop in the Presence of Surfactants",
     journal   = "Phys. Rev. Lett.",
     volume    = "87",
     year      = "2001",
     pages     = "048302",
}
@Article{YXB05,
     author    = "O. E. Yildrim and Q. Xu and O. A. Basaran",
     journal   = "Phys. Fluids",
     volume    = "17",
     year      = "2005",
     pages     = "062107",
}

@Article{AT05,
     author    = "S. Arscott and D. Troadec",
     journal   = "Appl. Phys. Lett.",
     volume    = "87",
     year      = "2005",
     pages     = "134101",
}
@Article{CY04,
     author    = "V. Christini Y.-C. Tan",
     journal   = "Lab Chip",
     volume    = "4",
     year      = "2004",
     pages     = "257",
}

@Article{W06,
     author    = "C. Williams",
     journal   = "Phys. World",
     volume    = "19",
     year      = "2006",
     pages     = "24",
}
@Article{Sch96,
     author    = "R. M. S. M. Schulkes",
     journal   = "J. Fluid Mech.",
     volume    = "309",
     year      = "1996",
     pages     = "277",
}
@Article{LRR00,
     author    = "J. Li and Y. Y. Renardy and M. Renardy",
     journal   = "Phys. FLuids",
     volume    = "12",
     year      = "2000",
     pages     = "269",
}
@Article{LT98,
     author    = "J. S. Lowengrub and L. Truskinovsky",
     journal   = "Proc. R. Soc. Lond. A",
     volume    = "454",
     year      = "1998",
     pages     = "2617",
}
@Article{LLG02,
     author    = "H.-G. Lee and J. S. Lowengrub and J. Goodman",
     journal   = "Phys. FLuids",
     volume    = "14",
     year      = "2002",
     pages     = "492",
}
@Book{LP82,
     author    = "L. Lapidus and G. F. Pinder",
     title     = "Numerical Solution of Partial Differential Equations
                  in Engineering",
     publisher = "Wiley: New York",
     year      = "1982",
}
@Article{OP01,
     author    = "S. Osher and R. P. Fedkiw",
     journal   = "J. Comp. Phys.",
     volume    = "169",
     year      = "2001",
     pages     = "463",

}
@Article{S01,
     author    = "J. A. Sethian",
     journal   = "J. Comp. Phys.",
     volume    = "169",
     year      = "2001",
     pages     = "503",
}
@Article{PZ99,
     author    = "S. Popinet and S. Zaleski",
     journal   = "Int. J. Numer. Meth. Fluids",
     volume    = "30",
     year      = "1999",
     pages     = "775",
}
@Article{P06,
     author    = "S. Popinet",
     journal   = "GERRIS",
     year      = "2006"
}
@Article{DPJZ02,
     author    = "L. Duchemin and S. Popinet and C. Josserand and S. Zaleski",
     journal   = "Phys. Fluids",
     volume    = "14",
     year      = "2002",
     pages     = "3000",
}
@Article{JZ03,
     author    = "C. Josserand and S. Zaleski",
     journal   = "Phys. Fluids",
     volume    = "15",
     year      = "2003",
     pages     = "1650",
}
@Article{GLSZ99,
     author    = "D. Gueyffier and J. Li and R. Scardiovelli and S. Zaleski",
     journal   = "J. Comput. Phys.",
     volume    = "152",
     year      = "1999",
     pages     = "423",
}
@Article{BMLV03,
     author    = "T. Biben and C. Misbah and A. Leyrat and C. Verdier",
     journal   = "Europhys. Lett.",
     volume    = "63",
     year      = "2003",
     pages     = "623",
}
@Book{Succi,
     author    = "S. Succi",
     title     = "The Lattice Boltzmann Equation, for Fluid Dynamics
                  and Beyond",
     publisher = "Oxford University Press",
     year      = "2001"
}
@Article{K05,
     author    = "A. Kitakawa",
     journal   = "Chem. Engin. Sci.",
     volume    = "60",
     year      = "2005",
    pages     = "5612",
}
@Article{RZ94,
     author    = "D. H. Rothman and S. Zaleski",
     journal   = "Rev. Mod. Phys.",
     volume    = "66",
     year      = "1994",
    pages     = "1417",
}
@Article{LDBY03,
     author    = "J. L{\'e}opold{\`e}s and A. Dupuis and D. G. Bucknall
                    and J. M. Yeomans",
     journal   = "Langmuir",
     volume    = "19",
     year      = "2003",
    pages     = "9818",
}
@Article{Edrop05,
     author    = "J. Eggers",
     title     = "Drop formation - an overview",
     journal   = "ZAMM",
     volume    = "85",
     year      = "2005",
    pages     = "400",
}
@Article{BWT05,
     author    = "J. C. Burton and R. Waldrep and P. Taborek",
     title     = "Scaling and Instabilities in Bubble Pinch-Off",
     journal   = "Phys. Rev. Lett.",
     volume    = "94",
     year      = "2005",
     pages     = "184502",
}

@Article{BRT04,
     author    = "J. C. Burton and J. E. Rutledge and P. Taborek",
     title     = "Fluid Pinch-Off Dynamics at Nanometer Length Scales",
     journal   = "Phys. Rev. Lett.",
     volume    = "92",
     year      = "2004",
     pages     = "244505",
}
@Article{BT07,
     author    = "J. C. Burton and P. Taborek",
     title     = "2D Inviscid Pinch-off: An Example of
          Self-Similarity of the Second Kind",
     journal   = "Phys. Fluids",
     volume    = "19",
     year      = "2007",
     pages     = "102109",
             }
@Article{BT08,
     author    = "J. C. Burton and P. Taborek",
     title     = "Bifurcation from Bubble to Droplet Behavior in
                  Inviscid Pinch-off",
     journal   = "Phys. Rev. Lett.",
     volume    = "101",
     year      = "2008",
     pages     = "214502"
}
@Article{BRT07,
     author    = "J. C. Burton and J. E. Rutledge and P. Taborek ",
     title     = "Fluid pinch-off in superfluid and normal Helium-4",
     journal   = "Phys. Rev. E",
     volume    = "75",
     year      = "2007",
    pages     = "036311",
}
@Article{KMZN06,
     author    = "N. C. Keim and P. M{\o}ller and W. W. Zhang and S. R. Nagel",
     title     = "Breakup of Air Bubbles in Water: Memory and
                       Breakdown of Cylindrical Symmetry",
     journal   = "Phys. Rev. Lett.",
     volume    = "97",
     year      = "2006",
     pages     = "144503"
}

@Article{BZ09,
     author    = "F. Blanchette and W. W. Zhang",
     title     = "Force Balance at the Transition from Selective",
     journal   = "Phys. Rev. Lett.",
     volume    = "102",
     year      = "2009",
     pages     = "144501"
}

@Article{TET07,
     author    = "S. T. Thoroddsen and E. G. Etoh and K. Takeara",
     title     = "Experiments on bubble pinch-off",
     journal   = "Phys. Fluids",
     volume    = "19",
     year      = "2007",
    pages     = "042101",
}
@Article{T02,
     author    = "S. T. Thoroddsen",
     title     = "The ejecta sheet generated by the impact of a drop",
     journal   = "J. Fluid Mech.",
     volume    = "451",
     year      = "2002",
    pages     = "373",
}

@Article{SGM05,
     author    = "A. Sevilla and J. M. Gordillo and C. Martinez-Bazan",
     journal   = "Phys. Fluids",
     volume    = "17",
     year      = "2005",
    pages     = "018105",
}

@Article{MCG07,
     author    = "A G. Marin and F. Campo-Cort{\'e}s and J. M. Gordillo",
     title     = "Generation of micron-sized drops through viscous
              coflows",
     journal   = "submitted",
     year      = "2007",
}
@Article{GSRM05,
     author    = "J. M. Gordillo and A. Sevilla and J. Rodriguez-Rodrigues
             and C. Martinez-Bazan",
     title     = " Axisymmetric Bubble Pinch-Off at High Reynolds Numbers",
     journal   = "Phys. Rev. Lett.",
     volume    = "95",
     year      = "2005",
    pages     = "194501",
}

@Article{GP06,
     author    = "J. M. Gordillo and and M. Perez-Sabroid",
     title     = "Axisymmetric breakup of bubbles at high Reynolds numbers",
     journal   = "J. Fluid Mech.",
     volume    = "562",
     year      = "2006",
     pages     = "303",
}
@Article{GF07,
     author    = "J. M. Gordillo and M. A. Fontelos",
     title     = "Satellites in inviscid breakup of bubbles",
     journal   = "Phys. Rev. Lett.",
     volume    = "98",
     year      = "2007",
     pages     = "144503",
}
@Article{S45,
     author    = "G. G. Stokes",
     journal   = "Trans. Camb. Phil. Soc.",
     volume    = "8",
     year      = "1845",
     pages     = "287",
}
@Article{P50,
     author    = "J. A. F. Plateau",
     journal   = "Ann. Phys. Chem.",
     volume    = "80",
     year      = "1850",
     pages     = "566",
}

@Article{B55,
     author    = "A. Beer",
     title     = "Uber die Oberfl{\"a}chen rotirender Fl{\"u}ssigkeiten
                   im Allgemeinen, insbesondere {\"u}ber den Plateau'schen
                   Rotationsversuch",
     journal   = "Ann. Phys. Chem.",
     volume    = "96",
     year      = "1855",
     pages     = "1",
}
@Article{F98,
     author    = "M. A. Fontelos",
     title     = "Pinching of liquid threads",
     journal   = "PhD Thesis, Universidad Complutense de Madrid",
     year      = "1998",
}
@Article{F03,
     author    = "M. A. Fontelos",
     title     = "Break-up and no break-up in a family of models
                 for the evolution of viscoelastic jets",
     journal   = "Z. angew. Math. Phys.",
     volume    = "54",
     pages     = "84",
     year      = "2003",
}
@Article{FV99,
     author    = "M. A. Fontelos and J. J. L. Vel{\'a}zquez",
     title     = "On some breakup and singularity formation
       mechanisms for inviscid liquid jets",
     journal   = "SIAM J. Appl. Math.",
     volume    = "59",
     pages     = "2274",
     year      = "1999",
}
@Article{FV00,
     author    = "M. A. Fontelos and J. J. L. Vel{\'a}zquez",
     title     = "Fractal-like singularities for an inviscid
        one-dimensional model of fluid jets",
     journal   = "European J. Appl. Math.",
     volume    = "11",
     pages     = "29",
     year      = "2000",
}
@Article{HF08,
     author    = "F. de la Hoz and M. A. Fontelos",
     title     = "On the structure of singularities in nonlocal
          transport equations",
     journal   = "J. Phys. A: Math. Theor.",
     volume    = "41",
     pages     = "185204",
     year      = "2008"
}
@Article{CKN82,
     author    = "L. Caffarelli and R. Kohn and L. Nirenberg",
     title     = "Partial regularity of suitable weak solutions
                 to the Navier-Stokes equations",
     journal   = "Comm. Pur. Appl. Math.",
     volume    = "35",
     pages     = "771-831",
     year      = "1982",
}

@Article{Souplet,
     author    = "P. Souplet",
     title     = "Recent results and open problems on parabolic
                equations with gradient nonlinearities",
     journal   = "Electron. J. Diff. Eqns.",
     volume    = "20",
     pages     = "1-19",
     year      = "2001",
}

@Article{ZL99,
     author    = "W. W. Zhang and J. R. Lister",
     journal   = "Phys. Rev. Lett.",
     volume    = "83",
     year      = "1999",
     pages     = "1151",
}
@Article{CN01,
     author    = "I. Cohen and S. R. Nagel",
     journal   = "Phys. Fluids",
     volume    = "13",
     year      = "2001",
     pages     = "3533",
}
@Article{ON00,
     author    = "L. Oddershede and S. R. Nagel",
     title     = "Singularity during the onset of an electrohydrodynamic
                  spout",
     journal   = "Phys. Rev. Lett.",
     volume    = "85",
     year      = "2000",
     pages     = "1234",
}
@Article{K98,
     author    = "S. Kawano",
     journal   = "Phys. Rev. E",
     volume    = "58",
     year      = "1998",
     pages     = "4468",
}
@Book{Graham,
     author    = "R. Graham",
     title     = "Springer Tracts in Modern Physics",
     publisher = "Springer: Berlin",
     year      = "1973",
     volume    = "66",
}
@Book{GV04,
     author    = "V. A. Galaktionov and J. L. Vazquez",
     title     = "A Stability Technique for Evolution Partial
              Differential Equations: A Dynamical Systems Approach",
     publisher = "Birkhauser",
     year      = "2004",
}
@Book{Vazquez,
     author    = "J. L. Vazquez",
     title     = "Smoothing and Decay Estimates for Nonlinear
                   Diffusion Equations. Equations of Porous Medium Type",
     publisher = "Oxford University Press",
     year      = "2006",
}
@Article{J76,
     author    = "H. K. Janssen",
     journal   = "Z. Physik B",
     volume    = "23",
     year      = "1976",
     pages     = "377",
}
@Article{HM90,
     author    = "P. Huerre and P. A. Monkewitz",
     journal   = "Annu. Rev. Fluid Mech.",
     volume    = "22",
     year      = "1990",
     pages     = "473",
}
@Inproceedings{Udine,
     author    = "J. Eggers",
     title     = "Singularities and Similarities",
     year      = "2007",
     booktitle = "Thin films of soft matter",
     editor    = "S. Kalliadasis and U. Thiele",
     pages     = "95",
     publisher = "Springer, Berlin"
}

@Article{BMSSPL06,
     author    = "R. Bergmann and D. {van der Meer} and M. Stijnman
                    and M. Sandtke and A. Prosperetti and D. Lohse",
     title     = " Giant Bubble Pinch-Off",
     journal   = "Phys. Rev. Lett.",
     volume    = "96",
     year      = "2006",
     pages     = "154505",
}
@ARTICLE{CN02,
   author = "I. Cohen and S. R. Nagel",
   title     = "Scaling at the Selective Withdrawal Transition
           through a Tube Suspended above the Fluid Surface",
   year = "2002",
   journal = "Phys. Rev. Lett.",
   volume = "88",
   pages = "074501"
}
@ARTICLE{C04,
   author = "I. Cohen",
   title     = "Scaling and transition structure dependence on the
       fluid viscosity ratio in the selective withdrawal transition",
   year = "2004",
   journal = "Phys. Rev. E",
   volume = "70",
   pages = "026302"
}
@ARTICLE{LRQ03,
   author = "\'E. Lorenceau and F. Restagno and D. Qu\'{e}r\'{e}",
   title     = " Fracture of a Viscous Liquid",
   year = "2003",
   journal = "Phys.\ Rev. \ Lett.",
   volume = "90",
   pages = "184501"
}
@Inproceedings{T66,
     author    = "G. I. Taylor",
     title     = "Conical free surfaces and fluid interfaces",
     year      = "1964",
     booktitle = "Proceedings of the 11th International Congress of
                    Applied Mathematics, Munich (Germany)",
     editor    = "H. G{\"o}rtler",
     pages     = "790-796",
     publisher = "Springer, Heidelberg",
}
@Inproceedings{E98,
     author    = "J. Eggers",
     title     = " Hydrodynamic Singularities",
     year      = "1998",
     booktitle = "A Perspective Look at Nonlinear Media in Physics,
                   Chemistry, and Biology",
     editor    = "J. Parisi and S. C. Mueller and W. Zimmermann",
     pages     = "305-312",
     publisher = "Springer, Berlin"
}

@ARTICLE{E93,
   author = "J. Eggers",
   title     = " Universal Pinching of 3D Axisymmetric Free-Surface Flow",
   year = "1993",
   journal = "Phys. Rev. Lett.",
   volume = "71",
   pages =  "3458"
}
@ARTICLE{RRR01,
   author = "A. Rothert and R. Richter and I. Rehberg",
   year = "2001",
   journal = "Phys. Rev. Lett.",
   volume = "87",
   pages =  "084501"
}
@ARTICLE{LSB99,
   author = "J. R. Lister and H. A. Stone and M. P. Brenner",
   year = "1999",
   journal = "Proc. Roy. Soc. London A",
   volume = "455",
   pages =  "329"
}
@ARTICLE{LL03,
   author = "D. Leppinen and J. Lister",
   title  = "Capillary pinch-off in inviscid fluids",
   year = "2003",
   journal = "Phys. Fluids",
   volume = "15",
   pages =  "568"
}
@Book{LLQu,
     author    = "L. D. Landau and E. M. Lifshitz",
     title     = "Quantum Mechanics",
     publisher = "Pergamon, Oxford",
     year      = "1984"
}

@ARTICLE{K97,
   author = "L. P. Kadanoff",
   title  = "Singularities and Blowups",
   year = "1997",
   journal = "Phys. Today",
   volume = "50(9)",
   pages =  "11-12"
}

@ARTICLE{K00,
   author = "L. P. Kadanoff",
   title  = "Making a splash, breaking a neck: the development
              of complexity in physical systems",
   year = "2000",
   journal = "Univ. Chicago Record",
   volume = "35",
   pages =  "2"
}

@ARTICLE{BCKSV99,
   author = "M. P. Brenner and P. Constantin and L. P. Kadanoff
         and A. Schenkel and S. C. Venkataramani",
   title  = "Diffusion, attraction and collapse",
   year = "1999",
   journal = "Nonlinearity",
   volume = "12",
   pages =  "1071"
}

@ARTICLE{ABS03,
   author = "S. L. Anna and N. Bontoux and H. A. Stone",
   year = "2003",
   journal = "Appl. Phys. Lett.",
   volume = "82",
   pages =  "364"
}
@ARTICLE{LAWS04,
   author = "D. Link and S. L. Anna and D. Weitz and H. A. Stone",
   title  = "Geometrically mediated breakup of drops in microfluidic devices",
   year = "2004",
   journal = "Phys. Rev. Lett.",
   volume = "92",
   pages =  "054503"
}
@ARTICLE{UFSW07,
   author = "A. S. Utada and A. Fernandez-Nieves and H. A. Stone and
               D. Weitz",
   title  = "Dripping to jetting transitions in coflowing liquid streams",
   year = "2007",
   journal = "Phys. Rev. Lett.",
   volume = "99",
   pages =  "094502"
}
@ARTICLE{J02,
   author = "D. Jacqmin",
   title  = "Very, very fast wetting",
   year = "2002",
   journal = "J. Fluid Mech.",
   volume = "455",
   pages =  "347-358"
}
@ARTICLE{GSW05,
   author = "P. Garstecki and H. A. Stone and G. M. Whitesides",
   year = "2005",
   journal = "Phys. Rev. Lett.",
   volume = "94",
   pages =  "164501"
}
@ARTICLE{G97,
   author = "A. M. Ga{\~n}{\'a}n-Calvo",
   title  = "Cone-jet analytical extension of Taylor's electrostatic
              solution and the asymptotic universal scaling laws in
              electrospraying",
   year = "1997",
   journal = "Phys. Rev. Lett.",
   volume = "79",
   pages =  "217"
}
@ARTICLE{G97b,
   author = "A. M. Ga{\~n}{\'a}n-Calvo",
   year = "1997",
   journal = "J. Fluid Mech.",
   volume = "335",
   pages =  "165"
}
@ARTICLE{G-C04,
   author = "A. M. Ga{\~n}{\'a}n-Calvo",
   year = "2004",
   journal = "J. Fluid Mech.",
   volume = "507",
   pages =  "203"
}
@ARTICLE{GLR06,
   author = "A. M. Ga{\~n}{\'a}n-Calvo and J. M. L{\'o}pez-Herrera and
            P. Riesco-Chueca",
   title = "The combination of electrospray and flow focusing",
   year = "2006",
   journal = "J. Fluid Mech.",
   volume = "566",
   pages =  "421"
}

@ARTICLE{LRG05,
   author = "J. M. L{\'o}pez-Herrera and P. Riesco-Chueca and
          A. M. Ga{\~n}{\'a}n-Calvo",
   title = "Linear Stability Analysis of Axisymmetric Perturbations
       in Imperfectly Conducting Liquid Jets",
   year = "2005",
   journal = "Phys. Fluids",
   volume = "17",
   pages =  "034106"
}
@ARTICLE{Hig03,
   author = "F. J. Higuera",
   title  = "Flow rate and electric current emitted by a Taylor cone",
   year = "2003",
   journal = "J. Fluid Mech.",
   volume = "484",
   pages =  "303"
}
@ARTICLE{HBCMS99,
   author = "R. P. A. Hartman and D. J. Brunner and D. M. A. Camelot and
               J. C. M. Marijnissen and B. Scarlett",
   title  = "Electrohydrodynamic atomization in the cone-jet mode physical
              modeling of the liquid cone and jet",
   year = "1999",
   journal = "J. Aerosol Sci.",
   volume = "30",
   pages =  "823"
}
@ARTICLE{LBGCMG02,
   author = "I. G. Loscertales and A. Barrero and I. Guerrero
 and R. Cortijo and M. Marquez and A. M. Ga{\~n}{\'a}n-Calvo",
   year = "2002",
   journal = "Science",
   volume = "295",
   pages =  "1695"
}
@ARTICLE{C99,
   author = "L. T. Cherney",
   year = "1999",
   journal = "J. Fluid Mech.",
   volume = "378",
   pages =  "167"
}
@ARTICLE{GG01,
   author = "A. M. Ga{\~n}{\'a}n-Calvo and J. M. Gordillo",
   title     = "Perfectly Monodisperse Microbubbling by Capillary
                 Flow Focusing",
   year = "2001",
   journal = "Phys. Rev. Lett.",
   volume = "87",
   pages =  "274501"
}
@ARTICLE{Ga04,
   author = "A. M. Ga{\~n}{\'a}n-Calvo",
   year = "2004",
   journal = "Phys. Rev. E",
   volume = "69",
   pages =  "027301"
}
@Book{HB65,
     author    = "J. Happel and H. Brenner",
     title     = "Low Reynolds Number Hydrodynamics",
     publisher = "Prentice-Hall, Englewood Cliffs, NJ",
     year      = "1965"
}

@Book{Whithambook,
     author    = "G. B. Whitham",
     title     = " Linear and Nonlinear Waves",
     publisher = "John Wiley \& Sons",
     year      = "1974"
}

@ARTICLE{Whithampaper,
   author = "D. W. Schwendeman and G. B. Whitham",
   title  = "On converging shock waves",
   year = "1987",
   journal = "Proc. R. Soc. Lond. A",
   volume = "413",
   pages =  "297-311"
}

@Incollection{ Dafermos,
     author    = "C. M. Dafermos",
     title     = " Hyperbolic conservation laws in continuum physics,
               2nd edition",
     booktitle = " Grundlehren der Mathematischen Wissenschaften",
     year      = " 2005",
     volume    = " 325",
     publisher = " Springer, Berlin",
         }

@Book{Bressan,
     author    = "A. Bressan",
     title     = " Hyperbolic Systems of Conservation Laws.
           The One Dimensional Cauchy Problem",
     publisher = "Oxford University Press",
     year      = "2000"
}

@misc{H04,
   author = "E. J. Hinch",
   year = "2004",
   howpublished = "private communication"
}
@misc{V-A04,
   author = "M. Vignes-Adler",
   year = "2004",
   howpublished = "Talk delivered at Euromech 450, Marseille"
}
@ARTICLE{BL86,
   author = "B. J. Bentley and L. G. Leal",
   year = "1986",
   journal = "J. Fluid Mech.",
   volume = "167",
   pages =  "219"
}
@ARTICLE{SL90,
   author = "H. A. Stone and L. G. Leal",
   year = "1990",
   journal = "J. Fluid Mech.",
   volume = "220",
   pages =  "161"
}

@ARTICLE{Ch04,
   author = "S. Chaieb",
   year = "2004",
   journal = "arXiv:physics/0404088",
   volume = "",
   pages =  ""
}
@ARTICLE{B93,
   author = "R. A. {De Bruijn}",
   year = "1993",
   journal = "Chem. Eng. Sci.",
   volume = "48",
   pages =  "277"
}
@ARTICLE{Z04,
   author = "W. W. Zhang",
   year = "2004",
   journal = "Phys. Rev. Lett.",
   volume = "93",
   pages =  "184502"
}
@ARTICLE{BCZ05,
   author = "M. {Kleine Berkenbusch} and I. Cohen and W. W. Zhang",
   title     = "Liquid interfaces in viscous straining flows:
     Numerical studies of the selective withdrawal transition",
   year = "2008",
   journal = "J. Fluid Mech.",
   volume = "613",
   pages =  "171"
}
@ARTICLE{BZ06,
   author = "F. Blanchette and W. W. Zhang",
   title     = "Transition flow rate in viscous withdrawal",
   year = "2006",
   journal = "Bull. Am. Phys. Soc.",
   volume = "51",
   pages =  "OJ.00006"
}
@ARTICLE{SRC05,
   author = "L. W. Schwartz and D. Roux and J. J. Cooper-White",
   title     = "On the shapes of droplets that are sliding on a
                  vertical wall",
   year = "2005",
   journal = "Physica D",
   volume = "209",
   pages =  "236"
}
@Article{W01,
     author    = "D. B. Wallace",
     title     = "Ink-Jet Applications, Physics, and Modelling
                - an Industrial/Applied Research View",
     journal   = "http://www.ima.umn.edu/multimedia/
                     abstract/1-10abs.html\#wallace",
     year      = "2001"
}
@ARTICLE{CP89,
   author = "M. Clopeau and B. Prunet-Foch",
   year = "1989",
   journal = "J. Electrost.",
   volume = "22",
   pages =  "135"
}
@ARTICLE{S97,
   author = "D. A. Saville",
   title     = "Electrohydrodynamics: the Taylor-Melcher leaky
            dielectric model",
   year = "1997",
   journal = "Annu. Rev. Fluid Mech.",
   volume = "29",
   pages =  "27"
}
@ARTICLE{MT69,
   author = "J. R. Melcher and G. I. Taylor",
   title     = "Electrohydrodynamics: a review of the role of
                interfacial shear stresses",
   year = "1969",
   journal = "Annu. Rev. Fluid Mech.",
   volume = "1",
   pages =  "46"
}
@ARTICLE{HSRB01a,
   author = "M. M. Hohman and M. Shin and G. C. Rutledge and M. P. Brenner",
   title =   {Electrospinning and electrically forced jets I.
                     Stability theory.},
   year = "2001",
   journal = "Phys. Fluids",
   volume = "13",
   pages =  "2201"
}
@ARTICLE{HSRB01b,
   author = "M. M. Hohman and M. Shin and G. C. Rutledge and M. P. Brenner",
   title =   {Electrospinning and electrically forced jets II. Applications.},
   year = "2001",
   journal = "Phys. Fluids",
   volume = "13",
   pages =  "2221"
}
@ARTICLE{SHBR01,
   author = "Y. M. Shin and M. M. Hohman and M. P. Brenner and G. C. Rutledge",
   year = "2001",
   journal = "Appl. Phys. Lett.",
   volume = "78",
   pages =  "1149"
}
@ARTICLE{FYBR03,
   author = "S. V. Fridrikh and J. H. Yu and M. P. Brenner and G. C. Rutledge",
   year = "2003",
   journal = "Phys. Rev. Lett.",
   volume = "90",
   pages =  "144502"
}
@ARTICLE{B71,
   author = "P. K. Baumgarten",
   title  = "Electrostatic spinning of acrylic microfibers",
   year = "1971",
   journal = "J. Colloid Interface Sci.",
   volume = "36",
   pages =  "71"
}
@ARTICLE{FZ05,
   author = "L. G. Fel and Y. Zimmels",
   title  = "Plateau instability of a liquid crystalline cylinder
                  in a magnetic field",
   year = "2005",
   journal = "J. Colloid Interface Sci.",
   volume = "288",
   pages =  "553"
}
@ARTICLE{RF94,
   author = "J. Rosell-Llompart and J. {Fernandez de la Mora}",
   year = "1994",
   journal = "J. Aerosol Sci.",
   volume = "25",
   pages =  "1093"
}
@ARTICLE{LVB03,
   author = "A. Lindner and J. Vermant and D. Bonn",
   year = "2003",
   journal = "Physica A",
   volume = "319",
   pages =  "125"
}
@ARTICLE{MRF95,
   author = "J. Magnaudet and M. Rivero and J. Fabre",
   year = "1995",
   journal = "J. Fluid Mech.",
   volume = "284",
   pages =  "97"
}
@ARTICLE{PS06,
   author = "Y. Pan and K. Suga",
   year = "2006",
   journal = "Phys. Fluids",
   volume = "18",
   pages =  "052101"
}
@ARTICLE{MTB05,
   author = "T. Menard and S. Tanguy and A. Berlemont",
   year = "2007",
   journal = "Int. J. Multiphase Flows",
   volume = "33",
   number="5",
   pages="510-524",
}
@ARTICLE{TPLB00,
   author = "H. Temmen and H. Pleiner and M. Liu and H. R. Brand",
   year = "2000",
   journal = "Phys. Rev. Lett.",
   volume = "84",
   pages =  "3228"
}
@ARTICLE{BGKO01,
   author = "A. N. Beris and M. D. Graham and I. Karlin and
                   H. C. {\"O}ttinger",
   year = "2001",
   journal = "Phys. Rev. Lett.",
   volume = "86",
   pages =  "744"
}
@ARTICLE{M04,
   author = "S. T. Milner",
   title     = "Thermodynamic admissability of the reptation model",
   year = "2004",
   journal = "J. Rheol.",
   volume = "48",
   pages =  "53"
}
@ARTICLE{VT91,
   author = "F. Vollrath and E. K. Tillinghast",
   title     = "Glycoprotein glue beneath a spider web's aqueous coat",
   year = "1991",
   journal = "Naturwissenschaften",
   volume = "78",
   pages =  "557"
}
@ARTICLE{OSY99,
   author = "M.-H. Oh and J.-H. So and S.-M. Yang",
   title     = "Rheological evidence for the silica-mediated gelation of
               Xanthan gum",
   year = "1999",
   journal = "J. Colloid Interf. Sci.",
   volume = "216",
   pages =  "320"
}
@ARTICLE{CW99,
   author = "J. M. Cheny and K. Walters",
   title     = "Rheological influences on the splashing experiment",
   year = "1999",
   journal = "J. Non-Newtonian Fluid Mech.",
   volume = "86",
   pages =  "185"
}
@ARTICLE{HMCB99,
   author = "G. M. Harrison and R. Mun and G. Cooper and D. V. Boger",
   title     = "A note on the effect of polymer rigidity and concentration
               on spray atomization",
   year = "1999",
   journal = "J. Non-Newtonian Fluid Mech.",
   volume = "85",
   pages =  "93"
}
@ARTICLE{ZBT99,
   author = "M. A. Zirnsak and D. V. Boger and V. Tirtaatmadja",
   title     = "Steady shear and rheological properties of Xanthan
               gum solutions in viscous solvents",
   year = "1999",
   journal = "J. Rheol.",
   volume = "43",
   pages =  "627"
}
@ARTICLE{JLB91,
   author = "D. A. R. Jones and B. Leary and D. V. Boger",
   title     = "The rheology of a concentrated colloidal suspension
              of hard spheres",
   year = "1991",
   journal = "J. Colloid Interf. Sci.",
   volume = "147",
   pages =  "479"
}
@ARTICLE{FB00,
   author = "D. R. Foss and J. F. Brady",
   title     = "Structure, diffusion and rheology of Brownian suspensions
               by Stokesian dynamics simulation",
   year = "2000",
   journal = "J. Fuid Mech.",
   volume = "407",
   pages =  "167"
}
@ARTICLE{BA82,
   author = "J. F. Brady and A. Acrivos",
   title     = "The deformation and breakup of a slender drop
              in extensional flow: intertial effects",
   year = "1982",
   journal = "J. Fuid Mech.",
   volume = "115",
   pages =  "443"
}
@ARTICLE{BAH03,
   author = "A. Bach and K. Almdal and H. K. Rasmussen and O. Hassager",
   title     = "Elongational viscosity of narrow molar mass distribution
                 polystyrene",
   year = "2003",
   journal = "Macromolecules",
   volume = "36",
   pages =  "5174"
}
@ARTICLE{GT03,
   author = "R. E. Grisenti and J. P. Toennies",
   title     = "Cryogenic microjet source for orthotropic beams of
                 ultralarge superfluid helium droplets",
   year = "2003",
   journal = "Phys. Rev. Lett.",
   volume = "90",
   pages =  "234501"
}
@ARTICLE{JNB96,
   author = "H. M. Jaeger and S. R. Nagel and R. P. Behringer",
   title     = "",
   year = "1996",
   journal = "Rev. Mod. Phys.",
   volume = "68",
   pages =  "1259"
}
@ARTICLE{LBMZMVWHK04,
   author = "D. Lohse and R. Bergmann and R. Mikkelson and C. Zeilstra and
             D. {van der Meer} and M. Versluis and K. {van der Weele}
              and M. {van der Hoef} and H. Kuipers",
   title     = "Impact on soft sand: void collapse and jet formation",
   year = "2004",
   journal = "Phys. Rev. Lett.",
   volume = "93",
   pages =  "198003"
}
@ARTICLE{LKL91,
   author = "M. S. Longuet-Higgins and B. R. Kerman and K. Lunde",
   title     = "The release of air bubbles from an underwater nozzle",
   year = "1991",
   journal = "J. Fluid Mech.",
   volume = "230",
   pages =  "365"
}
@ARTICLE{OP93,
   author = "H. N. O{\~g}uz and A. Prosperetti",
   title     = "Dynamics of bubble growth and detachment from a needle",
   year = "1993",
   journal = "J. Fluid Mech.",
   volume = "257",
   pages =  "111"
}
@ARTICLE{L46,
   author = "N. Levinson",
   title     = " On the asymptotic shape of the cavity behind an axially
              symmetric nose moving through an ideal fluid",
   year = "1946",
   journal = "Ann. Math.",
   volume = "47",
   pages =  "704"
}

@book{Agricola56,
   author =    {Georg Bauer--Agricola},
   title =     {De Re Metallica},
   publisher = {Froben, Ble},
   year =      1556,
}

@article{Alid96,
   author =  {Alidibirov, M. and Dingwell, D. B. },
   title =   {Magma fragmentation by rapid decompression},
   journal = {Nature},
   volume = {380},
   pages = {146-148},
   year =  1996,
}

@Article{Andreas2001,
	author={E. L. Andreas and M. L. Pattison  and S. E. Belcher},
	title={Production rates of sea-spray droplets:
	Clarification and elaboration},
	journal={J. Phys. Res.},
	year={2001},
	volume={106},
	number={C4},
	pages={7157--7161}
}


@inCollection{Ande95,
   author =    {Anderson, W. E. and Ryan, H. M. and Santoro, R. J. },
   title =     {Impinging jet injector atomization.},
   booktitle = {Liquid rocket engine combustion instability.},
   publisher = {AIAA},
   volume =  169,
   year =  1995,
}

@article{Ash90,
   author =  {Ashgriz, N. and Poo, Y. L.},
   title =   {Coalescence and separation in binary collisions of
                 liquid drops.},
   journal = {J. Fluid Mech.},
   volume = {221},
   pages = {183--204},
   year =  1990,
}

@article{Antko07,
   author =  {Antkowiak, A. and Bremond, N. and {Le Dizes}, S.
              and Villermaux, E.},
   title =   {Short-term dynamics of a density interface following an impact},
   journal = {J. Fluid Mech.},
   volume = {577},
   pages = {241-250},
   year =  2007,
}

@article{Blan79,
   author =  {Alusa, A. L. and Blanchard, D. C.},
   title =   {Drop size disribution produced by the
           breakup of large drops under turbulence.},
   journal = {Journal de Recherches Atmosph{\'e}riques.},
   volume = {VII},
   number={1},
   pages = {1--9},
   year =  1971,
}


@Article{Anguelova&Barber1999,
	author={M. Anguelova and R. P. Barber},
	title={Spume Drops Produced by the Wind Tearing of Wave Crests},
	journal={J.  Phys. Oceanogr.},
	year={1999},
	volume={29},
	pages={1156--1165}
}



@article{Asar81,
   author =  {Asare, H. R. and Takahashi, R. K. and Hoffman, M. A.},
   title =   {Liquid sheet jet experiments: comparison with
   linear theory.},
   journal = {Trans. ASME: J. Fluids Engng},
   volume = 103,
   pages = {395-604},
   year =  1981,
}

@article{Back69,
   author =  {Back, L. H. and Cuffel, R. F. and Massier, P. F.},
   title =   {Laminarization of a turbulent boundary layer in
   nozzle flow.},
   journal = {AIAA Journal},
   volume = 7,
   pages = {730-733},
   year =  1969,
}

@article{Basset94,
   author =  {Basset, A. B.},
   title =   {Waves and jets in a viscous liquid.},
   journal = {American J. Math.},
   volume = 16,
   pages = {93-110},
   year =  1894,
}


@book{Bayv93,
   author =    {Bayvel, L. and Orzechowski, Z.},
   title =     {Liquid atomization},
   publisher = {Taylor \& Francis.},
   year =      1993,
}

@article{belmonte07,
   author =  {Grumpstrup, T. and Keller, J. B. and Belmonte, A.},
   title =   {Cavity Ripples Observed during the Impact of Solid
            Objects into Liquids.},
   journal = {Phys. Rev. Letters},
   volume = 99,
   pages = {114502},
   year =  2007,
}


@article{Bent04,
   author =  {Bentley, W. A.},
   title =   {Studies of raindrops and raindrop phenomena.},
   journal = {Monthly Weather Review},
   volume = 10,
   pages = {450-456},
   year =  1904,
}

@Article{Bernal&Roshko1986,
	author={L. P. Bernal and A. Roshko},
	title={Streamwise vortex structure in plane mixing layers},
	journal={J. Fluid Mech.},
	year={1986},
	volume={170},
	pages={499--525}
}



@Article{Betchov&Szewczyk1963,
	author={R. Betchov and A. Szewczyk},
	title={Stability of a shear layer between parallel streams},
	journal={Phys. Fluids},
	year={1963},
	volume={6},
	number={10},
	pages={1391--1396}
}


@book{Blan66,
   author =    {Blanchard, D. C.},
   title =     {From Raindrops to Volcanoes},
   publisher = {Dover.},
   year =      1966,
}



@article{Bogy79,
   author =  {Bogy, D. B.},
   title =   {Drop formation in a circular liquid jet.},
   journal = {Annu. Rev. Fluid Mech.},
   volume = 11,
   pages = {207},
   year =  1979,
}

@Article{Bohr1939,
	author={N. Bohr},
	title={Disintegration of Heavy Nuclei},
	journal={Nature},
	year={1939},
	volume={143},
	number={},
	pages={330}
}

@Article{BW39,
	author={N. Bohr and J. A. Wheeler},
	title={The Mechanism of Nuclear Fission},
	journal={Phys. Rev.},
	year={1939},
	volume={56},
	number={},
	pages={426}
}


@article{Bond35 ,
   author =  {Bond, W. N.},
   title =   {The surface tension of a moving water sheet.},
   journal = {Proc. Phys. Soc.},
   volume = 47,
   pages = {549-558},
   year =  1935,
}

@article{BP37 ,
   author =  {W. N. Bond and H. O. Puls},
   title =   {The change of surface tension with time},
   journal = {Phil. Mag.},
   volume = 24,
   pages = {864-888},
   year =  1937,
}

@book{Born69,
   author =    {Born, M.},
   title =     {Atomic Physics},
   publisher = {Dover},
   year =      1969,
}

@book{BornWolf,
   author =    {M. Born and E. Wolf},
   title =     {Principles of Optics},
   publisher = {Oxford, Pergamon},
   year =      1980,
}

@book{Goodman,
   author =    {J. W. Goodman},
   title =     {Introduction to Fourier Optics},
   publisher = {Roberts \& Company Publishers},
   year =      2004,
}

@book{Sneddon,
   author =    {I. N. Sneddon},
   title =     {Elements of Partial Differential Equations},
   publisher = {McGraw-Hill},
   year =      1957,
}

@book{Duffy,
   author =    {D. G. Duffy},
   title =     {Green's Functions with Applications},
   publisher = {Chapman \& Hall},
   year =      2001,
}

@article{Brech02,
   author =  {Br{\'e}chignac, C. and Cahuzac, Ph. and Carlier,
    F. and Colliex, C. and Leroux, J. and Masson, A. and Yoon, B. and
                 Landman, U.},
   title =   {Instability driven fragmentation of nanoscale fractal islands.},
   journal = {Phys. Rev. Letters.},
   volume = 88,
   number={19},
   pages = {196103},
   year =  2002,
}

@article{Bren07 ,
   author =  {Paruchuri, S. and Brenner, M. P.},
   title =   {Splitting of a jet.},
   journal = {Phys. Rev. Lett.},
   volume = 98,
   pages = {134502},
   year =  2007,
}

@article{Brem02,
   author =  {Bremond, N. and Clanet, C. and Villermaux, E.},
   title =   {From jets to drops via jet. },
   journal = {Bull.  Am.  Phys.  Soc.},
   volume = 47,
   number = 10,
   pages = {43},
   year =  2002,
}

@phdThesis{Brem03,
   author = {Bremond, N.},
   title =  {Stabilit? et atomisation des nappes liquides.},
   school = {Universit? de Provence, Marseille},
   year =   2003,
}

@article{Brem05 ,
   author =  {Bremond, N. and Villermaux, E.},
   title =   {Bursting thin liquid films.},
   journal = {J. Fluid Mech.},
   volume = 524,
   pages = {121-130},
   year =  2005,
}

@article{Brem05b ,
   author =  {Bremond, N. and Villermaux, E.},
   title =   {Atomization by jet impact.},
   journal = {J. Fluid Mech.},
   volume = 549,
   pages = {273-306},
   year =  2006,
}

@article{Brem07 ,
   author =  {Bremond, N. and Clanet, C. and Villermaux, E.},
   title =   {Atomization of undulated liquid sheets.},
   journal = {J. Fluid Mech.},
   volume = {585},
   pages = {421-456},
   year =  2007,
}

@article{DCDYBC07,
   author =  {V. Duclaux and F. Caille and C. Duez and
        C. Ybert and L. Bocquet and C. Clanet},
   title =   {Dynamics of transient cavities},
   journal = {J. Fluid Mech.},
   volume = {591},
   pages = {1},
   year =  2007,
}


@article{Brou02,
   author =  {Brouillette, M.},
   title =   {The Ritchtmyer-Meshkov instability.},
   journal = {Annu. Rev. Fluid Mech.},
   volume = 34,
   pages = {445-468},
   year =  2002,
}

@article{Burt05 ,
   author =  {Burton, J. C. and Waldrep, R. and Taborek, P.},
   title =   {Scaling and Instabilities in Bubble Pinch-Off.},
   journal = {Phys. Rev. Letters.},
   volume = 94,
   pages = {184502},
   year =  2005,
}



@article{Bush04 ,
   author =  {Bush, J. W. M. and Hasha, A. E.},
   title =   {On the collision of laminar jets: fluid chains and
   fishbones.},
   journal = {J. Fluid Mech.},
   volume = 511,
   pages = {285-310},
   year =  2004,
}

@book{Chan61,
   author =    {Chandrasekhar, S.},
   title =     {Hydrodynamic and hydromagnetic stability},
   publisher = {New York: Dover publication.},
   year =      1961,
}

@Article{CS97,
	author={Y.-J. Chen and P. H. Steen},
	title={Dynamics of inviscid capillary breakup: collapse and
	pinchoff of a film bridge},
	journal={J. Fluid Mech.},
	year={1997},
	volume={341},
	number={},
	pages={245--267}
}
@Article{Chou1998,
	author={W.-H. Chou and G. M. Faeth},
	title={Temporal properties of secondary drop
                        breakup in the bag breakup regime},
	journal={Int. J. Multiphase Flow},
	year={1998},
	volume={24},
	number={},
	pages={889--912}
}

@article{Clan01 ,
   author =  {Clanet, C.},
   title =   {Dynamics and stability of water bells.},
   journal = {J. Fluid Mech.},
   volume = 430,
   pages = {111-147},
   year =  2001,
}

@article{Clan02 ,
   author =  {Clanet, C. and Villermaux, E.},
   title =   {Life of a smooth liquid sheet.},
   journal = {J. Fluid Mech.},
   volume = 462,
   pages = {307-340},
   year =  2002,
}

@article{Clar72,
   author =  {Clark, D. J. and Dombrowski, N.},
   title =   {On the formation of drops from the rims of fan
   spray sheets.},
   journal = {J. Aerosol Sci.},
    volume = 3,
   pages = {173-183},
   year =    1972,
}

@article{Clay40,
   author =  {Clay, P. H.},
   title =   {The mechanism of emulsion formation in turbulent flow. 1,
                Experimental part.},
   journal = {Proc. Roy. Acad. Sci. (Amstrerdam)},
    volume = 43,
   pages = {852-865},
   year =    1940,
}

@article{Clou94,
   author =  {Cloupeau, M. and Prunet-Foch, B.},
   title =   {Electrodynamic spraying functioning modes: a critical review},
   journal = {J. Aerosol Sci},
    volume = 25,
    number = 6,
   pages = {1021-1036},
   year =    1994,
}



@Article{Cohen1990,
	author={R. D. Cohen},
	title={Steady-state Cluster Size Distribution in Stirred Suspensions},
	journal={J. Chem. Soc. Faraday Trans.},
	year={1990},
	volume={86},
	number={12},
	pages={2133--2138}
}
@Article{Cohen1991,
	author={R. D. Cohen},
	title={Shattering of a liquid drop due to impact},
	journal={Proc. R. Soc. London},
	year={1991},
	volume={A},
	number={435},
	pages={483--503}
}

@article{Culi60,
   author =  {Culick, F. E. C.},
   title =   {Comments on a  ruptured soap film.},
   journal = {J. Appl. Phys.},
   volume = 31,
   pages = {1128},
   year =  1960,
}

@article{Choo01,
   author =  {Choo,Y. J. and Kang,B. S.},
   title =   {Parametric study on impinging-jet liquid sheet
   thickness distribution using an interferometric method.},
   journal = {Exp. Fluids},
   volume = 31,
   pages = {56-62},
   year =  2001,
}

@article{Choo02,
   author =  {Choo,Y. J. and Kang,B. S.},
   title =   {The velocity distribution of the liquid sheet
   formed by two low-speed impinging jets.},
   journal = {Phys. Fluids},
   volume = 14,
   pages = {622-627},
   year =  2002,
}

@article{Clanet99,
   author =  {Clanet, C. and Lasheras, J.},
   title =   {Transition from dripping to jetting.},
   journal = {J. Fluid Mech.},
   volume = 383,
   pages = {307},
   year =  1999,
}

@article{SB05,
   author =  { U. S. Sauter and H. W. Buggisch},
   title =   {Stability of initially slow viscous jets driven by gravity},
   journal = {J. Fluid Mech.},
   volume = 533,
   pages = {237},
   year =  2005,
}

@article{Cheong,
   author =  { B. S. Cheong and T. Howes},
   title =   { Capillary jet instability under the influence of gravity},
   journal = {Chem. Engin. Science},
   volume = {59},
   pages = {2145},
   year =  2004,
}

@article{HOOPS05,
   author =  { S. D. Howison and J. R. Ockendon and J. M. Oliver and
                R. Purvis and F. T. Smith},
   title =   {Droplet impact on a thin fluid layer},
   journal = {J. Fluid Mech.},
   volume = {542},
   pages = {1},
   year =  2005,
}

@article{W32,
   author =  { H. Wagner},
   title =   {{\"U}ber Sto{\ss}- und {G}leitvorg{\"a}nge an der
               Oberfl{\"a}che von Fl{\"u}ssigkeiten},
   journal = {ZAMM},
   volume = {12},
   pages = {193},
   year =  {1932}
}

@article{SBohr05,
   author =  { S. Senchenko and T. Bohr},
   title =   { Shape and stability of a viscous thread},
   journal = {Phys. Rev. E},
   volume = {71},
   pages = {056301},
   year =  2005,
}

@article{CH05,
   author =  { B. S. Cheong and T. Howes},
   title =   { Effect of initial disturbance amplitude in gravity affected
                 jet breakup},
   journal = {Chem. Engin. Science},
   volume = {60},
   pages = {3715},
   year =  2005,
}

@article{Coula77,
   author =  {Coulaloglou, C. A. and Tavlarides, L. L.},
   title =   {Description of interaction processes in agitated
            liquid-liquid dispersions.},
   journal = {Chem. Eng. Sci.},
   volume = 32,
   pages = {1289-1297},
   year =  1977,
}

@book{Couls68,
   author =    {Coulson, J. M. and Richardson, J. F.},
   title =     {Chemical Engineering.},
   publisher = {Pergamon Press},
   year =      1968,
}

@article{Crapp73 ,
   author =  {Crapper, G. D. and Dombrowski, N. and Jepson, W. P.
   and Pyott, G. A. D.},
   title =   {A note on the growth of Kelvin-Helmholtz waves on
   thin liquid sheets.},
   journal = {J. Fluid Mech.},
   volume = 57,
   pages = {671-672},
   year =  1973,
}

@article{Dean02 ,
   author =  {Dan, G. B. and Stokes, M. D.},
   title =   {Scale dependence of bubble creation mechanisms in
       breaking waves.},
   journal = {Nature},
   volume = 418,
   pages = {839-844},
   year =  2002,
}
@book{deGe02,
   author =    {de Gennes, P.-G. and Brochart-Wyart, F. and
   Qu{\'e}r{\'e} D.},
   title =     {Gouttes, bulles, perles et ondes.},
   publisher = {Belin},
   year =      2002,
}

@article{Della05 ,
   author =  {Della Porta, G. and De Vittori, C. and Reverchon, E.},
   title =   {Supercritical Assisted Atomization: A Novel Technology
       for Microparticles Preparation of an Asthma-controlling Drug .},
   journal = {AAPS PharmSciTech},
   volume = 6,
   number={3},
   pages = {E421-E428},
   year =  2005,
}

@article{Der91,
   author =  {Derrida, B. and Godr{\`e}che, C. and Yekutieli, I.},
   title =   {Scale-invariant regimes in one-dimensional models
        of growing and coalescing droplets},
   journal = {Phys. Rev. A},
   volume = 44,
   number={10},
   pages = {6241-6251},
   year =  1991,
}

@article{DeVega96,
   author =  {Derrida, B. and Godr{\`e}che, C. and Yekutieli, I.},
   title =   {Self-gravity as an explanation of the fractal
          structure of the  interstellar medium},
   journal = {Nature},
   volume = 383,
   number={},
   pages = {56-58},
   year =  1996,
}

@article{vega,
   author =  {S. Guti errez and J. Rivas and L. Vega},
   title =   {Formation of singularities and self-similar vortex
             motion under the localized induction approximation},
   journal = {Comm. Part. Di . Eq.},
   volume = 28,
   pages = {927-968},
   year =  2003,
}

@article{Ignat,
   author =  {L. Ignat and C. Lefter and V. D. Radulescu},
   title =   {Minimization of the renormalized energy in the unit ball
             of $\boldsymbol{R}^{2}$},
   journal = {Nieuw Arch. Wiskd.},
   volume = 1,
   pages = {278-280},
   year =  2000
}

@article{PR91,
   author =  {L. M. Pismen and J. Rubinstein},
   title =   {Motion of vortex lines in the Ginzburg-Landau model},
   journal = {Physica D},
   volume = 47,
   pages = {353--360},
   year =  1991,
}

@article{Neu,
   author =  {J. C. Neu},
   title =   {Vortices in complex scalar fields},
   journal = {Physica D},
   volume = 43,
   pages = {385--406},
   year =  1990
}

@article{Lin,
   author =  {F.-H. Lin and J. X. Xin},
   title =   {On the dynamical law of the Ginzburg-Landau vortices
            on the plane},
   journal = {Comm. Pure Appl. Math.},
   volume = 52,
   pages = {1189--1212},
   year =  1999,
}

@article{Serfaty,
   author =  {E. Sandier and S. Serfaty},
   title =   {Gamma-convergence of gradient flows with applications to
            Ginzburg-Landau},
   journal = {Comm. Pure Appl. Math.},
   volume = 57,
   pages = {1627-1672},
   year =  2004,
}

@Book{Brezis,
   author =  {F. Bethuel and H. Brezis and F. H{\'{e}}lein},
   title =   {Ginzburg-Landau Vortices},
   publisher = {Birkh{\"{a}}user, Boston},
   year =  1994
}

@Article{Dimotakis1986,
	author={P. E. Dimotakis},
	title={Two-dimensional shear layer entrainment},
	journal={AIAA},
	year={1986},
	volume={24},
	number={11},
	pages={1791--1796}
}

@Article{Hagan,
	author={P. S. Hagan},
	title={Spiral waves in reaction-diffusion equations},
	journal={SIAM J. Appl. Math.},
	year={1982},
	volume={42},
	pages={762--786}
}

@Article{Maria,
	author={M. Aguareles and S. J.\ Chapman and T. Witelski},
	title={Motion of spiral waves in the Complex Ginzburg-Landau
               equation},
	journal={Physica D},
	year={2010},
	volume={},
	pages={}
}

@Article{Chapman,
	author={S. J. Chapman},
	title={A hierarchy of models for type-II superconductors},
	journal={SIAM Review},
	volume={42},
	pages={555-598},
	year={2000},
}

@Article{BC89,
	author={M. S. Berger and Y. Y. Chen},
	title={Symmetric vortices for the nonlinear Ginzburg-Landau
   equations of superconductivity and the nonlinear desingularization
           phenomenon},
	journal={J. Funct. Anal.},
	volume={82},
	pages={259-295},
	year={1989}
}

@Article{Abri,
	author={A. A. Abrikosov},
	title={On the magnetic properties of superconductors of the
             second group},
	journal={Soviet Physics JETP},
	volume={5},
	pages={1174},
	year={1957}
        }

@book{Dirac,
   author =    {Dirac, P. A. M.},
   title =     {The principles of quantum mechanics.},
   publisher = {Oxford University Press},
   year =      1958,
}

@article{Domb54,
   author =  {Dombrowski, N. and Fraser, R. P.},
   title =   {A photographic investigation into the
   disintegration of liquid sheets.},
   journal = {Phil. Trans. A},
   volume = 247,
   pages = {101-130},
   year =  1954,
}

@article{Domb60,
   author =  {Dombrowski, N. and Hasson, D. and Ward, D. E.},
   title =   {Some aspects of liquid through fan spray nozzles.},
   journal = {Chem. Eng. Sci.},
   volume = 12,
   pages = {35-50},
   year =  1960,
}

@article{Domb63,
   author =  {Dombrowski, N. and Jonhs, W. R.},
   title =   {The aerodynamics instability and disintegration of
   viscous liquid sheets.},
   journal = {Chem. Eng. Sci.},
   volume = 18,
   pages = {203-214},
   year =  1963,
}

@article{DombHooper63,
   author =  {Dombrowski, N. and Hooper, P. C.},
   title =   {A study of the sprays formed by impinging jets in
   laminar and turbulent flow.},
   journal = {J. Fluid Mech.},
   volume = 18,
   pages = {392-400},
   year =  1963,
}

@article{Domb74,
   author =  {Dombrowski, N. and Neale, N. D.},
   title =   {Formation of streams of uniform drops from fan
   spray pressure nozzles.},
   journal = {J. Aerosol Sci.},
    volume = 5,
   pages = {551-555},
   year =    1974,
}

@article{Doua90,
   author =  {Douady, S.},
   title =   {Experimental study of the Faraday instability.},
   journal = {J. Fluid Mech.},
   volume = 221,
   pages = {383-409},
   year =  1990,
}

@book{Draz81,
   author =    {Drazin, P. G. and Reid, W. H.},
   title =     {Hydrodynamic stability},
   publisher = {Cambridge University Press, Cambridge},
   year =      1981,
}

@book{Draz92,
   author =    {Drazin},
   title =     {Nonlinear systems},
   publisher = {Cambridge University Press, Cambridge},
   year =      1992,
}

@article{Ducl06,
   author =  {Duclaux, V. and Clanet, C. and Qu{\'e}r{\'e} D.},
   title =   {The effects of gravity on the capillary instability in tubes.},
   journal = {J. Fluid Mech.},
   volume = 556,
   pages = {217-226},
   year =  2006,
}

@article{Dupr68,
   author =  {Dupr{\'e}, A.},
   title =   {Th{\'e}orie m{\'e}canique de la chaleur.},
   journal = {Ann. de chim. Phys.},
   volume = 11,
   pages = {194},
   year =  1868,
}

@article{eaton94,
	author={Eaton, J. K. and Fessler, J. R.},
	title={Preferential Concentration of Particles by Turbulence.},
	journal={Int. J. Mult. Flows.},
	year={1994},
	volume={20},
	pages={169--209}

}

@article{Engl91,
   author =  {Englman, R.},
   title =   {Fragments of matter from maximum-entropy viewpoint.},
   journal = {J. Phys.: Condens. Matter},
   volume = 3,
   pages = {1019-1053},
   year =  1991,
}


@article{Eins64,
   author =  {Einsenklam, P.},
   title =   {On ligament formation from spinning disks and cups.},
   journal = {Chem. Eng. Sci.},
   volume = 19,
   pages = {693-694},
   year =  1964,
}

@article{Eins61,
   author =  {Einsenklam, P.},
   title =   {Atomisation of liquid fuel for combustion.},
   journal = {J. Inst. fuel},
   volume = 0,
   pages = {130-143},
   year =  1961,
}

@article{Elb94,
   author =  {Elbaum, M. and Lipson, S. G.},
   title =   {How does a thin wetted film dry up?},
   journal = {Phys. Rev. Letters},
   volume = 72,
   number={22},
   pages = {3562-3565},
   year =  1994,
}

@article{Enge95,
   author =  {Engelbert, C. and Hardalupas, Y. and Whitelaw, J. H.},
   title =   {Breakup phenomena in coaxial airblast atomizers},
   journal = {Proc. Roy. Soc.},
   volume = 451,
   pages = {189-229},
   year =  1995,
}


@Article{Eroglu&Chigier&Farago1991,
	author={H. Eroglu and N. Chigier and Z. Farag\'o},
	title={Coaxial atomizer intact lengths},
	journal={Phys. Fluids A},
	year=1991,
	volume=3,
	number=2,
	pages={303--308}
}
@Article{Eroglu&Chigier1991,
	author={H. Eroglu and N. Chigier},
	title={Wave characteristics of liquid jets from airblast
              coaxial atomizers},
	journal={Atom. and Sprays},
	year=1991,
	volume=1,
	pages={349--366}
}


@Article{Faith1995,
	author={Faeth, G. M. and Hsiang, L.-P. and Wu, P.-K.},
	title={Structure and Breakup propreties of Sprays},
	journal={Int. J. Multiphase Flows},
	year={1995},
	volume={21},
	pages={99--127}
}


@Article{Falko02,
	author={Falkovich, G. and Fouxon, A. and Stepanov, M. G.},
	title={Acceleration of rain initiation by turbulence},
	journal={Nature},
	year={2002},
	volume={419},
	pages={151--154}
}


@Article{Farago&Chigier1992,
	author={Z. Farag\'o and N. Chigier},
	title={Morphological classification of disintegration of round liquid
	jets in a coaxial air stream},
	journal={Atom. and Sprays},
	year={1992},
	volume={2},
	number={},
	pages={137--153}
}


@article{Fara91,
   author =  {Farago, Z. and Chigier, N.},
   title =   {Morphological classification of disintegration of
   round liquid jets in a coaxial air stream.},
   journal = {Atom. and Sprays},
   volume = 2,
   pages = {137-153},
   year =  1991,
}

@book{Fell71,
   author =    {Feller, W.},
   title =     {An introduction to probability theory and its
   applictions},
   publisher = {Wiley},
   year =      1971,
}

@article{Fish67,
   author =  {Fisher, M. E.},
   title =   {The theory of condensation and the critical point},
   journal = {Physics},
   volume = 3,
   pages = {255-283},
   year =  1967,
}


@article{Fran85,
   author =  {Frankel, I. and Weihs, D.},
   title =   {Stability of a capillary jet with linearly
   increasing axial velocity (with application to shaped charge). },
   journal = {J. Fluid Mech.},
   volume = 155,
   pages = {289-307},
   year =  1985,
}

@article{Fras62,
   author =  {Fraser, R. P. and Eisenklam, P. and Dombrowski, N.
   and Hasson, D.},
   title =   {Drop formation from rapidly moving liquid sheet.},
   journal = {A. I. Ch. E. Journal},
   volume = 8,
   pages = {672-680},
   year =  1962,
}

@article{Fras63,
   author =  {Fraser, R. P. and Dombrowski, N. and Routley, J. H.},
   title =   {Thin filming of liquids by spinning cups.},
   journal = {Chem. Eng. Sci.},
   volume = 18,
   pages = {323-337},
   year =  1963,
}

@article{Fried66,
   author =  {Friedlander, S. K. and Wang, C. S.},
   title =   {The self-preserving particle size distribution for
       coagulation by brownian motion.},
   journal = {J. Coll. Int. Sci.},
   volume = 22,
   pages = {126-132},
   year =  1966,
}

@book{Frie00,
   author =    {Friedlander, S. K.},
   title =     {Smoke, dust and haze.},
   publisher = {Oxford University press.},
   year =      2000,
}

@article{Frisch97,
   author =  {Frisch, U. and Sornette, D.},
   title =   {Extreme deviations and applications.},
   journal = {J. Phys.I France},
   volume = 7,
   pages = {1155-1171},
   year =  1997,
}

@article{Sor98,
   author =  {D. Sornette},
   title =   {Discrete-scale invariance and complex dimensions},
   journal = {Phys. Rep.},
   volume = 297,
   pages = {239-270},
   year =  1998,
}

@article{Sor03,
   author =  {D. Sornette},
   title =   {Critical market crashes},
   journal = {Phys. Rep.},
   volume = 378,
   pages = {1-98},
   year =  2003,
}

@article{HE97,
   author =  {E. W. Hirschmann and D. M. Eardley},
   title =   {Criticality and bifurcation in the gravitational
      collapse of a self-coupled scalar field},
   journal = {Phys. Rev. D},
   volume = 56,
   pages = {4696-4705},
   year =  1997,
}

@article{ABT06,
   author =  {P. C. Aichelburg and P. Bizon and Z. Tabor},
   title =   {Bifurcation and fine structure phenomena in
       critical collapse of a self-gravitating $\sigma$-field},
   journal = {Class. Quant. Grav.},
   volume = 23,
   pages = {S299-S306},
   year =  2006,
}

@article{MG03,
   author =  {J. M. Martin-Garcia and C. Gundlach},
   title =   {Global structure of Choptuik's critical solution
           in scalar field collapse},
   journal = {Phys. Rev. D},
   volume = 68,
   pages = {024011},
   year =  2003,
}

@article{MG07,
   author =  {J. M. Martin-Garcia and C. Gundlach},
   title =   {Critical phenomena in gratiational collapse},
   journal = {Living Rev. Rel.},
   volume = 10,
   pages = 5,
   url       = "http://www.livingreviews.org/lrr-2007-5",
   year =  2007,
}

@article{Gund03,
   author =  {C. Gundlach},
   title =   {Critical phenomena in gravitational collapse},
   journal = {Phys. Rep.},
   volume = 376,
   pages = {339-405},
   year =  2003,
}

@article{C93,
   author =  {M. W. Choptuik},
   title =   {Universality and scaling in gravitational collapse
   of a massless scalar field},
   journal = {Phys. Rev. Lett.},
   volume = 70,
   pages = {9},
   year =  1993,
}

@article{Full99,
   author =  {Fullana, J. M. and Zaleski, S.},
   title =   {Stability of a growing end rim in a liquid sheet of
   uniform thickness.},
   journal = {Phys. Fluids},
   volume = 11,
   pages = {952-954},
   year =  1999,
}

@article{Funf01 ,
   author =  {Funfschilling, D. and Plaut, E. and {Skali Lami}, S.},
   title =   {Etude exp?rimentale des instabilit?s des jets
   liquides plans.},
   journal = {Compte rendu du XV?me congr?s fran?ais de
   m?canique, Nancy},
   volume = 635,
   year =  2001,
}

@Article{Ganan-Calvo1998,
	author={A. M. Ga{\~n}{\'a}n-Calvo},
	title={Generation of Steady Liquid Microthreads and Micro-Sized
	Monodisperse Sprays in Gas Streams},
	journal={Phys. Rev. Lett.},
	year={1998},
	volume={80},
	number={2},
	pages={285--288}
}

@Article{Ganan-Calvo1999,
	author={A. M. Ga{\~n}{\'a}n-Calvo},
	title={The Surface Charge in Electrospraying:
              Its Nature and Its Universal Scaling Laws},
	journal={J. Aerosol Sci.},
	year={1999},
	volume={30},
	pages={863-872}
}

@article{Gast62,
   author =  {Gaster,M.},
   title =   {A note on the relation between
   temporally-increasing and spatially-increasing disturbances
   in hydrodynamic stability.},
   journal = {J. Fluid Mech.},
   volume = 14,
   pages = {222-224},
   year =  1962,
}

@Article{Gaudet&McKinley&Stone1996,
	author={S. Gaudet and G. H. McKinley and H. A. Stone},
	title={Extensional deformation of Newtonian liquid bridges},
	journal={Phys. Fluids},
	year={1996},
	volume={8},
	number={10},
	pages={2568--2579}
}

@Article{Gladd05,
	author={Gladden, J. R. and Handzy, N. Z. and Belmonte, A.
           and Villermaux, E.},
	title={Dynamic buckling and fragmentation in brittle rods},
	journal={Phys. Rev. Letters},
	year={2005},
	volume={94},
	pages={035503}
}

@article{Good96,
   author =  {Goodridge, C. L. and Shi, W. T. and Lathrop, D. P.},
   title =   {Treshold dynamics of singular gravity-capillary waves},
   journal = {Phys. Rev. Lett.},
   volume = 76,
   pages = {1824-1826},
   year =  1996,
}

@article{Gord01,
   author =  {J. M. Gordillo and M. P{\'e}rez-Saborid and
         A. M. Ga{\~n}{\'a}n-Calvo},
   title =   {Linear stability of co-flowing liquid-gas jets},
   journal = {J. Fluid Mech.},
   volume = 541,
   pages = {23--51},
   year = 2001
}

@article{Gord05b,
   author =  {J. M. Gordillo and M. P{\'e}rez-Saborid},
   title =   {Aerodynamic effects in the breakup of liquid jets:
      on the first wind-induced breakup regime},
   journal = {J. Fluid Mech.},
   volume = 541,
   pages = {1--20},
   year = 2005
}


@article{Gore62,
   author =  {Goren, S. L.},
   title =   {The instability of an annular thread of fluid.},
   journal = {J. Fluid Mech.},
   volume = 12,
   number = 2,
   pages = {309--319},
   year = 1962,
}



@article{Goro03,
   author =  {Gorokhovski, M. A. and Saveliev, V. L.},
   title =   {Analyses of Kolmogorov's model of breakup and its
      application into Lagrangian computation of liquid sprays
         under air-blast atomization.},
   journal = {Phys. Fluids},
   volume = 15,
   number={1},
   pages = {184-192},
   year =  2003,
}

@article{Grad85,
   author =  {Grady, D. E. and Kipp, M. E.},
   title =   {Geometric statistics and dynamic fragmentation.},
   journal = {J. Appl. Phys.},
   volume = 58,
   number={3},
   pages = {1210--1222},
   year =  1985,
}
@article{Gran66,
   author =  {Grant, R. P. and Middleman, S.},
   title =   {Newtonian Jet Stability.},
   journal = {AICHE J.},
   volume = 12,
   number={4},
   pages = {669--678},
   year =  1966,
}

@article{Hage55 ,
   author =  {Hagerty, W. W. and Shea, J. F.},
   title =   {A study of the stability of plane fluid sheets.},
   journal = {J. Appl. Mech.},
   volume = 22,
   pages = {509-514},
   year =  1955,
}

@Article{Hanson&al1963,
	author={A. R. Hanson and E. G. Domich and H. S. Adams},
	title={Shock tube investigation of the break-up of drops by air
	blasts},
	journal={Phys. Fluids},
	year={1963},
	volume={6},
	number={8},
	pages={1070--1080}
}

@Article{GB54,
	author={W. C. Griffith and W. Bleakney},
	title={Shock waves in gases},
	journal={Amer. J. Phys.},
	year={1954},
	volume={22},
	pages={597}
}

@article{Hark19,
   author =  {Harkins, W. D. and Brown, F. E.},
   title =   {The determination of surface tension (free surface
   energy), and the weight of falling drops: the surface tension
   of water and benzene by the capillary height method.},
   journal = {J. Am. Chem. Soc.},
   volume = 41,
   pages = {499-524},
   year =  1919,
}

@article{Hash02,
   author =  {Hasha, A. E. and Bush, J. W. M.},
   title =   {Fluid fishbones.},
   journal = {Phys. Fluids : Gallery of fluid Motion},
   volume = 14,
   pages = {8},
   year =  2002,
}

@article{Hass64,
   author =  {Hasson, D. and Peck,R. E.},
   title =   {Thickness distribution in a sheet formed by impinging jets.},
   journal = {AIChE J.},
   volume = 10,
   pages = {752-754},
   year =  1964,
}

@Article{Henderson&al2000,
	author={D. Henderson and H. Segur and L. B. Smolka and M.
	Wadati},
	title={The motion of a falling liquid filament},
	journal={Phys. Fluids},
	year={2000},
	volume={12},
	number={3},
	pages={550--565}
}
@Article{Henderson&Miles1990,
	author={D. Henderson and J. Miles},
	title={Single-mode Faraday waves in small cylinder},
	journal={J. Fluid Mech.},
	year={1990},
	volume={213},
	pages={95-109}
}


@article{Hend89,
   author =  {Henderson, L. F.},
   title =   {On the refraction of shock waves.},
   journal = {J. Fluid Mech.},
   volume = 198,
   pages = {365-386},
   year =  1989,
}


@article{Heid57,
   author =  {Heidmann, M. F. and Priem, R. J. and Humphrey, J. C.},
   title =   {A study of sprays formed by two impacting jets.},
   journal = {N. A. C. A. Tech. note number 3835},
   year =  1957,
}


@article{Helmholtz,
   author =  {von Helmholtz, H. },
   title =   {On discontinuous movements of fluids.},
   journal = {Philosophical magazine},
   volume = 36,
   pages = {337-346},
   year =  1868,
}

@article{W72,
   author =  {F. J. Wegner},
   title =   {Corrections to Scaling Laws},
   journal = {Phys. Rev. B},
   volume = {5},
   pages = {4529 - 4536},
   year =  1972,
}

@article{EFLS07,
   author =  {J. Eggers and M. A. Fontelos and D. Leppinen and
           J. H. Snoeijer},
   title =   {Theory of the collapsing axisymmetric cavity},
   journal = {Phys. Rev. Lett.},
   volume = 98,
   pages = 094502,
   year =  2007,
}

@article{GSLM09,
   author =  {S. Gekle and J. H. Snoeijer
        and D. Lohse and D {van der Meer}},
   title =   {Approach to universality in axisymmetric bubble pinch-off},
   journal = {Phys. Rev. E},
   volume = 80,
   pages = 036305,
   year =  2009,
}

@article{EF09,
   author =  {J. Eggers and M. A. Fontelos},
   title =   {The role of self-similarity in singularities of
             partial differential equations},
   journal = {Nonlinearity},
   volume = {22},
   pages = {R1},
   year =  {2009}
}

@article{FSE07,
   author =  {M. A. Fontelos and J. Eggers and
           J. H. Snoeijer},
   title =   {The spatial structure of a collapsing cavity},
   journal = {unpublished},
   year =  2007,
}

@article{Hey33,
   author =  {Heywood, H. },
   title =   {Characteristics of pulverized fuels.},
   journal = {The Institute of fuel},
   volume = {VI},
   pages = {241-248},
   year =  1933,
}


@article{Hil01,
   author =  {S. Hilgenfeldt and A. M. Kraynik and
                    S. A. Koehler and H. A. Stone},
   title =   {An accurate von Neumann's law for three-dimensional foams},
   journal = {Phys. Rev. Lett.},
   volume = 86,
   pages = {2685-2688},
   year =  2001,
}


@Article{Hinze1949,
	author={J. O. Hinze},
	title={Critical speeds and sizes of liquid globules},
	journal={Appl. Sci. Res.},
	year={1949},
	volume={A1},
	pages={273--288}
}


@article{Hinz50 ,
   author =  {Hinze, J. O. and Milborn, H.},
   title =   {Atomization of liquid by means of a rotating cup.},
   journal = {Trans. ASME : J. Appl. Mech.},
   volume = 17,
   pages = {145-153},
   year =  1955,
}

@Article{Hinze55,
	author={J. O. Hinze},
	title={Fundamentals of the hydrodynamic mechanism of
        splitting in dispersion processes},
	journal={AIChE J.},
	year={1949},
	volume={1},
	number = {3},
	pages = {289--295}
}

@InCollection{Hiroyasu82,
	author={Hiroyazu, H. and Shimizu, M. and Arai, M.},
	title={The breakup speed of high speed jet in a
         high pressure gaseous atmosphere},
	booktitle ={Proceedings of the 2nd Conference on Liquid
            Atomization and Spray Systems},
	publisher={Madison, Wisconsin},
	year={1982},
	pages = {69--74}
}

@article{HoHu84,
   author =  {Ho, C. M. and Huerre, P.},
   title =   {Perturbed free shear layers.},
   journal = {Annu. Rev. Fluid Mech.},
   volume = 16,
   pages = {365-424},
   year =  1984,
}

@article{Hoyt77,
   author =  {Hoyt, J. W.  and Taylor, J.},
   title =   {Waves on water jets.},
   journal = {J. Fluid Mech. },
   volume = 83,
   pages = {119-},
   year =  1977,
}

@Article{Hu&Pine&Leal2000,
	author={Y. T. Hu and D. J. Pine and L. G. Leal},
	title={Drop deformation, breakup, and coalescence with compatibilizer},
	journal={Phys. Fluids},
	year={2000},
	volume={12},
	number={3},
	pages={484--489}
}
@Article{Hu&Scriven1969,
	author={C. Huh and L. E. Scriven},
	title={Shapes of axisymmetric fluid interfaces of unbounded
	extent},
	journal={J. Colloid Interface Sci.},
	year={1969},
	volume={30},
	number={},
	pages={323--337}
}

@Article{Huebner71,
	author={Huebner, A. L. and Chu, H. N.},
	title={Instability and breakup of charged liquid jets},
	journal={J. Fluid Mech.},
	year={1971},
	volume={49},
	number={2},
	pages={361--372}
}


@article{Huan70,
   author =  {Huang, J. C. P.},
   title =   {The break-up of axisymmetric liquid sheets.},
   journal = {J. Fluid Mech.},
   volume = 43,
   pages = {305-319},
   year =  1970,
}

@inproceedings{Huerre&Rossi,
	author={Huerre, P. and Rossi, M.},
	title={},
	booktitle={Hydrodynamics and Nonlinear Instabilities},
	year={1998},
	editor={Godr{\`e}che, C. and Manneville, P.},
	pages={81--386},
	volume={},
	series={},
	organization={},
	publisher={Ala Saclay},
	address={},
	month={},
	note={}
}


@article{Ibra91,
   author =  {Ibrahim, E. A. and Przekwas, A. J.},
   title =   {Impinging jets atomization.},
   journal = {Phys. Fluids A},
   volume = 3,
   pages = {2981-2987},
   year =  1991,
}

@article{Ibra98,
   author =  {Ibrahim, E. A.},
   title =   {Instability of a liquid sheet of parabolic
   velocity profile.},
   journal = {J. Fluid Mech.},
   volume = 10,
   pages = {1034-1036},
   year =  1998,
}

@article{Jame03,
   author =  {James, A. J. and Vukasinovic, B. and Smith, M. K.
             and Glezer, A.},
   title =   {Vibration-induced drop atomization and bursting.},
   journal = {J. Fluid Mech.},
   volume = 476,
   pages = {1-28},
   year =  2003,
}

@Article{Jeans02,
	author={Jeans, J.},
	title={Stability of a spherical nebulae},
	journal={Phil. Trans. R. Soc. London A},
	year={1902},
	volume={199},
	number={},
	pages={1--53}
}


@Article{Jeffreys1925,
	author={H. Jeffreys},
	title={On the formation of water wave by wind},
	journal={Proc. R. Soc. London, Ser. A},
	year={1925},
	volume={107},
	number={},
	pages={189}
}

@Article{Joseph&al1999,
	author={D. D. Joseph and J. Belanger and G. S. Beavers},
	title={Breakup of a liquid drop suddenly exposed to a high-speed
	airsteam},
	journal={Int. J. Multiphase Flow},
	year={1999},
	volume={25},
	number={},
	pages={1263--1303}
}
@Article{Josser06,
	author={Bartolo, D. and Josserand, C. and Bonn, D.},
	title={Singular jets and bubbles in drop impact},
	journal={Phys. Rev. Lett.},
	year={2006},
	volume={96},
	pages={124501}
}
@Article{Kapur1983,
	author={J. N. Kapur},
	title={Twenty-five years of maximum-entropy principle},
	journal={Jour. Math. Phy. Sci.},
	year={1983},
	volume={17},
	number={2},
	pages={103--156}
	}
	
	
	
@book{Kapur1989,
   author =    {Kapur, J. N.},
   title =     {Maximum Entropy models in Science and engineering.},
   publisher = {John Wiley \& Sons.},
   year =      1989,
}



@Article{Keller1983,
	author={J. B. Keller},
	title={Breaking of liquid films and liquid threads},
	journal={Phys. Fluid},
	year={1983},
	volume={26},
	number={12},
	pages={3451--3453}
	}

@article{Kell54,
   author =  {Keller, J. B. and Kolodner, I.},
   title =   {Instability of liquid surfaces and the formation of
   drops.},
   journal = {J. Appl. Phys.},
   volume = 25,
   pages = {918-921},
   year =  1954,
}

@article{Kell83,
   author =  {Keller, J. B.},
   title =   {Breaking of liquid films and threads.},
   journal = {Phys. Fluids},
   volume = 26,
   pages = {3451-3453},
   year =  1983,
}

@Article{Keller&Miksis1983,
	author={Keller, J. B. and Miksis, M. J.},
	title={Surface tension driven flows},
	journal={SIAM J. Appl. Maths},
	year={1983},
	volume={43},
	number={},
	pages={268--277}
}

@article{Kelvin,
   author =  {Kelvin, Lord},
   title =   {Hydrokinetic solutions and observations.},
   journal = {Philosophical magazine},
   volume = 42,
   pages = {362-377},
   year =  1871,
}


@article{Kim00,
   author =  {Kim, I. and Sirignano, W. A.},
   title =   {Three-dimensional wave distortion and disintegration
        of thin planar liquid sheets.},
   journal = {J. Fluid Mech.},
   volume = 410,
   pages = {147-183},
   year =  2000,
}

@article{Kend86,
   author =  {Kendall, J. M.},
   title =   {Experiments on annular liquid jet instability
      and on the formation of liquid shells},
   journal = {Phys. Fluids},
   volume = 29,
   pages = {2086-2094},
   year =  1986,
}

@article{Kita86,
   author =  {Kitamura, Y. and Takahashi, T.},
   title =   {Stability of jets in liquid-liquid systems.},
   journal = {Encyclopedia of Fluid Mechanics},
   volume = 2,
   number = 19,
   pages = {474--510},
   year =  1986,
}

@article{Kolmogorov1941b,
	author={A. N. Kolmogorov},
	title={?ber das logarithmish normale verteilungsgesetz der
	dimensionen der teilchen bei zerst?ckelung},
	journal={Dok. Akad. Nauk SSSR},
	year={1941},
	volume={31},
	number={2},
	pages={99--101}
}

@article{Kolmogorov1941,
	author={Kolmogorov, A. N.},
	title={On the Lognormal distribution of the fragment sizes
	under grinding},
	journal={Dok. Akad. Nauk SSSR},
	year={1941},
	volume={31},
	number={2},
	pages={99--101}
}	
@article{K62,
	author={Kolmogorov, A. N.},
	title={A refinment of previous hypothesis concerning the
        local structure of turbulence in a viscous incompressible
           fluid at high Reynold numbers},
	journal={J. Fluid Mech.},
	year={1962},
	volume={13},
	pages={82}
}	
@article{Kolmogorov1949,
	author={Kolmogorov, A. N.},
	title={On the breakage of drops in a turbulent flow},
	journal={Dok. Akad. Nauk SSSR},
	year={1949},
	volume={66},
	number={5},
	pages={825--828}
}
@book{Tikhomirov1991,
    author={V. M. Tikhomirov},
	title={Selected Works of A. N. Kolmogorov :
                           Mathematics and Mechanics (Mathematics
                           and Its Applications. Soviet Series, 25)},
	publisher={Klewer Acad. Pale},
	address={Dordrecht},
	year={1991}
}



@article{Komba64,
	author={Kombayasi, M. and Gonda, T. and Isono, K.},
	title={Life time of Water drops before breaking
         and size distribution of fragment droplets},
	journal={J. Met. Soc. Japan},
	year={1964},
	volume={42},
	number={5},
	pages={330--340}
}



@Article{Konno83,
	author={M. Konno and M. Aoki and S. Saito},
	title={Scale effect on breakup process in liquid-liquid agitated tanks.},
	journal={J. Chem. Engin. Japan},
	year={1983},
	volume={16},
	number={4},
	pages={313--319}
}


@Article{Krzeczkowski1980,
	author={S. A. Krzeczkowski},
	title={Measurement of liquid droplet mechanism},
	journal={Int. J. Multiphase Flow},
	year={1980},
	volume={6},
	pages={227--239}
}


@conference{Kruh03,
   author =    {Kr?hsel, G.},
   title =     {Development of 55kg/s ethanol/LOX rocket steam
   generator-accompanying combustion stability study},
   number = 5044,
   booktitle = {AIAA, 39th Joint Propulsion Conference and Exhibit},

   year =      2003,
}




@article{Kric94,
   author =  {Krichevsky, O. and Stavans, J.},
   title =   {Surfactant-polymer interactions in freely
   suspended lyotropic films.},
   journal = {Phys. Rev. Lett.},
   volume = 73,
   pages = {696-699},
   year =  1994,
}

@Article{lagu04,
	author={Lagutkin, S. and Achelis, L. and Sheikhaliev, S.
           and Uhlenwinkel, V. and Srivastava, V.},
	title={Atomization process for metal powder},
	journal={Material science and engineering A},
	year={2004},
	volume={383},
	pages={1--6}
}	

@book{Lamb32,
   author =    {Lamb, H.},
   title =     {Hydrodynamics, 6th edition.},
   publisher = {Cambridge University Press, Cambridge},
   year =      1932,
}

@book{Milne,
   author =    {L. M. Milne-Thompson},
   title =     {Theoretical Hydrodynamics, 4th edition.},
   publisher = {Macmillan \& Co},
   year =      1962,
}

@Article{Lane1951,
	author={W. R. Lane},
	title={Shatter of drops in streams of air},
	journal={Industrial and Engineering Chemistry},
	year={1961},
	volume={43},
	number={6},
	pages={1312--1317}
}	

@article{Lang62,
   author =  {Lang, R. J.},
   title =   {Ultrasonic atomization of liquids.},
   journal = {J. Acoust. Soc. Am.},
   volume = 34,
   pages = {6-8},
   year =  1962,
}

@Article{Lasheras&Villermaux&Hopfinger1998,
	author={J. C. Lasheras and E. Villermaux and E. J. Hopfinger},
	title={Breakup and atomisation of a round water jet by a high-speed
	annular jet},
	journal={J. Fluid Mech.},
	year=1998,
	volume=357,
	pages={351-379}
}


@book{Lavoi89,
   author =    {Lavoisier, A. L.},
   title =     {Trait{'e} \'El{\'e}mentaire de Chimie},
   publisher = {Cuchet, Paris.},
   year =      1789,
}

@BOOK{lavrentievchabat,
   author    = "M. Lavrentiev and B. Chabat",
   title     = "Effets hydrodynamiques et mod\`eles math\'ematiques",
   publisher = "\'Editions MIR",
   year      = "1980",
   note      = "Translated from the 1977 russian edition",
}

@Article{Laws43,
	author={Laws, J. O. and Parsons, D. A.},
	title={The relation of raindrop-size to intensity, II},
	journal={Trans. Amer. Geophys. Union},
	year=1943,
	volume=24,
	pages={452-460}
}

@Article{LeDizes97,
	author={Le Dizes, S.},
	title={Global modes in falling capillary jets},
	journal={Eur. J. Mech. B/Fluids},
	year=1997,
	volume={16},
	pages={761}
}


@Article{Loews96,
	author={Loewen, M. R. and O'Dor, M. A. and Skafel, M. G.},
	title={Bubbles entrained by mechanically generated breaking waves},
	journal={J. Geophys. Res.},
	year=1996,
	volume={101},
	number={C9},
	pages={452-460}
}

@Article{tong01,
	author={Lei, X. and Ackerson, B. J. and Tong, P.},
	title={Settling Statistics of Hard Sphere Particles.},
	journal={Phys.  Rev.  Letters},
	year= 2001,
	volume= 86,
	number={15},
	pages={3300-3303}
}

@book{Lefe89,
   author =    {Lefebvre, A. H.},
   title =     {Atomization and sprays},
   publisher = {Hemisphere.},
   year =      1989,
}

@book{LeMa02,
   author =    {Le Masson, G.},
   title =     {Rapport de projet personnel: impact d'un jet
  d'eau sur un barreau cylindrique.},
   publisher = {E. N. S. T. A.},
   year =      2002,
}

@Article{Len04,
	author={Lenard, P.},
	title={{\"U}ber Regen},
	journal={Meteorologische Zeitschrift},
	year= 1904,
	volume= 21,
	pages={249-262}
}

@Article{Spil48,
	author={A. F. Spilhaus},
	title={Drop size, intensity, and radar echo of rain},
	journal={J. Atmos. Sci.},
	year= 1948,
	volume= 5,
	pages={161-164}
}

@techReport{Lesp65,
   author =      {Lespinard,G.},
   title =       {R?duction des irr?gularit?s de l'?coulement en
   soufflerie.},
   institution = {Laboratoire de m\'ecanique des fluides, Grenoble},
    pages = {11-24},
   year =        1965,
}



@phdThesis{Lesp68,
   author = {Lespinard,G.},
   title =  {Contribution ? l'?tude de la transition de la
   couche limite : effet de l'aspiration pari?tale.},
   school = {Universit? de Grenoble},
   year =   1968,
}

@book{Levy1965,
    author={P. Levy},
	title={Processus stochastiques et mouvement brownien},
	publisher={Gauthier-Villars},
	year={1965}
}

@article{Lewi50,
   author =  {Lewis, D. J.},
   title =   {The instability of liquid surfaces when accelerated in a
              direction perpendicular to their plane.II},
   journal = {Proc. R. Soc. Lond. A},
   volume =  202,
   pages =   {81-96},
   year =    1950,
}



@Article{Dri10,
	author={M. M. Driscoll and C. C. Stevens and S. R. Nagel},
	title={Thin film formation during splashing of viscous liquids},
	journal={Phys. Rev. E},
	year={2010},
	volume={82},
	pages={036302}
}

@Article{Lin&Reitz1998,
	author={S. P. Lin and R. D. Reitz},
	title={Drop and spray formation from a liquid jet},
	journal={Ann. Rev. Fluid Mech.},
	year={1998},
	volume={30},
	number={},
	pages={80--105}
}

@inproceedings{Loewen&O'Dor&Skafel1995,
	author={Loewen, M. R. and OÍDor, M. and Skafel, M.},
	title={Laboratory Measurements of Bubble Size
           Distributions Under Breaking Waves},
	booktitle={Third International Symposium on Air-Water
	Gas Transfer, University of Heidelberg, July 24-27},
	year={1995},
	pages={337--349},
}
@Article{Loewen&O'Dor&Skafel1996,
	author={Loewen, M. R. and OÍDor, M. and Skafel, M.},
	title={Bubbles entrained by mechanically generated breaking waves},
	journal={Journal of Geophysical Research},
	year={1996},
	volume={101},
	number={C9},
	pages={20759--20769}
}
@Article{Lowry&Steen1997,
	author={B. J. Lowry and P. H. Steen},
	title={Stability of slender liquid bridges subjected to axial
	flows},
	journal={J. Fluid Mech.},
	year={1997},
	volume={330},
	number={},
	pages={189--213}
}

@article{Lif61,
   author =  {Lifshitz, I. M. and Slyozov, V. V.},
   title =   {The kinetics of precipitation from supersaturated
       solid solutions.},
   journal = {J. Phys. Chem. Solids},
   volume = 19,
   pages = {35-50},
   year =  1961,
}

@article{Lima93,
   author =  {Limat, L.},
   title =   {Instabilit{\'e} d'un liquide suspendu sous un surplomb
        solide : influence de l'{\'e}paisseur de la couche.},
   journal = {C. R. Acad. Sci. II},
   volume = 317,
   pages = {563-568},
   year =  1993,
}

@book{Lin03,
   author =    {Lin, S. P.},
   title =     {Breakup of liquid sheets and jets.},
   publisher = {Cambridge University Press, Cambridge},
   year =      2003,
}

@article{Long83,
   author =  {Longuet-Higgins, M. S.},
   title =   {Bubbles breaking waves and hyperbolic jets at free
   surface.},
   journal = {J. Fluid Mech.},
   volume = 127,
   pages = {103-121},
   year =  1983,
}

@article{Long92,
   author =  {Longuet-Higgins, M. S.},
   title =   {Capillary rollers and bores},
   journal = {J. Fluid Mech.},
   volume = 240,
   pages = {659-679},
   year =  1992,
}

@Article{Longuet-Higgins1992,
	author={M. S. Longuet-Higgins},
	title={The crushing of air cavities in a liquid},
	journal={Proc. R. Soc. London A},
	year=1992,
	volume=439,
	pages={611--626}
}

@Article{Loren05,
	author={Utada, A. S. and Lorenceau, E. and Link, D. R.
    and Kaplan, P. D. and Stone, H. A. and Weitz, D. A.},
	title={The crushing of air cavities in a liquid},
	journal={Science},
	year=2005,
	volume=308,
	pages={537-541}
}

@Article{LowList1982,
	author={T. B. Low and R. List},
	title={Collision, coalescence and breakup of raindrops. Part I:
	Experimentally established coalescence efficiencies and
	fragment size distributions in breakup},
	journal={J. Atmos. Sci.},
	year=1982,
	volume=39,
	pages={1591--1606}
}

@article{Loza98,
   author =  {Lozano, A. and Garcia-Olivares, A. and Dopazo, C.},
   title =   {The instability growth leading to a liquid sheet
   break up.},
   journal = {Phys. Fluids},
   volume = 10,
   pages = {2188-2197},
   year =  1998,
}

@article{Mab03,
   author =  {Mabile, C. and Leal-Calderon, F. and
             Bibette, J. and Schmitt, V.},
   title =   {Monodisperse fragmentation in emulsions:
             Mechanisms and kinetics.},
   journal = {Europhys. Letters},
   volume = 61,
   number={5},
   pages = {708-714},
   year =  2003,
}

@article{McEn69a,
   author =  {McEntee, W. R. and Mysels, K. J.},
   title =   {The bursting of soap films. I. An experimental
   study.},
   journal = {J. Phys. Chem.},
   volume = 73,
   pages = {3018-3028},
   year =  1969,
}

@article{McEn69b,
   author =  {McEntee, W. R. and Mysels, K. J.},
   title =   {The bursting of soap films. II.Theoritical
   considerations.},
   journal = {J. Phys. Chem.},
   volume = 73,
   pages = {3028-3038},
   year =  1969,
}

@article{OM05,
   author =  {Oliveira, M. S. N. and McKinley, G. H.},
   title =   {Iterated stretching and multiple beads-on-a-string
      phenomena in dilute solutions of high extensible flexible polymers.},
   journal = {Phys. Fluids},
   volume = 17,
   pages = {071704},
   year =  2005
}

@article{Mans90,
   author =  {Mansour, A. and Chigier, N.},
   title =   {Disintegration of liquid sheets.},
   journal = {Phys. Fluids A},
   volume = 2,
   pages = {706-719},
   year =  1990,
}

@Article{Mansour&Chigier1994,
	author={A. Mansour and N. Chigier},
	title={Turbulence characteristics in cylindrical liquid jets},
	journal={Phys. Fluids},
	year={1994},
	volume={6},
	number={10},
	pages={3380--3391}
}

@book{Mar86,
    author={Mariotte, E.},
	title={Trait{\'e} du mouvement des eaux et des autres corps fluides},
	publisher={E. Michallet, Paris},
	year={1686}
}

@article{Mark57,
   author =  {Markstein, G. H.},
   title =   {Flow disturbances induced near a slightly wavy
   contact surface or flame front, traversed by a shock wave.},
   journal = {J. Aero. Sci.},
   volume = 24,
   pages = {238-239},
   year =  1957,
}



@article{Marm00,
   author =  {Marmottant, P. and Villermaux, E. and Clanet, C.},
   title =   {Transient surface tension of an expanding liquid
   sheet.},
   journal = {J. Colloid Interface},
   volume = 230,
   pages = {29-40},
   year =  2000,
}

@phdThesis{Marm01,
   author = {Marmottant, P.},
   title =  {Atomisation d'un liquide par un courant gazeux.},
   school = {L. E. G. I. Grenoble},
   year =   2001,
}

@article{Marm04,
   author =  {Marmottant, P. and Villermaux, E.},
   title =   {On spray formation.},
   journal = {J. Fluid Mech.},
   volume = 498,
   pages = {73-112},
   year =  2004,
}

@article{Marm04b,
   author =  {Marmottant, P. and Villermaux, E.},
   title =   {Fragmentation of stretched liquid ligaments.},
   journal = {Phys. Fluids},
   volume = 16,
   pages = {2732-2741},
   year =  2004,
}

@Article{Marmottant&Villermaux&Clanet2000,
	author={P. Marmottant and E. Villermaux
             and C. Clanet },
	title={Transient Surface Tension of an Expanding Liquid Sheet},
	journal={J. Colloid Interface Sci.},
	year={ 2000},
	volume={230},
	number={1},
	pages={29--40}
}

@Article{Marshall48,
	author={Marshall, J. S. and Palmer, W. McK},
	title={The distribution of raindrops with size},
	journal={J. Meteorol.},
	year={1948},
	volume={5},
	pages={165--166}
}


@Article{Martinez-Bazan&Montanes&Lasheras1999,
	author={Martinez-Bazan, C. and Montanes, J. L. and Lasheras, J. C.},
	title={On the breakup of an air bubble injected into a fully developed
	turbulent flow. Part 2. Size PDF of the resulting daughter bubbles},
	journal={J. Fluid Mech.},
	year={1999},
	volume={401},
	number={},
	pages={183--207}
}

@book{Mason71,
    author={B. J. Mason},
	title={The Physics of Clouds},
	publisher={Clarendon Press--Oxford},
	year={1971}
}

@book{Massel96,
    author={Massel, S. R.},
	title={Ocean Surface Waves: their physics and prediction},
	publisher={World scientific},
	year={1996}
}

@Article{Mastin07,
	author={Mastin, L. G.},
	title={Generation of fine hydromagmatic ash by growth and
         disintegration of glassy rinds},
	journal={J. Geophys. Research.},
	year={2007},
	volume={112},
	pages={B02203}
}

@book{MayerandMayer1966,
    author={J. E. Mayer and M. G. Mayer},
	title={Statistical Mechanics},
	publisher={John Wiley},
	year={1966}
}

@article{Mayer96,
   author =  {Mayer, W. and Tamura, H.},
   title =   {Propellant Injection in a Liquid Oxygen/Gaseous
             Hydrogen Rocket Engine.},
   journal = {J. Prop. and Power},
   volume = 12,
   number={6},
   pages = {1137-1147},
   year =  1996,
}

@article{Meie92,
   author =  {Meier, G. E. A. and Klopper, A. and Grabitz, G.},
   title =   {The influence of kinematic waves on jet break down.},
   journal = {Exp. in Fluids},
   volume = 12,
   pages = {173-180},
   year =  1992,
}
@article{Merr47,
   author =  {Merrington, A. C. and Richarson, E. G.},
   title =   {The Breakup of Liquid jets.},
   journal = {The proceeding of the physical society},
   volume = 59,
   pages = {1-13},
   year =  1947,
}

@article{Mesh69,
   author =  {Meshkov, E. E.},
   title =   {Instability of the interface of two gases
   accelerated by a shock wave.},
   journal = {Sov. Fluid Dyn.},
   volume = 4,
   pages = {101-108},
   year =  1969,
}

@Article{Mikaelian1995,
	author={K. O. Mikaelian},
	title={Rayleigh-Taylor and Richtmyer-Meshkov instabilities in
	finite thickness fluid layers},
	journal={Phys. Fluids},
	year={1995},
	volume={7},
	number={4},
	pages={888--890}
}


@article{Mies57,
   author =  {Miesse, C. C.},
   title =   {The effect of ambient pressure oscillations in the
   disintegration and dispersion of a liquid jet },
   journal = {Jet Propulsion},
   year =  1957,
}

@article{Mies55,
   author =  {Miesse, C. C.},
   title =   {Correlation of experimental dataon the disintegration
                of liquid jets},
   journal = {Ind. Eng. Chem.},
   volume={47},
   number={9},
   year =  1955,
   pages = {1690-1701}
}

@article{Miles90,
   author =  {Miles, J. and Henderson, D.},
   title =   {Parametrically forced surface waves.},
   journal = {Ann. Rev. Fluids Mech.},
   volume = 22,
   pages = {143-165},
   year =  1990,
}

@article{Mill60,
   author =  {Miller, K. D.},
   title =   {Distribution of spray from impinging liquid jets.},
   journal = {J. Appl. Phys.},
   volume = 31,
   pages = {1132-1133},
   year =  1960,
}



@book{Monin75,
   author =    {Monin, A. S. and Yaglom, A. M.},
   title =     {Statistical Fluid Mechanics: Mechanics of Turbulence, Vol. 2},
   publisher = {The MIT Press.},
   year =      1975,
}




@article{Mos00,
   author =  {Moseler, M. and Landman, U.},
   title =   {Formation, Stability, and Breakup of Nanojets.},
   journal = {Science},
   volume = 289,
   pages = {1165-1169},
   year =  2000,
}

@article{Mott47,
   author =  {Mott, N. F.},
   title =   {Fragmentation of shell cases.},
   journal = {Proc. R. Soc. London A},
   volume = 189,
   pages = {300-308},
   year =  1947,
}


@article{Nabe88,
   author =  {Naber, J. D. and Reitz, R. D.},
   title =   {Modeling engine spray/wall impingement.},
   journal = {SAE Paper},
   pages = {880107},
   year =  1988,
}

@article{Neu52,
   author =  {von Neumann, J.},
   title =   {Discussion},
   journal = {Metal Interfaces},
   pages = {108-110},
   year =  1952,
}

@book{New87,
   author =    {Newton, I.},
   title =     {Principia Mathematica},
   publisher = {London},
   year =      1687,
}



@book{New04,
   author =    {Newton, I.},
   title =     {Opticks},
   publisher = {London},
   year =      1704,
}


@article{Nied03,
   author =  {Niederhaus, C. E. and Jacobs, J. W.},
   title =   {Experimental study of the Richtmyer-Meshkov
              instability of incompressible fluids.},
   journal = {J. Fluid Mech.},
   volume =  485,
   pages =   {243--277},
   year =    2003,
}

@article{Nikito00,
   author =  {Nikitopoulos, E. and Kelly, A. J.},
   title =   {Formation of a Net-Negative Charged Liquid Spray.},
   journal = {Phys. Fluids.},
   volume =  12,
   number = 9,
   pages =   {S7},
   year =  2000,
}

@book{nollet49,
    author={Abb{\'e} Nollet},
	title={Recherches sur les causes particuli{\`e}res
       des ph{\'e}nom{\`e}nes {\'e}lectriques},
	publisher={les Fr{\`e}res Guerin, Paris},
	year={1749}
}


@Article{Novikov&Dommermuth1997,
	author={E. A. Novikov and D. G. Dommermuth},
	title={Distribution of droplets in a turbulent spray},
	journal={Phys. Rev. E},
	year={1997},
	volume={56},
	number={5},
	pages={5479--5482}
}


@Article{Odd93,
	author={Oddershede, L. and Dimon, P. and Bohr, J.},
	title={Self organized criticality in fragmenting},
	journal={Phys. Rev. Letters},
	year={1993},
	volume={71},
	number={19},
	pages={3107--3110}
}




@article{Pand90,
   author =  {Pandit, A. B. and Davidson, J. F.},
   title =   {Hydrodynamics of the rupture of thin liquid films.},
   journal = {J. Fluid Mech.},
   volume = 212,
   pages = {11-24},
   year =  1990,
}

@article{Park04,
   author =  {Park, J. and Huh, K. Y. and Li, X. and Renksizbulut, M.},
   title =   {Experimental investigation on cellular breakup of a
        planar liquid sheet from an air-blast nozzle.},
   journal = {Phys. Fluids},
   volume = 16,
   pages = {625-632},
   year =  2004,
}

@book{Pere94,
   author =    {P?rez,J. P.},
   title =     {Optique g?om?trique et ondulatoire, 4?me ?dition},
   publisher = {Masson},
   year =      1994,
}

@Article{Peerho03,
	author={Lemenand, T. and Della Valle, D. and Zellouf, Y.
            and Peerhossaini, H.},
	title={Droplet formation in turbulent mixing of two
         immiscible fluids in a new type of static mixer},
	journal={Int. J. Mutli. Flows},
	year={2003},
	volume={29},
	pages={813-840}
}
@Article{Peregrine&Shoker&Symon1990,
	author={D. H. Peregrine and G. Shoker and A. Symon},
	title={The bifurcation of liquid bridges},
	journal={J. Fluid Mech.},
	year={1990},
	volume={212},
	number={},
	pages={25-39}
}

@Article{Pilch&Erdman1987,
	author={M. Pilch and C. A. Erdman},
	title={Use of breakup time data and velocity history data to
	predict the maximum size of stable fragments for
	acceleration-induced breakup of a liquid drop},
	journal={Int. J. Multiphase Flow},
	year={1987},
	volume={13},
	number={6},
	pages={741--757}
}

@article{Ples17,
   author =  {Plesset, M.},
   title =   {????.},
   journal = {J. Appl. Mech.},
   volume = 16,
   pages = {277--??},
   year =  1917,
}


@article{Pom06,
   author =  {Pomeau, Y. and Villermaux, E.},
   title =   {Two hundred years of capillarity research.},
   journal = {Phys. Today},
   volume = 3,
   pages = {39--44},
   year =  2006,
}

@article{PS05,
   author =  {Y. Pomeau and D. Sciamarella},
   title =   {An unfinished tale of nonlinear PDEs: Do solutions
             of 3D incompressible Euler equations blow up in
             finite time ?},
   journal = {Physica D},
   volume = 205,
   pages = {215},
   year =  2005,
}

@article{Ponst59,
   author =  {Ponstein, J.},
   title =   {Instability of rotating cylindrical jets.},
   journal = {Appl. Sci. Res. A},
   volume = 8,
   pages = {425--456},
   year =  1959,
}

@article{Potts01,
   author =  {Potts, H. E. and Diver, D. A.},
   title =   {Large-amplitude ferrofluid surface waves and
           jets.},
   journal = "New J. Phys.",
   volume = 3,
   pages = {7.1-7.14},
   year =  2001,
}

@article{WDKS02,
   author =  {I. M. Wallwork and S. P. Decent and A. C. King
              and R. M. S. M. Schulkes},
   title =   {The trajectory and stability of a spiralling liquid
         jet. Part 1. Inviscid theory},
   journal = {J. Fluid Mech.},
   volume = 459,
   pages = {43},
   year =  2002,
}

@article{PDSWK07,
   author =  {E. I. Parau and S. P. Decent and M. J. H. Simmons
         and D. C. Y. Wong and A. C. King},
   title =   {Nonlinear viscous liquid jets from a rotating orifice},
   journal = {J. Engin. Math.},
   volume = 57,
   pages = {159},
   year =  2007,
}


@article{Poul94,
   author =  {Pouliquen, O. and Chomaz, J. and Huerre, P.},
   title =   {Propagating holmboe waves at the interface between
   two immiscible fluids.},
   journal = {J. Fluid Mech.},
   volume = 266,
   pages = {277-302},
   year =  1994,
}

@Article{Ranger&Nicholls1969,
	author={A. A. Ranger and J. A. Nicholls},
	title={Aerodynamic shattering of liquid drops},
	journal={AIAA Journal},
	year={1969},
	volume={7},
	number={2},
	pages={285--290}
}

@Article{Qian97,
	author={Qian, J. and Law, C. K.},
	title={Regimes of coalescence and separation in droplet collision},
	journal={J. Fluid Mech.},
	year={1997},
	volume={331},
	pages={59--80}
}



@article{Ranz59,
   author =  {Ranz, W. E.},
   title =   {Some experiments on the dynamics of liquid films.},
   journal = {J. Appl. Phys},
   volume = 30,
   pages = {1950},
   year =  1959,
}

@article{Rayl79a,
   author =  {Rayleigh, Lord},
   title =   {On the instability of jets.},
   journal = {Proc. Lond. Math. Soc.},
   volume = 4,
   pages = {4--13},
   year =  1879,
}

@article{Rayl79b,
   author =  {Rayleigh, Lord},
   title =   {On the capillary phenomena of jets.},
   journal = {Proc. R. Soc. Lond.},
   volume = 29,
   pages = {71-97},
   year =  1879,
}

@article{Rayl80,
   author =  {Rayleigh, Lord},
   title =   {On the stability, or instability of certain fluid
   motion.},
   journal = {Proc. Lond. Math. Soc.},
   volume = 11,
   pages = {57},
   year =  1880,
}

@article{Rayl80b,
   author =  {Rayleigh, Lord},
   title =   {On the resultant of a large number of vibrations
        of the same pitch and of arbitrary phase.},
   journal = {Phil. Mag.},
   volume = {10},
   pages = {73--78},
   year =  1880,
}


@article{Rayl91,
   author =  {Rayleigh, Lord},
   title =   {Some applications of photography},
   journal = {Nature},
   volume = {44},
   pages = {249--254},
   year =  1891,
}

@article{Rayl82,
   author =  {Rayleigh, Lord},
   title =   {On the equilibrium of liquid conducting masses
           charged with electricity.},
   journal = {Phil. Mag.},
   volume = {14},
   pages = {184-186},
   year =  1882,
}



@article{Rayl83,
   author =  {Rayleigh, Lord},
   title =   {Investigation of the character of the equilibrium
   of an incompressible heavy fluid of variable density.},
   journal = {Proc. R. Soc. Lond.},
   volume = 14,
   pages = {170-177},
   year =  1883,
}

@article{Rayl92,
   author =  {Rayleigh, Lord},
   title =   {On the instability of a viscous cylinder
          under the capillary force.},
   journal = {Phil. Mag.},
   volume = 34,
   pages = {145-154},
   year =  1892 ,
}

@article{Rayl92b,
   author =  {Rayleigh, Lord},
   title =   {On the instability of cylindrical fluid surfaces.},
   journal = {Phil. Mag.},
   volume = 34,
   pages = {177-180},
   year =  1892 ,
}

@article{Rayl17,
   author =  {Rayleigh, Lord},
   title =   {????},
   journal = {Phil. Mag.},
   volume = {34},
   pages = {94-???},
   year =  1917,
}



@phdThesis{Rayn97,
   author = {Raynal, L.},
   title =  {Instabilit? et entra?nement ? l'interface d'une
   couche de m?lange liquide-gaz.},
   school = {Universit? Joseph Fourier, Grenoble},
   year =   1997,
}

@Article{Razumovskii&Chesnokov1999,
	author={N. A. Razumovskii and Yu. G. Chesnokov },
	title={Capillary waves on the surface of an extending cylindrical jet},
	journal={Fluid Dynamics},
	year={1999},
	volume={34},
	number={6},
	pages={856--861}
}

@Article{Rehab98,
	author={Rehab, H. and Villermaux, E. and Hopfinger, E. J.},
	title={Geometrical effects on the near field flow
              structure of coaxial jets},
	journal={AIAA J.},
	year={1998},
	volume={36},
	number={5},
	pages={867--869}
}

@Article{Reiner92,
	author={Reiner, G.},
	title={Dewetting of thin polymer films},
	journal={Phys. Rev. Letters},
	year={1992},
	volume={68},
	number={1},
	pages={75--78}
}


@Article{Reitz&Bracco1982,
	author={R. D. Reitz and F. V. Bracco},
	title={Mechanism of atomisation of a liquid jet},
	journal={Phys. Fluids},
	year={1982},
	volume={25},
	number={10},
	pages={1730--1742}
}

@Article{Renardy&Cristini2001b,
	author={Y. Renardy and V. Cristini},
	title={Scalings for fragments produced from drop breakup in
	shear flow with inertia},
	journal={Phys. Fluids},
	year={2001},
	volume={13},
	number={9},
	pages={2161--2164},
	}
	
@article{Rich60,
   author =  {Richtmyer, R. D.},
   title =   {Taylor instability in shock acceleration of
   compressible fluids.},
   journal = {Comm. Pure Appl. Math.},
   volume = 8,
   pages = {297-319},
   year =  1960,
}

@article{Righ97,
   author =  {Rightley, P. M. and Vorobieff, P. and Benjamin, R. F.},
   title =   {Evolution of a shock-accelerated thin fluid layer.},
   journal = {Phys. Fluids},
   volume =  9,
   pages =   {1770-1782},
   year =    1997,
}

@book{Rob99,
   author =    {Roberts, J. B. and Spanos, P. D.},
   title =     {Random vibrations and statistical linearization},
   publisher = {Dover},
   year =      1999,
}

@book{Rose85,
   author =    {Rosensweig, R. E.},
   title =     {Ferrohydrodynamics},
   publisher = {Cambridge University Press, Cambridge},
   year =      1985,
}


@article{Rosin33,
   author =  {Rosin, P. and Rammler, E.},
   title =   {The laws governing the fineness of powered coal.},
   journal = {The Institute of Fuel},
   volume =  {X},
   pages =   {29-36},
   year =    1933,
}



@book{Row02,
   author =    {Rowlinson, J. S.},
   title =     {Cohesion},
   publisher = {Cambridge University Press, Cambridge},
   year =      2002,
}




@article{Ryan95,
   author =  {Ryan, H. M. and Anderson, W. E. and Pal, S. and
   Santoro, R. J.},
   title =   {Atomization characteristics of impinging liquid jets.},
   journal = {J. Prop. and Power},
   volume = 11,
   pages = {135-145},
   year =  1995,
}


@article{Saff56,
   author =  {Saffman, P. G. and Turner, J. S.},
   title =   {On the collision of drops in a turbulent cloud},
   journal = {J. Fluid Mech.},
   volume = 1,
   pages = {16-30},
   year =  1956,
}

@article{Saff74,
   author =  {Saffman, P. G.},
   title =   {The structure and decay of trailing vortices},
   journal = {Archives of Mechanics},
   volume = 26,
   pages = {423-439},
   year =  1974,
}

@book{Saff_book,
   author =  {Saffman, P. G.},
   title =   {Vortex dynamics},
   publisher = {Cambridge University Press, Cambridge},
   year =  1992,
}

@book{Saf03,
   author =    {Safran, S. A.},
   title =     {Statistical thermodynamics of surfaces, interfaces,
                      and membranes},
   publisher = {Westview Press, Boulder, CO},
   year =      2003,
}

@book{Ellis85,
   author =    {Ellis, R. S.},
   title =     {Entropy, large deviations, and statistical mechanics},
   publisher = {Springer},
   year =      1885,
}

@article{HJKPS86,
   author =  {T. C. Halsey and M. H. Jensen and L. P. Kadanoff and
               I. Procaccia and B. I. Shraiman},
   title =   {Fractal measures and their singularities: the characterization
                 of strange sets},
   journal = {Phys. Rev. E},
   volume = 33,
   pages = {1141},
   year =  1986,
}

@article{Sall04,
   author =  {Sallam, K. A. and Aalburg, C. and Faeth, G. M.},
   title =   {Breakup of round nonturbulent liquid jets in gaseous crossflow},
   journal = {AIAA Journal},
   volume = 42,
   number = 12,
   pages = {2529-2540},
   year =  2004,
}

@article{Savart2,
   author =  {Savart, F.},
   title =   {M?moire sur le choc de deux veines liquides
   anim?es de mouvements directement oppos?s.},
   journal = {Ann. de chimie.},
   volume = 55,
   pages = {257-310},
   year =  1833,
}

@article{Savart1a,
   author =  {Savart, F.},
   title =   {M?moire sur le choc d'une veine liquide
   lanc?e sur un plan circulaire.},
   journal = {Ann. de chimie.},
   volume = 54,
   pages = {56-87},
   year =  1833,
}

@article{Savart1b,
   author =  {Savart, F.},
   title =   {Suite du m?moire sur le choc d'une veine liquide
   lanc?e sur un plan circulaire.},
   journal = {Ann. de chimie.},
   volume = 54,
   pages = {113-145},
   year =  1833,
}


@article{Savart0,
   author =  {Savart, F.},
   title =   {M?moire sur la constitution des veines liquides
   lanc?es par des orifices circulaires en mince paroi.},
   journal = {Ann. de chimie.},
   volume = 53,
   pages = {337-398},
   year =  1833,
}

@article{saville71,
   author =  {Saville, D. A.},
   title =   {Stability of electrically charged viscous cylinders},
   journal = {Phys. Fluids.},
   volume = 14,
   number = 6,
   pages = {1095-1099},
   year =  1971,
}


@book{Schlichting1987,
    author={Schlichting, H.},
	title={Boundary layer theory},
	publisher={McGraw-Hill},
	address={New York},
	edition={7th},
	year={1987}
}

@book{Sobey00,
    author={I. J. Sobey},
	title={Introduction to interactive boundary layer theory},
	publisher={Oxford University Press},
	year={2000}
}

@book{Sychev98,
    author={V. V. Sychev and A. I. Ruban and V. V. Sychev and G. L. Korolev},
	title={Aymptotic theory of separated flows},
	publisher={Cambridge University Press, Cambridge},
	year={1998}
}

@Article{Y58,
	author={K. T. Yang},
	title={Unsteady laminar boundary layers in an incompressible
           stagnation flow},
	journal={Trans. A.S.M.E. J. Appl. Mech.},
	year={1958},
	volume={25},
	pages={421}
}

@Article{Y58b,
	author={K. T. Yang},
	title={On certain similar solutions to unsteady laminar
         boundary-layer equations in low-speed flow},
	journal={J. aero Space Sci.},
	year={1958},
	volume={25},
	pages={471}
}

@Article{Schum1940,
	author={Schumann, T. E. W.},
	title={Theoretical aspects of the size distribution of fog particles},
	journal={Quart. J. Roy. Meteorol. Soc.},
	year={1940},
	volume={66},
	pages={195-207}
}



@Article{Schulkes1996,
	author={R. M. S. M. Schulkes},
	title={The contraction of liquid filaments},
	journal={J. Fluid Mech.},
	year={1996},
	volume={309},
	number={},
	pages={277-300}
}


@book{Sein98,
    author={Seinfeld, J. H. and Pandis, S. N.},
	title={Atmospheric Chemistry and Physics},
	publisher={John Wiley \& Sons, Inc.},
	year={1998}
}

@article{Shen98,
   author =  {Shen, Y. B. and Poulikakos, D.},
   title =   {Thickness variation of liquid sheet formed by two
   impinging jets using holographic interferometry.},
   journal = {J. Fluids Eng.},
   volume = 120,
   pages = {482-487},
   year =  1998,
}

@article{Shimo94,
   author =  {Shimozuru, D.},
   title =   {Physical parameters governng the formation of Pele's hair and tears.},
   journal = {Bull. Volcanol.},
   volume = 56,
   pages = {217-219},
   year =  1994,
}

@article{Shin61,
   author =  {Shinnar, R.},
   title =   {On the behaviour of liquid dispersions in mixing vessels.},
   journal = {J. Fluid Mech.},
   volume = 10,
   pages = {259-275},
   year =  1961,
}


@article{Simm77-1,
   author =  {Simmons, H. C.},
   title =   {The correlation of drop-size distributions in fuel
   nozzle sprays. Part I : the drop-size/volume-fraction
   distribution.},
   journal = {J. Eng. Power},
   volume = 7,
   pages = {309-314},
   year =  1977,
}

@article{Simm77-2,
   author =  {Simmons, H. C.},
   title =   {The correlation of drop-size distributions in fuel
   nozzle sprays. Part II : the drop-size$/$number distribution.},
   journal = {J. Eng. Power},
   volume = 7,
   pages = {315-319},
   year =  1977,
}

@Article{Sklavenites1997,
	author={D. Sklavenites},
	title={Wave pattern on a water column},
	journal={Am. J. Phys.},
	year={1997},
	volume={65},
	number={3},
	pages={225--230}
}


@article{Squi53 ,
   author =  {Squire, H. B.},
   title =   {Investigation of the stability of a moving liquid
   film.},
   journal = {British J. Appl. Physics},
   volume = 4,
   pages = {167-169},
   year =  1953,
}

@article{SQ05 ,
   author =  {Squires, T. M. and Quake, S. R.},
   title =   {Microfluidics: Fluid physics at the nanoliter scale.},
   journal = {Rev. Mod. Phys.},
   volume = 77,
   pages = {977-1026},
   year =  2005,
}

@article{SSA04,
   author =  {H. A. Stone and A. D. Stroock and A. Ajdari},
   title =   {Engineering flows in small devices.
             Microfluidics toward lab-on-a-chip},
   journal = {Ann. Rev. Fluid Mech.},
   volume = 36,
   pages = {381},
   year =  2004,
}

@Article{Smoluchowski1917,
	author={M. von Smoluchowski},
	title={Versuch einer mathematischen Theorie der
         Koagulationskinetik kolloider L{\"o}sungen},
	journal={Z. Phys. Chem.},
	year={1917},
	volume={92},
	number={},
	pages={129--168}
}

@Article{Smolka&al2003,
	author={L. B. Smolka and A. Belmonte},
	title={Drop pinch-off and filament dynamics of wormlike
	micellar fluids},
	journal={J. Non-Newtonian Fluid Mech.},
	year={2003},
	volume={115},
	number={},
	pages={1--25}
}

@Article{Sovani00,
	author={Sovani,S. D. and Sojka, P. E. and Lefebvre, A. H.},
	title={Effervescent Atomization},
	journal={Progr. Ener. Combust. Sci.},
	year={2000},
	volume={27},
	number={},
	pages={483--521}
}




@Article{Srivasta71,
	author={Srivastava, R. C.},
	title={Size distribution of Raindrops generated by
       their breakup and coalescence},
	journal={J. Atmo. Sci.},
	year={1971},
	volume={28},
	pages={410--415}
}

@Article{Stern06,
	author={S. A. Stern and H. A. Weaver and A. J. Steffl and
      M. J. Mutchler and W. J. Merline and M. W. Buie and E. F. Young
         and L. A. Young and J. R. Spencer},
	title={A giant impact origin for Pluto's small moons
          and satellite multiplicity in the Kuiper belt},
	journal={Nature},
	year={2006},
	volume={439},
	pages={946--948}
}



@Article{Stockmaker1943,
	author={Stockmayer, W. H.},
	title={Theory of Molecular Size Distribution and Gel Formation
	in Branched-Chain Polymers},
	journal={J. Chem. Phys.},
	year={1943},
	volume={11},
	number={2},
	pages={45--55}
}

@Article{Stow77,
	author={Stow, C. D. and Stainer, R. D.},
	title={The physical products of a splashing water drop},
	journal={J. Met. Soc. Japan},
	year={1977},
	volume={55},
	number={5},
	pages={518--531}
}


@Article{Spiegelberg&Ables&McKinley1996,
	author={S. H. Spiegelberg and D. C. Ables and G. H.
	McKinley},
	title={The role of end-effects on measurements of extensional
	viscosity in filament stretching rheometers},
	journal={J. Non-Newtonian Fluid Mech.},
	year={1996},
	volume={64},
	number={},
	pages={229--267}
}
@Article{Spiegelberg&McKinley1996,
	author={S. H. Spiegelberg and G. H.
	McKinley},
	title={Stress relaxation and elastic decohesion of viscoelastic
	polymer solutions in extensional flow},
	journal={J. Non-Newtonian Fluid Mech.},
	year={1996},
	volume={67},
	number={},
	pages={49--76}
}

@Article{Stone&Bentley&Leal1986,
	author={H. A. Stone, B. J. Bentley and L. G. Leal},
	title={An experimental study of transient effects in the breakup of
	viscous drops},
	journal={J. Fluid Mech.},
	year={1986},
	volume={173},
	pages={131--158}
}

@article{Stone04,
   author =  {Stone, H. A. and Stroock, A. D. and Adjari, A.},
   title =   {Engineering Flows in Small Devices:
               Microfluidics Towards a Lab-on-a-Chip},
   journal = {Annu. Rev. Fluid Mech.},
   volume = 36,
   pages = {381-411},
   year =  2004,
}

@article{Poni00,
   author =  {A. Poniewierski},
   title =   {Shape of the nematic-isotropic interface in conditions
              of partial wetting},
   journal = {Liq. Cryst.},
   volume = {27},
   pages = {1369-1380},
   year =  2000,
}

@article{JeromeBoix92,
   author =  {B. J{\'e}r{\^o}me and M. Boix},
   title =   {Wetting Instability in Nematic Liquid Crystals},
   journal = {Europhys. Lett.},
   volume = {17},
   pages = {169},
   year =  1992,
}

@article{SZBLW06,
   author =  {I. I. Smalyukh and O. V. Zribi and J. C. Butler and
               O. D. Lavrentovich and G. C. L. Wong},
   title =   {Structure and Dynamics of Liquid Crystalline Pattern
                Formation in Drying Droplets of DNA},
   journal = {Phys. Rev. Lett.},
   volume = 96,
   pages = {177801},
   year =  2006,
}

@article{Stone96,
   author =  {Stone, H. A. and Brenner, M. P.},
   title =   {Note on the capillary thread instability
          for fluids of equal viscosities},
   journal = {J. Fluid Mech.},
   volume = 318,
   pages = {373-374},
   year =  1996,
}


@article{Sult06 ,
   author =  {Sultan, E. and Boudaoud, A.},
   title =   {The statistcs of crumpled paper},
   journal = {Phys. Rev. Letters},
   volume = {96},
   pages = {136103},
   year =  2006,
}

@article{AB03 ,
   author =  {B. Audoly and A. Boudaoud},
   title =   {Self-similar structures near boundaries in strained systems},
   journal = {Phys. Rev. Letters},
   volume = {91},
   pages = {086105},
   year =  2003,
}

@article{Sund02 ,
   author =  {S{\"un}derhauf, G. and Raszillier, H. and Durst, F.},
   title =   {The retraction of the edge of a planar liquid sheet.},
   journal = {Phys. Fluids},
   volume = 14,
   pages = {198-208},
   year =  2002,
}

@Incollection{Tayl40,
   author =  {Taylor, G. I.},
   title =   {Generation of Ripples by wind blowing over a viscous fluid.},
   booktitle = {G. I. Taylor Scientific Papaers},
   volume = {III},
   pages = {244-254},
   year =  1940,
   editor    = "G. K. Batchelor",
   publisher = {Cambridge University Press, Cambridge},
}

@article{Tayl50 ,
   author =  {Taylor, G. I.},
   title =   {The instability of liquid surfaces when
   accelerated in a direction perpendicular to their plane.I},
   journal = {Proc. R. Soc. Lond. A},
   volume = 201,
   pages = {192-196},
   year =  1950,
}

@article{Tayl590 ,
   author =  {Taylor, G. I.},
   title =   {The dynamics of thin sheets of fluid I. Water bells.},
   journal = {Proc. R. Soc. Lond.},
   volume = 253,
   pages = {289-295},
   year =  1959,
}

@article{Tayl59a ,
   author =  {Taylor, G. I.},
   title =   {The dynamics of thin sheets of fluid II. Waves on fluid sheets.},
   journal = {Proc. R. Soc. Lond.},
   volume = 253,
   pages = {296-312},
   year =  1959,
}

@article{Tayl59b ,
   author =  {Taylor, G. I.},
   title =   {The dynamics of thin sheets of fluid III.
        Disintegration of fluid sheets.},
   journal = {Proc. R. Soc. Lond.},
   volume = 253,
   pages = {313-321},
   year =  1959,
}
@article{Tayl60 ,
   author =  {Taylor, G. I.},
   title =   {Formation of thin flat sheets of water.},
   journal = {Proc. R. Soc. Lond.},
   volume = 259,
   pages = {1-17},
   year =  1960,
}

@article{Tayl61,
   author =  {Taylor, G. I. in an Appendix to Brown, D. R.},
   title =   {A study of the behavior of a thin sheet of a moving liquid.},
   journal = {J. Fluid Mech.},
   volume = 10,
   pages = {305},
   year =  1961,
}

@article{Tayl69,
   author =  {Taylor, G. I.},
   title =   {Electrically driven jets},
   journal = {Proc. R. Soc. Lond. A},
   volume = {313},
   pages = {453-475},
   year =  1969,
}


@Article{Thoroddsen&Sakakibara1998,
	author={S. T. Thoroddsen and J. Sakakibara},
	title={Evolution of the fingering pattern of an impacting drop},
	journal={Phys. Fluids},
	year={1998},
	volume={10},
	number={6},
	pages={1359--1374}
}
@Article{Thoroddsen&Takehara2000,
	author={S. T. Thoroddsen and K. Takehara},
	title={The coalescence cascade of a drop},
	journal={Phys. Fluids},
	year={2000},
	volume={12},
	number={6},
	pages={1265--1267}
}

@Article{Thor06,
	author={Thoroddsen, S. T. and Etoh, T. G. and Takehara, K.},
	title={Crown-breakup by Marangoni Instability},
	journal={J. Fluid Mech.},
	year={2006},
	volume={557},
	pages={63--72}
}

@Article{Tom35,
	author={Tomotika, S.},
	title={On the instability of a cylindrical thread of
        a viscous liquid surrounded by another viscous fluid},
	journal={Proc. Roy. Soc Lond. A},
	year={1935},
	volume={150},
	pages={322--337}
}

@Article{Tom36,
	author={Tomotika, S.},
	title={Breaking up of drop of viscous liquid immersed in
        another fluid which is extending at uniform rate},
	journal={Proc. Roy. Soc Lond. A},
	year={1936},
	volume={153},
	pages={302--318}
}

@article{T06,
   author =  {Trouton, F. T.},
   title =   {On the coefficient of viscous traction and its
             relation to that of viscosity.},
   journal = {Proc. R. Soc. Lond.},
   volume = 77,
   pages = {426-440},
   year =  1906,
}

@article{Tuck02,
   author =  {Tucker, C. L. and Moldenaers, P.},
   title =   {Microstructural evolution in polymer blends.},
   journal = {Annu. Rev. Fluid Mech.},
   volume = 34,
   pages = {177--210},
   year =  2002,
}





@article{Val66,
   author =  {Valentas, K. J. and Amundson, N. R.},
   title =   {Breakage and coalescence in dispersed phase systems.},
   journal = {I\&EC Fundamentals},
   volume = 5,
   number={4},
   pages = {533-542},
   year =  1966,
}



@article{Vill98-a,
   author =  {Villermaux, E.},
   title =   {On the role of viscosity in shear instabilities.},
   journal = {Phys. Fluids},
   volume = 10,
   pages = {368-373},
   year =  1998,
}

@article{Vill98-b,
   author =  {Villermaux, E.},
   title =   {Mixing and spray formation in coaxial jets.},
   journal = {J. Prop. and Power},
   volume = 14,
   pages = {807-817},
   year =  1998,
}


@article{Vill02 ,
   author =  {Villermaux, E. and Clanet, C.},
   title =   {Life of a flapping liquid sheet.},
   journal = {J. Fluid Mech.},
   volume = 462,
   pages = {341-363},
   year =  2002,
}

@article{Vill03 ,
   author =  {Villermaux, E. and Duplat, J.},
   title =   {Mixing as an aggregation process.},
   journal = {Phys. Rev. Letters.},
   volume = 91,
   number={18},
   pages = {184501},
   year =  2003,
}


@article{Vill04,
   author =  {Villermaux, E. and Marmottant, P. and Duplat, J.},
   title =   {Ligament-mediated spray formation.},
   journal = {Phys. Rev. Let. },
   volume = 92,
   pages = {074501},
   year =  2004,
}

@article{Vill06,
   author =  {Villermaux, E. and Duplat, J.},
   title =   {Coarse grained scale of turbulent mixtures},
   journal = {Phys. Rev. Letters},
   volume = {97},
   pages = {144506},
   year =  2006,
}

@article{CBH05,
   author =  {B. Chan and N. J. Balmforth and A. E. Hosoi},
   title =   {Building a better snail: Lubrication and
                gastropod locomotion},
   journal = {Phys. Fluids},
   volume = {17},
   pages = {113101},
   year =  2005,
}

@article{Vill07,
   author =  {Villermaux, E. and Eggers, J.},
   title =   {Honey, why are you so thin ?},
   journal = {In preparation},
   volume = {},
   pages = {},
   year =  2007,
}


@article{Vuka00,
   author =  {Vukasinovic, B. and Glezer, A. and Smith, M. K.},
   title =   {Vibration-induced droplet atomization.},
   journal = {Phys. Fluids : Gallery of fluid Motion},
   volume = 12,
   pages = {12},
   year =  2000,
}

@article{Vuka07,
   author =  {Vukasinovic, B. and Smith, M. K. and Glezer, A.},
   title =   {Mechanisms of free-surface breakup in
         vibration-induced liquid atomization.},
   journal = {Phys. Fluids},
   volume = 19,
   pages = {012104},
   year =  2007,
}


@article{Walt49,
   author =  {Walton, W. H. and Prewett, W. C.},
   title =   {The production of sprays and mists of uniform drop
        size by means of spinning disc type sprayers.},
   journal = {Proc. Phys. Soc. B},
   volume = 62,
   number = 6,
   pages = {341-350},
   year =  1949,
}


@article{Wats64 ,
   author =  {Watson, E. J.},
   title =   {The radial spread of a liquid jet over a horizontal
   plane.},
   journal = {J. Fluid Mech.},
   volume = 20,
   pages = {481-499},
   year =  1964,
}

@Article{Weber1931,
	author={C. Weber},
	title={Zum zerfall eines fl?ssigkeitsstrahles},
	journal={Z. angew. Math. U. Mech.},
	year={1931},
	volume={2},
	pages={136}
}

@article{Weidman07,
   author =  {Kubitschek,J. P. and Weidman, P. D.},
   title =   {Helical instability of a rotating viscous liquid jet.},
   journal = {Phys. Fluids},
   volume = 19,
   pages = 114108,
   year =  2007,
}


@article{Weih78,
   author =  {Weihs, D.},
   title =   {Stability of thin, radially moving liquid sheets.},
   journal = {J. Fluid Mech.},
   volume = 87,
   pages = {289-298},
   year =  1978,
}

@article{Witt04,
   author =  {Wittel, F. and Kun, F. and Hermann, H. J. and Kreplin, B. H.},
   title =   {Fragmentation of shells.},
   journal = {Phys. Rev. Letters},
   volume = 93,
   number={3},
   pages = {035504},
   year =  2004,
}

@article{Wong04,
   author =  {D. C. Y. Wong and M. J. H. Simmons and S. P. Decent
           and E. I. Parau and A. C. King},
   title =   {Break-up dynamics and drop size distributions created
from spiralling liquid jets},
   journal = {Int. J. of Mult. Flow},
   volume = 30,
   pages = {499-520},
   year =  2004,
}


@Article{Wu&Faeth1995,
	author={P.-K. Wu and G. M. Faeth},
	title={Onset and end drop formation along the
            surface of turbulent jets
	in still gases},
	journal={Phys. Fluids},
	year={1995},
	volume={7},
	number={11},
	pages={2915--2917}
}
@Article{Wu&Faeth1993,
	author={P.-K. Wu and G. M. Faeth},
	title={Aerodynamic effects on primary breakup of turbulent liquids},
	journal={Atom. and Sprays},
	year={1993},
	volume={3},
	pages={265--289}
}

@Article{Wu81,
	author={Wu, J.},
	title={Bubble populations and spectra in near-surface ocean:
          summary and review of field measurements},
	journal={J. Geophys. Research},
	year={1981},
	volume={86},
	number={C1},
	pages={457--463}
}

@Article{Wu&Ruff&Faeth1991,
	author={P.-K. Wu and G. A. Ruff and G. M. Faeth},
	title={Primary break-up in liquid-gas mixing layers},
	journal={Atom. and Sprays},
	year={1991},
	volume={1},
	number={},
	pages={421--440}
}

@Article{XZN05,
	author={L. Xu and W. W. Zhang and S. R. Nagel},
	title={Drop splashing on a dry smooth surface},
	journal={Phys. Rev. Lett.},
	year={2005},
	volume={94},
	pages={184505}
}

@misc{SJZZ09,
	author={R. D. Schroll and C. Josserand and S. Zaleski and
           W. W. Zhang},
	title={Impact of a viscous liquid drop},
	year={2009},
        url         = {http://arxiv:physics.flu-dyn/0904.0483},
}

@Article{Xu06,
	author={L. Xu and L. Barcos and S. R. Nagel},
	title={Splashing of Liquids: interplay of
           surrounding gas and surface roughness},
        journal = "arXiv:physics/0608079",
	year={2006},
            }

@book{Yang95,
   author =    {Yang, V. and Anderson, W.},
   title =     {Liquid rocket engine combustion instability},
   publisher = {AIAA},
   volume = 169,
   year =      1995,
}

@book{Watson62,
   author =    {G. N. Watson},
   title =     {A treatise on the theory of Bessel functions},
   publisher = {Cambridge University Press, Cambridge},
   year =      1962,
}

@book{Strogatz94,
   author =    {S. H. Strogatz},
   title =     {Nonlinear Dynamics and Chaos},
   publisher = {Westview Press},
   year =      1994,
}

@Article{L63,
	author={E. N. Lorenz},
	title={Deterministic nonperiodic flow},
	journal={J. Atmos. Sci.},
	year={1963},
	volume={20},
	pages={130}
}

@Article{Yarin06,
	author={Yarin, A. L.},
	title={Drop Impact Dynamics: Splashing, Spreading,
            Receding, Bouncing... },
	journal={Annu. Rev. Fluid Mech.},
	year={2006},
	volume={38},
	pages={159--192}
}

@Article{RPV06,
	author={A. Rozhkov and B. Prunet-Foch and M. Vignes-Adler},
	title={Dynamics and disintegration of drops of polymeric liquids},
	journal={J. Non-Newtonian Fluid Mech.},
	year={2006},
	volume={134},
	pages={44}
}

@Article{VBM06,
	author={R. L. {Vander Wal} and G. M. Berger and S. D. Mozes},
	title={Droplet splashing upon films of the same fluid of various
               depths },
	journal={Exp. Fluids},
	year={2006},
	volume={40},
	pages={33}
}

@Article{Yatsuyanagi&Sakamoto&Sato1994,
	author={N. Yatsuyanagi and H. Sakamoto and K. Sato},
	title={Atomization Characteristics of Liquid Jets Injected Into a
	High-Velocity Flow Field},
	journal={Atom. and Sprays},
	year={1994},
	volume={4},
	pages={451--471}
}
@Article{Yatsuyanagi&Sakamoto&Sato1998,
	author={N. Yatsuyanagi and H. Sakamoto and K. Sato},
	title={Empirical Calculation Model of the atomization of a
     liquid sheet and a round liquid jet in a gazeous flow},
	journal={Atom. and Sprays},
	year={1998},
	volume={8},
	number={},
	pages={267--289}
}

@book{Yari93,
   author =    {Yarin, A. L.},
   title =     {Free liquid jets and films: hydrodynamics and rheology},
   publisher = {Longman},
   year =      1993,
}

@article{York53,
   author =  {York, J. L. and  Stubbs, H. E. and Tek, M. R.},
   title =   {The mechanism of disintegration of liquid sheets.},
   journal = {Trans. ASME},
   pages = {1279-1286},
   year =  1953,
}

@article{You05,
   author =  {Young, T.},
   title =   {An Essay on the Cohesion of Fluids},
   journal = {Proc. Roy. Soc.},
   volume = 95,
   pages = {65-87},
   year =  1805,
}

@article{Yule00,
   author =  {Yule, A. J. and Al-Suleimani, Y.},
   title =   {On droplet formation from capillary waves on a
               vibrating surface},
   journal = {Proc. Roy. Soc. A},
   volume = 456,
   pages = {1069-1085},
   year =  2000,
}

@Article{Zef&al2000,
	author={Benjamin W. Zef and B. Kleber and
	J. Fineberg and D. P. Lathrop},
	title={Singularity dynamics in curvature collapse and
            jet erruption on a
	fluid surface},
	journal={Nature},
	year={2000},
	volume={403},
	number={},
	pages={401--404}
}

@article{Zeldo80,
   author =  {Istratov, A. G. and Kidin, N. I. and Librovich, V. B.
                 and Zeldovich, Y. B.},
   title =   {Flame propagation in tubes: hydrodynamics and stability},
   journal = {Comb. Sci. and Tech.},
   volume = 24,
   pages = {1-13},
   year =  1980,
}

%Additional references introduced by Joseph

 @Article{ Kahlweit,
     author    = " M. Kahlweit and R. Strey and G. Busse",
     title     = " Weakly to strongly structured mixtures",
     journal   = " Phys. Rev. E",
     volume    = " 47",
     year      = " 1993",
     pages     = " 4197"
}

@Article{ BCM01,
     author    = " L. Bruschi and A. Carlin and G. Mistura",
     title     = " Wetting on a geometrically structured substrate",
     journal   = " J. Chem. Phys.",
     volume    = " 115",
     year      = " 2001",
     pages     = " 6200"
}

  @Article{ BCPM03,
     author    = " L. Bruschi and A. Carlin and A. O. Parry and G. Mistura",
     title     = " Crossover effects in the wetting of adsorbed films in linear wedges",
     journal   = " Phys. Rev. E",
     volume    = " 68",
     year      = " 2003",
     pages     = " 021606"
}

@Article{ BCM03,
     author    = " L. Bruschi and E. Carlin and G. Mistura",
     title     = " Wetting of geometrically structured surfaces",
     journal   = " J. Phys.: Condens. Matter",
     volume    = " 15",
     year      = " 2003",
     pages     = " S315"
}

@Article{ BFM06,
     author    = " L. Bruschi and G. Fois and G. Mistura and M. Tormen and V. Garbin and E. di Fabrizio and A. Gerardino and M. Natali",
     title     = " Complete wetting of curved microscopic channels",
     journal   = " J. Chem. Phys.",
     volume    = " 125",
     year      = " 2006",
     pages     = " 144709"
}

@Article{ Pomeau,
     author    = " Y. Pomeau",
     title     = " Wetting in a corner and related questions",
     journal   = " J. Colloid Interface Sci.",
     volume    = " 113",
     year      = " 1986",
     pages     = " 5"
}

@Article{ LLPR01,
     author    = "R. Lacaze and P. Lallemand and Y. Pomeau and S. Rica",
     title     = " Dynamical formation of a Bose Einstein condensate",
     journal   = " Physica D",
     volume    = " 152",
     year      = " 2001",
     pages     = " 779"
}

@Article{ JPR06,
     author    = "C. Josserand and Y. Pomeau and S. Rica",
     title     = " Self-similar singularities in the kinetics of
                    condensation",
     journal   = " J. Low Temp. Phys.",
     volume    = " 145",
     year      = " 2006",
     pages     = " 231"
}

@Article{ Cheng,
     author    = " E. Cheng and M. W. Cole",
     title     = " Physical adsorption near an oblique corner ",
     journal   = " Phys. Rev. B",
     volume    = " 41",
     year      = " 1990",
     pages     = " 9650"
}

@Article{ NaKoDi,
     author    = " M. Napi\'orkowski and W. Koch and S. Dietrich",
     title     = " Wedge wetting by van der Waals fluids",
     journal   = " Phys. Rev. A",
     volume    = " 45",
     year      = " 1992",
     pages     = " 5760"
}

@Article{ Hauge1992,
     author    = " E. H. Hauge",
     title     = " Macroscopic theory of wetting in a wedge",
     journal   = " Phys. Rev. A",
     volume    = " 46",
     year      = " 1992",
     pages     = " 4994"
}

@Article{ Rejmer,
     author    = " K. Rejmer and S. Dietrich and M. Napi\'orkowski",
     title     = " Filling transition for a wedge",
     journal   = " Phys. Rev. E",
     volume    = " 60",
     year      = " 1999",
     pages     = " 4027"
}

@Article{ ParryRW,
     author    = " A. O. Parry and C. Rasc\'on and A. J. Wood",
     title     = " Critical effects at 3D wedge wetting",
     journal   = " Phys. Rev. Lett.",
     volume    = " 85",
     year      = " 2000",
     pages     = " 345"
}

@Article{ PWCD,
     author    = " A. O. Parry and A. J. Wood and E. Carlon and
                    A. Drzewi\'nski",
     title     = " Universal phase boundary shifts for corner
                        wetting and filling",
     journal   = " Phys. Rev. Lett.",
     volume    = " 87",
     year      = " 2001",
     pages     = " 196103"
}

@Article{ PGW,
     author    = " A. O. Parry and M. J. Greenall and A. J. Wood",
     title     = " Wedge covariance for two-dimensional filling and wetting",
     journal   = " J. Phys.: Condens. Matter",
     volume    = " 14",
     year      = " 2002",
     pages     = " 1169"
}

@Article{ APW,
     author    = " D. B. Abraham and A. O. Parry and A. J. Wood",
     title     = " Drumhead model of 2D wetting, filling and wedge covariance",
     journal   = " Europhys. Lett.",
     volume    = " 60",
     year      = " 2002",
     pages     = " 106"
}


@Article{ IndRob,
     author    = " J. O. Indekeu and A. Robledo",
     title     = " Hyperscaling and nonclassical exponents for the line tension at wetting",
     journal   = " Phys. Rev. E",
     volume    = " 47",
     year      = " 1993",
     pages     = " 4607"
}

@Article{ IndekeuLT,
     author    = " J. O. Indekeu",
     title     = " Line tension at wetting",
     journal   = " Int. J. Mod. Phys. B",
     volume    = " 8",
     year      = " 1994",
     pages     = " 309"
}

@Article{ GPRE,
     author    = " M. J. Greenall and A. O. Parry and J. M. Romero-Enrique",
     title     = " Three-dimensional wedge filling in ordered
                        and disordered systems",
     journal   = " J. Phys.: Condens. Matter",
     volume    = " 16",
     year      = " 2004",
     pages     = " 2515"
}

@Article{ PGRE,
     author    = " A. O. Parry and M. J. Greenall and J. M. Romero-Enrique",
     title     = " Fluid adsorption at an apex:
           covariance between complete wetting and critical wetting",
     journal   = " Phys. Rev. Lett.",
     volume    = " 90",
     year      = " 2003",
     pages     = " 046101"
}

@Article{ RP05,
     author    = " C. Rasc\'on and A. O. Parry",
     title     = " Covariance for cone and wedge complete filling",
     journal   = " Phys. Rev. Lett.",
     volume    = " 94",
     year      = " 2005",
     pages     = " 096103"
}

@Article{ REP,
     author    = " J. M. Romero-Enrique and A. O. Parry",
     title     = " 3D wedge filling and 2D random-bond wetting",
     journal   = " Europhys. Lett.",
     volume    = " 72",
     year      = " 2005",
     pages     = " 1004"
}

@Article{ AM02,
     author    = " D. B. Abraham and A. Maciolek",
     title     = " Filling Transition: Exact Results for Ising Corners",
     journal   = " Phys. Rev. Lett.",
     volume    = " 89",
     year      = " 2002",
     pages     = " 286101"
}

@Article{ AMW,
     author    = " D. B. Abraham and V. Mustonen and A. J. Wood",
     title     = " Triangular lattice solution for filling in a wedge",
     journal   = " Europhys. Lett.",
     volume    = " 63",
     year      = " 2003",
     pages     = " 408"
}

@Article{ ADVMB,
     author    = " E. V. Albano and A. De Virgiliis and
                M. M{\"u}ller and K. Binder",
     title     = " Corner wetting in the two-dimensional Ising model: Monte Carlo results",
     journal   = " J. Phys.: Condens. Matter",
     volume    = " 15",
     year      = " 2003",
     pages     = " 333"
}

@Article{ MMBL,
     author    = " A. Milchev and M. M{\"u}ller and K. Binder
                   and D. P. Landau",
     title     = " Wedge filling and interface delocalization in finite Ising lattices with antisymmetric surface fields",
     journal   = " Phys. Rev. E",
     volume    = " 68",
     year      = " 2003",
     pages     = " 031601",
}

@Article{ MBin05,
     author    = " M. M{\"u}ller and K. Binder",
     title     = " The interplay between wetting and phase behaviour in binary polymer films and wedges: Monte Carlo simulations and mean-field calculations",
     journal   = " J. Phys.: Condens. Matter",
     volume    = " 17",
     year      = " 2005",
     pages     = " S333",
}

@Article{ JRHen104,
     author    = " J. R. Henderson",
     title     = " Interfacial statistical geometry: Fluids adsorbed in wedges and at edges",
     journal   = " J. Chem. Phys.",
     volume    = " 120",
     year      = " 2004",
     pages     = " 1535",
}

@Article{ JRHen204,
     author    = " J. R. Henderson",
     title     = " Statistical mechanics of fluids adsorbed in planar wedges: Finite contact angle",
     journal   = " Phys. Rev. E",
     volume    = " 69",
     year      = " 2004",
     pages     = " 061613",
}

@Article{ PDie04,
     author    = " G. Pal\'agyi and S. Dietrich",
     title     = " Critical adsorption and Casimir torque in wedges and at ridges",
     journal   = " Phys. Rev. E",
     volume    = " 70",
     year      = " 2004",
     pages     = " 046114",
}

@Article{ Hernandez06,
     author    = " E. S. Hern\'andez and F. Ancilotto and
       M. Barranco and R. Mayol and M. Pi",
     title     = " Condensation of helium in nanoscopic alkali wedges
                        at zero temperature",
     journal   = " Phys. Rev. B",
     volume    = " 73",
     year      = " 2006",
     pages     = " 245406",
}

@Article{ TasinDieLet,
     author    = " M. Tasinkevych and S. Dietrich",
     title     = " Complete wetting of nanosculptured substrates",
     journal   = " Phys. Rev. Lett.",
     volume    = " 97",
     year      = " 2006",
     pages     = " 106102"
}

@Article{ TasinDie,
     author    = " M. Tasinkevych and S. Dietrich",
     title     = " Complete wetting of nanosculptured substrates",
     journal   = " Eur. Phys. J. E",
     volume    = " 23",
     year      = " 2007",
     pages     = " 117"
}

@Article{ Gang05,
     author    = " O. Gang and K. J. Alvine and M. Fukuto and
        P. S. Pershan and C. T. Black and B. M. Ocko",
     title     = " Liquids on topologically nanopatterned surfaces",
     journal   = " Phys. Rev. Lett.",
     volume    = " 95",
     year      = " 2005",
     pages     = " 217801"
}

@Article{ Arscott,
     author    = " S. Arscott and M. Gaudet and M. Brinkmann
          and A. E. Ashcroft and R. Blossey",
     title     = " Capillary filling of miniaturized sources for
                         electrospray mass spectrometry",
     journal   = " J. Phys.: Condens. Matter",
     volume    = " 18",
     year      = " 2006",
     pages     = " S677"
}

@Article{ Ishino,
     author    = " C. Ishino and K. Okumura and D. Qu\'er\'e",
     title     = " Wetting transitions on rough surfaces",
     journal   = " Europhys. Lett.",
     volume    = " 68",
     year      = " 2004",
     pages     = " 419"
}

@Article{ LipoCO,
     author    = " R. Lipowsky",
     title     = " Morphological wetting transitions at chemically structured surfaces",
     journal   = " Current Opinion in Colloid and Interface Science",
     volume    = " 6",
     year      = " 2001",
     pages     = " 40"
}

@Article{ BrinkLipo,
     author    = " M. Brinkmann and R. Lipowsky",
     title     = " Wetting morphologies on substrates with striped surface domains",
     journal   = " J. Appl. Phys.",
     volume    = " 92",
     year      = " 2002",
     pages     = " 4296"
}

@Article{ SeemannBKLL,
     author    = " R. Seemann and M. Brinkmann and E. J. Kramer and
               F. F. Lange and R. Lipowsky",
     title     = " Wetting morphologies at microstructured surfaces",
     journal   = " PNAS",
     volume    = " 102",
     year      = " 2005",
     pages     = " 1848"
}

@Article{ LLS00,
     author    = " R. Lipowsky and Peter Lenz and P. S. Swain",
     title     = " Wetting and dewetting of structured and imprinted surfaces",
     journal   = " Colloids and Surfaces A",
     volume    = " 161",
     year      = " 2000",
     pages     = " 3"
}

@Article{ SwainLipo,
     author    = " P. S. Swain and R. Lipowsky",
     title     = " Wetting between structured surfaces:
               liquid bridges and induced forces",
     journal   = " Europhys. Lett.",
     volume    = " 49",
     year      = " 2000",
     pages     = " 203"
}

@Article{ LBDFKZ,
     author    = " R. Lipowsky and M. Brinkmann and R. Dimova and
                     T. Franke and J. Kierfeld and X. Zhang",
     title     = " Droplets, bubbles, and vesicles at chemically
                         structured surfaces",
     journal   = " J. Phys.: Condens. Matter",
     volume    = " 17",
     year      = " 2005",
     pages     = " S537"
}

@Article{ LBDHKS,
     author    = " R. Lipowsky and M. Brinkmann and R. Dimova and
             C. Haluska and J. Kierfeld and J. Shillcock",
     title     = " Wetting, budding, and fusion - morphological
                    transitions of soft surfaces",
     journal   = " J. Phys.: Condens. Matter",
     volume    = " 17",
     year      = " 2005",
     pages     = " S2885"
}

@Article{ Checco06,
     author    = " A. Checco and Y. Cai and O. Gang and B. M. Ocko",
     title     = " High resolution non-contact AFM imaging of liquids condensed onto chemically nanopatterned surfaces",
     journal   = " Ultramicroscopy",
     volume    = " 106",
     year      = " 2006",
     pages     = " 703"
}

@Article{ Mechkov,
     author    = " S. Mechkov and G. Oshanin and M. Rauscher and
                 M. Brinkmann and A. M. Cazabat and S. Dietrich",
     title     = " Contact line stability of ridges and drops",
     journal   = " Europhys. Lett.",
     volume    = " 80",
     year      = " 2007",
     pages     = " 66002"
}

@Inproceedings{DietrichPattiM,
     author    = "S. Dietrich",
     title     = "Fluids in contact with structured substrates",
     year      = "1999",
     booktitle = "New approaches to problems in liquid state
                    theory (NATO ASI series C vol 529)",
     editor    = "C. Caccamo and J.-P. Hansen and G. Stell",
     pages     = "197",
     publisher = "Kluwer, Dordrecht",
}


@Article{ KoDiNa,
     author    = " W. Koch and S. Dietrich and M. Napi\'orkowski",
     title     = " Morphology and line tension of liquid films
               adsorbed on chemically structured substrates",
     journal   = " Phys. Rev. E",
     volume    = " 51",
     year      = " 1995",
     pages     = " 3300"
}

@Article{ Getta,
     author    = " T. Getta and S. Dietrich",
     title     = " Line tension between fluid phases and a substrate",
     journal   = " Phys. Rev. E",
     volume    = " 57",
     year      = " 1998",
     pages     = " 655"
}

@Article{ BauerEPJ,
     author    = " C. Bauer and S. Dietrich",
     title     = " Quantitative study of laterally inhomogeneous wetting",
     journal   = " Eur. Phys. J. B",
     volume    = " 10",
     year      = " 1999",
     pages     = " 767"
}

@Article{ BauerPRE,
     author    = " C. Bauer and S. Dietrich",
     title     = " Wetting films on chemically heterogeneous substrates",
     journal   = " Phys. Rev. E",
     volume    = " 60",
     year      = " 1999",
     pages     = " 6919"
}

@Article{ BauerDP,
     author    = " C. Bauer and S. Dietrich and A. O. Parry",
     title     = " Morphological phase transitions of thin fluid films on chemically structured substrates",
     journal   = " Europhys. Lett.",
     volume    = " 47",
     year      = " 1999",
     pages     = " 474"
}

@Article{ BauerPRE00,
     author    = " C. Bauer and S. Dietrich",
     title     = " Phase diagram for morphological transitions of
                  wetting films on chemically structured substrates",
     journal   = " Phys. Rev. E",
     volume    = " 61",
     year      = " 2000",
     pages     = " 1664"
}

@Article{ BiekerD,
     author    = " T. Bieker and S. Dietrich",
     title     = " Wetting of curved surfaces",
     journal   = " Physica A",
     volume    = " 252",
     year      = " 1998",
     pages     = " 85"
}

@Article{ BRMD,
     author    = " P. Bryk and R. Roth and K. R. Mecke and S. Dietrich",
     title     = " Hard sphere fluids in contact with curved substrates",
     journal   = " Phys. Rev. E",
     volume    = " 68",
     year      = " 2003",
     pages     = " 031602"
}

@Article{ SSD05,
     author    = " M. Sprenger and F. Schlesener and S. Dietrich",
     title     = " Critical adsorption at chemically structured substrates",
     journal   = " Phys. Rev. E",
     volume    = " 71",
     year      = " 2005",
     pages     = " 056125"
}

@Article{ HPD04,
     author    = " L. Harnau and F. Penna and S. Dietrich",
     title     = " Colloidal hard-rod fluids near geometrically structured substrates",
     journal   = " Phys. Rev. E",
     volume    = " 70",
     year      = " 2004",
     pages     = " 021505"
}

@Article{ SchimmeleND,
     author    = " L. Schimmele and M. Napi\'orkowski and S. Dietrich",
     title     = " Conceptual aspects of line tensions",
     journal   = " J. Chem. Phys. ",
     volume    = " 127",
     year      = " 2007",
     pages     = " 164715"
}

@Article{ RothED00,
     author    = " R. Roth and R. Evans and S. Dietrich",
     title     = " Depletion potential in hard-sphere mixtures:
                        theory and applications",
     journal   = " Phys. Rev. E",
     volume    = " 62",
     year      = " 2000",
     pages     = " 5360"
}

@Article{ GotzelED98,
     author    = " B. G{\"o}tzelmann and R. Evans and S. Dietrich",
     title     = " Depletion forces in fluids",
     journal   = " Phys. Rev. E",
     volume    = " 57",
     year      = " 1998",
     pages     = " 6785"
}

@Article{ Biben,
     author    = " T. Biben and P. Bladon and D. Frenkel",
     title     = " Depletion effects in binary hard-sphere fluids",
     journal   = " J. Phys.: Condens. Matter",
     volume    = " 8",
     year      = " 1996",
     pages     = " 10799"
}

@Article{ Dickman,
     author    = " R. Dickman and P. Attard and V. Simonian",
     title     = " Entropic forces in binary hard sphere mixtures: theory and simulation",
     journal   = " J. Chem. Phys.",
     volume    = " 107",
     year      = " 1997",
     pages     = " 205"
}

@Article{ DijkstraRE,
     author    = " M. Dijkstra and R. {van Roij} and R. Evans",
     title     = " Direct simulation of the phase behaviour of binary hard-sphere mixtures: test of the depletion potential description",
     journal   = " Phys. Rev. Lett.",
     volume    = " 82",
     year      = " 1999",
     pages     = " 117"
}

@Article{ GotzelRDDE,
     author    = " B. G{\"o}tzelmann and R. Roth and S. Dietrich
                       and M. Dijkstra and R. Evans",
     title     = " Depletion potential in hard-sphere fluids",
     journal   = " Europhys. Lett.",
     volume    = " 47",
     year      = " 1999",
     pages     = " 398"
}

@Article{ MaoCL,
     author    = " Y. Mao and M. E. Cates and H. N. W. Lekkerkerker",
     title     = " Depletion force in colloidal systems",
     journal   = " Physica A",
     volume    = " 222",
     year      = " 1995",
     pages     = " 10"
}

@Article{ YangTYNS,
     author    = " S. Yang and H. Tan and D. Yan and E. Nies and A. C. Shi",
     title     = " Effect of polydispersity on the depletion
            interaction in nonadsorbing polymer solutions",
     journal   = " Phys. Rev. E",
     volume    = " 75",
     year      = " 2007",
     pages     = " 061803"
}

@Article{ BrykRSD,
     author    = " P. Bryk and R. Roth and M. Schoen and S. Dietrich",
     title     = " Depletion potentials near geometrically
                    structured substrates",
     journal   = " Europhys. Lett.",
     volume    = " 63",
     year      = " 2003",
     pages     = " 233"
}

@Article{ salima2,
     author    = " S. Rafa{\"\i} and D. Bonn and J. Meunier",
     title     = " Repulsive and attractive critical Casimir forces",
     journal   = " Physica A",
     volume    = " 386",
     year      = " 2007",
     pages     = " 31"
}

@Article{ KarGo,
     author    = " M. Kardar and R. Golestanian",
     title     = " The `friction' of vacuum, and other
                    fluctuation-induced forces",
     journal   = " Rev. Mod. Phys.",
     volume    = " 71",
     year      = " 1999",
     pages     = " 1233"
}

@Article{ balibar,
     author    = " S. Balibar and S. Ishiguro",
     title     = " Critical Casimir forces and anomalous wetting",
     journal   = " Pramana, J. Phys.",
     volume    = " 64",
     year      = " 2005",
     pages     = " 743"
}

@Article{ Sohaili,
     author    = "M. Sohaili and J. Klier and P. Leiderer",
     title     = "Triple-point wetting of molecular hydrogen isotopes",
     journal   = "J. Phys.: Condens. Matter",
     volume    = "17",
     year      = "2005",
     pages     = "S415",
}

@Article{ HankeED,
     author    = " A. Hanke and E. Eisenriegler and S. Dietrich",
     title     = " Polymer depletion effects near mesoscopic particles",
     journal   = " Phys. Rev. E",
     volume    = " 59",
     year      = " 1999",
     pages     = " 6853"
}

@Article{ MeckeD,
     author    = " K. R. Mecke and S. Dietrich",
     title     = " Effective Hamiltonian for liquid-vapour interfaces",
     journal   = " Phys. Rev. E",
     volume    = " 59",
     year      = " 1999",
     pages     = " 6766"
}

@Article{ DieNap91,
     author    = " S. Dietrich and M. Napi\'orkowski",
     title     = " Microscopic derivation of the effective
           interface Hamiltonian for liquid-vapor interfaces",
     journal   = " Physica A",
     volume    = " 177",
     year      = " 1991",
     pages     = " 437"
}

@Article{ NapiDi93,
     author    = " M. Napi\'orkowski and S. Dietrich",
     title     = " Structure of the effective Hamiltonian
                for liquid-vapor interfaces",
     journal   = " Phys. Rev. E",
     volume    = " 47",
     year      = " 1993",
     pages     = " 1836"
}

@Article{ BechingerRLRD,
     author    = " C. Bechinger and D. Rudhardt and P. Leiderer and
                  R. Roth and S. Dietrich",
     title     = " Understanding Depletion Forces beyond Entropy",
     journal   = " Phys. Rev. Lett.",
     volume    = " 83",
     year      = " 1999",
     pages     = " 3960"
}

@Article{ Mora,
     author    = " S. Mora and J. Daillant and K. R. Mecke and D. Luzet
                      and A. Braslau and M. Alba and B. Struth",
     title     = " X-Ray Synchrotron Study of Liquid-Vapor Interfaces
 at Short Length Scales: Effect of Long-Range Forces and Bending Energies",
     journal   = " Phys. Rev. Lett.",
     volume    = " 90",
     year      = " 2003",
     pages     = " 216101"
}
